Yoneda lemma

We are studying properties of the name appointment in various categories of enriched graphs. The Yoneda lemma is generalized for continuous transforms between transports of enriched original graphs.

==> neda.tex <==
%2023.02.15 Pradójau traukõ clattice/neda.tex
\vskip\tarpas
             At the end of this paper I shall fulfill my promise to
prove the Yoneda lemma. We wanted to follow the proving from \baf G. Kelley 1982*.
But our way appear more simple. The former complex proving of G. Kelley
rests some doubt
about its validity. We would wish that a reader would get more beautiful
impression from our text.

We remember that a monoidal category $\VV$ is closed if we have
truly joint pair of
functors. For chosen an assistant object $s\in \VV_0$ the adjoint
functor is defined by biproduct $s\otimes r$
and for it we demand existence of coadjoint exponential functor $t^s $
with natural bijective name mapping
$$\VV(s\otimes r;t)=\rightarrow \VV(r;t^s) \tsk$$

We have changed the place of assistant object $s$ in biproduct $s\otimes r$.
So we shall interchange the prefixes ^{=pre} with ^{=post}.
The prefix { \it pre} is applied when we maintain  the order of factors, and
the prefix { \it post}  is applied  when we change the order of factors to
opposite one.

We shall weaken our assumptions. We shall ask that a monoidal category
would be
^{almost =closed}. For the joint pair of functors $s\otimes r$ and $t^s$
we ask only existence of unit and counit transforms.

The unit transform is defined by ^{=sections arrows}
$$\lambda_r: r\rightarrow (s\otimes r)^s \kbl$$

and the counit transform is defined by ^{=evaluation arrows}
$$\ev_t: s\otimes t^s\rightarrow  t\tsk$$

The sections  arrow and the changing of target space by taken form
$f: p\otimes s\rightarrow p$
provide  the ^{=name form}
$$f^\sharp: p\mapright \lambda_p (s\otimes p)^s \mapright f^s p^s \tsk$$
 The biproduct of taken name form
$g: p\rightarrow r^s$ with identity $\Identity_s:s \rightarrow s$
and  the evaluation  arrow and provide   ^{=realization}
$$g^\flat : s\otimes p\mapright 1_s\otimes g s\otimes  r^s
 \mapright \ev_r r\tsk$$

In the values category $\VV$ defined exponential space $t^s\in \VV_0$
will be called an ^{inner hom =set} $[s;t]=t^s$. It provides
the  edges sets for an $\VV$-enriched
graph $\VV^e$
$$\VV^e(p;r)= [p;r]\tsk$$

For the projection to the left factor of biproduct
$\sigma: r\otimes *\rightarrow r$
we get the ^{=name arrow}
$$i_r : * \mapright \lambda_* (r\otimes *)^r \mapright \sigma^r  r^r \tsk$$
We shall take it as choosing of unit arrow $i_r\in \VV^e (r;r) $
for an object $r\in \VV_0$.
So we  construct  an original $\VV$-graph $\VV^e$.

Using an associative arrow  for biproduct $s\otimes t$
$$s: p\otimes (q\otimes r)\rightarrow (p\otimes q)\otimes r$$
together with double evaluation  we get
^{=contact arrows  mappings}  between inner hom sets
$$\cdot: q^p\otimes r^q \rightarrow q^p \cdot r^q \subset r^p \tsk$$

First we take the composition  of arrows
$$p\otimes (q^p\otimes r^q)\mapright s (p\otimes q^p)\otimes r^q
\mapright \ev_q  q\otimes r^q \mapright \ev_r  r \tsk$$
Then its name arrow will be taken as needed contact arrows mapping.

It is some problem to check under what conditions the chosen unit arrows
are neutral for such contact arrows mappings.
For the true joint pair of functors $r\otimes s$ and $t^s$ we have bijective
name appointment. In our more general case we can demand that
chosen special projection $\sigma: r\otimes *\rightarrow r $  would be
a realization of its name. We could demand this property also for
arbitrary ^{left =projection} $\sigma: r\otimes s\rightarrow r$.
Such  property is expressed as commuting diagram
$$\matrix{ r\otimes s & \mapright 1_r\otimes \lambda_s  &
r\otimes (r\otimes s)^r & \mapright 1_r\otimes \sigma^s  & r\otimes r^r \cr
 & \searrow & \mapdownd\ev_{r\otimes s} & & \mapdownd \ev_r \cr
 & & r\otimes s& \maprightap {\sigma} & r \cr} $$
\vskip\tarpas
It will be provided by the first triangular equality
$$\matrix{ r\otimes s & \mapright 1_r\otimes \lambda_s &
r\otimes (r\otimes s)^r \cr
& \searrow & \mapdownd \ev_{r\otimes s} \cr
& &r\otimes s \cr} $$
\hskip\tarpas
and commuting quadrat
$$\matrix{ r\otimes (r\otimes s)^r &\mapright  1_r\otimes \sigma^r &
r\otimes r^r \cr
\mapdownk \ev_{r\otimes s} &    & \ev_r \cr
r\otimes s & \maprightap {\sigma}  & r \cr}$$
\vskip\tarpas
First we shall check the neutral property for the arrow's source
$$i_r(*)\cdot t^r=t^r \tsk$$
It is expressed as commuting diagram
with right projection $\rho: *\otimes t^r \rightarrow t^r$
$$ \matrix {*\otimes t^r  & \mapright i_r\otimes 1_{t^r}  &
 r^r\otimes t^r \cr
\mapdownk {\rho}   &   \swarrow \cdot &  \cr
t^r &  & \cr}$$
\vskip\tarpas
We shall draw a commuting diagram for the  realization of
contact arrow  mappings over the biproduct
$r\otimes (*\otimes t^r)\rightarrow (r\otimes *) \otimes t^r$
$$\matrix{ (r\otimes *)\otimes t^r\hskip -10pt  &
 \mapright  (r\otimes \lambda_*)\otimes 1_{t^r}  &
(r\otimes (r\otimes *)^r)\otimes t^r  &
\mapright  (r\otimes \sigma^r)\otimes 1_{t^r}
& \hskip -5pt (r\otimes r^r)\otimes t^r  \cr
&\searrow & \mapdownk \ev_{r\otimes *}\otimes 1_{t^r} &
&\mapdownd  \ev_r \otimes 1_{t^r} \cr
& & (r\otimes *)\otimes t^r  & \maprightap \sigma\otimes 1_{t^r}
& r\otimes t^r  \cr}$$
\vskip\tarpas
which provide needed equality for the name form  defining
contact arrows mapping for the  inner
home sets.

In similar way we shall check the neutral property for the arrow's target
$$r^p \cdot i_r(*)= r^p \tsk$$
It is expressed as a commuting diagram
$$ \matrix {r^p \otimes  *  & \mapright 1_{r^p}\otimes 1_r
& r^p\otimes r^r \cr
\mapdownk {\sigma}  &   \swarrow \cdot &  \cr
r^p &  & \cr}$$
\vskip\tarpas
We shall draw a commuting diagram  for the realization of contact arrows
mapping over biproduct $p\otimes (r^p \otimes *)$
$$\hskip -10pt \matrix{p\otimes (r^p\otimes *) &
\hskip -5pt \mapright  1_p\otimes (1_{r^p}\otimes \lambda_*) \hskip -5pt &
p\otimes (r^p\otimes (r^p\otimes *)^{r^p})  &
\hskip -10pt \mapright 1_p\otimes  (1_{r^p}\otimes \sigma^{r^p}) \hskip -10pt
 &  p\otimes (r^p\otimes (r^p)^{r^p})  \cr
&\searrow & \mapdownk 1_p\otimes \ev_{(r^p\otimes *)} & &
\mapdownd  1_p\otimes \ev_{(r^p)}   \cr
& & p\otimes (r^p\otimes * )& \maprightap 1_p\otimes {\sigma}
& p\otimes r^p \cr}$$
\vskip\tarpas
which provide needed equality for the name arrow  defining
contact arrows mapping between inner hom sets.

We shall notice that constructed contact arrows mappings between inner
hom sets provides predecomposable form
$$q^p\otimes r^q \rightarrow q^p\cdot r^q \subset r^p $$
as we have an equality
$$q^p \cdot r^q =  (q^p\cdot i_{q})\cdot (1_{q}\cdot r^q) \tsk$$
This property will be changed to another  decomposability property, if
we take another notation of biproduct. For the biproduct
$r^q\otimes q^p $  we get postdecomposable form
$$r^q\otimes q^p \rightarrow q^p\cdot r^q \subset r^p \tsk$$
For general joint pair of functors $s\otimes r$ and $t^s$
we can have
another unit arrows $i_r(*)\subset [r;r]$ and another
contact arrows mappings between inner hom sets
$q^p \times r^q \rightarrow r^p $.


We want to check that the associativity of arrow composition in the
values category
$\VV$ provides also the associativity arrow for contact arrows mappings
between inner hom sets. 

The associativity arrow of biproduct isn't necessary.
Later we shall give example of concrete value
s category, which isn't  banal.

So we probe to define contact arrows mappings between inner hom sets
without using such associativity of biproduct $r\otimes s$.
We should  demand that sections arrows would define natural transform.
For arbitrary arrow $f:r\rightarrow t$ we used the  commuting diagram
$$\matrix{ r & \mapright \lambda_r & (s\otimes r)^s \cr
     \mapdownk f & & \mapdownd (1_s\otimes f)^s \cr
     t & \maprightap \lambda_t  & (s\otimes t)^s \cr} $$
\vskip\tarpas
In usual cases such property is fulfilled.

Also we demand that evaluation arrow would be natural on its functional
argument. For an arrow $g: r \rightarrow t$ we get commuting diagram
$$\matrix { s\otimes r^s & \mapright \ev_r & r \cr
\mapdownk 1_s\otimes g^s  & & \mapdownd g \cr
        s\otimes t^s  & \maprightap \ev_t & t \cr} $$
        \vskip\tarpas
More special property we ask for inner hom sets and biproducts.
We need to have isomorphic arrows
$$[p;q] \otimes r= [p;q\otimes r] \tsk$$
Then the contact arrows mappings between inner hom sets will be defined
as a annulation  of middle object
$$A_q: q^p \otimes r^q = (q\otimes r^q)^p \mapright (\ev_r)^p  r^p \tsk$$

The associativity arrow
$$q^p \cdot (r^q \cdot s^r) \rightarrow (q^p \cdot r^q)\cdot s^r $$
will be checked from diagrams with different annulation  order.
$$ q^p\otimes (r^q\otimes s^r) =
(q\otimes (r^q\otimes s^r))^p =(q\otimes (r\otimes s^r)^q )^p
\mapright A_r (q\otimes s^q)^p \mapright A_q  s^p \tsk$$
and
$$(q^p\otimes r^q) \otimes s^r = (q\otimes r^q)^p \otimes s^r \mapright A_q
q^p \otimes s^r = (r\otimes s^r)^p \mapright A_r s^p \tsk$$

So it rests to check a wanted associativity property
by equality or inequality of these two concrete processes.

We shall study a concrete value category produced with recursive schema
from the less complex values category.
We begin with a category of original graphs
with chosen set of original graphs transports
$$\VV= \OGrph\tsk$$

 The  graph $p$ is defined over the set of vertexes $p_0$
with the edges sets $p(u;v)\in \Set_0$
for arbitrary couple of vertexes $ u,v\in p_0$.
An  original graph $p$ has chosen unit arrows
$1_u\in p(u;u) $.
The crude functor $f: p\doublerightarrow r$ must maintain the unit arrows
$$f_{x,x}(1_x)= 1_{f(x)} \tsk$$

In the category of original graphs $\OGrph$ we can't  expect
to have truly joint pair of superfunctors $p\otimes s $ and $r^s$.

Let we have in the target graph $r$ the contact arrows mappings
$$\cdot: r(u;v) \times r(v;w) \rightarrow r(u;w) \tsk$$

Then for original graphs we can  construct
the ^{=form} $\Phi: p\otimes s\doublerightarrow r$
from its ^{partial =forms}
$\Phi( p,-) :s\doublerightarrow r$ and $\Phi(- ,s): p\doublerightarrow r$
with the help of contact arrows  in the target graph $r$.
We ask the  coherent vertexes mappings.
For vertexes $a\in p_0$ and $b\in r_0$ we need the equality
for  both partial forms
$$\Phi_0(a,b)= \Phi(a,-)_0(b)= \Phi(-,b)_0(a)\tsk$$
But for the edges $u\in p(a;a')$ and $v\in s(b;b')$ we have two choices.
One is prerealization
$$\Phi^+(u,v)= \Phi(u,b)\circ \Phi(a',v)\kbl$$
another is postrealization
$$\Phi^-(u,v)= \Phi(a, v)\circ \Phi(u, b')\tsk$$
The partial forms  are defined again from taken form $\Phi$
with the help of chosen unit arrow
$$\Phi(a,-)(v):=\Phi(1_a,u)\kbl \Phi(-,b)(u):= \Phi(u,1_b) \tsk$$

The biproduct of two graphs $p\otimes r$  is defined over the Carte tensor
product of vertexes sets $p_0\times r_0$ with the Carte tensor product
of edges sets
$$p\otimes r(\lan a,a'\ran;\lan b,b'\ran):= p(a;a')\times r(b;b') \tsk$$
It will present a Carte product in the category of graphs $\Grph$.

Taking a unit arrow
$$1_{\lan a,a'\ran} = \lan 1_a,1_{a'}\ran \in p\otimes r(\lan a,a'\ran;
\lan a,a' \ran) $$
we get a presentation of Carte product in the category
of original graphs $\OGrph$ with crude functors.

Additionally taking a  product of contact arrows mappings
$$\lan u,u'\ran \cdot \lan v,v'\ran = \lan u\cdot v, u'\cdot v'\ran $$
such biproduct will become  a presentation  of Carte  product  in the smaller
 category   of original graphs  $\OGrph^=$ with natural functors.

Such  biproduct defines  superfunctor in the category of original graphs.
It is true  not only for the category of crude functors $\OGrph$,
but also for smaller
categories of continuous functors $\OGrph^-$,  cocontinuous functors
$\OGrph^+$, or natural  functors $\OGrph^=$.

For the functors $f: p\doublerightarrow  p'$ and $g: r\doublerightarrow r'$
we take a product functor $f\otimes g: p\otimes r\doublerightarrow
p'\otimes r'$.
We have the product of vertexes mappings
$$(f\otimes g)_0= f_0\times g_0\kbl$$
and for edges set mappings   $f\otimes g_{\lan x,y\ran,\lan x',y'\ran}$
we take a Cauchy tensor product
$$ f_{x,x'}\times g_{y,y'}:
p(x;x')\times r(y;y')\rightarrow p(f_0(x);f_0(x'))\times r(g_0(y);g_0(y'))
\tsk$$

If we have continuous quadrats for the graphs transports
$f: X\doublerightarrow X'$ and $g: Y\doublerightarrow Y'$
$$\matrix{ X\otimes_p X &\mapright f\otimes f & X'\otimes_p X'& \cr
   \mapdownk {\circ} & & \mapdownd {\circ} &\cr
   X & \maprightap f & X' &  \cr
   & & & \hskip-15pt \nearrow \hfill \cr}\hskip 20 pt
\matrix{ Y\otimes_p Y &\mapright g\otimes g & Y'\otimes_p Y'& \cr
   \mapdownk {\circ} & & \mapdownd {\circ} &\cr
   Y & \maprightap g & Y' &  \cr
   & & & \hskip-15pt \nearrow \hfill \cr}$$
then we get again a continuous quadrats for the product of graphs transports
$f\otimes g: X\otimes Y \doublerightarrow X'\otimes Y'$
$$\matrix{ (X\otimes Y) \otimes_p (X\otimes Y)  &
\mapright (f\otimes g)\otimes_p(f\otimes g) &(X'\otimes g')\otimes_p
(X'\otimes Y')&\cr
   \mapdownk {\circ} & & \mapdownd {\circ} &\cr
   X\otimes Y & \maprightap f\otimes g  & X'\otimes Y' &  \cr
   & & & \hskip-25pt \nearrow \hfill \cr}$$

We could take some relator as a larger biproduct
$p\otimes r\subset p\sqprod r$, but it would be hard task to check
when we can get needed biproduct of taken  functors
$f: p\doublerightarrow p'$
and $g: r\doublerightarrow r'$.  This can be imagine as a problem to have
some integral of taken functors.

Necessarily we need to have a biproduct
$$f\sqprod g: *\sqprod * \rightarrow X\sqprod Y$$
of arbitrary  points $f:*\doublerightarrow X$
and $g: *\doublerightarrow Y$.

Also we want  to have biproduct for  arbitrary functor
$f:p \doublerightarrow p'$
with identity functor of assistant graph  $\Identity_s: s\doublerightarrow s$
$$f\sqprod \Identity_s:p\sqprod s\doublerightarrow p'\sqprod s\tsk$$
\vskip\tarpas
The exponential space $p^s$ is constructed as a graph
with vertexes set  compounded
of all functors
$$(p^s)_0= \lbrace \phi: s\doublerightarrow p\rbrace\tsk$$
The edges set will be compounded by all transforms
$$p^s(\phi;\psi)= \lbrace \alpha:\phi\rightarrow \psi\rbrace \tsk$$
Such transforms will be defined by collection of edges
$$\alpha= \lan \alpha_a\uparrow a\in s_0\ran \in \Prod_{a\in s_0}
p(\phi_0(a);\psi_0(a))\tsk$$

A unit arrow will be defined by collection of unit arrows
$$1_{\phi}=\lan 1_{\phi_0(a)}\uparrow a\in A\ran\in
 \Prod_{a\in A_0} p(\phi_0(a);\phi_0(a))\tsk$$
A contact arrows mapping
$$\cdot : p^s(\phi;\psi)\times p^s(\psi;\xi) \rightarrow  p^s(\phi;\xi)$$
is also defined as a product of contact arrows mappings in
the target space. For transforms
$\alpha\in \Prod_{a\in A_0} p(\phi_0(a);\psi_0(a))$ and
$\beta\in \Prod_{a\in A_0} p(\psi_0(a);\xi_0(a))$
it appoints
$$ \alpha\cdot \beta= \Prod_{a\in s_0} \alpha_a\cdot \beta_a\in
\Prod_{a\in s_0}p(\phi_0(a);\xi_0(a)) \tsk$$
Such exponential space $r^s$ also  defines a superfunctor within the
category $\OGrph$.
For a functor between target spaces $f: p\doublerightarrow r$
we  appoint the changing of target space
$f^s: p^s\doublerightarrow r^s $.  Such appointment
maintains the identity functor
$$(\Identity_p )^s= \Identity_{p^s}\kbl $$
also it maintains composition of functors
$$(f\circ g)^s= f^s\circ g^s\kbl$$
as we have associative the composition in the category $\OGrph$.

We would want to  work also
 with a smaller exponential space $p^{(s)}$
which has  smaller edges sets $p^{(s)}(\phi;\psi)$
compounded by natural transforms $\alpha: \phi\rightarrow \psi$, i. e.
having commuting diagrams for arbitrary edge $u\in s(a;b)$
$$\matrix{ \phi_0(a) & \mapright \alpha_a & \psi_0(a) \cr
\mapdownk \phi(u) & & \mapdownd \psi(u) \cr
\phi_0(b) & \maprightap \alpha_b & \psi_0(b) \cr} $$
\vskip\tarpas
However without the property of associativity for contact arrows mappings
we can't guaranty that contact arrows mappings rest
in the set of natural transforms.
Such exponential space would  define superfunctor only for
natural functors. If functor $f: p\doublerightarrow r$
maintains the contact arrows mappings
$$f(u\cdot v)= f(u)\cdot f(v) \uparrow u\in p(x;y), v\in p(y;z)\kbl$$
then transported transform
$\alpha\star f $ rests natural transform as we get commuting diagram
again for arbitrary edge $u\in s(a;b)$
$$\matrix{ f_0(\phi_0(a)) & \mapright f(\alpha_a) & f_0(\psi_0(a)) \cr
\mapdownk f(\phi(u)) &\searrow  & \mapdownd f(\psi(u)) \cr
f_0(\phi_0(b)) & \maprightap f(\alpha_b) & f_0(\psi_0(b)) \cr} $$
\vskip\tarpas

For the joint pair of superfunctors $s\sqprod p$ and $r^s$ we shall define
unit transform by collection of sections transports
$\lambda_p: p\doublerightarrow (s\sqprod p)^s $.
The sections $\lambda_p(x): s\doublerightarrow s\sqprod p$ are defined
by biproduct of identity transport
$\Identity_s: s\doublerightarrow s$ with chosen unit arrow
$1_x\in p(x;x) $, i. e.  we have
vertexes mapping
$$a\to \lan a,x\ran\in p_0\times s_0 $$
and edges set mappings
$$\lambda_p(x)_{a,b} : s(a;b) \rightarrow   s(a;b) \sqprod 1_x
\subset  s(a;b)\sqprod p(x;x)\tsk$$


The counit transform is defined by collection of evaluation transports
$$\ev_r: s \sqprod r^s \doublerightarrow r\tsk$$
It for a functor $\phi: s  \doublerightarrow r$ and vertex $a\in s_0$
appoints the value $\phi_0(a)\in r_0$ and have edges set mappings
$$ s(a;b)\sqprod r^s(\phi;\psi)\rightarrow r(\phi_0(a);\psi_0(b))\tsk$$

It can be done in two ways.
A postevaluation map  is provided  for an edge $u\in s(a;b)$  and  a
transform $\alpha:\phi\rightarrow \psi$
 by extension over the larger  new biproduct
of postcontact arrows mapping
$$ s(a;b) \sqprod r^s(\phi;\psi)\rightarrow .\alpha_a\circ \psi_{a,b} (u) \in r(\phi_0(a);\psi_0(b))\tsk$$
 May be we shall take a smaller
exponential space $(r^s)'$ to achieve this  task.

A preevaluation map for an edge $u\in s(a;b)$  and a transform
$\alpha:\phi\rightarrow \psi$
 is provided by extension over the larger new biproduct of
 precontact arrows mapping
$$ s(a;b) \sqprod r^s(\phi;\psi)\rightarrow \phi_{a,b}
(u)\circ \alpha_b \in p(\phi_0(a);\psi_0(b))\tsk$$
Also may be we shall take  a smaller
exponential space $(r^s)'$ to achieve this  task.

We get a bijective name  appointment
$$\OGrph( s\sqprod p ;r) =\rightarrow  \OGrph(p;r^s) $$
for the  forms
 $\Phi: s\sqprod p\doublerightarrow p$
with  a predecomposition property
$$\Phi(s(a;b); p(x;y))= \Phi(1_x,s(a;b))\cdot \Phi(p(x;y),1_b)\tsk$$

A postevaluation map for an edge $u\in s(a;b)$  and a transform
$\alpha:\phi\rightarrow \psi$
 is provided by extension over the larger new biproduct of
 postcontact arrows mapping
$$ s(a;b) \sqprod r^s(\phi;\psi)\rightarrow \alpha_a\circ
\psi_{a,b} (u) 
 \in p(\phi_0(a);\psi_0(b))\tsk$$
Also may be we shall take  a smaller
exponential space $(r^s)'$ to achieve this  task.

We get a bijective name  appointment
$$\OGrph( s\sqprod p ;r) =\rightarrow  \OGrph(p;r^s) $$
for the  forms
 $\Phi: s\sqprod p\doublerightarrow p$
 with a postdecomposition  property
$$\Phi(s(a;b);p(x;y))= \Phi(p(x;y), 1_a)\cdot \Phi(1_y; s(a;b))\kbl$$
                   
It is hard task to construct  a new biproduct by some topological extension.
For example in the category of metric spaces  $\Cat_{[0,\infty]^+}$
we can apply a  metric of
uniform convergence in the space of nonexpanding mappings
$\Cat_{[0,\infty]^+}(X;Y)$, but  such metric space is already complete.
Therefore we haven't got  any interesting completion.

There is a more easy task to take some new biproduct
in the values category $\VV= \OGrph$ which would be relator to
the former biproduct
$$p\otimes r\rightarrow p\sqprod r $$
and take as  target space only
such original graphs $t\in \VV_0$ which would have contact arrows mappings
 extended over the new biproduct
$$\circ: t(x;y)\sqprod t(y;z) \rightarrow t(x;z)   \tsk$$

For the partial forms as functors
$\Phi(p,-): r\doublerightarrow t$ and $\Phi(-,r) :p \doublerightarrow t$
we get again the predecomposable form
$\Phi^+: p\sqprod r \doublerightarrow t$
with equal appointments
$$\Phi^+(p(x;x')\sqprod r(y;y')):=\Phi(p(x;x'),y) \sqprod \Phi(x';r(y;y'))$$
and postdecomposable form $\Phi^-:p\sqprod r \doublerightarrow t$
with  another appointment
$$\Phi^-(p(x;x'),r(y;y')):= \Phi(x; r(y;y'))\sqprod \Phi(p(x;x'),y')\tsk$$

Later we prefer to talk about $\VV$-enriched graphs. The ordinary graph
is also $\Set$-enriched graph.
A $\VV$-graph $X$   is defined by the set of vertexes $X_0\in \Set_0$
and edges sets $X(a;b)\in \VV_0$. The $\VV$-graphs transport
$f: X\doublerightarrow Y$ is defined by  the  mapping of vertexes
$f_0: X_0\rightarrow Y_0$ as an arrow in  the category of sets
$\Set$ and edges set mappings
$$f_{a,b}: X(a;b)\rightarrow Y(f_0(a);f_0(b))$$
as an arrows in the values category $\VV$.
All $\VV$-graphs transports compound  the category $\Grph_{\VV}$.

Now  we can take the category of original
$\VV$-graphs as a new values category.
 At first we can take the category compounded by all
 crude functors
$\VW=\OGrph_\VV$.
Such functors will be $\VV$-graphs transports $f: X\doublerightarrow Y$
 with edges $\VV$-object
mappings
$$f_{x,y} : X(x;y) \rightarrow Y(f_0(x);f_0(y))$$
maintaining unit arrow choosing
$$f_{x,x}(1_x(*))= 1_{f_0(x)}(*)\tsk$$
We shall apply the words ^{$\VV$-=objects} and ^{$\VV$-=arrows} for the object and arrows
in the category $\VV$.

For two parallel arrows we can define inequality by  existing transform
between correspondent functors
$f,g: X\doublerightarrow Y $. We have the $\VV$-object of all transforms
equal for the Carte product of edges $\VV$-objects in the target $\VV$-graph $Y$
$$Y^X (f;g)= \Prod_{a\in X_0} Y(f_0(a);g_0(a)) $$
and we shall say $f\dgl g$ if exists some point in this product as
an arrow from former values category $\VV$
$$(* \rightarrow  \Prod_{a\in X_0} Y(f_0(a)'g_0(a)))= \Prod_{a\in X_0}
(*\rightarrow Y_0(f_0(a);g_0(a)))\tsk$$
Also we can take a stronger order relation provided by the partial
$\VV$-object  of continuous, cocontinuous or natural  transforms, But
for it we shall need contact arrows $\VV$-mappings in the target space $Y$.
An inequality with existing special transform  will  provide
the inequality defined with existing of general transforms.

As usually we take the Carte tensor product of vertexes sets
$X_0\times Y_0$ with biproduct of edges $\VV$-objects from the former
values category $\VV$.
For the monotone biproduct in $p\otimes r$ values category $\VV$
we get again monotone biproduct of original $\VV$-graphs $X\otimes Y$.

For  any assistant space $T$ we get a superfunctor in the category
$\OGrph_{\VV}$ defined by biproduct with assistant space $T\otimes X$.
For a functor $f:X\doublerightarrow Y$ it appoints the biproduct
$$\Identity_T\otimes f : T\otimes T \doublerightarrow T\otimes Y \tsk$$.

For cocontinuous relator's involution
$$m_{\lan p,r\ran,\lan s,t\ran} : (p\otimes r)\otimes (s\otimes t)
\rightarrow  (p\otimes s)\otimes (r\otimes t)$$
we get such superfunctor  restricted in the category $\OGrph_{\VV}^-$
of  continuous transports  between  original $\VV$-graphs.
Also for continuous  relator's involution we get restriction in the
category $\OGrph_{\VV}^- $ of cocontinuous transports between original
$\VV$-graphs,

It is possible to choose a larger biproduct
$$X\otimes Y \doublerightarrow X\sqprod Y$$
with relator's transport to the former biproduct
$$N_{\lan X,Y\ran, \lan Z,W\ran} :(X\sqprod Y)\otimes (Z\sqprod W)
\doublerightarrow (X\otimes Z)\sqprod (Y\otimes W)\tsk$$
We can choose such new biproduct being monotone superfunctor
$$\OGrph_{\VV} \otimes \OGrph_{\VV} \doublerightarrow \OGrph_{\VV} \kbl$$
or having continuous or cocontinuous relator's involution
$$M_{\lan X,Y\ran,\lan Z,W\ran}: (X\sqprod Y)\sqprod (Z\sqprod W)
\doublerightarrow  (X\sqprod Z)\sqprod(Y\sqprod W) \tsk$$

Also we are choosing the  ^{=exponential space} $Y^T$
defined with
the partial set of original $\VV$-graphs transports
as the vertexes set
$$(Y^T )_0\subset \lbrace f: T\doublerightarrow Y\rbrace$$
and the edges $\VV$-objects taken as
as a partial object from all transforms
$$Y^T(\phi;\psi)\subset \Prod_{a\in T_0} Y(\phi_0(a);\psi_0(a))\tsk$$

For  a  target space  $Y$ with
 contact arrows $\VV$-mappings
$$\circ : Y(x;y) \otimes Y(y;z) \rightarrow Y(x;y)\circ Y(y;z)\subset
Y(x;z) $$
we get an ^{=exponential superfunctor} provided by the target changing
with an  original $\VV$-graphs transport $f: X\doublerightarrow Y$.
For a $\VV$-graphs transport $\phi: T\doublerightarrow X$
 we get the new $V$-graphs transport $\phi\circ f:T\doublerightarrow Y$.
For continuous taken transport we get continuous changing of target space.
And for cocontinuous one we get cocontinuous changing of target space.
It rests to check the maintenance of edges $\VV$-object.

Such superfunctor will be monotone one.
For the inequality between parallel $\VV$-graphs transports
$f,f': X\doublerightarrow Y$, i. e. we
have equal first projection
$$f_0(x)= f'_0(x)\uparrow x\in X_0$$
and inequalities for edges $\VV$-objects mappings
$$f_{x,y} \dgl f'_{x,y} \uparrow x,y\in X_0\kbl$$
we get $\VV$-graphs transports
$$f^T, (f')^T: X^T\doublerightarrow Y^T $$
 with equality of mappings for the
equal secondary projection
$$(f_0)^{T_0} = (f'_0)^{T_0} : (X_0)^{T_0} \rightarrow (Y_0)^{T_0}\tsk $$
We get the inequalities for the $\VV$-graphs transports of  first projection
$$\phi\cdot f \dgl \phi\cdot f'\uparrow \phi\in X^T \kbl $$
i. e. we have for edges $\VV$-objects mappings we have
inequalities
$$T(s;t) \rightarrow f_{\phi_0(s),f'_0(t)} (\phi_{s,t} (T(s;t)) \dgl
$$$$f'_{\phi_0(s),f'_0(t)} (\phi_{s,t} (T(s;t))
\subset Y(f_0'(\phi_0(s));f_0'(\phi_0(t)))\tsk$$
Also we get inequalities for edges $\VV$-objects mappings
$$X(a;b)\rightarrow f_{a,b}(X(a;b))\dgl $$$$
f_{a,b}'(X(a;b))\subset Y^T(f_0'(a);f'_0(b)) = \Prod_{s\in T_0}
Y(f'_0(a)_s; f'_0(b)_s)\tsk$$

Also the sections transport becomes monotone
$$\lambda_X: X\doublerightarrow (T\otimes X)^T \tsk$$

Additionally we demand that changing of target with contact arrows
$\VV$-mappings
would be monotone for arbitrary $\VV$-object $r\in \VV_0$
$$\VV(r;Y(x;y)) \rightarrow \VV(r;Y(x;y) \circ Y(y;z))\subset Y(r;Y(x;z) )
\uparrow  r\in\VV_0\kbl$$
Such assumption provides the monotone preevaluation transports
$$\ev_{Y}^+: T\otimes Y^T \doublerightarrow Y$$
defined with precontact arrows mappings
 $$T(s;t)\otimes Y^T(\phi;\psi)\rightarrow
 \phi_{s,t} (T(s;t))\circ Y(\phi_0(t);\psi_0(t))\subset
  Y(\phi_0(s);\psi_0(t))\kbl$$

For the monotone target's changing
$$\VV(r;Y(y;z)) \rightarrow \VV(r;Y(x;y) \circ Y(y;z))\subset Y(r;Y(x;z) )
\uparrow  r\in\VV_0\tsk$$
we get monotone
$$\ev_{Y}^-: T\otimes Y^T \doublerightarrow Y$$
defined with postcontact arrows mappings
 $$T(s;t)\otimes Y^T(\phi;\psi)\rightarrow
Y(\phi_0(s);\psi_0(s)) \circ \psi_{s,t} (T(s;t)) \subset
  Y(\phi_0(s);\psi_0(t))\tsk$$

So the category $\OGrph_{\VV} $ can be consider as a new values category.
\vskip\tarpas
We wish to convert the category of $\VV$-graphs $\Grph_{\VV}$
into an enriched  graph by itself.
 .
We have constructed the exponential space $Y^X$ in the category of $\VV$-graphs
$\Grph_{\VV} (X;Y) $ taking all $\VV$-graphs transports
$f: X\doublerightarrow  Y$ as vertexes and the sets of transforms
between them
$$Y^X(\phi;\psi)= \Prod_{a\in X_0} Y(\phi_0(a);\psi_0(a))$$
as edges sets.
Usually we denote this exponential space
$$Y^X= [X;Y]\tsk$$

We have composition of arrows in this category
$$\Grph_{\VV} (X;Y)\times \Grph_{\VV} (Y;Z)\rightarrow
\Grph_{\VV} (X;Z)\tsk$$
Now the set of transforms between two $\VV$-graphs transports
$\phi,\psi: X\doublerightarrow Y$ will provide an edges $\VV$-object
$Y^X(\phi;\psi)$ in the exponential space $Y^X$.
We need to define  contact arrows mappings for such exponential spaces.
They will be edges $\VV$-object mappings for the $\VV$-graphs transport
over pullbacked biproduct
$$\circ :Y^X\otimes_p Z^Y   \doublerightarrow Z^X\tsk$$

We shall define the contact arrows mappings $Y^X\otimes Z^Y
\doublerightarrow  Z^Y$ similarly to the double evaluation.

At first we shall construct the $\VV$-enriched continuous quadrats as $\VV$-enriched
graph and produce the horizontal contact mappings between them
in arbitrary category of original $\VV$-graphs.
In the category of $\VV$-enriched graphs $\Grph_{\VV}$
a continuous quadrat $\VQ$ is a diagram
$$\matrix{  \bigcirc & \mapright M & \cdot & \cr
  \mapdownk I_1 & &\mapdownd I_2 & \cr
  \cdot & \maprightap N & \bullet & \hskip -10 pt \nearrow \hfill \cr}$$
  \vskip\tarpas
A ^{=source of diagram} is a $\VV$-graph  $\bigcirc$ and
a ^{=target of diagram} is a $\VV$-graph $\bullet$.
 A^{=circuit in diagram} is a chain of composable functors from the source
 $\VV$-graph
 to the  target  $\VV$-graph.  For taken quadrat $\VQ$ we have only two circuits.
 One is $I_1N :\bigcirc\doublerightarrow \bullet$ and another
 is $MI_2: \bigcirc\doublerightarrow \bullet$.
The continuous quadrat $\VQ$ is defined by the partial  set of transforms
defined in the product of edges sets from the final $\VV$-graph
$$\VQ(I_1N;MI_2)\subset [\bigcirc;\bullet] (I_1N;MI_2)=
\Prod_{a\in \bigcirc_0 } \bullet((I_1N )_0(a);(MI_2)_0(a))\tsk$$
For a general diagram we construct a new
 original graph with all circuits as vertexes, and the sets of
 transforms between two circuits can  be
 defined by  products of edges sets in diagram's
 target space.

We shall try to define horizontal composition of two continuous
quadrats  $\VQ_1\bullet \VQ_2$  as decomposable form
$$\matrix {\bigcirc & \mapright M_1 & \cdot & & \mapright M_2 &\cdot &\cr
       \mapdownk I_1 &      &\mapdownd I_2 &  &  &\mapdownd I_3 & \cr
  \cdot &\maprightap N_1 &\cdot & & \maprightap N_2 &\bigcirc & \cr
 &  & &\hskip -15pt \nearrow  \hfill   & & &\hskip -10pt \nearrow \hfill \cr}
 $$
 \hskip\tarpas

 First we shall define partial forms.
We shall demand that arrows in value category $\VV$ provides the images
of partial objects, i. e. such category is a ^{=regular} by \baf I. Freyd,
A. Scedrov 1990 * \S 1.5.

The new graphs transport
$$\alpha\ast 1_{N_2}:= \alpha\star N_2 $$
will be defined by transport of diagrams target with the functor $N_2$.
The edges set mapping of functor $N_2$ will provide the image of partial set
$$N_2(\VQ(I_1N_1;M_1I_2))\subset [\circ;\bullet](I_1N_1N_2; M_1N_2N_2) \tsk$$
Another partial transport
$$1_{M_1} \ast \beta := M_1\star \beta $$
will be defined by transport of diagram source by functor $M_1$.
In the case of $\Set$-enriched graphs we take the same arrows of transform $\beta$,  only indexes are
vertexes from the new source object. For more general values category $\VV$
we can take the  projection of product
$$\Prod_x \bullet( ((I_2N_2)_0(x); (M_2I_3)_0(x))\rightarrow
\Prod_{x= (M_1)_0(a)} \bullet ( (M_1I_2N_2)_0(a); (M_1M_2I_3)_0(a))$$
and the image of partial object
$O_2\subset \Prod_{x} \bullet((I_2M_1)_0(x);
(M_2I_3)_0(x))$.

If the target object  of new diagram has  contact arrows
mappings, then  we get predecomposable appointment
$$\alpha\ast^+\beta: =( \alpha\star N_2)\circ (M_1\star \beta)\tsk$$
It will define the ^{=prehorizontal composition} of continuous quadrats.

Also we can get postdecomposable appointment for cocontinuous quadrats
$$\alpha\ast^- \beta =(M_1\star  \beta)\circ (\alpha\star N_1 ) \tsk$$

If the target object has associative contact arrows mappings, then
we get again the associative composition of continuous or cocontinuous
quadrats.


The deformed quadrats with identic functors
$I_1= \Identity_X$, $I_2= \Identity_Y$
will be identified with transforms between functors
$M, N:X\doublerightarrow Y$.
\vskip\tarpas

The  ^{prehorizontal =composition} $\alpha\ast^+ \beta: \phi\circ \xi
\rightarrow \psi\circ \kappa $   of two transforms
$\alpha: \phi\rightarrow \psi$  between functors
$\phi,\psi: X\doublerightarrow Y$
and $\beta: \xi\rightarrow \kappa $  between functors
$\xi,\kappa: Y\doublerightarrow Z$ are calculated
as ^{horizontal =composition of two continuous  quadrats}
$$\matrix{
 &  & &\hskip-10pt \searrow^\alpha\hfill & &
  &\hskip -10pt \searrow^\beta \hfill\cr
 X &\mapright {\phi} &Y & & \mapright {\xi } & Z & \cr
         \uparrow &  &\uparrow &  & & \uparrow & \cr
       X &\maprightap {\psi} &Y & & \maprightap {\kappa} & Z & \cr}$$
 \vskip\tarpas
$$\alpha\ast^+ \beta= (\alpha\star \xi )\circ (\psi\star \beta) \tsk$$

The edges set mapping of preevaluation functor
$\ev_Y: X\otimes Y^X \doublerightarrow Y$ is  expressed as
horizontal composition between  continuous  quadrats. For an edges set
$ X(a;b) $  we get
a set of precontact arrows
$$ \alpha_a\circ \psi(w): \phi (a)\rightarrow \psi(b) $$
$$\matrix{  &  & &\hskip-10pt \searrow^w \hfill & & &\hskip -10pt
 \searrow^\alpha \hfill\cr
* &\mapright  a  &X & & \mapright {\psi} & Y & \cr
          &  &\uparrow &  & & \uparrow & \cr
        * &\maprightap b &X & & \maprightap {\phi} & Y & \cr }$$
\vskip\tarpas
In the case of associative contact arrows mappings from final $\VV$-graph  $Z$
the ^{double =preevaluation} provides  the horizontal composition of
three continuous  quadrats
$$\matrix{& &  &  & \hskip -15 pt \searrow^w \hfill &
&\hskip-10pt \searrow^\alpha \hfill &
& &\hskip -10pt \searrow^\beta \hfill\cr
* & \mapright a & X & &\mapright {\phi} &Y & & \mapright {\xi } & Z & \cr
    & &     \uparrow &  &  &\uparrow & & & \uparrow & \cr
   * & \maprightap b &     X &  &\maprightap {\psi} &Y & & \maprightap
   {\kappa} & Z & \cr }$$
\vskip\tarpas
and coincides with the preevaluation of earlier defined prehorizontal
composition.

This can be produced also for the horizontal composition of cocontinuous
quadrats.

$$\matrix{
 X &\mapright {\phi} &Y & & \mapright {\xi } & Z & \cr
         \uparrow &  &\uparrow &  & & \uparrow & \cr
       X &\maprightap {\psi} &Y & & \maprightap {\kappa} & Z & \cr
  &  & &\hskip-10pt \swarrow_\alpha\hfill & &
  &\hskip -10pt \swarrow_\beta \hfill\cr
 }$$
 \vskip\tarpas
$$\alpha\ast^- \beta= (\phi\ast \beta) \circ (\alpha\star \kappa) \tsk$$

\vskip\tarpas



For G. Kelley it was important to explain his  notation
by constructing a functor
$\Hom_X: X^\op \otimes X \doublerightarrow \VV$
which would have the  appointment of vertexes
$$(\Hom_X)_0(a;b)=X(a;b)\in \VV_0 $$
and the edges sets mappings
$$\Hom_X: X^\op(a;b)\times X(c;d) \rightarrow [X(a;c);X(b;d)]$$
extending target's changing  mappings $X(1;\beta): X(a;b)\rightarrow X(a;c) $
and source' changing mappings
$X(\alpha;1): X(b;d)\rightarrow X(a;d)$.
For us it will be an interesting exercise.

For the form's  $\Phi: X_1\otimes X_2\doublerightarrow Y$
name $X_1\doublerightarrow [X_2; Y]$ 
we shall apply  more special notation.
 We take the exponential space $[X_1\otimes X_2; Y]$ and construct
 partial form over the first argument
 applying identic mapping $X_1\doublerightarrow X_1$
 composed with taken exponential space
$$X_1 \doublerightarrow [ \bigcirc \otimes X_2; Y]\tsk$$

Also we can construct another name
with another composition  over the second argument
$$X_2\doublerightarrow [X_1\otimes \bigcirc ; Y] \tsk$$

So we can express different partial forms more graphically.
\vskip\tarpas


We shall use a diagram to explain  the notation  in our problem
of functor $Hom_X$
$$\matrix{ b &\rightarrow & d \cr
      \mapdownk {\alpha} & & \mapupd {\beta} \cr
      a& \rightarrow &c  \cr } $$
\vskip\tarpas
Such functor can be get in two ways.
One is defined as an predecomposable form, another is defined
as an postdecomposable form.
We shall apply the names of predecomposable form
defined by contact arrows mappings in taken original
$\VV$-graph  $X$.
$$X(a,b)\otimes X(b;c) \rightarrow X(a;b)\circ X(b;c) \subset X(a;c) \tsk$$
For it we can check equality
 $$X(a;b)\circ X(b;c)= (X(a;b) \circ 1_b(*))\circ (1_b(*)\circ A(b;c))\tsk$$
One  name will be
$$X(b;c) \rightarrow [ X(a;c)\circ \bigcirc ; X(a;c)] = [X(a;b);X(a;c)]\tsk$$
Another ^{dual =name} will be
$$X(b;c)\rightarrow [\bigcirc\circ  X(b;c);X(a;c)] = [X(b;c);X(a;c)]\tsk$$

With  such names we define partial forms for desired predecomposable
form
$$\Hom_X^+ (X^\op(a;b)\times X(c;d))= \Hom_X(X^\op (a;b)\otimes 1_c(*))
\cdot \Hom_X(1_b(*)\times X(c;d)) $$

One partial form will be
$$\Hom_X(X^\op(a;b)\times 1_c(*))= [\bigcirc\circ X(a;c);X(b;c)]\subset
 [X(a;c);X(b;c)]$$
$$\matrix{ b &&\cr
\downarrow &\searrow & \cr
a &\rightarrow c \cr}$$
\vskip\tarpas
and  another partial form
$$ \Hom_X (1_b(*)\times X(c;d))= [X(b;c)\circ \bigcirc;X(b;d)]
\subset [X(b;c);X(c;d)]$$
$$\matrix { b &\rightarrow & d\cr
        & \searrow &\uparrow \cr
        & & c \cr}$$
\vskip\tarpas

The defined predecomposable form can be explain by diagram
$$\matrix{ b &\rightarrow & d\cr
         \downarrow & \searrow &\uparrow \cr
         a &\rightarrow & c\cr }$$
\vskip\tarpas

We shall calculate such mappings in more details
for the prehorizontal composition between  exponential spaces  in our
values category $\VV=\OGrph$. Later such category will be called a
^{=pointed } one.

Let we have original graphs $p= X^\op(a;b)$, $q=X(a;c)$, $r= X(c;d)$. We denote
the vertexes $u\in p_0$, $v\in q_0$, $w\in r$ and edges
$\alpha\in p(u,u')$, $\beta\in q(v;v')$, $ \gamma\in r(w;w')$.

The functor between original graphs
$$ X^\op(a;b)\times X(c;d) \doublerightarrow [\bigcirc\circ X(a;c);X(b;c)]\cdot
 [\bigcirc\circ  X(c;d);X(b;d)]  $$
is composed as
functor to the ^{first =factor}
$$X^\op(a;b)\doublerightarrow [\bigcirc\circ X(a;c);X(a;d)]\kbl$$
then the functor over two arguments to the ^{second =factor}
$$X^\op(a;b)\times [\bigcirc\circ X(a;c);X(a;d)]\times X(c;d)
\doublerightarrow
[\bigcirc\circ X(c;d); X(b;d)]\kbl$$
and finally we calculate the form over such two mappings
$$[\bigcirc\circ  X(a;c);X(b;c)]\cdot  [\bigcirc\circ
X
(c;d);X(b;d)]\tsk$$
We shall calculate the realization of such composition.
For the first  functor we get a realization defined with
contact arrows mappings in $\VV$-graph $X$
$$X^\op(a;b)\times X(a;c) \doublerightarrow X(b;a)\circ X(a;c)\subset X(b;c)\tsk$$
For the second factor we get a realization
$$X^\op (a;b)\times  X(b;c)\times X(c;d)\doublerightarrow
(X(b;a)\circ X(a;c)) \circ X(c;d) \subset X(b;d)\tsk$$

Finally we need to calculate the prehorizontal composition of transforms
between provided original graphs transports.
$$\matrix{
 &  & &\hskip-10pt \searrow^{A(\alpha)}\hfill & &
  &\hskip -10pt \searrow^{A(\gamma)}\hfill\cr
 X^\op(a;b) &\mapright T_u & X(b;c) & & \mapright T_w & X(b;d) & \cr
         \uparrow &  &\uparrow &  & & \uparrow & \cr
   X^\op(a;b) &\maprightap T_{v'} &X(b;c) & & \maprightap T_{w'} & X(b;d)
    & \cr}$$
 \vskip\tarpas
$$A(\alpha)\ast^+ A(\gamma)=
 (A(\alpha)\star T_w)\cdot (T_{v'}\star A(\gamma))
\tsk$$

For a vertex $u\in p_0$ we get a functor
$T_u: X(a;c)\doublerightarrow X(b;c)$
in the first factor
defined with contact arrow mappings from taken  $\VV$-graph $X$.
For a vertex $v\in q_0 $ it appoints $u\circ v\in X(b;c)$ and
for an edge $\beta:v\rightarrow v'$ it appoints the new edge
$1_u\circ \beta:u\circ v\rightarrow u\circ v'$.

For an edge $\alpha: u\rightarrow u'$ it appoints the transform
between former functors $A(\alpha): T_u\rightarrow T_{u'}$
 defined with collection of edges
$\alpha\circ 1_v: u\circ v\rightarrow u'\circ v$

For a vertex $w\in r_0$  we get a functor
$ T_w: X(b;c)\doublerightarrow X(b;d)$
in the second factor
defined with contact arrows mappings from taken $\VV$-graph $X$.
For a vertex $u\circ v\in X(b;c)_0$ it appoints the  new vertex
$(u\circ v)\circ w$ and for an edge $(\alpha\circ\beta): u\circ v\rightarrow u'\circ v'$
it appoints the new edge $(\alpha\circ\beta) \circ 1_w :
(u\circ v)\circ w\rightarrow (u'\circ v')\circ w $.
For an edge $\gamma: w\rightarrow w'$ it appoints the transform between
such functors $A(\gamma): T_w\rightarrow T_{w'}$  defined with collection of edges
$$(1_u\circ 1_v)\circ \gamma: (u\circ v)\circ w\rightarrow (u\circ v)\circ w;\tsk$$

The prehorizontal composition of such transforms
$$A(\alpha)=\alpha\circ 1_v: u\circ v\rightarrow u'\circ v\kbl$$
$$A(\gamma)=(1_u\circ 1_v)\circ \gamma: (u\circ v)\circ w\rightarrow
(u\circ v)\circ w'$$
will be
$$(\alpha\circ 1_v)\circ 1_w: (u\circ v )\circ w\rightarrow (u'\circ v)\circ w$$
composed with
$$(1_{u'}\circ 1_v )\circ\gamma: (u'\circ v)\circ w \rightarrow
(u'\circ v)\circ w'
\kbl$$
i.e. we get transform defined with collection of arrows
$$(\alpha\circ 1_v)\circ \gamma : (u\circ v)\circ w \rightarrow
(u'\circ v  )\circ w'$$
between functors  defined by the  vertexes $u\in p_0$ and $w\in r_0$
with appointment for a  vertex $v\in q_0$
the vertex $(u\circ v)\circ w $ and for an edge $\beta: v\rightarrow v'$
appointing the new edge
$$(1_u \circ  \beta )\circ 1_w : (u\circ v)\circ w\rightarrow (u\circ v')\circ w\tsk$$
For an edges $\alpha:u'\rightarrow u$ and $\gamma: w\rightarrow w'$
we appoint
the transform  between such functors
$$(\alpha\circ 1_v)\circ \gamma : (u\circ v) \circ w\rightarrow
(u'\circ v)\circ w'\tsk $$

This can be expressed as a new functor to the new exponential space
$$X^\op (a;b)\times X(c;d) \doublerightarrow
[(\bigcirc \circ X(a;c))\circ \bigcirc; X(b;d)]\subset [X(a;c);X(b;d)] \tsk$$
It will be a partial form  got from  the form
$$ X^\op (a;b)\times X(c;d)\times X(a;c) \doublerightarrow (X^\op(a;b)\circ
X(a;c) )\circ X(c;d) \subset X(b;d) \tsk$$

There is no surprise that the same result will be got
also for posthorizontal composition of edges
in value category $\VV$.
$$A(\alpha)\ast^- A(\gamma)= (T_v\star A(\gamma))\cdot
(A(\alpha)\star T_{w'})
\tsk$$

For the postdecomposable form
$$\Hom_X^+ (X^\op(a;b)\times X(c;d))= \Hom_X(1_a(*)\otimes X(c;d))
\cdot \Hom_X(X^\op(a;b) \times 1_d(*)) $$
we take one partial form
$$\Hom_X(1_a(*)\times X(c;d) = [\bigcirc\circ X(a;c);X(a;d)] \subset
[X(a;c);X(a;d)] $$
$$\matrix { & & d\cr
&\nearrow &\uparrow \cr
a &\rightarrow &c \cr } $$
\vskip\tarpas
and another partial form
$$\Hom_X(X^\op(a;b)\times 1_d(*))=[\bigcirc\circ X(c;d);X(b;d)] $$
$$\matrix { b&\rightarrow &d\cr
\downarrow & \nearrow & \cr
a & & \cr }$$
\vskip\tarpas
The defined postdecomposable form can be explain  by diagram
$$\matrix { b &\rightarrow &d\cr
\downarrow &\nearrow &\uparrow \cr
a &\rightarrow &c \cr }$$
\vskip\tarpas
For the values category $\VV= \OGrph$
the postdecomposable form can be expressed  again as
 a functor to the new exponential space
 $$X^\op (a;b)\times X(c;d) \doublerightarrow
 [\bigcirc \circ (X(a;c) \circ \bigcirc ); X(b;d)]\subset [X(a;c);X(b;d)]
 \tsk$$
 It will be a partial form got from the  form
 $$X^\op(a;b)\times X(c;d) \times X(a;c)
 \doublerightarrow X^\op(a;b)\circ ( X(a;c)\circ X( c;d)) \subset X(b;d)
 \tsk $$
Having associativity arrows in  taken
original $\VV$-graph $X$
$$S : X(a;b) \circ (X(b;c)\circ
X(c;d))\rightarrow
(X(a;b)\circ (X(b;c))\circ X(c;d)\kbl$$

we get an  arrow  also between predecomposable and postdecomposable forms
$$\Hom_X^+=\rightarrow \Hom_X^-$$
which are partial forms for the correspondent forms.
The same is true for an opposite arrow, or for isomorphic arrows.

\vskip\tarpas
Now we are ready to prove the Yoneda lemma.
It will be proved for arbitrary original $\VV$-graph $X$ with
contact arrows mappings
$$X(a;b)\otimes X(b;c) \rightarrow X(a;b)\circ X(b;c) \subset X(a;c) \tsk$$

Let  we have an  $\VV$-graphs transport
from the opposite $\VV$-graph $X^\op$ to the values
category $\VV$   considered as $\VV$-graph
$$F: X^\op\doublerightarrow \VV^e\tsk$$
It will be  called a ^{=character}
 over taken original  $\VV$-graph $X$.
The representable character is defined by any vertex $x\in X_0$
$$X(-; x): X^\op \doublerightarrow \VV^e \tsk$$
Such appointment  will be understood as a Yoneda mapping
$$(\Yoneda_X)_0: X_0\rightarrow  (\VV^{X^\op} )_0\tsk$$
It can be extended as graphs transport
$$\Yoneda_X: X\doublerightarrow \VV^{X^\op} $$
and this extension will be ^{=fullfaithful  imbedding}.
It will be called a ^{=Yoneda imbedding}.
Usually mathematicians were interesting when such embedding
can be corestricted in the set of natural transforms $\VV^{(X^\op)}$.
We extend such  problematic with the set
of continuous transforms $\VV^{(X^\op)}_-$.

The Yoneda lemma will  describe the set of  transforms
between representable character $X(-;x) $ and other character
$F: X^\op\doublerightarrow \VV$ which is  an original  $\VV$-graphs
transport, i. e. we get identity mapping
$$F(i_x) = \Identity_{F_0(x)}: F_0(x) \rightarrow F_0(x)\tsk$$
\Proposition
For an original $\VV$-graphs transport $F: X^\op \doublerightarrow \VV^e$
we get a fullfaithful mapping from the value object $F_0(x)$
to the exponential space of transforms between representable character
$X(-;x)$ and taken $\VV$-graphs transport $F$
$$F_0(x)\rightarrow [ X(-;x); F] \tsk$$
\Proof:
For a $\VV$-graphs transport $F: X^\op\doublerightarrow \VV^e$
we have a mapping
$$X(a;x)\rightarrow [F_0(x);F_0(x)]\tsk$$
It is a name mapping for predecomposable form
$$X(a;x) \otimes F_0(x) \rightarrow F(x) \tsk$$
The dual name form will be
$$F_0(x) \rightarrow [ X(a;x); F_0(a)] \tsk$$
So we have got a mapping to the product
$$\rho:F_0(x) \rightarrow \Prod_{a\in X_0} [X(a;x);F_0(a)] \tsk$$
The inverse mapping is provided by projection to the factor
$$\Prod_{x\in X_0} [X(a;x );F_0(a)] \rightarrow [X(x;x);F_0(x)]$$
and taking image of unit arrow $i_x(*) \subset  X(x;x)$
$$[i_x(*); F_0(x)] \subset F_0(x) \tsk$$

 By our assumption taken  functor $F: X^\op \doublerightarrow \VV^e$
 is an original $\VV$-graphs transport, therefore it maintains
 the choosing of unit arrows, therefore  we have got
the  composition  as identity mapping
$$F_0(x) \rightarrow \Prod_{a\in X} [X(a;x);F_0(a)] \rightarrow
[i_x(x); F_0(x)] \subset F_0(x)\tsk$$
Otherwise we have also identic mapping
$$\Prod_{a\in X_0} [X(a;x);F_0(a) ] \rightarrow [i_x(*);F_(x)]
\mapright {\rho} \Prod_{a\in X_0} [X(a;x);F_0(a)]\tsk$$
It is enough to notice that every factor  is defined by the value object
$F_0(x)$.

\irodymopabaiga

Let we have an original $\VV$-graph $X$ with upper
associative contact arrows mappings, i. e. we have associative
arrow  between
mappings
$$X(a;b)\circ (X(b;c)) \circ X(c;x)) \rightarrow (X(a;b)\circ
X(b;c))\circ X(c;x) \tsk$$
Every representable character now will be continuous one
$$\matrix { X(a;b) \otimes X(b;c)  & \mapright {\circ} \cr
\mapdownk X(-;x) \otimes X(-;x) &    \cr
[\bigcirc \circ X(b;c); X(a;c) ]\otimes [ \bigcirc\circ X(c:x); X(b;x)] &
\maprightap {\cdot} \cr}$$
\vskip\tarpas
$$\matrix {   \rightarrow & X(a;c) &\cr
   & \mapdownd X(-;x) &\cr
\rightarrow  & [\bigcirc\circ X(c;x);X(b;x)]\cdot [\bigcirc
\circ X(b;x); X(a;x)] &\cr
 & & \hskip-10pt \nearrow \cr }$$
\vskip\tarpas
We need only to calculate the  double evaluation for composition
of contact arrows mappings in $\VV$-graph $\VV^e$
$$X(b;c) \otimes( [\bigcirc\circ X(c;x);X(b;x)]\cdot [\bigcirc
\circ X(b;x); X(a;x) ] \mapright {\ev} $$$$
(X(b;c)\circ X(c;x)) \otimes [\bigcirc \circ  X(b;x); X(a;x)]
\mapright {\ev}
$$$$ X(a;b)\circ (X(b;c)\circ X(c;x) \subset X(a;x) \tsk$$
For it we have associativity arrow to another predecomposable form
$$X(a;b)\circ (X(b;c)\circ X(c;x) \rightarrow
(X(a;b)\circ X(b;c)) \circ X(c;x) \subset X(a;x) \tsk$$

We shall improve the former proposition for continuous functor
between original $\VV$-graphs  $F: X^\op \doublerightarrow \VV^e $.

\Proposition
In original $\VV$-graph $X$ with upper associative contact arrows mappings
$$X(a;b)\circ (X(b;c)) \circ X(c;x)) \rightarrow (X(a;b)\circ
X(b;c))\circ X(c;x)$$
the set of transforms between a representable functor
$X(-;x): X^\op\doublerightarrow \VV^e$ and a continuous original
$\VV$-graphs transport $F: X\op \doublerightarrow \VV^e$
coincides with the set of continuous transforms
$\VV^{(X^\op)}_-(X(-;x);F) $.
\Proof:
We need to check continuous inequality between two forms
One is get with preevaluation transport
$$ X^\op(a;b) \otimes \Prod_{a\in X_0} [X(a;x);F_0(a)]
\rightarrow [\bigcirc \circ X(a;x); X(b;x)] \cdot [X(b;x) ; F_0(b) ]
$$
and another is get with postevaluation transport
$$ X^\op(a;b) \otimes \Prod_{a\in X_0} [X(a;x);F_0(a)]
\rightarrow [X(a;x);F_0(a)]\cdot [F_0(a);F_0(b)]\tsk$$
The predecomposable form
will be calculated  with the double evaluation
$$X^\op (a;b) \otimes [\bigcirc \circ X(a;x); X(b;x)] \cdot
[X(b;x) ; F_0(b) ]\mapright {\ev} $$$$
 (X(b;a)\circ X(a;x))\otimes [ X(b;x);F_0(b)]
\mapright [(X(b;a)\circ X(a;x);F_0(b)] \tsk$$
It was calculated as
$$F_{x,b} (X(b;a)\circ X(a;x))\subset [F(x);F(b)] \tsk$$
The postdecomposable form
will be calculated also with double evaluation
$$X^\op (a;b) \otimes [X(a;x);F_0(a)]\cdot
[F_0(a); F_0(b) ]\rightarrow
$$$$ [X(a;x);F_0(a)] \cdot X^\op(a;b)\otimes
[F_0(a);F_0(b)]_)$$
It was calculated as
$$F_{x,a} (X(a;x)) \cdot F_{a;b} (X(b;a))\subset F_{x,b} ( X(b;x) \tsk$$
For the continuous original $\VV$-graphs transport $F$
we have an arrow
$$F_{x,a) (X(a;x)) \cdot F_{a;b} (X(b;a)) =\rightarrow
F(b;x} (X(b;a)\circ X(a;x)) \tsk$$
\irodymopabaiga
As corollary we get fullfaithful imbedding of original $\VV$-graphs transport
with upper associative contact arrows mappings
into the set of continuous transforms between representable characters,  i. e.
we have isomorphic objects in values category $\VV$
$$X(x;y)\rightarrow \VV^{(X^\op)}_- ( X(-;x); X(-;y) ) \tsk$$

As partial case we get this result also for the $\VV$-enriched categories,
as they are original $\VV$-graphs with associative contact arrows mappings.

The isometry of metric spaces will be example of such isomorphism for
$\VV$-enriched categories. We shall remark that for
morphism of $\VV$-enriched categories
such property of isometry is  more weak than  to be isomorphic.

We append  some theoretical constructions which will provide more insight
about the set of natural or continuous transforms.
We shall use  a translation $\VV\doublerightarrow \Set$
of values category to the category of sets. The image will be called
a ^{pointed =category}. We shall denote it as
an exponential space over final object
$\VV^*$.
For the ^{=object} $r\in \VV_0$ we take the set of its ^{=points}
$$r^*= \lbrace *\rightarrow r\rbrace\tsk$$
A point is understood as a mapping from category's final object.
For the mapping $u:a\rightarrow b $ between the objects $a, b\in \VV_0$
we get a mapping between the sets of points $u^*: a^*\rightarrow b^*$.
$$\matrix { * & & \cr
       \downarrow  & \searrow & \cr
       a &\maprightap u & b \cr}$$
\vskip\tarpas
For a point $*\rightarrow a$ it appoints another point
$*\rightarrow b$. Obviously such appointing of mappings
maintains an identity arrow and composition of arrows, therefore we get
indeed a functor $\VV\doublerightarrow \Set$.

For the biproduct $r\otimes s$ the points  will be defined by biproduct
of correspondent mappings
$$*=\rightarrow * \otimes * \rightarrow r\otimes s \tsk$$
So we get a mapping of points
$$r^*\times s^*\rightarrow (r\otimes s)^*\tsk$$
For two mappings between the objects $u: a\rightarrow a'$ and
$v: b\rightarrow b'$ we get a biproduct $u\otimes v: a\otimes b\rightarrow
a'\otimes b'$.  Correspondingly for points $*\rightarrow a$
and $*\rightarrow  b$ we get the point in the biproduct
$*\rightarrow *\otimes * \rightarrow a\otimes b$. So we defined the mapping
$a^*\otimes b^*\rightarrow (a\otimes b)^*$
from the product of points sets $a^*\times b^*$ to the set of points in
the biproduct of objects $(a\otimes b)^*$.

We have got a ^{=natural  translation} with isomorphic comparison arrows
$$t_{a,b}: r^*\otimes b^* =\rightarrow (r\otimes t)^*\tsk$$
In the  final object $*\in\VV_0$ we get the  unique point $*\rightarrow *$,
The onepoint set is a final in the category of sets $\Set$,
therefore the translation of pointed category maintains the final object.

For the partial category of ^{Birkhoff =algebras}
in the category of sets $\Set$
the final object will be onepoint set and for each such algebra $X\in \Set_0$
the points coincide with members of the  set carrying this algebra.
Every transport of algebras is defined by some mapping between the carrying
sets.  So we get
that functor of pointed category is identic for this category.

In the category of Banach spaces $\Ban$ the objects are Banach spaces with arrows
being nonexpanding linear mappings
$u: X\rightarrow Y$
$$|u(x)|\mzl |x| \tsk$$
The final object will be any $1$-dimensional space $x\cdot \VR$ with
norm $|x|\mzl 1$.
So the points in Banach space $X$ will be any $1$-dimensional subspace
$x\cdot \VR$ with the points $x$ of unit ball $|x|\mzl 1$.
The set of points of Banach space for the category of nonexpanding linear
mappings
can be identified with the unit ball
$$X^*= \lbrace x\in X: |x|\mzl 1\rbrace \subset X\tsk$$
However in bigger category of arbitrary bounded linear
mappings  $u: X\rightarrow Y$ the points of Banach space will coincide
with the whole  space $X^*= X$.

For us will be interesting to note that in the scalar category
$[0,\infty]^+$ we have the  final
object $0\in [0;\infty]$  and only  one  point
$0\dgl 0$.

In the category of graphs $\Grph$ the final object will be the graph
with  the unique vertex and the unique  edge. For another graph $X$ all vertexes
$x\in X_0$ with some loop  $x\rightarrow x$ defines some points. If we have
different loops, we shall have different points with the same vertex.

The situation will be simpler in the category $\OGrph$  of
original graphs with their transports.
The original graphs transport must maintain chosen unit arrows,
so the points coincide with the vertexes of taken graph
$$(X^*)_0=X_0\tsk$$

The transform $\alpha: S\rightarrow T$ between
two parallel graphs transports $S, T: X\doublerightarrow Y$
is defined by collection of edges  $$\alpha_a\in Y( S_0(a);T_0(a))\tsk$$
The transform between two points $a,b:*\doublerightarrow X$
will be defined by one edge $\alpha\in (X(a;b)$.
And all edges are possible. So we get the same graph
$$X^*= X\tsk$$

For $\VV$-enriched graphs $X$ we haven't any particular transform
between two $\VV$-graphs transforms. We have  defined only the set  of
 transforms between two graphs transports $\phi,\psi: X\doublerightarrow Y$
 $$Y^X(\phi;\psi)= \Prod_{a\in X_0} Y(\phi_0(a);\psi_0(a))\tsk$$

The compromise is achieved by defining $\two$-category over
$\Grph_{\VV}$.  Between parallel
graphs transports $\phi,\psi: X\doublerightarrow Y$ we are chosen
the particular transforms. We understand the
$2$-category  only as possibility to define order relation in the set
 of parallel graphs transports $\Grph_{\VV} (X;Y) $.
The transform will be defined
by arbitrary collection of edges in the target space
$$\alpha= \Prod_{a\in X_0} \alpha_a(*)\subset \Prod_{a\in X_0}
Y(\phi_0(a);\psi_0(a))\tsk$$

The final object in the category of $\VV$-graphs $\Grph_{\VV}$
will be arbitrary onepoint set with unique edge $*\in \VV_0$.
For original $\VV$-graph $X$ we again have the same set of vertexes
$$(X^*)_0= X_0\tsk$$
The edge between two points $a\in\VV_0$ and $b\in\VV_0$ will be a transforms
between corespondent original $\VV$-graphs transports $a: *\doublerightarrow X$
and $b:*\doublerightarrow X$. It is defined by some edge $\alpha\in X(a;b)$.
We get a new graph.                              
For an original $\VV$-graphs transport between two
original $\VV$-graphs  $f: X\doublerightarrow Y$
we get mapping of  particular edge between two points $\alpha\in X(a;b)$
to the new edge between new points
$$f(\alpha)\in Y(f_0(a);f_0(b))\tsk$$

So we get superfunctor $\OGrph_{\VV} \superrightarrow \OGrph$
defined by translation of pointed category $\VV\doublerightarrow \VV^*$.
Appointed new graph  will be called an ^{=underlying graph}.

With translation of underlying category $\VV\doublerightarrow \VV^*$
we get a new $\VV^*$-graph  $X^* $ with the same vertexes $X^*_0= X_0$
but remaining only points in edges sets
$$X^*(a;b)= \lbrace *\rightarrow X(a;b)\rbrace\tsk$$
For $\VV$-graphs transport $f: X\doublerightarrow Y$ we get mappings
in the category of sets
$$(f^*)_{a,b}: X(a;b)^*\rightarrow Y(f_0(a);f_0(b))^*\tsk$$

The using of such notation could be dangerous, but it will be useful for us.
Therefore we used two different names for these different situations.

The set of all
transform  $\alpha: f\rightarrow g$ between two parallel $\VV$-graphs transports
$f: X\doublerightarrow Y$ and $g: X\doublerightarrow Y$ will be defined
by collection of chosen edges
$$\alpha_a (*)\subset Y(f_0(a);g_0(a))\uparrow a\in X_0\tsk$$

Let we have  $\VV$-graph $Y$ with contact arrows mappings defining
functor over pullbacked biproduct
$$\circ : Y\otimes_p Y \doublerightarrow Y\tsk$$
Then we get the  postevaluation functor
$$\ev_Y^-: X\otimes Y^X \doublerightarrow Y$$
defined with postcontact arrows mappings
$$ \ev_Y^-:  X(a;b)\otimes Y^X(\phi;\psi) \rightarrow
Y(\phi_0(a);\psi_0(a)) \circ\psi( X(a;b)) \subset Y(\phi_0(a);\psi_0(b)) \tsk$$
Also we have the preevaluation  functor
$$\ev_Y^+: X\otimes Y^X \doublerightarrow Y$$
defined with precontact arrows mappings
$$\ev_Y^+: X(a;b) \otimes  Y^X(\phi;\psi)\rightarrow \phi(X(a;b)) \circ
Y(\phi_0(b);\psi_0(b)) \subset Y(\phi_0(a);\psi_0(b))\tsk$$



In the values category $\VV$
for arbitrary objects $p\in\VV_0$ and $r\in\VV_0$
we have defined an  exponential space $r^p\in \VV_0$
Using contact arrows mappings in any object $r\in\VV_0$
we have defined  also contact arrows mappings between exponential spaces
$$q^p\times r^q\rightarrow r^p\tsk$$

The underlying graph coincides with taken  values category
$$[p;r]^*= \VV(p;r)\tsk$$
In \baf G. Kelly 1982* p. 14 author uses   also the
equality
$$p = [*;p ]\kbl$$
i. e. every object can be get as exponential space over the set of its
points.
It is fulfilled in the scalar category $[0,\infty]^+$
$$p= (p-0)^+\tsk$$
But it isn't universal even in monoidal closed categories.
So we shall try to apply such property more carefully.

We demanded isomorphic arrow for the right projection
$\rho: *\otimes p \rightarrow p$.
For almost coadjoint biproduct the inverse arrow will be provided
as a biproduct with the uniquely defined arrow to the final object
 $*\in \VV_0$
 $$p\mapright ! *\tsk$$
Then we can get an arrow begun with diagonal arrow
$$p\rightarrow p\otimes p \mapright !\otimes 1_p * \otimes p\tsk$$

In values category $\VV$ we have associative composition of arrows,
therefore the  isomorphic arrow $\pi : *\otimes r \rightarrow r$ provides a natural
transform of representable characters defined with collection of
arrows set mappings
$$\alpha_a: \VV(a; *\otimes p) \rightarrow \VV(a;p) \tsk$$
We need to check that such natural transform is bijective. The inverse natural
transform will be defined with inverse arrows
$$\beta_a : \VV( a;p) \rightarrow \VV(a;*\otimes p) \tsk$$
In values category we can apply associative property for arrows composition.
So we get commuting diagrams for arbitrary arrow $f\in \VV(a;x)$
$$\matrix { x & \mapright \theta_x  & *\otimes x & \mapright \pi_x  & x \cr
\mapupk f &\nearrow  & \mapupd 1_*\otimes f  &\nearrow  & \mapupd f \cr
a &\maprightap \theta_a & *\otimes x & \maprightap \pi_a  & a \cr }$$
\vskip\tarpas
Also we have commuting diagram for arbitrary arrow
$g: a\rightarrow *\otimes x $.

We continue with introduction some notion which were essential
for G. Kelley way of proving Yoneda lemma for $\VV$-enriched categories.

A natural transform  $\alpha: F\rightarrow g$ between two graphs transports
$f, g X\doublerightarrow Y $ is defined with collection of
edges  $\alpha_a\in Y(f_0(a);g_0(a))\uparrow a\in X_0$  and
demands commuting diagram for each edge
$u\in X(a;b)$
$$\matrix { f_0(a) & \mapright  \alpha_a & g_0(a) \cr
  \mapdownk f(u) & & \mapdownd g(u) \cr
     f_0(b) & \maprightap \alpha_b & g_0(b) \cr} $$
\vskip\tarpas
A natural transform  between two $\VV$-graphs  transports needs more
sophisticate definition. Such transform is defined by taking some edges
as mappings from  final object of values category $*\in \VV_0$
$$*\mapright \alpha_a Y(f_0(a);g_0(a))\tsk$$
Now we demand the commuting diagrams

$$\matrix{
&*\otimes X(a;b) & \mapright \alpha_a\otimes g &
Y(f_0(a);g_0(a))\otimes Y(g_0(a);g_0(b)) &  \cr
 &\nearrow   & &\hfill \searrow \circ\hskip -20 pt& \cr
\hfill X(a;b) \hskip -10pt &  & & &\hskip -20pt  Y(f_0(a);g_0(b)) \hfill \cr
& \searrow & & \hfill\nearrow \circ \hskip -20 pt& \cr
 &X(a;b)\otimes * & \maprightap f\otimes \alpha_b &
Y(f_0(a);f_0(b))\otimes Y(f_0(b);g_0(b)) &  \cr } $$
\vskip\tarpas
We shall rewrite such diagram more compactly.

$$\matrix{ X(a;b) & \mapright g & Y(g_0(a);g_0(b)) \cr
 \mapdownk f & & \mapdownd Y(\alpha_a;1) \cr
 Y(f_0(a);f_0(b)) & \maprightap Y(1;\alpha_b)  &Y(f_0(a);g_0(B)) \cr}$$
 \vskip\tarpas

The mapping $Y(1;\beta): Y(x;y)\rightarrow Y(x;z) $
is defined as changing of target space with an edge $\beta:*\rightarrow
 Y(y;z)$
$$\beta_*: Y(x;y)\rightarrow Y(x;y)\otimes * \mapright {1\otimes \beta}
Y(x;y)\otimes Y(y;z) \mapright {\circ} Y(x;z)  \tsk$$

The mapping $Y(\alpha;1): Y(y;z)\rightarrow Y(x;z)$
is defined as changing of source space with an edge
$\alpha:*\rightarrow Y(x;y)$
$$\alpha^*: Y(z;z)\rightarrow  *\otimes Y(y;z)\mapright \alpha\otimes 1
Y(x;y)\otimes Y(y;z)\mapright {\circ} Y(x;z)\tsk$$


 Between two  $\VV$-graphs transports
$X(-;x), F: X^\op \doublerightarrow \VV^e $  the set of natural transforms
is defined as an  exponential space of natural
transforms  $K= F^{(X(-;a)) }$
identified with the equalizer as partial object within the space of all
transforms between taken functors
$$\rightarrow K \rightarrow \Prod_{a\in X_0} [X(a;x);F_0(x)]
\tworightarrows \Prod_{a,b\in X_0} [X(a;x); F_0(b)]^{X^\op(a;b)}\tsk$$
The two   mappings were defined as names  for
postevaluation and preevaluation  mappings with the set of edges
 $  X^\op(a;b)$
$$ X^\op(a;b) \otimes
\Prod_{a\in X_0} [X(a;x);F_0(a)] \rightarrow [X(a;x);F_0(a)]\cdot  F_{a,b} (X^\op(a;b))\kbl$$
$$ X^\op(a;b)\otimes \Prod_{a\in X_0} [X(a;x);F_0(a)]
\rightarrow [X(a;x);X(b;x)] \cdot [X(b;x); F_0(b)]\tsk$$
% \subset [X(a;x);F_0(b)] \tsk$$
Such equalizer categorically is
expressed as an end for the  ^{=bifunctor}
$$T(a,b)= [X(-;x);K]:X^\op \times X
\doublerightarrow \VV^e\kbl$$
 clr.  \baf S. MacLane 1971*
part IX. Special limits. It is a partial object embedded
in the product of all values $T(a,a)$
$$\rightarrow \int_{a\in X_0} T(a,a)\rightarrow \Prod_{a\in X_0} T(a,a)
\tworightarrows
\Prod_{a,b\in X_0} T(a,b)^{X^\op(a;b)} \tsk$$
A bifunctor
$T: X^\op \times X \doublerightarrow \VV^e $
is defined by mapping over the set of vertexes
$$T(a,b)= \VV( X(a;x); F_0(b))$$
and is a $\VV$-graphs
  functor for each argument. In our case one functor is
$$T(a,-): X^\op\doublerightarrow \VV^e $$
with edges set mappings
$$ X^\op(a;b)\rightarrow [X(a;x);F_0(a)]\cdot F_{a,b} (X^\op(a;b))
\subset [X(a;x);F_0(b)]$$
We express such mappings with a diagram
$$\matrix {  X(a;x) & \rightarrow & F_0(a)\hphantom { ^{X^\op (a;b)}} \cr
    &\searrow & \mapdownd  X^\op(a;b) \cr
    & & F_0(b) \hphantom{ ^{F^\op(a;b)}} \cr}$$
\vskip\tarpas
The  contact arrows mappings in original $\VV$-graph $\VV^e$
was defined as predecomposable form
$$q^p \otimes r^q \rightarrow q^p\cdot r^q \subset r^p $$
so we get
 a postdecomposable form
$$X^\op(a;b)\otimes T(a,a)\rightarrow T(a,a)\cdot F_{a,b} (X^\op(a;b))
\subset T(a,b)$$ and its name form
$$\sigma_{a;b} : T(a,a) \rightarrow T(a;b)^{X^\op(a;b)} \tsk$$
Another functor is
$$T(-,b) : X\doublerightarrow \VV^e$$
with edges set mappings
$$ X^\op (a;b)\rightarrow [\bigcirc \circ X(a;x);X(b;x)]\cdot
[X(b;x);F_0(b)]
\subset [X(a;x);K_0(b)]$$
We express such mappings with a diagram

$$\matrix{ \hphantom { ^{X(a;b)}}X(a;x) &  & \cr
  \mapdownk X^\op(a;b)  & \searrow  &\cr
  \hphantom{ ^{X(a;b)}} X(b;x) & \rightarrow & F(b)\cr }$$
\vskip\tarpas
It defines another predecomposable form
$$X^\op(a;b)\otimes T(b,b) \rightarrow
[\bigcirc \circ X(a;x);X(b;x)]\cdot T(b,b) $$
with its name form
$$\rho_{a,b}: T(b,b)\rightarrow T(a,b)^{X^\op(a;b)} \tsk$$

So the end $K$ will be defined as initial object
for all commuting diagrams
$$\matrix{\searrow &  & & \cr
 & K &\mapright \lambda_a & T(a;a)\cr
&\mapdownk \lambda_b  & &\mapdownd \rho_{a,b} \cr
&T(b,b) & \maprightap \sigma_{a,b} & [X^\op(a;b);T(a,b)]\cr}$$
\vskip\tarpas

For the postdecomposable form
$$X^\op (a;b)\otimes T(a,a)  \rightarrow T(a,b)$$
we have bijection between ^{=dual  name forms} defined as mappings
$$ T(a,a)\rightarrow [X^\op (a;b);T(a;b)]\kbl
X^\op (a;b) \rightarrow [T(a,a) ;T(a,b)] \tsk$$
Such bijection exists even without existence of
predecomposable or postdecomposable
form as a functor over biproduct $ X^\op(a;b)\otimes T(a,a)$.
For name forms  we need to have only partial forms of
arbitrary  bifunctor
$$T: X^\op(a;b)\times  T(a,a)\doublerightarrow T(a,b)\tsk$$
However for the next property existence of predecomposable or postdecomposable form
is essential.

We shall check that a triangular diagram for source changing
between the name mappings
$$\matrix { K & \mapright \lambda_a &   T(a,a) \cr
  & { _{\phi_1}} \searrow &\mapdownd \psi_1 \cr
  & &[ X^\op(a;b);T(a,b)]\cr } $$
provides the triangular diagram for target changing
between the dual name mappings
$$\matrix { X^\op(a;b )& \mapright \psi_2 & [T(a,a);T(a,b)] \cr
  & { _{\phi_2}} \searrow & \mapdownd  [\lambda_a; 1_{T(a,b)}] \cr
  & & [K;T(a,b)] \cr }$$
\vskip\tarpas
and vice versa.

\Proposition
Let we have a pair of dual name forms provided by a pair of predecomposable
forms. Then an existing source changing
between name forms
provides the target changing
 for the dual name forms. And vice versa an existing target changing
between  name forms  provides the source changing  for the dual name forms.
\Proof:
Let  we have a pair of predecomposable forms
$$\phi:  X(a;b)\otimes K \rightarrow T(a;b)\kbl
\psi: X(a;b)\otimes T(a,a) \rightarrow T(a,b) \tsk$$
If  we have source changing transform  $\theta: K\rightarrow T(a,a) $
between name forms

$$\matrix{ K  & \mapright {\theta} & T(a,a) \cr
 & _{\phi_1} \searrow & \mapdownd  \psi_1  \cr
& & [X(a;b); T(a,b)] \cr }$$
\vskip\tarpas
then we get the source changing transform between predecomposable forms

$$\matrix{ X(a;b) \otimes K & \mapright 1_{X(a;b)}\otimes \phi_1  &
 X(a;b)\otimes [X(a;b);T(a,b)] &\hskip -10pt
 \mapright \ev_{T(a,b)} & \hskip -15pt T(a,b) \cr
\mapdownk {1_{X(a;b)}\otimes \theta}
& \nearrow & { _{1_{X(a;b)}\otimes \psi_1}} &  & \cr
X(a;b) \otimes T(a,a) & & & & &\cr }$$
\vskip\tarpas
For the dual name forms we get commuting diagram

$$ \matrix{ &  & [T(a,a) ; T(a,a)\otimes X(a;b) ] &
\mapright [1_{T(a,b)};\psi]
&T(a,a); T(a,b)] \cr
& { ^{\lambda_{X(a;b)}}} \nearrow
& \mapdownk  [\theta;1_{T(a,a)\otimes X(a;b)}]   &
&\mapdownd [\theta;1_{T(a,b)}]  \cr
X(a;b) & & [K;T(a,a)\otimes X(a;b)] &
\mapright [1_K;\psi] & [K;T(a;b)] \cr
& _{\lambda_{X(a;b)}}   \searrow  & \mapupk [1_K;\theta\otimes 1_{T(a,b)}]
 & \nearrow  {  _{[K;\phi]}} & \cr
& & [K; K\otimes X(a,b)] & & \cr } $$
\vskip\tarpas
Otherwise for the target changing of dual name mappings

$$\matrix { X(a;b) & \mapright \psi_2 & [ T(a,a) ; T(a,b)] \cr
 &  _{\phi_2} \searrow & \mapdownd [\theta;1_{T(a;b)}]  \cr
& & [K;T(a,b)\cr }$$
\vskip\tarpas
we get the source changing of predecomposable forms

$$\matrix{ T(a;a)\otimes X(a;b) & \mapright 1_{T(a,a)}\otimes \psi_2
& T(a,a) \otimes [T(a,a);T(a,b)] &   &   \cr
\mapupk  \theta\otimes 1_{X(a;b)}  &
& \mapupk \theta\otimes 1_{[T(a,a);T(a,b)]} &
\hskip -5pt \searrow { ^{\ev_{T(a,b)}}} \cr
K\otimes X(a;b) &  \mapright 1_K\otimes \psi_2 & K\otimes [T(a,a);T(a,b)] & &
T(a,b) \cr
& { ^{\phi_2}} \searrow  & \mapdownk 1_k\otimes [\theta;1_{T(a,b)}] &
\hskip -5pt  \nearrow { _{\ev_{T(a,b)}}} & \cr
& & K\otimes [K;T(a,b)] & & \cr}$$
\vskip\tarpas
This produces the source changing transform between  dual name forms

$$\matrix{ K & \mapright \lambda_K & [X(a;b); K \otimes X(a;b)] &
\mapright {\phi} & [X(a;b);T(a,b)] \cr
\mapdownd {\theta}  &  & \mapdownd [1_{X(a;b)};\theta\otimes 1_{X(a;b)}]
&\nearrow { _\psi}  & \cr
T(a,a)  & \maprightap \lambda_{T(a,a)} & [X(a;b);T(a,a)\otimes X(a;b)]  & &\cr}
$$
\vskip\tarpas
We must remark  that for the  dual name forms we used the dual
sections arrows
$$\lambda_K : K\rightarrow [X(a;b); K\otimes X(a;b)]\kbl$$
$$\lambda_{T(a,a)} : T(a,a) \rightarrow [X(a;b); T(a,a)\otimes X(a;b)] \tsk$$
Also we used  the dual evaluation arrows
$$\ev_{T(a;b)} : [X(a;b) ; T(a;b)\otimes X(a;b)]\rightarrow T(a;b) \tsk$$
\irodymopabaiga

As a consequence we get a correspondence between commuting diagrams.
The commuting diagram of name mappings 

$$\matrix { K & \mapright \lambda_a &   T(a,a) \cr
\mapdownk \lambda_b   & \searrow &\mapdownd \sigma_{a,b} \cr
T(b,b)  &\maprightap \rho_{a,b}  &[ X^\op(a;b);T(a,b)]\cr } $$
provides also the commuting diagram between  dual name mappings

$$\matrix { X^\op(a;b )& \mapright \bar \sigma_{a,b} & [T(a,a);T(a,b)] \cr
\mapdownk \bar\rho {a,b}  & \searrow & \mapdownd  [\lambda_a;1_{T(a;b)}] \cr
[T(b,b);T(a,b)] &\maprightap [\lambda_b;1_{T(a,b)}] & [K;T(a,b)] \cr }$$
\vskip\tarpas
and vice versa.
\vskip\tarpas


%Uýbaigiau traukõ callatice/oneda.teû


==> oneda.tex <==
%2022.11.13 Pradójau traukõ clattice/oneda.tex
\vskip\tarpas
We shall try to recognize $\VV$-graphs for some concrete values categories.
For the category of small sets $\Set$  we get usual graphs.
The $\Set$-enriched graph will be arbitrary  graph $X$ with small edges sets
$X(a;b)$. So we get an original graphs or categories. The $\Set$-graphs
transport  $f: X\doublerightarrow Y$ will be transport
of usual graphs with edges set mappings
$$f_{a,b} : X(a;b) \rightarrow Y(f_0(a);f_0(b))\tsk$$
So all properties of $\Set$-enriched graphs or categories can be
verified for usual graphs or categories.
For the functors of  categories  $\phi,\psi: T\doublerightarrow Y$
we get the same set of natural transforms $Y^{(T)}(\phi;\psi)$.
These sets defines an exponential superfunctor $Y^{(T)}$
which is coadjoint to the superfunctor defined with biproduct  $X\otimes T$.

More interesting opportunities are provided by a larger
values category $\Cat$.
The points of such category   will be categories. They will be
denoted by hind Latin letters $p, q, r, s,t\in  \Cat_0$.
Further the points in such categories will be denoted $u,v, x, y,z\in p_0$.
In the category $\Cat$ the  arrows $f:p\rightarrow q$ will be functors
between such categories.
They will be denoted by fore Latin letters $f, g, h, k\in\Cat$.
The usual composition of functors defines the appointment
$$f\circ g\in  \Cat(p;q\uparrow \lan f,g\ran  \in \Cat(p;q)\times \Cat(q;r)$$
over ^{pullbacked =product}
$$\Cat\times_{\Cat_0} \Cat = \lbrace \lan f,g\ran: p_2(f)=p_1(g)
\rbrace \subset  \Cat\times \Cat\tsk$$
The identity functors are ^{neutral =arrows} for the  source and
the target of arrows
$$\Identity_p\circ f=f =f\circ \Identity_q \uparrow f\in \Cat(p;q) \tsk$$

The arrows from $\Cat(p;q)$ will be called parallel. For parallel
arrows we can define order relation with existing natural transform
between functors
$$\alpha: f\rightarrow g \uparrow f,g\in \Cat(p;q)\tsk$$
The natural transforms will be denoted by initial Greek letters $\alpha,
\beta, \gamma,\theta $.
We shall say $f\dgl g$ if exists a natural transform $\alpha: f\rightarrow g$.
For functors between categories it is possible to construct concrete
natural transforms, but we shall work with notion of continuity which
uses only order relation between parallel functors
defined by existing natural transform.

We choose Carte tensor product of categories as a  biproduct
$$ p\otimes q:= p\times q\tsk$$
The final category with unique point $*=\lbrace O\rbrace$ will be a
^{neutral  =point} for such biproduct, i. e.
we have uniquely defined canonical isomorphisms  of biproducts
$$*\otimes r= r= r\otimes * \tsk$$
We have an expression of functors to the  product of categories
$$\Cat (p;q\otimes r) \rightarrow \Cat (p; q)\times \Cat(p;r)\tsk$$

The Carte product of natural transforms
$\alpha:f\rightarrow g\uparrow f,g\in \Cat(p;q)$
and $\beta: h\rightarrow k\uparrow h,k\in \Cat(p;r)$
provides the natural transform between the functors  to
the Carte  product  of target spaces
$$\alpha\times \beta: f\times h\rightarrow g\times k \uparrow
\lan  f\times h\ran, \lan g\times k\ran \in \Cat(p;q\times r ) \tsk$$
This shows that  the biproduct of categories $p\times q $ defines
monotone bisuperfunctor.
For a natural transform $\alpha: f\rightarrow g$ between two functors
$f,g\in \Cat (p;q)$ we get the natural transform between biproducts
of these functors with any functor $h\in \Cat(r;s)$
$$\alpha\times 1_h: f\times h\rightarrow g\times h\tsk$$
Also  for a natural transform $\beta: h\rightarrow k$ between two functors
$h,k\in\Cat (r;s)$ we get the natural transform between biproducts  of these
functors with any functor $f\in\Cat(p;q)$
$$1_f\times \beta: f\times h\rightarrow f\times k \tsk$$

The same is true for arbitrary Carte product of categories
$$\Prod_u r_u\tsk$$
It defines monotone superfunctors with edges set mappings
 $$\Prod_u \Cat(p;r_s) \superrightarrow
  \Cat(p;\Prod_u r_u) \tsk$$

The chosen biproduct  $r\otimes s$
with an assistant category $s\in \Cat_0$  defines a superfunctor
within the $\Cat$. For a functor $f\in  \Cat ( p;r)$ we  shall  appoint the
biproduct with identity functor $\Identity_s\in \Cat(s;s)$
$$f\otimes \Identity_s\in \Cat (p\otimes s;r\otimes s)\tsk$$

Such superfunctor will be adjoint one. The coadjoint superfunctor is
provided by an  exponential space
 of natural transforms
$p^s(\phi;\psi)$.  The exponential space of natural transforms
$p^s$ is a category on the set of parallel functors
$\Cat(s;p)= (p^s)_0 $ having as arrows
natural transforms $\alpha: \phi\rightarrow \psi$ between  some functors
$\phi;\psi\in \Cat(s;p)$.
In  such category we take the ^{vertical =composition}  of natural
transforms
$$\alpha\circ \beta: f\rightarrow h\uparrow \alpha: f\rightarrow g,
\beta :g\rightarrow h \tsk$$
The identity transforms $\Identity_f: f\rightarrow f$ will be
^{neutral =units} for such composition
$$\Identity_f\circ \alpha= \alpha= \alpha\circ \Identity_g
\uparrow \alpha: f\rightarrow g\tsk$$

The exponential space $p^s$ indeed defines a superfunctor. It for a  functor
$f\in \Cat(p;q)$ appoints the changing of target space $f^s\in\Cat(p^s;q^s)$.
As usually it maintains the  identity functor
and  the composition of functors.

 We have another ^{horizontal =composition} of natural transforms
$$\alpha\ast\alpha': f\circ h \rightarrow g\circ k \uparrow
\alpha: f\rightarrow g, \alpha': h\rightarrow k \tsk$$
It will be a bifunctor over the exponential spaces of natural transforms
$$\ast\in \Cat (q^p\times r^q; r^p ) \tsk$$
Indeed. We have ^{=middle four exchange} equality for both vertical and
horizontal  compositions of natural transforms
$$(\alpha\circ\beta)\ast( \alpha'\circ\beta') = (\alpha\ast\alpha')
\circ (\beta\ast \beta')\tsk$$
Therefore we have commuting diagram
$$\matrix{ (q^p\times r^q)\times (q^p\times r^p ) &
\mapright{\ast\times \ast} &r^p\times r^p \cr
\mapdownk {\circ } & & \mapdownd {\circ} \cr
q^p\times r^q & \maprightap {\ast} & r^p \cr}$$
That means that horizontal composition is  graphs transport
natural  for vertical composition.
Also it maintains identity transforms
$$\Identity_f \ast \Identity_h = \Identity_{f\circ h} \tsk$$
So horizontal composition is a natural functor over Carte tensor product
 of categories  $ q^p\times r^q $ with vertical composition of arrows.

We are ready to prove that superfunctor of exponential space $p^s$
is monotone for the weaker  order relation  in   exponential space $r^s$
defined between ^{secondarily =parallel functionals}.If  we have
an inequality  between primarily parallel functors
$$f\dgl g: p\rightarrow  r$$ we get the inequality between secondarily
parallel functionals  $f^s,g^s: p^s\rightarrow r^s $.
We have coinciding secondarily projections  for changing of target space
$$(f_0)^{s_0}=(g_0)^{s_0}: (p_0)^{s_0}\rightarrow (r_0)^{s_0}\kbl$$
i. e. for arbitrary  functor $\phi \in p^s$ we have the equality
of composition
$$\phi_0\circ f_0= \phi_0\circ g_0\tsk$$
Also we get the inequalities of arrows set mappings
$$(\phi\circ f)_{u,v}\dgl (\phi\circ g)_{u,v}\uparrow u,v\in s \kbl$$
$$ f^s_{\phi;\psi}\dgl g^s_{\phi,\psi}
\uparrow \phi,\psi\in p^s\tsk$$
For a functor $\phi\in \Cat(s;p)$ the changing of target space with functor
$f\in \Cat(p;r)$ appoints the new functor $\phi\circ f\in \Cat(s;r)$,
or the changing of target space with another functor
$g\in \Cat(p;r)$  appoints
another new functor $\phi\circ g\in\Cat(s;r)$.
The horizontal composition  $1_\phi\ast \alpha: \phi\circ f\rightarrow
\phi\circ g$  provides needed natural transform for the first inequality.
This can be understood as transferred natural transform by source functor
$\phi\star \alpha$. For each point $u\in s_0$ it produces the arrow
in the target category $r$
$$\alpha_{\phi_0(u)}\in r(f_0(\phi_0(u));f_0(\psi_0(u)))$$
with commuting diagram  for arrows in assistant category $\theta\in s(u;v) $
between the
points $u,v\in s_0$
$$\matrix{  f_0(\phi_0(u)) &\mapright \alpha_{\phi_0(u)} & g_0(\phi_0(u))\cr
\mapdownk f(\phi(\theta))  & & \mapdownd f(g(\theta)) \cr
f_0(\phi_0(v)) &\maprightap \alpha_{\phi_0(v)} & g_0(\phi_0(v))\cr}$$

So the collection of these arrows $\alpha_{\phi_0(u)}\uparrow u\in s_0$
provides a natural transform $\phi\times\alpha_u: \phi\circ f\rightarrow
\phi\circ g$ between two functors $\phi\circ f,\phi\circ g\in (r^s)_0$,
i. e. an arrow in exponential space of natural transforms
$$\phi\star \alpha \in r^s(\phi\circ f;\phi\circ g) \tsk$$
The collection of such arrows defines the transform between two
functors defined by changing of target space
$\alpha^s: f^s\rightarrow g^s $.
We need to check that this transform is natural for the arrows in
the category $p^s$,
i. e. for arbitrary natural transforms $\theta: \phi\rightarrow \psi$
between two functors $\phi,\psi\in \Cat(s;p)$ we have commuting diagram
$$\matrix{\phi\circ f & \mapright  {\phi\times \alpha} & \phi\circ g \cr
\mapdownk \theta\star f & & \mapdownd\theta\star g \cr
\psi \circ f  &\maprightap { \psi\times \alpha } &\psi \circ g \cr}$$
\vskip\tarpas
This can be proved by equalities
$$(\phi\star \alpha)\circ ( \theta\star g)=
(1_\phi\ast \alpha ) \circ (\theta\ast 1_g)= $$$$
(1_\phi\circ \theta)\ast (\alpha\circ 1_g)=
\theta \ast \alpha \tsk$$
                                          
For each point $x\in p_0$ in the  category $p$ we have chosen a unit arrow
$1_x\in p(x;x)$, so we can define the sections functor
$\lambda_p\in \Cat(p;(p\otimes s)^s)$
and the name appointment
$$\Cat(p\otimes s; r) \rightarrow \Cat(p; r^s)$$
provided by composition of functors
$f^\#=\lambda_p\circ f^s$.

We can  check
that the name appointment
remains  monotone for the weaker order relation  in exponential space  $r^s$
defined with natural transforms
between secondarily parallel functors.

For a point $x\in p_0$ we get the section $\lambda_p(x)\in (p\otimes s )^s$
which   has edges set mappings
$$s(u;v)\rightarrow \lambda_p(x)(s(u;v))= 1_x\otimes s(u;v)\subset
p(x;x)\otimes s(u;v)  \tsk$$
The changing of target space with functor $f\in \Cat(p\otimes s;r)$
provides the
functor $\lambda_p(x)\circ f\in \Cat(p;r^s)$ with edges set mappings
$$s(u;v) \rightarrow f_{\lan x,u\ran,\lan x,v\ran} (1_x\otimes s(u;v))
\subset r(f_0(x,u); f_0(x,v))\tsk$$
Having a natural transform $\alpha: f\rightarrow g$ we get the
natural transform
$$\lambda_p(x)\times \alpha : \lambda_p(x)\circ f\rightarrow
\lambda_p(x)\circ g\tsk$$
between appointed functors
$\lambda_p(x)\circ f, \lambda_p(x)\circ g\in \Cat (p;r^s)$
with edges set mappings
$$s(u;v) \rightarrow f_{\lan x,u\ran,\lan x,v\ran} (1_x\otimes s(u;v))\dgl $$$$
g_{\lan x,u\ran,\lan x,v\ran} (1_x\otimes s(u;v))\subset
r(g_0(x,u);g_0(x,v))\tsk$$
Otherwise we get a  natural transform also for the  edges set mappings.
For the sections functor $\lambda_p\in\Cat(p;(p\otimes s)^s)$
the edges set mappings will be
$$p(x;y)\rightarrow\Prod_{u\in s_0}  p(x;y)\otimes 1_u \subset
\Prod_{u\in s_0}
p(x;y)\otimes s(u;u)\tsk$$
The changing of target space with
functor $f\in \Cat(p;r)$
provides a new edges set mapping
$$p(x;y) \rightarrow \Prod_{u\in s_0} f_{\lan x,u\ran,\lan y,u\ran} (p(x;y)
\otimes 1_u)\subset r(f_0(x,u);f_0(y,u))\kbl$$
and a  natural transform $\alpha: f\rightarrow g$ provides the natural transform
for the edges set mappings $\lambda_p \times \alpha^s:\lambda_p\circ f^s
 \rightarrow \lambda_p\circ g^s$
$$p(x;y) \rightarrow \Prod_{u\in s_0} f_{\lan x,u\ran,\lan y,u\ran} (p(x;y)
\otimes 1_u)\dgl $$$$
\Prod_{u\in s_0} g_{\lan x,u\ran,\lan y,u\ran} (p(x;y)
\otimes 1_u)\subset\Prod_{u\in s_0}  r(g_0(x,u);g_0(y,u))\tsk$$

The composition of arrows in a category $r$
provides the contact arrows, and we get the evaluation functor over exponential space
of natural transforms  $\ev_r\in \Cat (r^s\otimes s;r)$.
The composition with this functor
$$g^\flat =(g\otimes 1_s)\circ \ev_r \in \Cat(p\otimes s;r)\uparrow
g\in \Cat(p;r^s)$$
provides  the realization of functional
$$\Cat(p;r^s)\rightarrow \Cat(p\otimes s;r) $$
 which is monotone
from the functionals to the  exponential space of natural transforms
with order relation
defined by existing natural transform between the secondarily parallel
mappings to the forms into the target space $r$ with an  order
relation defined by existing natural transform between  (primarily )
parallel  functors.

Let we have two secondarily parallel functors $f,g\in \Cat(p;r^s)$
with  a natural transform   $\alpha : f\rightarrow g$.
defined by  collection of arrows
$$\alpha_x: f_0(x)\rightarrow g_0(x)\uparrow x\in p_0$$
between
functors $f_0(x),g_0(x)\in (r^s)_0$.
We have commuting diagrams for edges set mappings
for  every arrow in source category
$\theta\in p(x;y)$
$$\matrix{ f_0(x) & \mapright \alpha_x & g_0(x) \cr
 \mapdownk f_{x,y}(\theta) & & \mapdownd g_{x,y}(\theta) \cr
f_0(y) & \maprightap \alpha_x & g_0(y) \cr }$$
\vskip\tarpas
They are arrows in the exponential space of natural transforms
$\alpha_x\in r^s$,
so they will be the  natural transforms  between functors,
and they are defined as Carte product of
arrows in the target space $r$
$$\alpha_{x,u}\in r(( f_0(x) )_0(u);(g_0(x))_0(u))\uparrow u\in s_0\tsk$$
These arrows allows the commuting
diagram for any arrow in the source
category $\theta\in p(x;y)$
$$\matrix{(f_0(x))_0(u) & \mapright \alpha_{x,u} & (g_0(x))_0(u) \cr
\mapdownk f_{x,y}(\theta)_u &    & \mapdownd g_{x,y} (\theta)_u   \cr
(f_0(y))_0(u) & \maprightap \alpha_{y,u} & (g_0(y))_0(u) \cr}$$
\vskip\tarpas

For a  couple of arrows $\theta\in p(x,y)$ and $\kappa\in s(u;v)$
the evaluation functor $\ev_r \in \Cat(r^s\otimes s;r)$ can be defined by
precontact or
postcontact arrows
 $$\matrix { f_0(x,u) & \mapright f_0(x)_{u,v}(\kappa)  & f_0(x,v)\cr
\mapdownk f_{\lan x,u\ran, \lan y,u\ran}(\theta) & \searrow & \mapdownd
f_{\lan x,v\ran,\lan y,v\ran }(\theta) \cr
 f_0(y,u) & \maprightap f_0(y)_{u,v}(\kappa) & f_0(y;v) \cr}$$
 \vskip\tarpas

For the precontact arrow we have a
diagram
$$\matrix { f_0(x,u) &  &\cr
\mapdownk f_{\lan x,u\ran, \lan y,u\ran}(\theta) & \searrow &
 \cr
 f_0(y,u) & \maprightap f_0(y)_{u,v}(\kappa) & f_0(y;v) \cr}$$
 \vskip\tarpas
All mappings are arrows in the target category $r$, therefore  we have
for them associative composition, so the commuting transforms
for two arrows will provide commuting transform for their
composition
$$\matrix { f_0(x,u) & \mapright f_{\lan x,u\ran,\lan y,u\ran}(\theta) &
f_0(y,u) & \mapright f_0(y)_{u,v}(\kappa) &  f_0(y,v) \cr
\mapdownk  \alpha_{\lan x,u\ran} & &\mapdownd \alpha_{\lan y,u\ran} &  &
\mapdownd  \alpha_{\lan y,v\ran} \cr
 g_0(x,u) & \maprightap g_{\lan x,u\ran,\lan y,u\ran}(\theta) &
g_0(y,u) & \maprightap g_0(y)_{u,v}(\kappa)  &  g_0(y,v) \cr  }$$
\vskip\tarpas

So we get a natural transform between  the realizations of two functors
$f,g\in\Cat(p\otimes s;r)$, and we have shown that the  realization appointment
 is monotone
$$\Cat(p;r^s) \rightarrow \Cat(p\times s;r ) \tsk$$

Next we shall prefer to  use "small"  terminology. We shall
say that we have a category
$\Cat$ with  points $p\in \Cat_0$ and arrows $f:p\rightarrow q$.
For them we have truly joint pair of monotone  functors. The
adjoint functor defined   with biproduct  $p\otimes s$
is monotone for order relation defined with existing of natural transform
between  the primarily parallel arrows.
The coadjoint functor defined
with exponential space  of natural transforms $r^s$ is monotone
for the order relation defined by existing natural transform
between secondarily parallel arrows in exponential space $r^s$.
 For them we have the  name  appointment
  isomorphic for the order relation defined by existing natural transform
between the primarily parallel
arrows $\Cat(p\times s;r)$ and the secondarily parallel arrows $\Cat(p;r^s)$
in exponential space also defined by natural transform between two
functionals
$$\Cat(p\times s; r)=\rightarrow \Cat(p; r^s)\kbl$$
\vskip\tarpas

Now we shall study the ^{$\Cat$-enriched =spaces}.
 We shall call  the $\Cat$-enriched graph $X$   also as a $\Cat$-graph.
The edges sets between vertexes  $a,b\in X_0$ will be categories
$X(a;b)\in \Cat_0$ and functors between such categories
 will be taken as  mappings.

 The values category $\Cat$ is the first example of $\Cat$-enriched space.
It provides useful experience with new  notions of $\Cat$-enriched spaces.
The enriched $\Cat$-space has another structure as the category $\Cat$ itself.
Therefore we shall use another notation for it $\Cat^e$. The letter $e$
will remind that we are dealing with enriched space.
For arbitrary categories $p,r\in \Cat_0$ we take the  exponential space
as an edges set
$$\Cat^e(p;r) = r^p \in \Cat_0\tsk$$

The set of arrows between two points
$\Cat(p;r)$ defines the structure of $\Set$-enriched space.
We have projection
$$\Cat(p;r)= Cat^e(p;r)_0 \tsk$$

We shall say that these
projections are provided by ^{=translation} of
values category. For $\Cat$-enriched graphs we can also take
arbitrary graphs
transport   $\Cat \doublerightarrow \VV$. For a category $p\in\Cat_0$
the projection to its vertexes set $p_0\in \Set_0$ will define
very simple translation $\Cat\doublerightarrow \Set$ of
$\Cat$-enriched spaces with many good properties,
but we are conscious to know what exact properties we are using in each
investigation's step.

 The $\Cat$-graphs transport $f: X\doublerightarrow Y$ will be defined
by an appointment of vertexes $f_0: X_0\rightarrow Y_0$
and edges set mappings
  $$f_{a,b} : X(a;b)\rightarrow Y(f_0(a);f_0(b))\tsk$$
We get a category $\Grph_{\Cat}$  compounded of all $\Cat$-graphs transports.
Arbitrary graphs transport $D:\Cat\doublerightarrow \VV$
defines the superfunctor of
categories
$$(D):\Grph_{\Cat} \superrightarrow \Grph_{\VV} \tsk$$
For a $\Cat$-enriched graph $X$ it appoint the new
$\VV$-enriched graph  $X^{(D)}$
with the same vertexes and their appointments, and new
mappings for graphs transports  $f^{(D)}:X^{(D)} \doublerightarrow Y^{(D)}$
$$f^{(D)}_{a,b}: X^{(D)} (a,b)\rightarrow Y^{(D)}(f_0(a);f_0(b))\tsk$$

We shall call two $\Cat$-graphs transports $f, g: X\doublerightarrow Y$
^{primarily  =parallel} if they have the same  appointments of vertexes
$f_0=g_0: X_0\rightarrow Y_0$.
For a  primarily parallel $\Cat$-graphs transports
$f,g:X\doublerightarrow Y$
we get an order relation from values category $\Cat$.
For mappings between edges sets
$$f_{a,b}: X (a;b)\rightarrow f_{a,b}(X(a;b))\subset Y(f_0(a);f_0(b))\kbl$$
$$g_{a,b}: X (a;b)\rightarrow g_{a,b}(X(a;b))\subset Y(g_0(a);g_0(b))$$

the inequality
$f_{a,b} \dgl g_{a,b}$ means that we can find some natural transform
$\alpha_{a,b} :f_{a,b}\rightarrow g_{a,b} $ between functors
 of correspondent categories.
We shall  come down to the category $X(a;b)\in \Cat_0$.
For every point $u\in X(a;b)_0$ these functor appoints the couple
of points
$(f_{a,b})_0(u)\in Y(f_0(a);f_0(b))$ and $(g_{a,b})_0(u)\in Y(g_0(a);g_0(b))$
and such natural transform is defined by collection of arrows from category
$Y(f_0(a);f_0(b))=Y(g_0(a);g_0(b))$
$$\alpha_u:(f_{a,b})_0(u)\rightarrow (g_{a,b})_0(u)\uparrow u\in X(a;b)_0$$

We shall define a joint pair of superfunctors within the category
$\Grph_{\Cat}$. First we define biproduct of $\Cat$-graphs
$X\otimes Y$. We take the  Carte tensor product of vertexes sets
$$(X\otimes Y)_0= X_0\times Y_0$$
and biproduct of edges sets
$$X\otimes Y(\lan x,y\ran;\lan x',y'\ran)= X(x;x')\otimes Y(y;y')\tsk$$
The biproduct of $\Cat$-graphs transports $f: X\doublerightarrow X'$  and $
g: Y\doublerightarrow Y' $ will be defined by biproduct of
edges set mappings
$$f\otimes g_{\lan x,y\ran,\lan x',y'\ran}:
X(x;x')\otimes Y(y;y')\rightarrow f_{x,x'} (X(x;x'))\otimes g_{y,y'}(Y(y;y'))
\subset$$$$
 X'(f_0(x);f_0(x')) \otimes Y'(g_0(y);g_0(y'))\tsk$$
Such bisuperfunctor is monotone, as we have monotone biproduct in the values
category  $\Cat$.  We need to check this property only for the edges set
mappings. We shall not be lazy to come down inside  the categories $X(x;x')$
and $Y(y;y')$.

 Between two parallel functors
$f_{x,x'}, f'_{x,x'}
:X(x;x')\rightarrow X'(f_0(x);f_0(x'))$
a natural transform  $\alpha_{x,x'}: f_{x,x'}\rightarrow f'_{x,x'}$
is defined by some collection of arrows
from the category $X'(f_0(x);f_0(x'))$
$$\alpha_u: (f_{x,x'})_0(u)\rightarrow (f'_{x,x'})_0(u)\uparrow u\in
X(x;x')_0\tsk$$

Also a natural transform $\beta_{y,y'}: g_{y,y'}\rightarrow g'_{y,y'}$
between two parallel functors $g_{y,y'}, g'_{y,y'}
:Y(y;y')\rightarrow Y'(g_0(y);g_0(y'))$ is defined by another
collection of arrows
from category $Y'(g_0(y);g_0(y'))$
$$\beta_v: (g_{y,y'})_0(v)\rightarrow (g_{y,y'})_0(v)\uparrow v\in
Y(y;y')_0\tsk$$

The Carte product of such natural transforms will be defined
by collection of arrows couples from the category $X'(f_0(x);f_0(x'))\times
Y'(g_0(y);g_0(y'))$
$$\lan \alpha_u,\beta_v\ran: \lan (f_{x,x'})_0(u),g_{y,y'})_0(v)\ran
\rightarrow \lan (f'_{x,x'})_0(u),(g'_{y,y'})_0(v)\ran  \tsk$$
And it will be a natural transform between biproducts of taken functors
$$\alpha_{x,x'}\otimes \beta_{y,y'} : f_{x,x'}\otimes g_{y,y'}\rightarrow f'_{x,x'}
\otimes g'_{y,y'} \tsk$$
We shall work with a for chosen assistant $\Cat$-graph $T$  defined
 superfunctor.
For a $\Cat$-graph $X$ it appoints the biproduct with the assistant $\Cat$-graph
$X\otimes T$, and
for a $\Cat$-graphs transport $f: X\doublerightarrow X'$  it appoints
the biproduct with identity $\Cat$-graphs transport of the assistant
$\Cat$-graph $T$
$$f\otimes \Identity_{T}: X\times T \doublerightarrow X'\otimes T\tsk$$
We shall take it as an adjoint superfunctor within the category of
$\Cat$-graphs $\Grph_{\Cat}$.

The coadjoint superfunctor will be defined with exponential space $Y^T$
of all transforms  $\alpha: \phi\rightarrow \psi$
 between $\Cat$-graphs transports $\phi,\psi: T\doublerightarrow Y$.
The vertexes will be  all $\Cat$-graphs transports
$\phi: T\doublerightarrow Y$ and edges sets are  provided by the
Carte product
of edges sets in the target space $Y$
$$Y^T(\phi;\psi)= \Prod_{s\in T_0} Y(\phi_0(s);\psi_0(s))\tsk$$
Obviously an assistant $\Cat$-graph $T$ would have a vertexes set $T_0$
small enough that such Carte product could exist.

For  a $\Cat$-graphs transport $f:Y\doublerightarrow Y'$ such superfunctor
appoints  the changing of target space with taken $\Cat$-graphs transport
$$f^T: Y^T \doublerightarrow (Y')^T\tsk$$

For a $\Cat$-graphs transport $\phi: T\doublerightarrow Y$ it appoints
the composition of $\Cat$-graphs transports
$\phi\circ f: T\doublerightarrow Y'$ and for an edges set
$Y^T(\phi;\psi)$  the  mapping  is defined with the Carte product of edges
set mappings in the target space
$$f^T_{\phi,\psi}: Y^T(\phi;\psi) = \Prod_{s\in T_0} Y(\phi_0(s);\psi_0(s))
\rightarrow $$$$
\Prod_{s\in T_0} f_{\phi_0(s);\psi_0(s)} (Y(\phi_0(s);\psi_0(s)))
\subset
\Prod_{s\in T_0} Y'(f_0(\phi_0(s));f_0(\psi_0(s))) \tsk$$

For primarily parallel $\Cat$-graphs transports $f,g: Y\doublerightarrow Y'$
we get only secondarily parallel $Cat$-graphs transports
$f^T,g^T: Y^T\doublerightarrow (Y')^T $,  i. e. we don't
have  coincident appointments of vertexes $f^T_0(\phi)\not= g^T_0(\phi)$,
  but we get
coincidence only for the projection to  vertexes appointment
$$f_0(\phi_0(s))= g_0(\phi_0(s))\uparrow \phi\in (Y^T )_0, s\in T_0\tsk$$
For  a natural transform between the  edges set mappings
$f_{x,y}\dgl g_{x.y}$ we get the natural transform between  vertexes
appointments
$$T(s;t)\rightarrow  f_{\phi_0(s);\psi_0(t)} (\phi_{s,t} (T(s;t))
\dgl  g_{\phi_0(s);\psi_0(t)} (\phi_{s,t} (T(s;t)) \kbl$$
and another natural transform between the  edges set mappings
$$Y(x;y)\rightarrow \Prod_{s\in T_0} f_{\phi_0(s);\psi_0(s)}
(Y(\phi_0(s);\psi_0(s))) \dgl $$$$
\Prod_{s\in T_0} g_{\phi_0(s);\psi_0(s)}
(Y(\phi_0(s);\psi_0(s))) \subset \Prod_{s\in T_0} Y'(
g_0(\phi_0(s));g_0(\psi_0(s)))
\tsk$$
We needed to check this property only for the target space changing in
the values category $\Cat$. We shall come down inside
the categories $X(x;y)$
and $T(s;t)$ again. Let we have a natural transform
$\alpha_{x,y}: f_{x,y}\rightarrow g_{x,y}$ defined by collection of arrows
from the category $Y(f_0(x);f_0(y))$
$$\alpha_w: (f_{x,x'})_0(w)\rightarrow (g_{x,x'})_0(w)\uparrow w\in X(x;y)_0
\tsk$$
For some $\Cat$-graphs transport $\phi: T\doublerightarrow X$ the changing
of target space with another $\Cat$-graphs transport $f: X\doublerightarrow Y$
will appoint the composition of $\Cat$-graphs transports
$\phi\circ f:X\doublerightarrow Y$ which will have the edges set mappings
$$T(s;t)\rightarrow f_{\phi_0(s),\phi_0(t)}(\phi_{s,t}(T(s;t)))\subset
Y(f_0(\phi_0(s);f_0(\phi_0(t)))\tsk$$
The natural transforms $\alpha_{x,y}: f_{x,y}\rightarrow g_{x,y}$ now provides
a new natural transform
$\alpha^{\phi_{s,t}(T(s;t))}: \phi_{s,t}\circ f_{\phi_0(s),\phi_0(t))}
\rightarrow   \phi_{s,t}\circ g_{\phi_0(s);\phi_0(t)} $
defined with collection of arrows
from the  category $Y(f_0(\phi_0(s)); f_0(\phi_0(t))= Y(g_0(\phi_0(s));
g_0(\phi_0(t))) $
$$\alpha_{(\phi_{s,t})_0(u)}: (f_{\phi_0(s),\phi_0(t)} )_0((\phi_{s,t})_0(u))
\rightarrow
  (g_{\phi_0(s),\phi_0(t)} )_0((\phi_{s,t})_0(u))
$$  for $ u\
in T(s;t)_0$.
The notation $\alpha^{\phi_{s,t}(T(s;t))}$ denotes the collection of arrows
for the points in the category $\phi_{s,t} (T(s;t))$.

For a edges set $X^T(\phi;\psi)$ between  $\Cat$-graphs transports
$\phi,\psi: T\doublerightarrow X$ the changing of target space with
$\Cat$-graphs transport $f: X\doublerightarrow Y$ provides
the  edges set mapping
as the Carte product of mappings
$$\Prod_{s\in T_0} X(\phi_0(s);\psi_0(s))\rightarrow \Prod_{s\in T_0}
f_{\phi_0(s),\psi_0(s)}(X(\phi_0(s );\psi_0(s)))\subset $$$$
\Prod_{s\in T_0} Y(f_0(\phi_0(s ));f_0(\psi_0(s))) \tsk$$
The  natural transforms $\alpha_{x,y}: f_{x,y}\rightarrow g_{x,y}$ now provides
a new natural transform
$$\alpha^{X^T(\phi;\psi)}: \Prod_{s\in T_0}f_{\phi_0(s),\psi_0(s)}
 \rightarrow  \Prod_{s\in T_0} g_{\phi_0(s),\psi_0(s)} $$
with Carte product of arrows
$$(f_{\phi_0(s),\psi_0(s)})_0 (w)) \rightarrow
  (g_{\phi_0(s),\psi_0(s)})_0 (w)
\uparrow w\in X(\phi_0(s);\psi_0(s))_0, s\in T_0\tsk$$
\vskip\tarpas

We should want to take arbitrary arrow  $e_x\in X(x;x)$
as a unit arrow.
Let $e_x:u\rightarrow v$  is an arrow between two points $u,v\in X(x;x)_0$.
The choosing of unit arrow  would allow us to  define sections transport
$\lambda_X: X\doublerightarrow (X\otimes T)^T$.  The vertexes appointment
for a vertex $x\in X_0$ appoints the section $\lambda_X(x)\in X^T$.
It will be a $\Cat$-graphs transport for a vertex $s\in T$
appointing a vertex in the biproduct
$\lambda_X(x,s)=\lan x,s\ran \in X_0\otimes T_0$ and  having
 edges set mappings
$$\lambda_X(x)_{s,t} : T(s;t)\rightarrow e_x(*)\otimes T(s;t) \subset
X(x;x) \otimes T(s;t) \tsk$$
The edges set mappings for sections transport will be
$$(\lambda_X)_{x,y}: X(x;y)\rightarrow (X\otimes T)^T
(\lambda_X(x); \lambda_X(y)) = \Prod_{s\in T_0} X(x;y)\otimes e_s(*)\subset
$$$$\Prod_{s\in T_0} X(x;y)\otimes T(s;s)\tsk$$
These mappings for $\Cat$-enriched graphs $X$ and $T$ must be functors
between correspondent categories. However the edges set mappings
between  section $\Lambda_X(x)$
$$\Lambda_X(x)_{s,t}: T(s;t)\rightarrow e_x(*)\otimes T(s;t)$$
doesn't maintain composition of arrows from  category $T(s;t)$ if
the unit arrow doesn't allow the equality of idempotent
$$e_x\circ e_x= e_x \tsk$$
Otherwise for an arrow $e_x: v\rightarrow w$ with the different points
$v\in X(x;x)_0$ and $v\in X(x;x)_0$ defined  mapping
 $T(s;t)\rightarrow e_x(*)\otimes T(s;t)$
 can't be functor, as for some point
$u\in T(s;t)_0$ we get an arrow $\lan e_x , u\ran:\in X(x;x) \otimes T(s;t)$
between different couples $\lan v, u\ran\not=\lan w,u\ran $.
We need extend the stock of mappings allowing
new functors $f: p\rightarrow q^{\two}$. We have denoted the category
$\two=\lbrace \cdot \rightarrow \cdot\rbrace $ with two points
and three arrows. The composition  of such arrows
will  extends the stock of arrows. We must include also the  arrows
$f: p \rightarrow q^{\two^n} $ with arbitrary finite number $n\dgl 0$.
So we need to extend the values category $\Cat$ with
graphs transports $p\rightarrow q^{\two^n} $
between categories $p,q\in \Cat_0$. Such categories are original graphs,
and graphs transports $p\rightarrow q^{\two^n}$ can be taken maintaining unit
arrows. Such new category isn't closed one, but has name and realization
mappings with simply properties.

At this moment we shall work with our taken category $\Cat$.
The collection of sections transports defines the name appointment
from the set of $\Cat$-graphs transports over biproduct  $X\otimes T$
with the assistant
$\Cat$-graph  $T$  to the set of $\Cat$-graphs transports into the
exponential
space $Y^T$
$$\Grph_{\Cat} (X\otimes T;Y) \rightarrow \Grph_{\Cat} (X;Y^T) \tsk$$

For a $\Cat$-graphs transport $f:X\otimes T\doublerightarrow Y$  it provides
the composition of $\Cat$-graphs transports
$$f^\#= \lambda_X\circ f^T : X\doublerightarrow Y^T\tsk$$
It is monotone for order relation defined by existing natural transform
between  primarily parallel $\Cat$-graphs transports to the  target
$\Cat$-graph $Y$ and existing natural
transforms between secondarily parallel $\Cat$-graphs  transports to the
exponential   space of all transforms $Y^T$. It can be checked for edges set
mappings which will be functors between correspondent categories.

We again will come down inside the categories $p\in \Cat_0$.
The natural transform $\alpha_{\lan x,s\ran,\lan y, t\ran}:
f_{\lan  x,s\ran,\lan y,t\ran} \rightarrow f'_{\lan x,s\ran,\lan y,t\ran} $
between two $\Cat$-graphs transports $f,f'\in \Cat(X\otimes T;Y) $
is defined by collection of arrows from category  $Y(f_0(x,s); f_0(y,t))$
$$\alpha_{\lan w,u\ran } :( f_{\lan x,s\ran,\lan y,t\ran} )_0(w,u)
\rightarrow   ( f'_{\lan x,s\ran,\lan y,t\ran} )_0(w,u) \uparrow
w\in X(x;y)_0, u\in T(s;t)_0\tsk$$

For any  vertex $x\in X_0$  appointed section
$\Lambda_X(x): T\doublerightarrow X\otimes T$ is defined with vertexes
appointment $\lan e_x,s\ran\in X(x;x)_0\times T(s;t)_0$
and edges set mappings $\lambda_X(x)_{s,t}: T(s;t)\rightarrow
(X(x;x)\otimes T(s;t))^{\two}$.
Further the changing of target space
by a  $\Cat$-graphs transport $f: X\otimes T\doublerightarrow Y$ appoints
the $\Cat$-graphs transport $T\doublerightarrow Y$ which for the
vertex $s\in T_0$ appoints the vertex $f_0(x,s)\in Y_0$ and  have edges set
mappings
$$T(s,t)\rightarrow f^{\two}_{\lan x,s\ran,\lan x,t\ran}
(e_x(*)\otimes T(s;t))
\subset Y(f_0(x,s);f_0(x,t))^{\two} \tsk$$
We get a natural transform
$\alpha^{\lambda_X(x)_{s,t}(T(s;t))} : f_{\lan x,s\ran,\lan x,t\ran} \rightarrow
f'_{\lan x,s\ran,\lan x,t\ran} $ defined with collection of arrows
from category $Y(f_0(x,s);f_0(y,t))$
for the source and target points
$$\alpha^1_{(\lambda_X(x)_{s,t})_0(u)}= \alpha_ {\lan e_x^1,u\ran } :
(f_{\lan x,s\ran,\lan x,t\ran})_0(e_x^1,u)\rightarrow
(f'_{\lan x,s\ran,\lan x,t\ran})_0(e^1_x,u) \kbl$$
$$\alpha^2_{(\lambda_X(x)_{s,t})_0(u)}= \alpha_ {\lan e^2_x,u\ran } :
(f_{\lan x,s\ran,\lan x,t\ran})_0(e^2_x,u)\rightarrow
(f'_{\lan x,s\ran,\lan x,t\ran})_0(e^2_x,v) \tsk$$
For the  edges set mappings
$X(x,y)\rightarrow \Prod_{s\in T_0} f_{\lan x,s\ran,\lan y,s\ran}$
the natural transform is defined with natural transforms
between taken $\Cat$-graphs transports
$$\alpha_{\lan x,s\ran,\lan y,t\ran}:
f_{\lan x,s\ran,\lan y,t\ran}\rightarrow f'_{\lan x,s\ran,\lan y,t\ran}
\tsk$$
They provide a new natural transform  with arrows
$$\alpha ^{(X\otimes T )^T} : \Prod_{s\in T_0} (f_{\lan x,s\ran,
\lan y,s\ran})_0 (w) \rightarrow \Prod_{s\in T_0} (f_{\lan x,s\ran,
\lan y,s\ran})_0 (w)  $$
equal to Carte product of arrows couples
$$\alpha^1_{\lan x,s\ran,\lan y,s\ran}( w,e^1_s):
(f_{\lan x,s\ran,\lan y,s\ran})_0(w,e^1_s) \rightarrow
(f'_{\lan x,s\ran,\lan y,s\ran})_0(w,e^1_s) \uparrow u\in T(s;s)_0\kbl$$
$$\alpha^2_{\lan x,s\ran,\lan y,s\ran}( w,e^2_s):
f_{\lan x,s\ran,\lan y,s\ran_0})_0(w,e^2_s) \rightarrow
f'_{\lan x,s\ran,\lan y,s\ran})_0(w,e^2_s) \uparrow u\in T(s;s)_0\tsk$$

\vskip\tarpas

Now we shall construct an evaluation functor.
In a $\Cat$-graph  $X$
the contact arrows mappings
Will be defined  as bifunctors
$$h_{a,b,c}:X(a;b)\otimes X(b;c) \rightarrow X(a;c) \tsk$$
They defines some $\Cat$-graphs transport
over ^{pullbacked =product}
$$h:X\otimes _{X_0} X\doublerightarrow X\tsk$$
The pullbacked product of enriched graphs is defined
by the vertexes set  $X_0\times X_0$ and
the edges sets
$$X\otimes _{X_0} X(p;r) = \Cup_{q\in X_0} X(p;q)\otimes X(q;r)\tsk$$
The taken bifunctors  define edges set mappings
$$\Cup_{q\in X_0} h_{p,q,r}: \Cup_{q\in X_0} X(p;q)\otimes X(q;r)
\rightarrow  X(p;r)\tsk$$

We demand that changing of target space with such bifunctors would be
monotone
$$\Cat(r, X(a,b)\otimes X(b;c))\rightarrow \Cat(r; X(a;b)\circ X(b;c)
)\subset \Cat(r;X(a;c)) \kbl$$

This means that for the couple of natural transforms
$\alpha: f\rightarrow f'$ between  any two functors
$ f,f'\in \Cat(r; X(a;b))$ and  $\beta: g\rightarrow  g' $ between
two functors $g,g'\in \Cat(r;X(b;c))$
such changing of target space  would  provide a new natural transform.
In our case the $\Cat$-graphs functors always keeps natural transforms.
The image of natural transform $\alpha$ by functor $F$ can  be
denoted $\alpha\times F$.

The contact arrows mappings allows us to define preevaluation
$$\ev_Y^+: Y^T\otimes T \doublerightarrow Y \tsk$$
Preevaluation for the edges sets $Y^T(\phi;\psi) $ and $T(s;t)$
appoints precontact
edges set
$$Y^T(\phi;\psi)\otimes T(s;t)\rightarrow
Y(\phi_0(s);\psi_0(t))\circ \psi_{s,t} (T(s;t)) \subset
Y(\phi_0(s);\psi_0(t))\tsk$$
The prerealization appointment
$$\Grph_{\Cat} (X;Y^T)\rightarrow \Grph_{\Cat} (X\otimes T;Y)$$
is provided by composition of $\Cat$-graphs transports.
For a $\Cat$-graphs transport $g: X \doublerightarrow Y^T $ it appoints
the composition
$$g^\flat= (g\otimes \Identity_T ) \circ \ev_Y^+: X\otimes T\doublerightarrow Y\tsk$$
We can check that for  a natural transforms
$\alpha_x: g_0(x)\rightarrow g'_0(x)$ between $
\Cat$-graphs transports $g_0(x),g'_0(x): T\doublerightarrow Y$ for vertexes
$x\in  X_0$  and natural transforms
$\alpha_{x, y} : g_{x,y}
\rightarrow g'_{x,y}$
between the edges set mappings
$$X(x;y)\rightarrow g_{x,y} (X(x;y))\dgl g'_{x,y}(X(x;y))
\subset Y^T (g'_0(x);g'_0(y)) $$
of secondarily parallel $\Cat$-graphs transports
$g,g': X\doublerightarrow Y^T$ we get a new natural transform between
edges set mappings
$$X(x;y)\otimes T(s;t) \rightarrow Y(g_0(x,s); g_0(y, s))  \dgl
 Y(g'_0(x,s); g'_0(y,s)) \tsk$$
Let we have  a   natural transforms  $\alpha_x: g_0(x)\rightarrow g'_0(x)$
between edges set mappings  $g_0(x)_{s,t},g'_0(x)_{s,t}: T(s;t)\doublerightarrow
Y (g_0(x,s);g_0(x,t) $
defined by collection of arrows
$$(\alpha_{x})_u: (g_0(x)_{s,t})_0(u)\rightarrow  (g'_0(x)_{s,t})_0(u)
\uparrow u\in T(s;t)_0$$

and natural transforms $\alpha_{x,y}: g_{x,y}\rightarrow g'_{x,y} $
between two edges set mappings
 $X(x;y)\rightarrow Y^T(g_0(x);g_0(y)))$.
These mappings  are defined as a Carte product
$$g_{x,y}= \Prod_{s\in T_0} g_{x,y}(s)$$
of functors $g_{x;y}(s): X(x;y)\rightarrow Y(g_0(x;s); g_0(y;s))$, therefore
we get the  Carte product$$\alpha_{x,y} = \Prod_{s\in T_0} \alpha_{x,y}(s)$$
 of natural transforms
$$(\alpha_{x,y}(s))_w: (g_{x,y}(s))_0 (w) \rightarrow
(g'_{x,y}(s))_0 (w)) \uparrow w\in X(x;y) $$
defined with arrows in the  category $ Y(g_0(x,s);g_0(y,s))$.

The realization provided by  the preevaluation transport
is defined
as precontact arrows mappings
$$X(x;y)\otimes T(s;t)\rightarrow Y((g_0(x))_0(s);
( g_0(y))_0(s))\circ Y( (g_0(y))_0(s);(g_0(y))_0(t))\subset
$$$$  Y((g_0(x))_0(s);(g_0(y))_0(t))\tsk$$
Having the natural transforms between edges set mappings
$$f_{\lan x,s\ran,\lan y,t\ran}, f'_{\lan x,s\ran,\lan y,t\ran}:
 X(x;y)\otimes T(s;t)\rightarrow  Y( g_0(x,s); g_0(y,t)) )$$
we get the needed natural transform for the precontact arrows mappings
by monotone property of changing target space
by contact arrows mappings.

In the case of mappings $g_0(x)_{s,t}:
T(s;t)\rightarrow Y(g_0(x,s);g_0(x,t))^{\two}$
and
$$g_{x,y}: X(x;y)\rightarrow Y(g_0(x,s);g_0(y,s))^{\two}$$
we would get a realization  $f: X\otimes T\doublerightarrow Y$
with edges set mappings
$$X(x;y)\otimes T(s;t) \rightarrow Y(g_0(x,s);g_0(y,t))^{\two^2} \tsk$$
Such realization remains monotone for order relation defined with
existent natural transforms between functors.

\vskip\tarpas
We begin studies of original $\Cat$-graphs.
The original $\Cat$-enriched graph  $X$ needs equalities
for chosen unit arrows  and contact arrows mappings
$$X(a;b)\rightarrow e_a(*)\circ X(a;b) = X(a;b)= X(a;b) \circ e_b(*)\subset
X(a;b)\tsk$$

At first we shall check such equalities for translation of values category
$ \Cat \doublerightarrow \Set $.  The unit arrow $e_x\in X(x;x)$
becomes some  point  among all points  $   O_x\in X(x;x)_0$ of category
$X(x;x)$.
For original $\Set$-graph  $X_0 $ we need the equalities
$$X(a;b)_0\rightarrow O_a(*)\circ X(a;b)_0 = X(a;b)_0= X(a;b)\circ O_b(*)
\tsk$$
It means that for arbitrary point $u\in X(a;b)_0$ we have the equalities
$$O_a\circ u= u = u\circ O_b\tsk$$

Otherwise for  points $u\in X(a;a)$
and the  unit point $O_a\in X(a;a)_0$
we get  the equalities
$$O_a\circ u = u= u\circ O_a \uparrow u\in X(a;a)_0\tsk$$

We can see that a unit point is unique.
If we have another unit point $u\in X(a;a)_0$, then we get
equalities
$$O_x= O_x\circ u = u\tsk$$

So for the original $\Set$-graph  $X_0$ all sets $X(x;x)_0$
has unique unit point $$O_x\in X(x;x)_0\tsk$$


In arbitrary set $X(x;x)_0$  we can add a new unit
$O_x\in X(x;x)_0$
and in the set $X(x;x)^*_0 = X(x;x)_0 \cup \lbrace O_x\rbrace $
we can extend contact arrows mapping by taking
$$O_x\circ u=u\circ O_x =u\uparrow u\in X(x;x)_0\kbl
O_x\circ O_x= O_x \tsk$$
The old unit $e\in X(x;x)_0$
looses the property of unit in $X(x;x)^*_0$
as  we have
$$e\circ O_x = e\tsk$$

Such construction allows us arbitrary $\Set$-graph $X$ to change with
original $\Set$-graph  $X^*$. More exactly the category of $\Set$-graphs
$\Grph_{\Set}$ is isomorphic to the category of original $\Set$-graphs
$\OGrph_{\Set}$ with arrows of all original $\Set$-graphs transports.
For a $\Set$-graphs transport $f_0: X_0\doublerightarrow Y_0$ we appoint
its extension $f^*: X^*\doublerightarrow Y^*$  with
$$(f^*_{x,x})_0 (O_x) = O_{f_0(x)} \in Y(f_0(x);f_0(x))_0\tsk$$
Obviously we get a superfunctor
$\Grph_{\Set} \superrightarrow \OGrph_{\Set}$,
and inverse superfunctor will be defined by restriction of
edges set mappings
$$(f^*_{x,x})_0 : X(x;x)^*_0\rightarrow Y^*(f_0(x);f_0 (x))_0 $$

The same construction can be repeated for a $\Cat$-enriched graph $X$.
For a category $X(x;x)$ we appoint the set of category's points
$X(x;x)_0$. Let we have find one origin point $O_x\in  X(x;x)_0$
which is a neutral for the projection of contact arrows mapping
to the mappings of $\Set$-enriched graph
$$X(x;x)_0\times X(x;x)_0 \rightarrow  X(x;x)_0\tsk$$
In the set of loops with source and target point $O_x$ we shall look
for a unit arrow $1_x:O_x\rightarrow O_x$ with  the equality
for the contact arrows mapping
$$1_x\ast 1_x = 1_x\tsk$$
Otherwise we can add such unit arrow formally.
In such way we extend taken category $X(x;x)^*$.
Such extension is possible also even having true unit arrow.
We again can  unanimously extended  every functor to
the original functor over extended category $X(x;x)^* $. For arbitrary
$\Cat$-graphs transport $f:X \doublerightarrow Y$ we get
original $\Cat$-graphs transport
$$f^*: X^*\doublerightarrow Y^* \tsk$$
The restriction of original
$\Cat$-graphs transport $g: X^*\doublerightarrow Y^*$
provides non original $\Cat$-graphs transport  $\hat g: X
\doublerightarrow  Y$. We again get isomorphism of categories
$$\Grph_{\Cat} =\rightarrow \OGrph_{\Cat} \tsk$$
However we don't need to apply such construction for all $\Cat$-graphs.
When we are studying the name appointment
$$\Grph_{\Cat(} (X\otimes T;Y)\rightarrow \Grph_{\Cat} (X; Y^T)\kbl$$
we shall  apply such construction only for  three taken $\Cat$-graphs $X^*$,
$Y^*$, $T^*$ and we shall probe to construct needed  correct  extension
for biproduct $X\otimes T$ and exponential space $Y^T$.

We shall add a unit loop $1_x: O_x\rightarrow O_x$ with additional
arrows to other points of category $X(x;x)$. We shall say that we have
a category $X(x;x) $ with  a ^{leading =unit}.
Also the $\Cat$-graph  $X$ will be called ^{=leading } if it have  a leading
unit.
Let  we take leading extensions of source and assistant $\Cat$-graphs $X$
and $T$. For the target $\Cat$-graph  $Y$ we ask existence of correspondent
limits, needed to define extension of taken  $\Cat$-graphs transport
$f: X\otimes T\doublerightarrow Y$.
In ordered spaces such limits coincide with lower boundaries for
the points. In general case we should  work with arrow spaces
defined as an exponential space $p^{\two}$.

For   mapping
$f_{\lan x,s\ran,\lan y,s\ran}  X(x;y)\rightarrow Y(f_0(x,s);f_0(y,s))$
we take
$$f^*_{\lan x,s\ran,\lan y,s\ran}(w,1_s)= \lim_{u\to 1_s} f_{\lan x,s\ran,
\lan y,s\ran}(w,u) \in Y(f_0(x,s);f_0(y,s)) \kbl   $$
$$f^*_{ \lan x,s\ran,\lan x.t\ran} (1_x,u)= \lim_{w\to 1_x}
 f_{\lan x,s\ran,\lan x.t\ran} (w,u)\in Y(f_0(x,s);f_0(x,t))\kbl $$
$$f^*_{\lan x,s\ran,\lan x,s\ran} (1_x;1_s)= 1_{f_0(x,s)} \in
Y(f_0(x,s);f_0(x,s)) \tsk$$
These limits can be not unique, then we should get different possible
extensions. Any such extension will be useful to explain situation
with taken $\Cat$-graphs $X$, $Y$, $T$.
Also the ^{=partial transport}  $g: X\doublerightarrow Y^T$ will be changed with its
extension.

We want to remark that we get opportunity to understand a  general theory
for the name appointment
$$\Grph_{\Cat} (X\otimes T;Y) \rightarrow \Grph_{\Cat} (X;Y^T) \tsk$$
From original graphs $X$, $Y$, $T$ we can remove unit arrows, and
to produce all patterns of general case.

Let we have an   original $\Cat$-graphs transport
$f : X\otimes T \doublerightarrow Y$
with upper predecomposition
$$f_{\lan a,s\ran,\lan b,s\ran }(X(a;b)\otimes 1_s(*))\circ
f_{\lan b,s\ran,\lan b,t\ran} (1_b(*)\otimes T(s;t))\dgl$$$$
f_{\lan a,s\ran,\lan b,t\ran}(X(a;b)\otimes T(s;t))\tsk$$

Then appointed prerealization of name $f^+\dgl f $ is the smallest
preregular upper bound,  i. e. a original $\Cat$-graph transport
coinciding with the name's prerealization.

For this $\Cat$-graphs transport we have  the  predecomposition equality
$$f^+_{\lan a,s\ran,\lan b,s\ran }(X(a;b)\otimes 1_s(*))\circ
f^+_{\lan b,s\ran,\lan b,t\ran} (1_b(*)\otimes T(s;t))=$$$$
f^+_{\lan a,s\ran,\lan b,t\ran}(X(a;b)\otimes T(s;t))\tsk$$

Otherwise each  original $\Cat$-graphs transport
$f: X\otimes T\doublerightarrow Y$
with predecomposition equality is preregular.

The name appointment is bijective  over the set of preregular $\Cat$-graphs
transports. This means that for arbitrary $\Cat$-graphs transport
$g: X\doublerightarrow Y^T$ we have the realization
$f: X\otimes T\doublerightarrow Y$
being some preregular $Cat$-graphs
transport.

We want to remark that for original $\Cat$-graphs transports
$f: X\otimes T \doublerightarrow Y$ we use the properties
of contact arrows mappings
only in the target space $Y$. In the source space $X$
we need only that chosen units
will be neutral for taken contact arrows mappings.

Finally we have seen that the name $g: X\doublerightarrow Y^T$
 of  arbitrary  original $\Cat$-graphs transport $f: X\times T\doublerightarrow Y$
with upper predecomposition  and lower postdecomposition

$$f_{\lan a,s\ran,\lan b, s\ran } (X(a;b) \otimes 1_s((*)) \circ
f_{\lan b, s\ran,\lan b,t\ran} (1_b(*)\otimes T(s;t))
\dgl  $$$$
 f_{\lan a,s\ran, \lan b,t\ran} (X(a;b)\otimes T(s;t))\dgl $$$$
f_{\lan a,s\ran,\lan a,t\ran} (1_a(*)\otimes T(s;t)) \circ
f_{\lan a, t\ran,\lan b,t\ran} (X(a;b)\otimes 1_t(*)) $$
 is corestricted  in exponential space
of natural transforms
$$ g: X\doublerightarrow Y^{(
T)}\tsk$$
\vskip\tarpas

It rests to consider the $\Cat$-enriched categories.
The $\Cat$-enriched category $X$ will be arbitrary original $\Cat$-graph
with contact arrows mappings providing associative composition, i. e.
we can apply  for the ^{=associativity  mappings}
$$S_{p,q,r}p\otimes (q\otimes r)\rightarrow( p \otimes q)  \otimes r $$
the ^{=associativity diagram }
$$S_{X(x;y),X(y;z),X(z;u)}\circ (X_{x,y,z}\otimes 1_{X(z,u)})\circ X_{x,z,u}
=$$$$
(1_{X(x,y)}\otimes X_{y,z,u})\circ X_{x,y,u}$$
\vskip\tarpas
$$\hskip -10 pt\matrix{X(x;y)\otimes (X(y;z)\otimes X(z;u)) \hskip -10 pt &
  & \mapright S & &
  (X(x;y)\otimes X(y;z))\otimes X(z,;u) \cr
%
\mapdownk {1_{X(x;y)}\otimes X_{y,z,u}} \hskip 20 pt & & & &
\mapdownd {X_{x,y,z}\otimes 1_{X(z,u)}} \cr
%
\hskip 20 pt X(x;y)\otimes X(y;u) \hskip-20 pt&   & &  &
\hskip -20pt X(x;z)\otimes X(z;u) \hskip 20 pt \cr
%
X_{x,z,u} \hskip -20pt & \searrow &  & \swarrow & \hskip -20 pt X_{x,z,u} \cr
%
& & X(x;u) & & \cr} $$
\vskip \tarpas
We shall work with various categories of $\Cat$-enriched categories.
Their transports $f: X\doublerightarrow Y$
will be called functors. The crude functors
are transports of original $\Cat$-graphs. They maintain the unit arrows
$$f_{x,x} (1_x(*)) = 1_{f_0(x)}(*)\subset Y(f_0(x);f_0(x))\tsk$$
This category I shall denote, in contrast of other users, most simply
$\Cat_{\Cat}$.

Then  we take continuous or cocontinuous functors having correspondent
diagrams for contact arrows mappings
$$\matrix{
X(a;b) \otimes X(b;c) & \mapright f_{a,b}\otimes f_{b,c} &
Y(f_0(a);f_0(b)) \otimes Y(f_0(b);f_0(c)) & \cr
\downarrow & &\downarrow & \cr
X(a;c) & \maprightap f_{a,c} & Y(f_0(a); f_0(c)) & \cr
  &        &  &\hskip-25pt \nearrow \hfill \cr}$$
   \vskip\tarpas
$$  \matrix{
X(a;b) \otimes X(b;c) & \mapright f_{a,b}\otimes f_{b,c} &
Y(f_0(a);f_0(b)) \otimes Y(f_0(b);f_0(c)) & \cr
\downarrow & &\downarrow & \cr
X(a;c) & \maprightap f_{a,c} & Y(f_0(a); f_0(c)) & \cr
  &        &  &\hskip-25pt \swarrow \hfill \cr} $$
\vskip \tarpas
 Their categories will be denoted $\Cat^+_{\Cat}$ and $\Cat^-_{\Cat} $.
Their intersection
also will have own denotation
$$\Cat^\pm_{\Cat}= \Cat^+_{\Cat} \Cap \Cat^-_{\Cat}\tsk$$

 I shall call the usual functors $f: X\doublerightarrow Y$  as natural
  functors.
They maintain the contact arrows mappings, i. e. we have commuting
diagrams
$$  \matrix{
X(a;b) \otimes X(b;c) & \mapright f_{a,b}\otimes f_{b,c} &
Y(f_0(a);f_0(b)) \otimes Y(f_0(b);f_0(c)) \cr
\downarrow & &\downarrow  \cr
X(a;c) & \maprightap f_{a,c} & Y(f_0(a); f_0(c))  \cr } $$
\vskip \tarpas
 Their category will be denoted
$\Cat^=_{\Cat} $.
For it the name appointment  provides  the true
conjunction between adjoint superfunctor
of biproduct $X\otimes T$ and coadjoint functor of exponential space $Y^{(T)}$
of natural transforms. Therefore the biproduct
is defined by exponential space
unanimously up unique isomorphism.

We can  see that the values category $\Cat$ becomes a $\Cat$-graph $\Cat^e$
with edges sets $p^s$ between vertexes $s,p\in \Cat_0$. The
true edges sets $\Cat(s;p)$ will be the edges sets for $\Set$-graph $\Cat$.
It can be identified with the set of all functors $\Cat^{\two}$,
where $\two =\lbrace \cdot \rightarrow \cdot\rbrace$

The defined functors $q^p\times r^q\rightarrow r^p$ defines edges sets
mappings for $\Cat$-graphs transport over pullbacked product of
$\Cat$-graphs
$$\Cat^e\times_{\Cat_0} \Cat^e \doublerightarrow \Cat^e \tsk$$
The pullbacked product for the $\Set$-graphs $\Cat$ can be defined as
the set of composable functors couples
$$\Cat^{\two}\times_{\Cat_0} \Cat^{\two} = \Cup_{q\in\Cat_0} \Cat(p;q)\times
\Cat(q;r)\tsk$$

Its projection to $\Set$-graph $\Cat^{\two}$
 $$\Cat^{\two}\times_{\Cat_0}\Cat^{\two}  \doublerightarrow \Cat^{\two}$$
is  defined with the composition of functors
$$f\circ g\in \Cat(p;r)\uparrow f \in \Cat(p;q), g\in\Cat(q;r)\tsk$$

It is interesting to understand is  the horizontal composition of
natural transform  a  unique possibility for the $\Cat$-graph $\Cat^e$ to
become   $\Cat$-enriched category.

In the category $\Cat^e$ we have evaluation mappings
$$\ev_q: p\otimes q^p \rightarrow q\tsk$$
We can compose two evaluation mappings
$$p\otimes (q^p\otimes r^q)=(p\otimes q^p )\otimes r^q\rightarrow q\otimes r^q
\rightarrow r\kbl$$
and get the arrow with the name
$$q^p\otimes r^q\rightarrow r^p \tsk$$

I am sure that we could find also another useful contact arrows mappings
in $\Cat$-graph $\Cat^e$. But then we need to check that we have got
mappings coincided with horizontal composition of natural transforms,
This can be done by careful calculation. We present the ^{graphical
=instruction} for such calculations.

In \baf G. Valiukevi\v cius 1992* p. 102 I have proposed  to express
the transform
$\alpha: \phi\rightarrow \psi $
between
parallel functors $\phi, \psi: p\doublerightarrow  q$
with ^{deformed =squares}

$$\matrix{
  &         & &\hskip -10 pt  \searrow  \hfill \cr 
 p  & \mapright {\phi} &  q & \cr
        \uparrow &   & \uparrow & \cr
        p &\maprightap {\psi} & q & \cr}$$
\vskip\tarpas
We take identity  functors $\Identity_p : p\doublerightarrow  p $ and
$\Identity_q: q\doublerightarrow q $ as ^{=uparrows} in such  diagrams.
In this article we have called such squares as continuous squares.

The  ^{prehorizontal =composition} $\alpha\ast \beta: \phi\circ \xi
\rightarrow \psi\circ \kappa $   of two transforms
$\alpha: \phi\rightarrow \psi$  between functors
$\phi,\psi: p\doublerightarrow q$
and $\beta: \xi\rightarrow \kappa $  between functors
$\xi,\kappa: q\doublerightarrow r$ are calculated
as ^{horizontal =composition of two deformed  quadrats}
$$\matrix{
 &  & &\hskip-10pt \searrow^\alpha \hfill & &
 &\hskip -10pt \searrow^\beta \hfill\cr
 p &\mapright {\phi} &q & & \mapright {\xi } & r & \cr
         \uparrow &  &\uparrow &  & & \uparrow & \cr
        p &\maprightap {\psi} &q & & \maprightap {\kappa} & r & \cr}$$
 \vskip\tarpas
$$\alpha\ast^+ \beta= (\alpha\star \xi )\circ (\psi\star \beta) \tsk$$
The associative composition  of functors is essential for such application
of deformed  quadrats.

The edges set mapping of preevaluation functor
$\ev_q: p\otimes q^p \doublerightarrow q$ is also expressed as
horizontal composition of deformed  quadrats. For an arrow
$w\in p(u;v) $  we get
a precontact arrow
$$ \alpha_u\circ \psi(w): \phi (u)\rightarrow \psi(v) $$
$$\matrix{  &  & &\hskip-20pt \searrow^w \hfill & & &\hskip -20pt
 \searrow^\alpha \hfill\cr
* &\mapright  u  &p & & \mapright {\psi} & q & \cr
          &  &\uparrow &  & & \uparrow & \cr
        * &\maprightap v &p & & \maprightap {\phi} & q & \cr }$$
\vskip\tarpas
So the ^{double =evaluation} provides  the horizontal composition of
three deformed quadrats
$$\matrix{
& &  &  & \hskip -10 pt \searrow^w \hfill & &\hskip-10pt \searrow^\alpha
\hfill & & &\hskip -10pt \searrow^\beta \hfill\cr
* & \mapright u & p & &\mapright {\phi} &q & & \mapright {\xi } & r & \cr
    & &     \uparrow &  &  &\uparrow & & & \uparrow & \cr
   * & \maprightap v &     p &  &\maprightap {\psi} &q & & \maprightap
   {\kappa} & r & \cr }$$
\vskip\tarpas
and coincides with the preevaluation of earlier defined prehorizontal
composition.
\vskip\tarpas

Also we can express the same transform
$\alpha: \phi\rightarrow \psi $
between
parallel functors $\phi, \psi: p\doublerightarrow  q$
with a ^{dual deformed =quadrat}. Such duality was introduced in
\baf G. Valiukevi\v cius 1992* and thoroughly exploited in
\baf G. Valiukevi\v cius 2009*.

For dual diagram we take the identity arrows
$\Identity_p : p\doublerightarrow  p $ and
$\Identity_q: q\doublerightarrow q $ as the ^{=downarrows}.

$$\matrix{ p  & \mapright {\phi} &  q & \cr
        \downarrow &   & \downarrow & \cr
        p &\maprightap {\psi} & q & \cr
          &         & &\hskip -10 pt  \nearrow  \hfill \cr} $$
\vskip\tarpas
Such deformed quadrats we have called  as  cocontinuous quadrats.

A  ^{posthorizontal =composition} $\alpha\ast \beta: \phi\circ \xi
\rightarrow \psi\circ \kappa $   of two transforms
$\alpha: \phi\rightarrow \psi$  between functors
$\phi,\psi: p\doublerightarrow q$
and $\beta: \xi\rightarrow \kappa $  between functors
$\xi,\kappa: q\doublerightarrow r$ is calculated
as ^{horizontal =composition of two deformed  quadrats}
$$\matrix{ p &\mapright {\phi} &q & & \mapright {\xi } & r & \cr
         \downarrow &  &\downarrow &  & & \downarrow & \cr
        p &\maprightap {\psi} &q & & \maprightap {\kappa} & r & \cr
 &  & &\hskip-10pt \swarrow_\alpha \hfill & &
 &\hskip -10pt \swarrow_\beta \hfill\cr }$$
 \vskip\tarpas
$$\alpha\ast^- \beta=  (\phi\star \beta) \circ (\alpha\star \kappa )\tsk$$

The edges set mapping of postevaluation functor
$\ev_q: p\otimes q^p \doublerightarrow q$ also is expressed as
horizontal composition of deformed  quadrats. For an arrow
$w\in p(u;v) $  we get
a postcontact arrow
$$ \phi(w) \circ \alpha_v: \phi (u)\rightarrow \psi(v) $$
$$\matrix{ * &\mapright  u  &p & & \mapright {\phi} & q & \cr
          &  &\downarrow &  & & \downarrow & \cr
        * &\maprightap v &p & & \maprightap {\psi} & q & \cr
 &  & &\hskip-20pt \swarrow_w  w\hfill & & &\hskip -20pt \swarrow_\alpha
 \hfill\cr }$$
\vskip\tarpas
So the ^{double =evaluation} provides  the horizontal composition of
three deformed quadrats
$$\matrix{ * & \mapright u & p & &\mapright {\phi} &q & & \mapright {\xi } & r & \cr
    & &     \downarrow &  &  &\downarrow & & & \downarrow & \cr
   * & \maprightap v &     p &  &\maprightap {\psi} &q &
   & \maprightap {\kappa} & r & \cr
& &  &  & \hskip -20 pt \swarrow_w \hfill & &\hskip-10pt \swarrow_\alpha
\hfill &
& &\hskip -10pt \swarrow_\beta \hfill\cr }$$
\vskip\tarpas
and coincides with the  postevaluation of  defined
posthorizontal composition.

For a natural transform $\beta: \xi\rightarrow \kappa$
the prehorizontal composition coincides with the posthorizontal composition.
We need to check only
coincidence of  preevaluation with postevaluation

$$\hskip-12pt \matrix{
& &  &  & \hskip -20 pt \searrow^w \hfill &
&\hskip-10pt \searrow^\alpha \hfill &
& &\hskip -10pt \searrow^\beta  \hfill\cr
* & \mapright u & p & &\mapright {\phi} &q & & \mapright {\xi } & r & \cr
    & &     \uparrow &  &  &\uparrow & & & \uparrow & \cr
   * & \maprightap v &     p &  &\maprightap {\psi} &q & & \maprightap
   {\kappa} & r & \cr
   \cr}=
\matrix{ \cr
* & \mapright u & p & &\mapright {\phi} &q & & \mapright {\xi } & r & \cr
    & &     \downarrow &  &  &\downarrow & & & \downarrow & \cr
   * & \maprightap v &     p &  &\maprightap {\psi} &q & &
    \maprightap {\kappa} & r & \cr
& &  &  & \hskip -20 pt \swarrow_w \hfill & &\hskip-10pt \swarrow_\alpha
 \hfill & & &\hskip -10pt \swarrow_\beta \hfill\cr } $$
\vskip\tarpas

For two natural transforms $\alpha: \phi\rightarrow \psi$ and
$beta:\xi\rightarrow \kappa$ we get  a horizontal composition being
natural transform
$$\alpha\ast\beta: \phi\circ \xi\rightarrow \psi\circ \kappa\tsk$$
First we can check that the horizontal composition of dual de\-formed qua\=drats
is dual for a horizontal composition of taken deformed quadrats.
It is true not only for the pair of opposite identity functors, but
also for arbitrary truly joint pair of functors as it was done in
\baf G. Valiukevi\v cius 1992* p. 104.

Then the conclusion for horizontal composition of natural transforms will
be obvious.
\vskip\tarpas
We can see an instance of our proposition in metric spaces.
The scalar space  $[0,\infty]$ is compounded of positive real numbers
$r\dgl 0$ and  infinite point $+\infty$.
Taking inequality $r\dgl s$ as an arrow $r\rightarrow s $,
we get a graph structure. We need a new sign for it $[0,\infty]^+$.
The scalar space will be  a set of its vertexes
$$[0,\inf]^+_0= [0,\infty] \tsk$$

The contact arrows mapping is provided  by transitivity
of inequalities
$$r\dgl s, s\dgl t \duoda r\dgl t \tsk$$
Such implication can be understood as a rule for definition of
graphs transport over pullbacked product
$$[0,\infty]^+\times _{[0,\infty] } [0,\infty]^+\doublerightarrow
[0,\infty]^+
\tsk$$
Such contact arrow mapping  defines associative composition of arrows
as we have commuting diagram of graphs transports
$$\matrix{  (p\dgl q, q\dgl r), r\dgl s & &\rightarrow  &  &
p\dgl q, (q\dgl r,r \dgl s) \cr
\downarrow  & &     && \downarrow  \cr
p\dgl r, r\dgl s & &    & & p\dgl q, q\dgl s  \cr
 & \searrow &   & \swarrow & \cr
 & & p\dgl s  & & \cr} $$
\vskip \tarpas
Commuting for such diagram is get automatically, as an inequality in ordered
space  means the unique arrow.

The inequality $r\dgl r$ will be a unit arrow for such contact
arrows  mapping. It also can  be expressed as two commuting
diagrams of graphs transports

$$ \matrix { r\dgl s  & \rightarrow & r\dgl r , r\dgl s  \cr
 &\searrow & \downarrow \cr
 &    & r\dgl s \cr } \hskip 20 pt
\matrix { r\dgl s, s\dgl s & \leftarrow & r\dgl s \cr
\downarrow & \swarrow & \cr
r\dgl s & & \cr}$$
\hskip\tarpas
So indeed the graph $[0,\infty]^+ $ is a category.
The point $0\in [0,\infty]$ is a final point for it
as we have exactly one arrow from any
 point
$$r\dgl 0 \uparrow r\in [0,\infty] \tsk$$

It is true for arbitrary ordered space $X$ with the smallest member
$0\in  X$. Taking inequality $r\dgl s$ as an arrow, we get
a category $X^+$  with final point $0\in \VF$.

Every graphs transport between the categories provided by ordered
spaces $f: X^+\doublerightarrow Y^+$
defines monotone appointment of points
$$p\dgl r \duoda f_0(p)\dgl f_0(r) \tsk$$
And conversely any monotone appointment of points defines
graphs transport for categories provided of taken ordered spaces.
Usually we don't distinguish ordered space $X$ from its provided category
$X^+$.

We can check that every graphs transport $f: X^+\doublerightarrow Y^+$
is exact functor between correspondent categories.

Indeed. Every unit arrow $p\dgl p$ will be maintained by arbitrary
graphs transport, as $f(p)\dgl f(p)$.
As edge between two points can be only unique, so we get
maintained unit arrow.

Also for two ^{connected =inequalities}
$p\dgl q$ and $q\dgl r$ we get connected inequalities in the target
space $f(p)\dgl f(q)$ and $f(q)\dgl f(r)$. Their composition
$p\dgl r$ is maintained also maintained $f(p)\dgl f(q)$.

These properties are sufficient for  graphs transport
between categories provided by ordered spaces $f: X^+\doublerightarrow Y^+$
to be an exact functor.

In the category $[0,\infty]^+$ we shall take a  biproduct
as a graphs transport
$$[0,\infty]^+\times [0,\infty]^+ \doublerightarrow [0,\infty]^+$$
defined  with appointment of vertexes provided by addition of real numbers.
For edges we have appointment of inequality provided by monotone  addition
$$(p\dgl q, r\dgl s) \duoda p+r\dgl q+ s\tsk$$
Obviously such biproduct is commutative and associative. The final
vertex $0\in [0,\infty]$ will be neutral for such biproduct
$$ 0+ p = p = p+0\tsk$$
So we have got a monoidal category $[0,\infty]^+$.

For a chosen number $s$ we get a functor $[0,\infty]^+ \doublerightarrow
[0,\infty]^+ $
$$p\dgl r \duoda p+s\dgl r+s \tsk$$
For it we  define another coadjoint exponential functor
$$p\dgl r \duoda (p-s)^+\dgl (r-s)^+ \tsk$$
The equivalence of inequalities
$$r+s\dgl t\lygiavertu r\dgl ( t-s)^+ $$
provides the adjunction for true joint pair of functors $r+s$ and $t^s$.
So  we have got  the closed monoidal category $[0,\infty]^+$

This category  is complete for arbitrary Carte product
$$\Prod_\alpha r_\alpha = \sup_\alpha r_\alpha\tsk$$

The $[0,\infty]^+$-enriched graph $X$ is defined by the set of vertexes
$X_0$
and the edges sets $X(x;y) \in [0,\infty]$ being positive real numbers.
The $[0,\infty]^+$-graphs transport $f: X\doublerightarrow Y$
is defined by appointment of vertexes $f_0: X_0\rightarrow Y_0$
and edges set mappings
$$f_{x,y} : X(x;y) \rightarrow f_{x,y}(X(x;y))\subset Y(f_0(x);f_0(y))\tsk$$
Obviously this  expression  is only symbolic. It is only
the  inequality between real numbers
$$X(x;y)\dgl Y(f_0(x);f_0(y))\tsk$$
Such expressions  remain mappings
in the category of sets
$\Set$ and they can be useful for constructing some
needed commuting diagrams
which  will be common for all $\VV$-enriched spaces with different values
categories $\VV$.

The $[0,\infty]^+$-graph $X$ will be called as ^{=distance space}, and
$[0,\infty]^+$-graphs transport between $[0,\infty]^+$-enriched graphs
$f: X\doublerightarrow Y$ can be called as ^{nonexpanding =mapping}
of distance spaces.

The original $[0,\infty]^+$-graph needs to have chosen unit arrows
 $$* \rightarrow 1_x(*)\subset X(x;x)\tsk$$
It will be expressed as an inequality
$$0\dgl X(x;x)\uparrow x\in X_0\tsk$$

Also it needs to have  chosen  contact arrows mappings
$$X_{x,y,z}:
X(x;y)\otimes X(y;z) \rightarrow X(x;y)\circ X(y;z) \subset X(x;z)\tsk$$
It will be expressed as a triangular inequality for distance
$$X(x;y)+ X(y;z) \dgl X(x;z) \uparrow x,y,z\in X_0\tsk$$
The chosen unit arrows in original $[0,\infty]^+$-graphs  automatically will
be  neutral for contact arrows mappings
$$X(x;y)\rightarrow 1_x(*)\circ X(x;y)= X(x;y)= X(x;y)\circ 1_y(*)\uparrow
x,y\in X_0 \kbl$$
i. e. we have equalities between different mappings
$$X(x;y) \dgl 0+X(x;y)= X(x;y)= X(x;y)+0 \tsk$$
It must be expressed as commuting diagrams
$$\matrix{ X(x;y) & \rightarrow & 1_x(*)\circ X(x;y) \cr
     & \searrow & \downarrow \cr
     & & X(x;y) \cr } \hskip 10 pt
 \matrix { X(x;y) \circ 1_y(*) & \leftarrow & X(x;y) \cr
    \downarrow & \swarrow & \cr
    X(x;y) & & \cr }$$
\vskip\tarpas

So in an original $[0,\infty]^+$-graph $X$ the distance is a true metric.
Such graph will be called a metric space $X$.
We can check that original $[0,\infty]^+$-graph is an $[0,\infty]^+$-enriched
category, We need to check only commuting diagram
for associativity of contact arrows mappings
$$X(x;y)+ (X(y;z)+ X(z;w)) = (X(x;y)+X(y;z))+ X(x;z)\tsk $$
Such diagram is constructed for mapping over pullbacked product
$$S: X\times_{X_0} (X\times _{X_0} X) =\rightarrow
(X\times _{X_0} X)\times_{X_0} X $$

$$\hskip -10 pt\matrix{X(x;y)\otimes (X(y;z)\otimes X(z;u)) \hskip -10 pt &
  & \mapright s & &
  (X(x;y)\otimes_X(y;z))\otimes X(z,;u) \cr
%
\mapdownk {1_{X(x;y)}\otimes X_{y,z,u}} \hskip 20 pt & & & &
\mapdownd {X_{x,y,z}\otimes 1_{X(z,u)}} \cr
%
\hskip 20 pt X(x;y)\otimes X(y;u) \hskip-20 pt&   & &  &
\hskip -20pt X(x;z)\otimes X(z;u) \hskip 20 pt \cr
%
X_{x,z,u} \hskip -20pt & \searrow &  & \swarrow & \hskip -20 pt X_{x,z,u} \cr
%
& & X(x;u) & & \cr} $$
\vskip \tarpas
The commuting diagram in ordered space $[0,\infty]^+ $
is get automatically, as there between two points
can be only unique arrow.
The nonexpanding mapping between metric spaces $f: X\doublerightarrow Y$
will be crude functor of $[0,\infty]^+$-enriched categories.
It again will be  a natural  functor.
We need to  check the commuting diagram for contact arrows mappings
$$\matrix { X(x;y)\otimes X(y;z) & \mapright f_{x,y}\otimes f_{y,z} &
       Y(f(x);f(y)) \otimes Y(f(y);f(z)) \cr
    \downarrow & & \downarrow \cr
    X(x;y)\circ X(y;z)& \maprightap f_{x,z} &
    Y(f(x);f(y))\circ Y(f(y);f(z))\cr} $$
\vskip\tarpas
For metric spaces $X$ and $Y$ we have triangular inequalities
$$X(x;y)+ X(y;z)\dgl X(x;z) \kbl$$$$
 Y(f(x);f(y))+ Y(f(y);f(z))\dgl Y(f(x);f(z))\kbl$$
and for nonexpanding mapping we have  inequalities
$$X(x;y)\dgl Y(f(x);f(y))\kbl X(y;z)\dgl Y(f(y);f(z))\kbl $$$$
 X(x;z)\dgl  Y(f(x);f(y))\tsk$$
Therefore we get also the inequality
$$X(x,y)+X(y;z) \dgl Y(f(x);f(y))+ Y(f(z);f(z))\tsk$$
So we have all needed arrows for diagram
and this diagram in ordered space $Y$ must be commuting
$$\matrix { X(x;y)+ X(y;z) & \rightarrow &  Y(f(x);f(y))+Y(f(y);f(z)) \cr
\downarrow & & \downarrow \cr
X(x;z) & \rightarrow & Y(f(x);f(z))\cr } $$
\vskip\tarpas
Also it maintain chosen unit arrows
$$0\dgl X(x;x)\dgl Y(f(x);f(x))\tsk$$

We have shown that every nonexpanding mapping $f: X\doublerightarrow Y$
between  metric spaces   is natural functor between correspondent
$[0,\infty]^+$-enriched categories. So we have coinciding categories
$$\OGrph_{[0,\infty]^+}= \Cat^=_{[0,\infty]^+} \tsk$$

In these categories  for the  joint pair
of superfunctors we have a natural bijection. We shall check it directly.

\Proposition
It is equivalent  properties
for some mapping
$\Phi:X\times A\rightarrow Y$ to be nonexpanding over taken tensor product
of metric spaces $X\otimes A$
$$X(x;x')+A(a,a')\dgl Y(\Phi(x,a);\Phi(x',a'))$$
and for the partial mapping
$ \Phi_1: X\rightarrow Y^A$ to be nonexpanding for the metric of uniform
boundary  in functional space
$$ X(x;x')\dgl \sup_{a\in A} Y(\Phi(x,a);\Phi(x',a'))\tsk$$
\Proof:
Let we have the first inequality
$$ X(x,x')+ A(a;a')\dgl \Phi(x,a);\Phi(x';a'))\tsk$$
Then we get
$$ X(x;x')\dgl Y(\Phi(x,a);\Phi(x';a))\uparrow a\in A\kbl$$
$$X(x;x')\dgl \sup_{a\in A} Y(\Phi(x,a);\Phi(x',a'))\tsk$$

Otherwise from the second inequality  for arbitrary nonexpanding mapping
$\Phi_1(x)\in Y^A$
we get inequality
$$X(x;x') \dgl Y(\Phi(x,a);\Phi(x';a))\kbl $$
and for the metric in the space $Y$ we can apply triangular inequality
$$Y(\Phi(x,a);\Phi(x';a'))\mzl Y(\Phi(x;a);\Phi(x';a))+
Y(\Phi(x';a);\Phi(x';a')) \mzl $$$$
X(x;x')+ A(a;a')\tsk$$
\irodymopabaiga

We shall formulate this proposition in the  language  of
$[0,\infty]^+$-graphs.
At first we define biproduct $X\otimes Y$ of $[O,\infty]^+$-graphs $X$ and
$Y$. We take Carte tensor product of vertexes $(X\otimes Y)_0=X_0\times Y_0$
and tensor products of edges sets
$$X\otimes Y(\lan x,y\ran,\lan x',y'\ran) = X(x;x;) \otimes Y(y;y')\tsk$$
For distance  spaces we get $\ell_1$-distance  on product space
$$X\otimes Y(\lan x,y\ran,\lan x',y'\ran )= X(x;x')+ Y(y;y')\tsk$$
With an  assistant distance  space $T$ we define the adjoint superfunctor.
For a distance  space $X$ it appoints the biproduct with the
assistant space $X\otimes T$, and for a
nonexpanding mapping between distance  spaces $f: X\doublerightarrow Y$ it
appoints the biproduct with the identity mapping of the assistant space
$$f\otimes \Identity_T : X\otimes T \doublerightarrow Y\otimes T\tsk$$

The coadjoint superfunctor will
be define with the exponential space $Y^T$.
Its vertexes set will be compound by all nonexpanding mappings between
distance spaces $\phi: T\doublerightarrow Y$.
The edges set between two nonexpanding mappings
$\phi,\psi: T\doublerightarrow Y$
will  be defined by Carte product in value category $[0,\infty]^+$
$$Y^T (\phi;\psi)= \Prod_{s\in T_0 } Y(\phi_0(s); \psi_0(s)) \tsk$$
It is provided by upper boundary, therefore
$$Y^T(\phi;\psi)= \sup_{s\in T_0} Y(\phi_0(s);\psi_0(s)) ) \tsk$$
Between two nonexpanding mappings we have got
 a distance of uniform convergence.

The exponential  space  $Y^T$ defines a superfunctor in the category
of distance  spaces $\Grph_{[0,\infty]^+ }  $.
For arbitrary nonexpanding mapping $f: Y\doublerightarrow Y'$ it appoints
the changing of target space $f^T: Y^T\doublerightarrow (Y')^T $.
For a nonexpanding mapping  $\phi: T\doublerightarrow Y$
it appoints the new mapping $\phi\circ f: T\doublerightarrow Y'$
and  between changed mappings
it provides the new distance
$$(Y')^T(\phi\circ f;\psi\circ f)= \sup_{s\in T}
Y'(f_0(\phi_0(s));f_0(\psi_0(s)))
\uparrow \phi,\psi\in Y^T \tsk$$

Easy to check  the maintenance of mappings composition
$$(f\circ g)^T= f^T\circ g^T\tsk$$
It is true for general mappings in  the category $\Set$. We need only to
check that a changing of target space with composition of nonexpanding
mappings rests nonexpanding mapping.
We have inequalities of distances for nonexpanding mappings
$$X(x;y)\dgl Y(f_0(x);f_0(y) \kbl Y(f_0(x);f_0(y))\dgl
Y'(g_0(f_0(x));g_0(f_0(y)))  \tsk$$
Therefore
$$\sup_{s\in T} Y'(g_0(f_0(\phi_0(s)));g_0(f_0(\psi_0(s))))\mzl
$$$$\sup_{s\in T} Y(f_0(\phi_0(s)); f_0(\psi_0(s))) \mzl
$$$$ \sup_{s\in T} X(\phi_0(s);\psi_0(s))\tsk$$

Also the identity mapping defines the identity mapping
of exponential spaces
$$(\Identity_Y )^T= \Identity_{Y^T} \tsk$$

The mapping of  unit arrow  choosing
$$*\rightarrow 1_x(*)\subset X(x;x)$$
coincides with inequality for a distance
$$0\dgl X(x;x)\tsk$$
Such inequalities for all points in the source space $x\in X$ and
assistant space $s\in T$
allows us to define the sections transport of distance spaces
$$\lambda_X: X\doublerightarrow (X\otimes T)^T \tsk$$
For a point $x\in X$ it appoints the section
$\lambda_X(x): T\doublerightarrow X\otimes T $ which
for a point $s\in T$ appoints the couple $\lan x,s\ran\in X\times T$.
The section is nonexpanding mapping as in our case $X(x;x)=0$
and we have the inequality
$$ T(s;t)\dgl X(x;x)+T(s;t) \tsk$$
Also the sections transport is nonexpanding mapping
as $T(s;s)=0$
$$X(x;y)\dgl \sup_{s\in T} (X(x;y)+ T(s;s)) \tsk$$

The sections transport provides  the
 unit transform for joint pair of superfunctors.
 It will be  a natural transformation.
We have the commuting quadrats for arbitrary  nonexpanding
 mapping of distance spaces $f:X\rightarrow X'$
$$\matrix{ X&\mapright f & X \cr
          \mapdownk \lambda_X  &    &\mapdownd \lambda_{X'} \cr
          (X\otimes T)^T& \maprightap {(f\otimes 1_T)^T} &
         (X'\otimes T)^T \cr}$$
\vskip \tarpas

For an arrows set $X(x,x')$ we appoint the distance between sections
 mappings
$$(X\otimes T)^T(\lambda_X(x);\lambda_X(x'))= X(x;x')$$
and for a mapping $(f\otimes \Identity_T)^T: (X\otimes T)^T
\rightarrow  (X'\otimes T)^T$
we shall get the  new sections mappings with distances
$$(X'\otimes T)^T(\lambda_{(X')}(f(x));\lambda_{(X')}(f(x')))=
X'(f(x);f(x'))$$
the same as it would be a  distance for sections mappings
defined by the appointed points $f(x)\in X'$ and $ f(x')\in X'$.


For a distance space $Y$ the contact arrows mappings
$$Y(x;y)\otimes Y(y;z)\rightarrow Y(x;y)\circ Y(y;z) \subset Y(x;z)$$
are expressed as inequalities
$$Y(x;y)+ Y(y;z) \dgl Y(x;z) \tsk$$
In  such spaces we define evaluation transport
$$\ev_Y: Y^T\otimes T \doublerightarrow Y \tsk$$
It for a nonexpanding mapping
$\phi: T\doublerightarrow Y$ and point in assistant distance space  $s\in T$
appoints the value of taken mapping $\phi_0(s)\in Y$.
It is also nonexpanding.
For the pair of couples
$\lan \phi, s\ran \in Y^T\otimes T$ and $\lan \psi,t\ran\in
Y^T\otimes T$ we get the distance between values
$$Y(\phi_0(s);\psi_0(t))\mzl Y(\phi_0(s);\psi_0(s))+ \psi(T(s,t))\mzl
\sup_{s\in T} Y(\phi_0(s); \psi_0(s))+ T(s;t)\tsk$$
An evaluation transports provides  the natural transform between superfunctors.
We have the commuting quadrats for
 arbitrary nonexpanding mapping
$g: Y\doublerightarrow Y'$
$$\matrix{ (Y)^T\otimes T& \mapright { g^T\otimes 1_T} &
{Y'}^T\otimes T\cr
\mapdownk \ev_{Y} &    & \mapdownd \ev_{Y'} \cr
Y& \maprightap g & Y'\cr} $$
\vskip \tarpas
For a couple of nonexpanding mapping
$\phi: T\doublerightarrow Y$ and point $s\in T$
we appoint the mapping's  value $\phi(s)\in Y$, for a
nonexpanding map $g:Y\doublerightarrow Y'$ we get the  changed value
$g(\phi(s))\in Y'$.

For a pair of couples  $\lan \phi,s\ran$ and $\lan \psi,t\ran $
with distance
$$Y^T(\phi;\psi)+ T(s,t) $$
the evaluation $\ev_Y: Y^T\otimes T\doublerightarrow Y$   appoints
 the distance for appointed  values
$Y(\phi(s);\psi(t))$ and further the distance of changed values
$$Y'(g(\phi(s));g(\psi(t)))\tsk$$
It is the same as the distance calculated between two  mappings
$\phi:T\doublerightarrow Y$ and $\psi:T\doublerightarrow Y$
changed with nonexpanding mapping $g: Y\doublerightarrow Y'$
$$\lan (Y')^T(\phi\circ g;\psi\circ g)\tsk$$

For the truly joint  superfunctors $X\otimes A$ and $Y^A$ we need
to check both triangular equalities. However we can apply our proposition
about bijective name appointment.

For reversing realization appointment we need  to check decomposition
equality
$$X(a;b)\otimes T(s;t) \rightarrow
f_{\lan a,s\ran,\lan b,s\ran } (X(a;b)\otimes 1_s(*) ) \circ
f_{\lan y,s\ran,\lan y,t\ran} (1_b(*) \otimes T(s;t))=  $$$$
f_{\lan x,s\ran,\lan b,t\ran} (X(a;b)\otimes T(s;t))\subset
Y(f(a,s); f(b,t))$$
In our case we have commuting diagram of inequalities
$$X(a;b)+T(s;t)\dgl Y(f(a,s);f(b,s))+Y(f)b,s);f(b,t))
\dgl Y(f(a,s);f(b,t))$$
For the reversing  the name appointment we need to apply
the neutral equalities
$$ X(a;b)\rightarrow g_{a,b}(X(a;b))_s
 \circ g(b)_{s,s}(1_s(*)) = $$$$
 g_{a,b} (X(a;b))_s  \subset Y(g(a)_s;g(b)_s) \kbl$$
$$T(s;t)\rightarrow g_{a,a}(1_a(*) )
\circ g(a)_{s,t} (T(s;t)) = $$$$
g(a)_{s,t}(T(s;t)) \subset Y(g(a)_s;g(a)_t)$$
In our case we have such arrows only as  inequalities.
First we can see that nonexpanding mapping maintains the unit arrow
mappings. For a nonexpanding mapping $g(b): T\doublerightarrow X\otimes T$
we get the inequalities
$$0\dgl T(s;s)\dgl Y(g(b)_s;g(b)_s)\kbl$$
and the first neutral equality
$$X(a;b) \dgl Y(g(a)_s;g(b)_s)+ Y(g(b)_s;g(b)_s)= Y(g(a)_s;g(b)_s)\tsk$$
Also for a nonexpanding mapping $g: X\doublerightarrow Y^T$
we get the inequalities
$$0\dgl X(a;a)\dgl \sup_{s\in T} Y(g(a)_s; g(a)_s)\kbl$$
and the second neutral equality
$$T(s;t) \dgl Y(g(a)_s;g(a)_s) + Y(g(a)_s;g(a)_t) = Y(g(a)_s;g(a)_t)\tsk$$

We can see that there isn't any need to have the contact arrows mapping
in the source space $X$ or in the assistant space $T$.
\vskip\tarpas
We have another alternative metric space definition.
In scalar space we have Carte product $r\lor s\in [0,\infty]$. It will be
another tensor product. It defines a functor
which for a scalar $r\in [0,\infty$  appoints another scalar
$r\times s= r\lor s$.
We have a coadjoint exponential functor which for the scalar
$t\in [0,\infty]$  appoints another scalar $\Hom(s;t)\in [0,\infty]$
$$\Hom (a,v)= v\uparrow v\dg a; 0\uparrow v\mzl a \tsk$$
We get a joint pair of functors $r\lor s$ and $\Hom (s;t)$.

For the  unit transform we have an arrow $x\dgl \Hom (a;x\lor a )$.

In  the case $x\dg a$ we shall have
$x\lor a\dg a$ and
$$ x= x\lor a= \Hom (a;x\lor a)\tsk$$

In another case $x\mzl a$ we shall have
$x\lor a\mzl a$, therefore
$$\Hom (a;x\lor a)=0\mzl x \tsk$$

Also it is  an arrow for the  counit transform $\Hom(a,y)\lor a \dgl y $.

In the case $y\dg a$
we shall have
$\Hom (a;y)=y$ and
$$\Hom (a;y )\lor a=y\lor a \dgl y\tsk$$

In  another case $y\mzl a$ we shall have  $\Hom(a;y)=0$ and
$$\Hom (a;y)\lor a= a\dgl y\tsk$$

The triangular equalities are get  automatically, therefore we have
the true joint pair of functors $r\lor s$ and $ \Hom(s;t)$ provided
with assistant member
$s\in [0,\infty]$.

So we have got   a closed category again.
It will be called ^{Cartesian closed =category} in the
scalar space $[0,\infty]$.
 We shall use a sign
$[0,\infty]^+_{\Carte}$ for it.
Now we get a ^{=translation}  of monoidal categories
$$F:[0,\infty]^+\doublerightarrow [0,\infty]^+_{\Carte}\tsk$$
Denoting $r\sqprod s= r\lor s$
we have needed natural transform
$$t_{r,s}:(r\otimes s)^F\rightarrow r^F\sqprod s^F\kbl$$
and identity arrow for coinciding neutral points
$\bar e=e^F=0\in [0,\infty]^+_{\Carte} $.
$$t_e:e^F\rightarrow  \bar e\tsk$$

We recognize the original  $[0,\infty]^+_{\Carte}$-graph  $X$ as ultrametric
space, i. e. we have inequalities for scalars $X(x;y)$
$$0\dgl X (x,y)\kbl$$
$$X(x;y)\lor X(y;z)\dgl X(x;z)\tsk$$

The former translation provides imbedding for the
categories of original graphs
$$\OGrph_{[0,\infty]^+_{\Carte}} \subset \OGrph_{[0,\infty]^+}\tsk$$
The new tensor product of ultrametric spaces
$X\sqprod T$ is defined with smaller distance
$$X(x;y)\sqprod A(a,b)\mzl X(x;y)\otimes A(a;b)\kbl$$
but an exponential  superfunctor appoints the same functional space.
 It is compounded of all nonexpanding mappings
$\phi: T\rightarrow X$.
And for two nonexpanding mappings
$\phi:A\rightarrow Y$ and $\psi: A\rightarrow Y$
 we have again the distance of uniform convergence
$$\Hom(T;Y) (\phi;\psi)= \sup_{a\in A} Y(\phi(a);\psi(a))\tsk$$

This tensor product $X\sqprod Y$
   can be defined for arbitrary metric spaces  $X$ and $Y$
   defined with the initial  category $\Grph_{[0,\infty]}$,

In the case of ultrametric target space $Y$ we
again have equivalent properties for a  mapping
$\Phi: X\times A\rightarrow Y$
from
arbitrary metric spaces $X$ and $A$
to be  nonexpanding over the new tensor product of
ultrametric spaces
$$X(x;x')\lor  A(a;a')\dgl Y(\Phi(x,a);\Phi(x';a'))$$
and  for the partial mapping
$\Phi_1: X\rightarrow Y^A$   to be nonexpanding with  the metric of uniform
boundary
 $$X(x;x') \dgl \sup_{a\in A} Y(\Phi(x,a);\Phi(x';a))\tsk$$

\Proposition
For arbitrary metric spaces $X$ and $A$ and ultrametric space $Y$
we have equivalent properties  for mapping
$\Phi: X\times A\rightarrow Y$ to be  nonexpanding over the new
tensor product of
ultrametric spaces
$$X(x;x')\lor  A(a;a')\dgl Y(\Phi(x,a);\Phi(x';a'))$$
and  for the partial mapping
$\Phi_1: X\rightarrow Y^A$   to be nonexpanding with  the metric of uniform
boundary
 $$X(x;x') \dgl \sup_{a\in A} Y(\Phi(x,a);\Phi(x';a))\tsk$$
\Proof:
Let we have the first inequality
$$ X(x,x')\lor A(a;a')\dgl Y(\Phi(x,a);\Phi(x';a'))\tsk$$
Then we get
$$ X(x;x')\dgl Y(\Phi(x,a);\Phi(x';a))\uparrow a\in A\kbl$$
$$X(x;x')\dgl \sup_{a\in A} Y(\Phi(x,a);\Phi(x',a'))\tsk$$

Otherwise from the second inequality  for arbitrary nonexpanding mappings
$\Phi_1(x)\in Y^A$
we get the inequality
$$X(x;x') \dgl Y(\Phi(x,a);\Phi(x';a))\kbl $$
and for the ultrametric in space $Y$ we can apply triangular inequality
$$Y(\Phi(x,a);\Phi(x';a'))\mzl Y(\Phi(x;a);\Phi(x';a))\lor
Y(\Phi(x';a); \Phi(x';a')) \mzl
$$$$X(x;x')\lor A(a;a')\tsk$$
\irodymopabaiga

Seeking to understand this mathematical fact, I have gone astray
for one year in the theory of enriched graphs.
For the better illustration  we  could  work with more
general values category
$\Ban$ of Banach spaces.

We shall generalize the notion of monoidal category $\VV$. Let we have
defined some biproduct as bifunctor
$$\otimes : \VV\times \VV\doublerightarrow \VV$$
with neutral point $e\in\VV_0$. For it we have natural transforms
for left canceling defined with right projection
$$r_a: e\otimes a \rightarrow a$$
and another transform for right canceling  defined with left projection
$$\ell_a: a\otimes e \rightarrow a \tsk$$
Usually we shall take a category's $\VV$ final object $*\in \VV_0$
as a neutral point for taken biproduct.

Also we can ask a natural transform  for associativity
defined  with arrows
$$s_{a,b,c} : a\otimes (b\otimes c)\rightarrow (a\otimes b)\otimes c\tsk$$
So we  get the classical monoidal category if such natural transforms
are defined with isomorphic arrows.

Demanding the pentagon diagram
$$\matrix{
& a\otimes (b\otimes (c\otimes d))&\mapright s
&(a\otimes b)\otimes (c\otimes d) &  \cr
%
\hfill 1\otimes s \hskip -20 pt &\swarrow  &
 &\searrow &\hskip-20pt s\otimes 1 \hfill  \cr
\hfill a\otimes ((b\otimes c)\otimes d) \hskip -30pt & \maprightap s &
(a\otimes (b\otimes c))\otimes d &\maprightap s\otimes 1 &
\hskip-30pt ((a\otimes b)\otimes c)\otimes d \hfill\cr}$$
\vskip\tarpas
the triangular diagram
$$\matrix { & a\otimes (e\otimes c) & \mapright s & (a\otimes e)\otimes c& \cr
\hfill 1\otimes\ell \hskip -20 pt&\searrow  & & \swarrow & \hskip -20 pt
r\otimes 1 \hfill  \cr
&& a\otimes c & & \cr } $$
\vskip\tarpas
and  equal
arrows
$$\ell_e= r_e: e\otimes e\rightarrow e $$
for classical monoidal category we get  a tensor product.
By coherence theorem in \baf S. MacLane 1971*  part VII we get
a unique canonical isomorphic arrow
between  tensor products defined for arbitrary two binary words
of the same length.

Later for the working with $\VV$-enriched spaces we shall ask
a natural transform of ^{=relator's involution}
$$m_{p,r,s,t} : (p\otimes s)\otimes (r\otimes t) \rightarrow (p\otimes r)
\otimes (s\otimes t) \tsk$$
For associative tensor product this property is weaker than
commutativity property. 

Also we demand the ^{upper =continuity} for the Carte products
$$\Prod_i p_i\otimes \Prod_i r_i= \Prod_i p_i\otimes r_i\tsk$$

Let in the category $\VV$ we have another biproduct $r\sqprod s$ which is a
 relator for the first tensor product $r\otimes s$
with a natural transform defined with arrows
$$N_{p,r,s,t}: (p\sqprod s)\otimes (r\sqprod t)\rightarrow (p\otimes r)
\sqprod (s\otimes t ) $$
and the same neutral member with natural cancellation transforms defined by
 arrows
$$*\sqprod r\rightarrow  r\leftarrow r\sqprod *\tsk$$
We shall demand that these canceling arrows will be isomorphisms
$$*\sqprod r=\rightarrow  r\leftarrow= r\sqprod *\tsk$$
Then we have inclusion arrows
$$r\otimes s \rightarrow (r\sqprod *)\otimes (s\sqprod *)\rightarrow
(r\sqprod s) \otimes (*\sqprod *)\rightarrow r\sqprod s\tsk$$
which will be ^{=comparison arrows }
 between two biproducts
$$t_{r,s}: r\otimes s\rightarrow r\sqprod s \tsk$$
Translation of values category is defined by transport of monoidal
categories $F: \VV\doublerightarrow \VV'$  with comparison arrows
$$t_{a,b}: a^F\sqprod b^F\rightarrow (a\otimes b)^F\kbl$$
$$t_e: \bar e \rightarrow e^F\tsk$$

We get a ^{continuous =translation} of values category  $\VV$ to the
new values category $\VV'$  with the same points $r\in \VV_0$ and arrows
$\alpha\in \VV$ but with a new biproduct $x\sqprod s$
$$F:\VV \doublerightarrow \VV'\tsk$$
For
objects  and arrows we have identity functor
$$F_0(r)=r\kbl \alpha^F=\alpha\uparrow r\in\VV_0, \alpha\in V(r;s)\tsk$$

Such translation will be continuous for biproducts
$$\matrix { \VV\times \VV & \mapright F\times F & \VV' \times \VV'&\cr
\mapdownk { \otimes} &  & \mapdownd {\sqprod  } &  \cr
   \VV  & \maprightap F & \VV' & \cr
   &  & & \hskip-10pt \nearrow \hfill \cr}$$
   \vskip\tarpas
 i. e. we have
continuous square with natural transform of comparison defined
with arrows
$$t_{r,s}: (r\otimes s)^F\rightarrow r^F\sqprod s^F $$
Also we ask the continuity for chosen neutral member
 $e^F\rightarrow \bar e$
 $$\matrix { * & = &* & \cr
           \mapdownk e & &\mapdownd \bar e  & \cr
           \VV &\maprightap F & \VV' &\cr
           & & & \hskip-10pt \nearrow \hfill \cr }$$
\vskip\tarpas

If the new biproduct is associative with natural transform defined
by  arrows
$$s'_{a,b,c}: a\sqprod (b\sqprod c)\rightarrow (a\sqprod b)\sqprod c\kbl$$
we should demand that two continuous  quadrats would be coherent for
associativity transforms.
Such continuous quadrats
are defined for a  functor $F: \VV\doublerightarrow \VV'$
with ^{=convergences} defined by bifunctors  of different biproducts
$\VV\times \VV \doublerightarrow \VV\otimes \VV$  and $\VV'\times\VV'
\doublerightarrow \VV'\sqprod \VV'$
$$\matrix {\VV\times (\VV\times \VV) & \mapright F\times (F\times F) &
\VV'\times (\VV'\times \VV') & \cr
\downarrow & & \downarrow & \cr
\VV\times (\VV\otimes \VV) & \mapright F\times F  &
\VV'\times (\VV'\sqprod \VV') & \cr
& &  & &\hskip-15pt \nearrow \hfill \cr
\downarrow & &\downarrow & \cr
\VV\otimes (\VV\otimes \VV) & \maprightap F &\VV'\sqprod (\VV'\sqprod \VV')&
\cr
&  & & \hskip-10pt \nearrow t \hfill \cr }$$
\vskip\tarpas
and
$$\matrix{ (\VV\times \VV)\times \VV & \mapright (F\times F)\times F &
(\VV'\times \VV')\times \VV' & \cr
\downarrow & & \downarrow & \cr
(\VV\otimes \VV)\times \VV & \mapright F\times F  &
(\VV'\sqprod \VV')\times  \VV' & \cr
& &  & &\hskip-15pt \nearrow \hfill \cr
\downarrow & &\downarrow & \cr
(\VV\otimes \VV)\otimes \VV & \maprightap F &(\VV'\sqprod\VV')\sqprod \VV' &  \cr
&  & & \hskip-10pt \nearrow t \hfill \cr }$$
\vskip\tarpas
The natural transform between two coherent  graphs is defined
with vertexes in the same spaces and   arrows of transform between
them. It can be explain by graphs of continuous mapping for two
coherent convergences. In our case the convergences are defined by coherent
biproducts.
$$\hskip 55 pt\matrix {  &\bullet & \mapright (F\times F)\times F &  & \bullet  \cr
         \nearrow &  &  &\nearrow &  \cr
           & \downarrow  &    & & \downarrow  \cr
           &\bullet &\mapright F & &\bullet \cr
         \nearrow & &         &\nearrow & \cr}$$
\vskip -50pt
$$\matrix {  &\bullet & \mapright F\times (F\times F) &  & \bullet  \cr
        \phantom{ \nearrow} &  & \phantom{ \nearrow} &  & \cr
           & \downarrow  &    & & \downarrow  \cr
           &\bullet &\mapright F & &\bullet \cr
    \phantom{ \nearrow} & &         &\phantom{\nearrow} & \cr}
 $$

The coherence can be defined
by commuting diagram in the target space
$$\matrix { (\VV\otimes (\VV\otimes \VV))^F & \mapright s^F  &
((\VV \otimes \VV)\otimes  \VV)^F \cr
\mapdownk t & &\mapdownd t \cr
\VV'\sqprod (\VV'\sqprod \VV') & \mapright s' &
(\VV'\sqprod \VV')\sqprod \VV'\cr  }$$
For objects $a,b,c\in\VV$ we have equality of arrows compositions
$$ s^F_{a,b,c}\circ t_{(a,b),c}= t_{a,(b,c)} \circ s'_{a^F,b^F,c^F}:
(a\otimes (b\otimes c))^F \rightarrow ( a^F \sqprod b^F)\sqprod c^F \tsk$$
We have denoted arrows of horizontal composition for natural transforms
$$t_{a,(b,c)}=( 1_a\otimes t_{b,c})\circ t_{a, b\otimes c}\kbl$$
$$t_{(a,b),c} = (t_{a,b}\otimes 1_c ) \circ t_{a\otimes b,c}\tsk$$

For the inclusion of the sets $a\otimes b\subset a\sqprod b$
it demands that  a  mapping over the  larger  set would be restricted
to  the mapping over the smaller  set
$$\matrix{ (a\otimes (b\otimes c) & \subset & a\sqprod(b\sqprod c)\cr
\downarrow & & \downarrow \cr
(a\otimes b)\otimes c & \subset  & (a\sqprod b) \sqprod c \cr }$$
\vskip\tarpas
We shall say that translator $F: \VV\doublerightarrow \VV'$
is ^{=coherent for associativity transforms}.

In this case  the coherence theorem
for classical monoidal categories
will produce a restricted natural isomorphism for arbitrary binary word
with the smaller tensor product.

We want to explain why equality of
natural transforms in the ^{final =space} define the coherence
of the whole quadrat.
We can see that earlier defined equality is a unique choice.
We propose the procedure of reduction which can be applied also
for more complex coherent ^{=diagrams }.

Let we have the arrows of natural transform for every vertex  of diagram
$$\hskip 65 pt\matrix {  &\cdot & \rightarrow &  & \cdot &  \cr
         \nearrow &  &  &\nearrow & & \cr
           & \downarrow &    & & \downarrow & \cr
           &\cdot &\rightarrow &&\bullet&\hskip -10 pt{}_\nearrow\hfill \cr
                 \nearrow & &         &\nearrow & &\cr}$$
\vskip -45pt
$$\matrix {  &\circ & \rightarrow  &  & \cdot & \cr
        \phantom{ \nearrow} & & & \phantom{ \nearrow} &  & \cr
           & \downarrow  &    & & \downarrow &  \cr
           &\cdot &\rightarrow & &\cdot &\hskip -10pt {}_\nearrow \hfill \cr
    \phantom{ \nearrow} & &         &\phantom{\nearrow} && \cr}
 $$
We shall study all possible ^{=circuits} from initial vertex in the first quadrat
to the final vertex in the second quadrat.
We can "compress" two commuting quadrats in such diagram. This process
I have drawn by hand in \baf G. Valiukevi\v cius  1992* p. 123.
Now such drawing must be done by computer, and I haven't time for it
at this moment.

As the result we get a problem of coherent transforms for
 continuous triangle
$$\hskip 65pt \matrix{ &\cdot  & & & &\cr
             \nearrow &     & & &&  \cr
                      & \downarrow & \searrow & & & &\cr
  & \cdot    & \rightarrow  & & \bullet & \hskip-20 pt {}_\uparrow\hfill  \cr
 \nearrow &  & &
 \raise 3pt \hbox{$\nearrow$} \llap{\raise -3 pt\hbox{$\nearrow$}} & &\cr } $$
\vskip -52pt
$$\matrix{ &\circ  && && \cr
         \phantom{ \nearrow} &     & & & &\cr
           &\downarrow & \searrow& &&& \cr
      &\cdot  &  \rightarrow  & & \cdot &\hskip -20pt {}_\uparrow\hfill \cr
\phantom{\nearrow}          &   &   &\phantom{ \nearrow} & &\cr }
$$
\vskip\tarpas

We have drawn also another transported arrow in the final category.
It provides a commuting lower side.  So in the final category we get a
commuting quadrat  which is needed and provides
coherent transform for the whole diagram.

\vskip\tarpas
For more detailed work
it is possible to apply  another properties
of biproducts. We notice that we  are working with comparison arrows
for continuous translation. The opposite arrows  would define a
cocontinuous translation, and for it the product must be changed by
coproducts.

The biproduct $\otimes : \VV\times \VV\doublerightarrow \VV$
can be considered as a coadjoint functor
for the diagonal functor $\trik: \VV\doublerightarrow \VV\times \VV$.
The ^{=diagonal functor} for a object $r\in\VV_0$ appoints the couple
$\lan r,r\ran\in \VV_0\times \VV_0$ and for an arrow $u: r\rightarrow s$
appoints the couple of arrows
$$\lan u,u\ran: \lan r,r\ran\rightarrow \lan s,s\ran\tsk$$

The unit transform will be defined by ^{=diagonal arrows}
$$i_r: r\rightarrow r\otimes r \tsk$$
Such biproduct will be called ^{=diagonalized}. The counterexample
can be defined with non Hausdorff topology on the product space $X\times Y$.

In \baf G. Valiukevi\v cius 2009* p.107 the proposition 3c concludes
that comparison from  diagonalized  biproduct provides
another contact arrow  in the target category $\VV'$
$$t'= i^F\circ t: r^F\rightarrow r^F\otimes r^F\tsk$$
This was formulated as changing the  initial  point of diagram.
%
%
$$\matrix{\bigcirc \llap {1 }& \VV\times \VV &
\mapright F\times F & \VV'\times \VV'& \cr
& \mapdownk {\trik} \llap {$\mapupd {\otimes} $\hskip -5pt} &   &
\mapdownd {\sqprod'} & \cr
\bigcirc\llap {2 }  &\VV & \mapright F &\VV' &\cr
&    & && \hskip -10 pt \nearrow \hfill \cr}$$
\vskip\tarpas
We shall say that  we have got  contact arrows ^{=transported by  the
translation} $F: \VV\doublerightarrow \VV'$.
If we have  diagonal arrows also in the target category $\VV'$,
then translation $F: \VV\doublerightarrow \VV'$  will be called
^{=diagonalized  }  if the diagonal arrows  in the target category $\VV'$
extends the  transported diagonal  arrow.


The counit transform will be defined with pair of projections
$$\lan p_{r,s}^1,p_{r,s}^2 \ran: \lan r\otimes s,r\otimes s\ran \rightarrow
\lan r,s\ran\tsk$$
Such biproduct will be called projectable.

In \baf G. Valiukevi\v cius 1992* p. 171 we provide an example
of non projectable
biproduct for graphs.
In \baf G. Valiukevi\v cius 2009* p.  107  the proposition 3a concludes
that comparison from projectable biproduct  provides another projections
in the target category $\VV'$
$$t'= \lan t,t\ran \circ \lan p^1,p^2\ran \tsk$$
This was formulated as changing the final point of diagram
$$\matrix{\bigcirc\llap {1 }   & &   & & \hskip -10pt \nwarrow \hfill\cr
& \VV\times \VV & \mapright F\times F
& \VV'\times \VV' &\cr
&\mapdownk {\otimes} &  & \mapdownk {\trik } \llap {$\mapupd \sqprod' $
\hskip -7pt } & \cr
&\VV & \maprightap  F & \VV' &\cr
&  &                 &   & \hskip -10 pt \nearrow  \hfill \cr}$$
\vskip\tarpas
We shall call the  projections
$p^1: r^F\otimes s^F\rightarrow r^F$
and $p^2: r^F\sqprod s^F\rightarrow s^F$ ^{=transported by translation}
$F: \VV\doublerightarrow \VV'$. 
If we have projections  in the target category $\VV'$,  the translation
$F:\VV\doublerightarrow  \VV'$  will be called ^{=projectable}
 if the projections in target category $\VV'$ extends the transported
 projections.

We shall say that a biproduct $r\otimes s$ in a category $\VV$
is ^{almost =coadjoint} one, if it is projectable and diagonalized.
Accordingly the translation $F:\VV\doublerightarrow \VV'$ transports
the almost coadjoint biproduct if it is projectable and diagonalized.

The first triangular equality for a biproduct $r\otimes s$
$$\lan 1_r,1_r\ran=: \lan r,r\ran \mapright {\lan i_r,i_r\ran}
\lan r\otimes r,r\otimes r\ran \mapright {\lan p_1,p_2 \ran}  \lan r,r\ran$$
provides the injective name  appointment.
We express  that there is only one couple
of arrows $p\rightarrow r$ and
$p\rightarrow s$ providing  an arrow to this biproduct
$p\rightarrow r\otimes s $.


The faithful almost coadjoint translation
$F:\VV\doublerightarrow \VV'$ reflects the property of
target category $\VV'$ to have injective name appointment.

The second triangular equality for a biproduct $r\otimes s$
$$ 1_{r\otimes s}=: r\otimes s\mapright i_{r\otimes s}
\lan r\otimes s,r\otimes s\ran \mapright p^1\otimes p^2 r\otimes s $$
provides the injective realization appointment. We express  that there
is only one arrows
to the biproduct $p\rightarrow r\otimes s$  providing the couple of arrows
$p\rightarrow r$ and $p\rightarrow s$.

The faithful almost coadjoint translation
$F:\VV\doublerightarrow \VV'$ reflects the property of
target category $\VV'$ to have an injective realization appointment.

The almost coadjoint biproduct with both first and second triangular
equalities will be ^{truly =coadjoint} one, therefore it coincides
will the Carte product $r\times s$ up unique isomorphism.

These properties  were applied in \baf G. Valiukevi\v cius 1992 *  part 5.4
to study  the commuting diagrams in categories with abstract products. They
also will be useful for any detailed work with concrete categories.

The most special translation of monoidal categories
is defined with  isomorphic comparison arrows
$$t_{r,s}: (r\otimes s)^F=\rightarrow r^F\sqprod s^F\tsk$$
We shall call it a ^{strict =translation}. Such property
is meaningful even without the property of projectable tensor product.

\vskip\tarpas
In monoidal category $\VV$ the comparison arrow
$r\otimes s\rightarrow r\sqprod s$ provides the
restriction  of arbitrary arrow over the new biproduct
$r\square s\rightarrow t$. It is get as composition
$$r\otimes s \rightarrow r\sqprod s \rightarrow t\tsk$$

We can take the same exponential functor $t^s$ as coadjoint functor
for the functor defined with the new biproduct $r\sqprod s$.
We get again a sections arrow
$$\lambda'_r: r\rightarrow (
r\otimes s)^s \rightarrow( r\sqprod s)^s\tsk$$
However we can't get a truly joint pair again. We can't have  evaluation
arrows  $\ev_t:t^s\sqprod s\rightarrow t$ for arbitrary member $t\in\VV_0$.
It may be necessary also to use a smaller exponential space to
get possibility to define on it the evaluation arrow.

The same situation will be for the $\VV$-graphs.
In the category $\Grph_\VV$ we have a joint pair of superfunctors.
 An adjoint
functor of biproduct $X\otimes A$ is provided with the
tensor product $r\otimes s$ in the values category $\VV$ and a coadjoint functor
will be the exponential functor $Y^A$ provided by transforms between
$\VV$-graphs transports $\phi: A\doublerightarrow Y$. The new biproduct of
$\VV$-graphs $X\sqprod A$ is defined by the new biproduct $r\sqprod s$
in the values category $\VV$. We can work with another values category $\VV'$
and define the category of $\VV'$-graphs $\Grph_{\VV'}$.
Every $\VV'$-graphs transport $\phi: A\doublerightarrow Y$
will be also the $\VV$-graphs transport.  So the new category
 will be imbedded in the former category of $\VV$-graphs
$$\Grph_{\VV'}\subset \Grph_{\VV}\tsk$$
However the  exponential space $(Y^A)'$
for $\VV'$-graph $Y$ will be smaller and imbedded
in the  former exponential space from  category $\Grph_{\VV}$.
We expose such remarks more carefully.

Within the category of $\VV$-graphs  $\Grph_{\VV}$ we can  define
another biproduct $X\sqprod Y$.   For vertexes  sets we take
the same Carte tensor product $X_0\times Y_0$ and for edges sets
we take the $\sqprod$-biproducts in the values category $\VV$
$$X\sqprod Y(\lan x,y\ran;\lan x',y'\ran):= X(x;x')\sqprod Y(y;y')\tsk$$
For $\VV$-graphs transports $f: X\doublerightarrow X'$ and
$g: Y\doublerightarrow Y'$ we define a new biproduct
$$f\sqprod g: X\sqprod Y\doublerightarrow X'\sqprod Y' $$
having the new edges set mappings
$$(f\sqprod g)_{\lan x,y\ran,\lan x',y'\ran} = f_{x,x'}\sqprod g_{y,y'}:
$$$$X(x;x')\sqprod Y(y;y')\rightarrow X'(f_0(x);f_0(x'))\sqprod
Y'(g_0(y);g_0(y')) \tsk$$

We have got a new bisuperfunctor in the category of
$\VV$-graphs $\Grph_{\VV}$.
We additionally can check that we have got a bisuperfunctor also in smaller
categories of original $\VV$-graphs or in the category of $\VV$-enriched
categories  with continuous functors $\Cat_{\VV}^+$,
cocontinuous functors $\Cat_{\VV}^-$  or exact functors $\Cat_{\VV}^=$.

Indeed. We take the unit arrow mappings transported with such bisuperfunctor.
For the unit arrow mappings $1_x:*\rightarrow 1_x(*)\subset X(x;x)$ and
$1_y:*\rightarrow 1_y(*)\subset Y(y;y)$ it appoints the biproduct
$$1_{\lan x,y\ran}=1_x\sqprod 1_y: * \rightarrow 1_x(*)\sqprod 1_y(*)
\subset X(x;x)\sqprod Y(y;y)\tsk$$
If these $\VV$-graphs transports have maintained the  unit arrow
mappings
$$1_x \circ f_{x,x}= 1_{f_0(x)}\kbl 1_y\circ g_{y,y} = 1_{g_0(y)} \kbl$$
then we get maintained unit arrows mappings also in the biproduct of
$\VV$-graphs $X\sqprod Y$
$$(1_x\sqprod 1_y)\circ (f_{x,x}\sqprod g_{y,y}) =
(1_x \circ f_{x,x}) \sqprod (1_y\circ g_{y,y})=
 f_{f_0(x)}\sqprod 1_{g_0(y)}\tsk $$
The contact arrows mappings are also transported by
taken bisuperfunctor.
In the new biproduct of $\VV$-graphs  $X\sqprod Y$ the contact
arrows mappings
are defined with the $\sqprod$-product of contact arrows mappings
for each  component
$$(X\sqprod Y(\lan x,y\ran; \lan x',y'\ran) )\otimes
(X\sqprod Y(\lan x',y'\ran; \lan x'',y''\ran ))=
$$$$(X(x;x')\sqprod Y(y;y') )\otimes (X(x';x'')\sqprod Y(y';y''))\rightarrow
$$$$(X(x;x')\otimes X(x';x''))\sqprod (Y(y;y')\otimes Y(y';y'')\rightarrow
$$$$ (X(x;x')\circ X(x';x''))\sqprod (Y(y;y')\circ Y(y';y'')\subset
$$$$X(x;x'')\sqprod Y(y;y'')= X\sqprod Y(\lan x,y\ran ;\lan x'',y''\ran)\tsk$$

The equalities for the chosen unit arrow mappings
$$1_x(*)\circ X(x;x')= X(x;x')= X(x;x')\circ 1_{x'}(*) \kbl$$
$$1_y(*)\circ Y(y;y')= Y(y;y')\circ 1_{y'}(*) $$
provides correspondent equalities in the new biproduct of $\VV$-graphs
$X\sqprod Y$. We shall write only for the first equalities
$$1_{\lan x,y\ran}(*) \otimes (X\sqprod Y(\lan x,y\ran; \lan x',y'\ran) )
=
$$$$(1_x(*) \sqprod 1_y(*) )\otimes (X(x;x')\sqprod Y(y;y')\rightarrow
$$$$(1_x(*)\otimes X(x;x'))\sqprod (1_y(*)\otimes Y(y;y'))\rightarrow
$$$$(1_x(*)\circ  X(x;x'))\sqprod (1_y(*)\circ Y(y;y'))=
$$$$ X(x;x')\sqprod Y(y;y')=
$$$$ X\sqprod Y (\lan x,y\ran;\lan x',y'\ran) \tsk$$

So for  original $\VV$-graphs $X$and $Y$ we get the original $\VV$-graph
$X\sqprod Y$ again.
We have got that bisuperfunctor $X\otimes Y$ can be restricted in the
category of crude functors between original $\VV$-graphs $\OGrph_{\VV}$.

For a natural ^{=relator's transform} defined with arrows
$$n_{r,r',s,s'}: (r\sqprod r')\otimes (s\sqprod s')\rightarrow
  (r\otimes s)\sqprod (r'\otimes s')$$
we can prove that the new bisuperfunctor also maintains natural functors,
i. e. we have commuting diagram again for the contact arrows mappings.
First we have commuting diagram
$$\hskip-10pt \matrix{ (X(x;x')\sqprod Y(y;y')) \otimes (X(x';x'')\sqprod Y(y';y'')) &
\hskip-10pt \rightarrow \hfill\cr
%
\mapdownk (f_{x;x'}\sqprod g_{y;y'})\otimes (f_{x';x''}\sqprod g_{y',y''})
&\cr
%
(X'(f_0(x);f_0(x'))\sqprod Y'(g_0(y);g_0(y'))\otimes (X'(f_0(x');f_0(x'')
\sqprod Y'(g_0(x');g_0(y''))) & \hskip -10 pt \rightarrow \hfill \cr}$$
\vskip\tarpas
%
 $$\hskip -10 pt\matrix{
 (X(x;x')\otimes X(x';x''))\sqprod (Y(y;y')\otimes Y(y';y''))\cr
%
 \mapdownd (f_{x,x'}\otimes f_{x',x''})
\sqprod (g_{y,y'}\otimes g_{y',y''}) \cr
%
(X'(f_0(x);f_0(x'))\otimes X'(f_0(x');f_0(x''))\sqprod
(Y'(g_0(y);g_0(y'))\otimes Y'(g_0(y');g_0(y'')))\cr } $$
\vskip\tarpas

Having commuting diagrams
for a natural functor $f: X\doublerightarrow X'$

$$\matrix{ X(x;x')\otimes  X(x';x'') & \mapright {\circ }  & X(x;x'') \cr
\mapdownk f_{x,x'}\otimes f_{x';x''} &  & \mapdownd f_{x;x''} \cr
X'(f_0(x);f_0(x'))\otimes X'(f_0(x');f_0(x'')) & \maprightap {\circ } &
X'(f_0(x);f_0(x'')) \cr }$$
\vskip\tarpas
and  for another exact functor $g: Y\doublerightarrow Y'$
$$\matrix{ Y(y;y')\otimes  Y(y';y'') & \mapright {\circ }  & Y(y;y'') \cr
\mapdownk g_{y,y'}\otimes g_{y';y''} &  & \mapdownd g_{y;y''} \cr
Y'(g_0(y);g_0(y'))\otimes Y'(g_0(y');g_0(y'')) & \maprightap {\circ } &
Y'(g_0(y);g_0(y'')) \cr }$$
\vskip\tarpas
we get commuting diagram for the new biproducts of arrows
$$\hskip -10pt \matrix{ (X(x;x')\otimes  X(x';x''))
\sqprod(Y(y;y')\otimes  Y(y';y''))  \cr
%
\mapdownk (f_{x,x'}\otimes f_{x';x''})\sqprod (g_{y,y'}\otimes g_{y';y''}) \cr
%
(X'(f_0(x);f_0(x'))\otimes X'(f_0(x');f_0(x'')))\sqprod (
Y'(g_0(y);g_0(y'))\otimes Y'(g_0(y');g_0(y'')) ) \cr}$$
\vskip\tarpas
$$\matrix{   \rightarrow  & X(x;x'')\sqprod Y(y;y'') \cr
%
  & \mapdownd f_{x;x''}\sqprod g_{y,y''} \cr
 \rightarrow  &
X'(f_0(x);f_0(x''))\sqprod Y'(g_0(y);g_0(y'')) \cr }$$
\vskip\tarpas
and finally
the commuting diagram for the biproduct of functors
$$\hskip -10 pt \matrix{ (
X(x;x')\sqprod Y(y;y')) \otimes (X(x';x'')\sqprod Y(y';y'')) &
\hskip -10 pt \rightarrow \hfill\cr
%
\mapdownk (f_{x,x'}\sqprod g_{y,y'})\otimes (f_{x',x''}\sqprod g_{y',y''}) &
\cr
%
(X'(f_0(x);f_0(x'))\sqprod Y'(g_0(y);g_0(y'))\otimes (X'(f_0(x');f_0(x'')
\sqprod
Y'(g_0(x');g_0(y''))) & \hskip -10pt \rightarrow \hfill \cr}$$
 \vskip\tarpas
$$\matrix { \rightarrow & X(x;x'')\sqprod Y(y;y'')\cr
%
& \mapdownd f_{x,x''}\sqprod g_{y,y''} \cr
%
\rightarrow &
X'(f_0(x);f_0(x''))\sqprod Y'(g_0(y);g_0(y''))\cr } $$
\vskip\tarpas
So we have shown that taken bisuperfunctor can be restricted in
the category of original $\VV$-graphs with natural  functors $\OGrph_{\VV}^=$.

For weaker assumption about arrows
$n_{r,r',s,s'}$, we can prove restriction of taken bisuperfunctor
in larger partial categories.
For cocontinuous arrows $n_{r,r',s,s'}$ we get restriction in the category
of original $\VV$-graphs with continuous functors $\OGrph_{\VV}^+$,
and for continuous arrows $n_{r,r',s,s'}$ we get restriction in
the category of cocontinuous functors $\OGrph_{\VV}^-$.
The earlier proving for tensor product $X\otimes Y$ will be considered
as a partial case.

Finally we shall study biproducts in the category of $\VV$-enriched categories.
Let the new biproduct in values category $\VV$
is also associative with natural isomorphisms
$$s'_{r,s,t}:r\sqprod (s\sqprod t)= \rightarrow (r\sqprod s)\sqprod t $$
and comparison arrows
$$t_{p,r}: p\otimes r\rightarrow p\sqprod r $$
are coherent for associativity isomorphisms, i. e.we have commuting
diagram
$$ s^F_{a,b,c}\circ t_{(a,b),c}= t_{a,(b,c)} \circ s'_{a^F,b^F,c^F}:
(a\otimes (b\otimes c))^F \rightarrow ( a^F \sqprod b^F)\sqprod c^F \tsk$$

We shall use relator's involution, which is defined with
 isomorphic arrows
$$m_{p,r,s,t} : (p\otimes s)\otimes (r\otimes t)=\rightarrow (p\otimes r)
\otimes (s\otimes t) \kbl$$
The contact arrows mappings
$$X_{a,b,c}: X(a,b)\otimes X(b;c) \rightarrow X(a;c) $$
defines a functor over pullbacked tensor product
$$\circ : X\otimes_p X \doublerightarrow X\tsk$$
Repeating relator's mapping we get isomorphisms
$$( X\otimes Y )\otimes_p ((X\otimes Y)\otimes_p (X\otimes Y))=\rightarrow
$$$$ (X\otimes p (X\otimes_p X) \otimes (Y\otimes_p (Y\otimes_p Y))\kbl$$
$$((X\otimes Y)\otimes_p (X\otimes Y))\otimes_p (X\otimes Y)=\rightarrow
$$$$ ((X\otimes_p (X\otimes_p X))\otimes ((Y\otimes_p Y)\otimes_p Y)\tsk$$
Therefore the associativity transforms  for each component
$$X\otimes_p (X\otimes_p X)\rightarrow ( Y\otimes_p X)\otimes_p X\kbl$$
$$Y\otimes_p (Y\otimes_p Y)\rightarrow (Y\otimes_p Y)\otimes_p Y $$
provides the transform  for the associativity of tensor product
$$( X\otimes Y )\otimes_p ((X\otimes Y)\otimes_p (X\otimes Y))\rightarrow
((X\otimes Y)\otimes_p (X\otimes Y))\otimes_p (X\otimes Y)\tsk$$

There isn't any obvious way to define associativity transform
for the new biproduct of $\VV$-categories.
We can assume that  relator's arrows
$$n_{p,r,s,t}: (p\sqprod s)\otimes (r\sqprod t)=\rightarrow (p\otimes r)
\sqprod (s\otimes t ) $$
are get from involution arrows
$$m_{p,r,s,t} : (p\otimes s)\otimes (r\otimes t)\rightarrow (p\otimes r)
\otimes (s\otimes t) \kbl$$
by some topological extension of continuous mapping.
So the associativity  transform can be provided  also by topological
extension of continuous mapping
$$X\sqprod Y\otimes_p ( X\sqprod Y\otimes_p X\sqprod Y)\rightarrow
(X\sqprod Y \otimes_p X\sqprod Y) \otimes_p X\sqprod Y\tsk $$

Then in the new product of $\VV$-graphs defined contact arrows mappings
will  again provide an associative composition,  These
 contact arrows mappings
will define the functor over pullbacked product
$$(X\sqprod Y )\otimes_p (X\sqprod Y)\doublerightarrow X\sqprod Y$$
as composition of relator's transform
with contact arrows mappings  for each component $X$ and $Y$
$$(X\sqprod Y)\otimes_p (X\sqprod Y) \mapright N   (X\otimes _p X)\sqprod
(Y\otimes _p Y) \mapright {\circ \sqprod \circ} X\sqprod Y \tsk$$
In each $\VV$-enriched category we have commuting diagram for associative
composition
$$\matrix{X\otimes_p (X\otimes_p X) &  & \mapright S & &
  (X\otimes_pX)\otimes_p X) \cr
%
\mapdownk {1_X\otimes \circ} & & & &\mapdownd {\circ \otimes 1_X} \cr
%
\hskip 20 pt X\otimes_p X \hskip-20 pt&   & &  &
\hskip -20pt X\otimes X \hskip 20 pt \cr
%
\circ \hskip -20pt & \searrow &  & \swarrow & \hskip -20 pt \circ \cr
%
& & X & & \cr} $$
and
$$\matrix{Y\otimes_p (Y\otimes_p Y) &  & \mapright S & &
  (Y\otimes_pY)\otimes_p Y \cr
%
\mapdownk {1_Y\otimes \circ} & & & &\mapdownd {\circ \otimes 1_Y} \cr
%
\hskip 20 pt Y\otimes_p Y \hskip-20 pt&   & &  &
\hskip -20pt Y\otimes_p Y \hskip 20 pt \cr
%
\circ \hskip -20pt & \searrow &  & \swarrow & \hskip -20 pt \circ \cr
%
& & Y & & \cr} $$
\vskip\tarpas
We shall check such commuting diagram for the contact arrows mappings
from the biproduct $X\sqprod Y$.
It was for the tensor product $X\otimes Y$, i. e. we have commuting
^{double =diagram}.
For them we get  generated commuting diagrams. For example with
commuting triangles
$$\matrix { X &\rightarrow & Y\cr
              & \searrow &\downarrow \cr
              & & Z\cr}
              \hskip 20 pt
  \matrix { X' &\rightarrow & Y'\cr
              & \searrow &\downarrow \cr
              & & Z'\cr}$$
 we get also the commuting triangle of  biproducts
$$  \matrix { X\otimes X' &\rightarrow & Y\otimes Y'\cr
              & \searrow &\downarrow \cr
              & & Z\otimes Z'\cr}$$
So we can get  commuting diagrams of arrows composition
in the tensor product $X\otimes Y$. This diagram can be changed to the double
diagram using relator's involution
$$\hskip -17pt \matrix{(X\otimes Y)\otimes_p ((X\otimes Y)\otimes_p (X\otimes Y)) &
 \mapright S  &
  ((X\otimes Y)\otimes_p(X\otimes Y))\otimes_p (X\otimes Y) \cr
%
\mapdownk {1_{X\otimes Y}\otimes \circ}  & &
\mapdownd {\circ \otimes 1_{X\otimes Y}} \cr
%
\hskip 20 pt (X\otimes Y)\otimes_p (X\otimes Y) \hskip-20 pt    &  &
\hskip -20pt (X\otimes Y)\otimes_p (X\otimes Y )\hskip 20 pt \cr
%
\circ  \searrow &  & \swarrow  \circ \cr
%
&  X\otimes Y  & \cr} $$
\vskip\tarpas
Now we get again a commuting diagram for topological extended continuous
mappings
$$\matrix{(X\sqprod Y)\otimes_p ((X\sqprod Y)\otimes_p (X\sqprod Y)) &
 \mapright S  &
  ((X\sqprod Y)\otimes_p(X\sqprod Y))\otimes_p (X\sqprod Y) \cr
%
\mapdownk {1_{X\sqprod Y}\otimes \circ}  & &
\mapdownd {\circ \otimes 1_{X\sqprod Y}} \cr
%
\hskip 20 pt (X\sqprod Y)\otimes_p (X\sqprod Y) \hskip-20 pt&    &
\hskip -20pt (X\sqprod Y)\otimes_p (X\sqprod Y )\hskip 20 pt \cr
%
\circ  \searrow &  & \swarrow  \circ \cr
%
 & X\sqprod Y  & \cr} $$
\vskip\tarpas
We can get restriction of taken bisuperfunctor $X\sqprod Y$ in the categories of
$\VV$-enriched categories with crude functors $\Cat_{\VV}$,
with  continuous functors $\Cat_{\VV}^+$, with cocontinuous functors
$\Cat_{\VV}^-$ or with exact functors $\Cat_{\VV}^=$.
\vskip\tarpas

Let we take an assistant $\VV$-enriched category $A$.
Then we  define a superfunctor $F$ for a
$\VV$-enriched category $X$ appointing the $\sqprod$-product $X\sqprod A$ of
taken $\VV$-enriched
category $X$ with the assistant  $\VV$-enriched category $A$
 and for transports of $\VV$-enriched categories  $f:X\rightarrow Y$
 appointing the $\sqprod$-product of transports
 $f\sqprod \Identity_A:X\sqprod A\rightarrow Y\sqprod A$.
We get  a superfunctor in the category of $\VV$-graphs, also in
smaller categories
of original $\VV$-graphs or $\VV$-enriched categories.

We shall try for the new biproduct of $\VV$-graphs $X\sqprod Y$
to define a  coadjoint exponential  superfunctor.
We take a category of $\VV'$-graphs $\Grph_{\VV'}$.
We have continuous translation of values category
$\VV\doublerightarrow \VV'$ which change only biproduct
with natural arrows of comparison
$t_{r,s}: r\otimes s\rightarrow r\sqprod s $.
Therefore every $\VV'$-graph $X$ will be  a $\VV$-graph, and every
$\VV'$-graphs transport $f: X\doublerightarrow Y$ will rest
a $\VV$-graphs transport, i. e. we  get embedding of categories
$$\Grph_{\VV'}\subset \Grph_{\VV}\tsk$$
In reality we have coincidence of these two categories.

The choosing of unit arrows $1_x(*)\subset X(x;x)$ is also the same
for enriched graphs in both  categories.

The difference will appear only when we shall work with contact  arrows
mappings. Every contact arrows mapping
$X(a;b)\sqprod X(b;c) \rightarrow X(a;c)$ can be restricted over
the tensor product in values category $\VV$.
We get  a new mapping with  composition
$$X(x;y)\otimes X(y;z) \rightarrow X(x;y)\sqprod X(y;z)\rightarrow
X(y;z)\circ X(y;z)\subset X(x;z)\tsk$$
For a $\VV'$-graph $X$ with contact arrows mappings we appoint a new
$\VV$-graph $X'$ with restricted contact arrows mappings.

The choice of unit arrow remains neutral for such restricted
contact arrows mapping. The neutral property for the source of arrows
will be expressed by commuting diagram
$$\matrix {  & & X(x;y) \cr
        &\swarrow & \downarrow \cr
  *\otimes X(x;y) & = & *\sqprod X(x;y) \cr
  \mapdownk 1_x\otimes 1 &  & \mapdownd 1_x\sqprod 1 \cr
  X(x;x)\otimes X(x;y) & \mapright t & X(x;x)\sqprod X(x;y) \cr
  & \searrow & \mapdownd {\circ}  \cr
  & & X(x;y) \cr }$$
  \vskip\tarpas
The neutral property for the target of arrows will be expressed
with the similar commuting diagram.

So we get that every original $\VV'$-graph remains original $\VV$-graph
with  restricted contact arrows mappings i. e.
we have faithful imbedding of correspondent category with crude functors
$$\OGrph_{\VV'}\superrightarrow \OGrph_{\VV} \tsk$$

Any continuous, cocontinuous or natural functor between  original
$\VV'$-graphs rests such in the category of original $\VV$-graphs.
We apply the natural property of comparison arrows. There is
the diagram for a continuous transport $f: X\doublerightarrow Y$
$$\matrix { X(x;y)\otimes  X(y;z) & \rightarrow &
f(X(x;y))\otimes f(X(y;z))& \cr
\mapdownk t & & \mapdownd t & \cr
X(x;y)\sqprod  X(y;z) & \rightarrow & f(X(x;y))\sqprod f(X(y;z))& \cr
\mapdownk {\circ}  & & \mapdownd {\circ} & \cr
X(x;y)\circ X(y;z) & \rightarrow & f(X(x;y))\circ f (X(y;z)) &\cr
                   &   &  &\hskip-20pt \nearrow \hfill\cr }$$
\vskip \tarpas
We have checked faithful embedding of corresponding categories of
original graphs with continuous functors
$\OGrph_{\VV'}^+\superrightarrow \OGrph_{\VV}^+$, with cocontinuous
functors
$\OGrph_{\VV'}^-\superrightarrow \OGrph_{\VV}^-$, and with
natural functors $\OGrph_{\VV'}^=\superrightarrow \OGrph_{\VV}^=$.

Also we can check that restricted contact arrows mappings
maintain the property of associativity.

Let we have commuting diagram for edges set mappings in $\VV'$-graph
$X$
$$\hskip -10 pt\matrix{X(x;y)\sqprod (X(y;z)\sqprod X(z;u)) \hskip -10 pt &
  & \mapright s' & &
  (X(x;y)\sqprod X(y;z))\sqprod X(z,;u) \cr
%
\mapdownk {1_{X(x;y)}\sqprod X_{y,z,u}} \hskip 20 pt & & & &
\mapdownd {X_{x,y,z}\sqprod 1_{X(z,u)}} \cr
%
\hskip 20 pt X(x;y)\sqprod X(y;u) \hskip-20 pt&   & &  &
\hskip -20pt X(x;z)\sqprod X(z;u) \hskip 20 pt \cr
%
X_{x,z,u} \hskip -20pt & \searrow &  & \swarrow & \hskip -20 pt X_{x,z,u} \cr
%
& & X(x;u) & & \cr} $$
\vskip \tarpas
We must check commuting diagram for deformed restricted diagram  with
correspondent comparison arrows
$$\matrix {
&\hskip -10pt \nearrow \hfill && & & & & \hskip-10pt \nearrow\hfill\cr
\bullet & & &\rightarrow && &\bullet & \cr
\downarrow & & &      && & \downarrow & \cr
&\hskip -10pt  \nearrow \hfill & &  & & & & \hskip-10pt \nearrow \hfill\cr
\bullet & & &    &    & & \bullet & \cr
  & &\searrow & & & \swarrow &  & \cr
& & & & \hskip-12pt \nearrow \hfill & & & \cr
& & & \bullet & & & & & \cr}$$
\vskip\tarpas
We need only to check commuting quadrats  for corespondent comparison arrows.
For the upper side we have commuting diagram by
an assumption of coherence for associativity transforms by the
 continuous translation $\VV\doublerightarrow \VV"$
$$\matrix{ X(x;y)\otimes (X(y;z)\otimes X(z;u)) & \mapright s &
(X(x;y) \otimes X(y;z))\otimes X(z;u) \cr
\mapdownk t & & \mapdownd t \cr
X(x;y)\sqprod (X(y;z)\sqprod X(z;u)) & \mapright s' &
(X(x;y) \sqprod X(y;z))\sqprod X(z;u) \cr}$$
\vskip\tarpas
Now we shall check commuting diagram for the left side
$$\matrix { X(x;y)\otimes (X(y;z)\otimes X(z;u))&   & \cr
 \mapdownk 1\otimes t  &\searrow & \cr
 X(x;y)\otimes (X(y;z)\sqprod X(z;u)&  \maprightap t  &
  X(x;y)\sqprod (X(y;z)\sqprod X(z;u)\cr
\mapdownk 1\otimes {\circ} & & \mapdownd 1\sqprod {\circ} \cr
X(x;y) \otimes X(y;u) & \maprightap t & X(x;y)\sqprod X(y;u) \cr }$$
\vskip\tarpas
The commuting diagram for the lowest left side is get by definition
of restricted contact arrows mapping
$$\matrix { X(x;y) \otimes X(y;u) & \mapright t & X(x;y)\sqprod X(y;u) \cr
& \searrow & \mapdownd  {\circ} \cr
& & X(x;u) \cr }$$
\vskip\tarpas
So we get correspondent faithful embeddings for the different
categories of $\VV$-enriched categories.  For the crude functors
we get $\Cat_{\VV'}\superrightarrow \Cat_{\VV}$, for the continuous functors
we get $\Cat_{\VV'}^+\superrightarrow \Cat_{\VV}^+$, for the cocontinuous
functors we get $\Cat_{\VV'}^-\superrightarrow \Cat_{\VV}$ and finally
for the natural  functor we get $\Cat_{\VV'}^=\superrightarrow \Cat_{\VV}^=$.

For assistant $\VV$-graph  $A$ we can take the same
 exponential
superfunctor restricted over the image category of
faithful embedding of $\VV'$-graphs
$$\Grph_{\VV'}\superrightarrow \Grph_{\VV}\kbl$$
 i. e.
for $\VV'$-graph $X$ we take the set of $\VV$-graphs transports
$$Y^A_0= \lbrace  \phi: A\doublerightarrow Y\rbrace \kbl$$
and the edges set between two $\VV$-graphs transports
$\phi,\psi:A\doublerightarrow Y$  is  defined by the product of edges sets
$$Y^A(\phi; \psi)= \prod_{a\in A_0} Y(\phi_0(a);\psi_0(a))\tsk$$
We  choose the transported unit arrow
$$1_\phi(*)= \Prod_{a\in A_0} 1_{\phi_0(a)} (*)\subset \Prod_{a\in A_0}
Y(\phi_0(a);\phi_0(a))\tsk$$
This allows to have projections $p_a: Y^A\doublerightarrow Y$
as $\VV$-graphs transports maintaining the chosen unit arrows
$$1_\phi^{p_a}(*)= 1_{\phi_0(a)}(* )\subset Y(\phi_0(a);\phi_0(a))\tsk$$
Having the contact arrows mappings
$$\circ : Y(x;y)\sqprod Y(y;z) \rightarrow Y(x;z)$$
we take it's  restriction and define contact arrows mappings in
the exponential $\VV$-graph
$$Y^A(\phi;\psi) \otimes Y^A(\psi;\xi)= \Prod_{a\in A_0}
(Y(\phi_0(a);\psi_0(a))\otimes Y(\psi_0(a);\xi_0(a)))
\rightarrow $$$$
\Prod_{a\in A_0}
(Y(\phi_0(a);\psi_0(a))\sqprod  Y(\psi_0(a);\xi_0(a)))
\rightarrow
$$$$\Prod_{a\in A_0}
(Y(\phi_0(a);\psi_0(a))\circ  Y(\psi_0(a);\xi_0(a)))
\subset \Prod_{a\in A_0} Y(\phi_0(a);\xi_0(a))= Y^A(\phi;\xi)\tsk$$
For an original $\VV'$-graph $Y$ we get the original exponential
$\VV$-graph again.

For a $\VV'$-graphs transport $f: X\doublerightarrow Y$ we get
the $\VV$-graphs transport of imbedded $\VV$-graphs  and
the changing of target
space provides the $\VV$-graphs transport of exponential $\VV$-graphs
$$f^A: X^A \doublerightarrow Y^A\tsk$$

We get a superfunctor in the category of $\VV$-graphs $\Grph_{\VV}$
defined over the partial category of imbedded $\VV'$-graphs
$$\Grph_{\VV'}\superrightarrow \Grph_{\VV} \tsk$$

It can also be restricted in the categories of original graphs
with  natural functors
$\OGrph_{\VV'}\superrightarrow \OGrph_{\VV}$.
 with continuous functors
$\OGrph_{\VV'}^+\superrightarrow \OGrph_{\VV}^+$, with cocontinuous
functors $\OGrph_{\VV'}^-\superrightarrow \OGrph_{\VV}^-$,
or in the category with natural functors
$\Grph_{\VV'}^=\superrightarrow \Grph_{\VV}^=$.

The associativity of contact arrows mappings in $\VV'$-graph $Y$
provides the associativity of restricted contact arrows mappings in
imbedded $\VV$-graph, and also in exponential $\VV$-graph $Y^A$.
So we get superfunctors in smaller categories of $\VV$-enriched categories.
For the crude functors we get $\Cat_{\VV'}\superrightarrow \Cat_{\VV}$,
for the continuous functors we get $\Cat_{\VV'}^-\superrightarrow
\Cat_{\VV}^-$,
for the cocontinuous functors we get $\Cat_{\VV'}^+\superrightarrow
\Cat _{\VV}^+$, and for the natural functors we get
$\Cat_{\VV'}^=\superrightarrow \Cat_{\VV}^= $.

For the $\VV$-enriched categories we can also define the exponential space of
continuous transforms  $Y^{(A)}_-$, cocontinuous transforms $Y^{(A)}_+$,
or natural transforms $Y^{(A)}_=$. However these spaces defines superfunctors
only in the category of natural functors
$\Cat_{\VV}^=\superrightarrow \Cat_{\VV}^=$.

The unit transform  for the joint pair of superfunctors in the category
of $\VV$-graphs $\Grph_{\VV}$ is defined by collection of $\VV$-graphs
transports
$$\lambda_X: X\doublerightarrow (X\sqprod A)^A\tsk$$
They are sections transports defined with
chosen unit arrow mappings
$$e_x(*)\subset X(x;x)\kbl e_a(*)\subset A(a;a) \tsk$$
For a vertex $x\in X_0$ they  appoint the section
$\Lambda_X(x): A\doublerightarrow X\sqprod A$, which for
a vertex $a\in A_0$ appoints the couple $\lan x,a\ran \in X_0\times A_0$
and have edges set mappings
$$\lambda_X(x)_{a,b}: A(a;b)\rightarrow 1_x(*)\sqprod A(a;b) \subset
X(x;x)\sqprod A(a;b) \tsk$$
The edges set mappings for sections transport
$\Lambda_X: X\doublerightarrow   X\sqprod A$ is defined
by the set of transforms in exponential space $(X\sqprod A)^A $
$$\lambda_X: X(x;y)\rightarrow \Prod_{a\in A_0} X(x;y)\sqprod 1_a(*)\subset
\Prod_{a\in A_0} X(x;y)\sqprod A(a;a) \tsk$$

The counit transform may be defined by preevaluation
$\VV$-graphs transport defined with precontact arrows mappings
$$\ev_Y^+: Y^A\sqprod A\doublerightarrow Y\tsk$$
For the former  joint pair of superfunctors $X\otimes A$ and $Y^A$
we have preevaluation  over tensor product
$$\ev_Y^+: Y^A\otimes A\doublerightarrow Y\tsk$$
It for a $\VV$-graphs transport $\phi: A\doublerightarrow Y$ and a vertex
$a\in A_0$ appoints the value $\phi_0(a)\in Y_0$ and have edges set mappings
$$Y^A(\phi;\psi)\otimes A(a;b)\rightarrow
Y(\phi_o(a);\psi_0(a))\otimes Y(\psi_{a,b}(A(a;b)))\rightarrow
$$$$Y(\phi_o(a);\psi_0(b))\circ Y(\phi_{a,b}(A(a;b))) \subset
Y(\phi_0(a);\psi_0(b))\tsk$$
However for the new biproduct to have extension of these arrows isn't
obvious
$$Y^A(\phi;\psi)\sqprod A(a;b)\rightarrow
Y(\phi_o(a);\psi_0(a))\sqprod Y(\psi_{a,b}(A(a;b)))\rightarrow
$$$$Y(\phi_o(a);\psi_0(b))\circ Y(\phi_{a,b}(A(a;b))) \subset
Y(\phi_0(a);\psi_0(b))\tsk$$

Another counit transform may be defined by postevaluation $\VV$-graphs
transport defined with postcontact arrows mappings
$$\ev_Y^-: Y^A\sqprod A\doublerightarrow Y\tsk$$
It for a $\VV$-graphs transport $\phi: A\doublerightarrow Y$ and  a vertex
$a\in A_0$ appoints the value $\phi_0(a)\in Y_0$ and have edges set mappings
$$Y^A(\phi;\psi)\sqprod A(a;b)\rightarrow
Y(\phi_{a,b}(A(a;b)) \sqprod  Y(\phi_o(b);\psi_0(b))) \rightarrow
$$$$ Y(\phi_{a,b}(A(a;b))) \circ  Y(\phi_o(b);\psi_0(b))
 \subset  Y(\phi_0(a);\psi_0(b))\tsk$$

I am sorry that after wasting so many pages of paper I have got so miserable
result. We are return to the most general case studying the name
appointment  in the category  of $\VV$-graphs
$$\Grph_{\VV}(X\sqprod A; Y) \rightarrow \Grph_{\VV}(X;Y^A) \tsk$$

\Proposition
Let we have $\VV$-graphs $X$ and $A$ with chosen unit arrows
$$1_x(*)\subset X(x;x)\kbl 1_a(*)\subset A(a;a)$$
and $Y$ with chosen contact arrows mappings
$$\circ : Y(x;y)\sqprod Y(y;z)\rightarrow Y(x;z)$$
allowing preevaluation mappings
$$Y(\phi_o(a);\psi_0(a))\sqprod Y(\psi_{a,b}(A(a;b)))
\rightarrow $$$$
Y(\phi_o(a);\psi_0(b))\circ Y(\phi_{a,b}(A(a;b))) \subset
Y(\phi_0(a);\psi_0(b))\tsk$$
or postevaluation mappings
$$Y(\phi_{a,b}(A(a;b)) \sqprod  Y(\phi_o(b);\psi_0(b))) \rightarrow
$$$$ Y(\phi_{a,b}(A(a;b))) \circ  Y(\phi_o(b);\psi_0(b))
 \subset  Y(\phi_0(a);\psi_0(b))\tsk$$

For the $\VV$-graphs transport $\Phi: X\sqprod  A\doublerightarrow Y$
with continuous quadrat of contact arrows mappings
$$X(x;y)\sqprod A(a;b)\rightarrow  \Phi_{\lan x,a\ran,\lan x,b\ran}(1_x(*)\sqprod A(a;b)) \circ
\Phi_{\lan x,b\ran,\lan y,b\ran} (X(x;y)\sqprod 1_b(*)) \dgl
$$$$\Phi_{\lan x,a\ran,\lan y,a\ran} (X(x;y)\otimes 1_a(*))\circ
\Phi_{\lan y,a\ran,\lan y,b\ran} (1_y(*)\sqprod A(a;b))\subset
Y(\Phi_0(x,a); \Phi_0(y;b))$$
the name $\Psi: X\doublerightarrow Y^A$ is $\VV$-graphs transport
corestricted in the exponential space of continuous transforms
$Y^{(A)}_+\subset Y^A$.
The prerealization is provided with the precontact arrows mapping
$$\Phi'_{\lan x,a\ran,\lan y,b\ran}: X(x;y)\sqprod A(a;b)=
$$$$ \hskip -10 pt\Phi_{\lan x,a\ran,\lan y,a\ran} (X(x;y)\otimes 1_a(*))\circ
\Phi_{\lan y,a\ran,\lan y,b\ran} (1_y(*)\sqprod A(a;b))\subset
Y(\Phi_0(x,a); \Phi_0(y;b))\tsk$$
The postrealization is provided with  the postcontact arrows mappings
$$
\Phi'_{\lan x,a\ran,\lan y,b\ran}: X(x;y)\sqprod A(a;b)=
$$$$\hskip -10pt \Phi_{\lan x,a\ran,\lan y,b\ran}(1_x(*)\sqprod A(a;b))
 \circ
\Phi_{\lan x,b\ran,\lan y,b\ran} (X(x;y)\sqprod 1_b(*))
\subset Y(\Phi_0(x,a); \Phi_0(y;b))\tsk$$
If the name appointment is corestricted in the exponential space of natural
transforms $Y^{(A)}$, then we have coinciding both realizations.
It coincides with taken  $\VV$-graphs transport
$\Phi: X\sqprod A\doublerightarrow Y$ if we have inequalities  of
predecomposition and postdecomposition
$$X(x;y)\sqprod A(a;b)\rightarrow  \Phi_{\lan x,a\ran,\lan y,b\ran}(1_x(*)\sqprod A(a;b)) \circ
\Phi_{\lan x,b\ran,\lan y,b\ran} (X(x;y)\sqprod 1_b(*)) \dgl  $$$$
%
\Phi_{\lan x,a\ran,\lan y,b\ran} (X(x;y)\sqprod A(a;b))\dgl
$$$$\hskip -10pt\Phi_{\lan x,a\ran,\lan y,a\ran} (X(x;y)\otimes 1_a(*))\circ
\Phi_{\lan y,a\ran,\lan y,b\ran} (1_y(*)\sqprod A(a;b))\subset
Y(\Phi_0(x,a); \Phi_0(y;b))\tsk$$
\Proof:
The proving of such conclusion was provided
earlier in various propositions.

\irodymopabaiga

It can be useful to simplify the notation of contact arrows mappings
for $\VV$-graphs transport
$F: X\doublerightarrow Y$
$$F_{x,y}: X(x;y)\rightarrow F(X(x;y))\subset Y(F_0(x);F_0(y))\tsk$$
%
In former proposition we can choose  $\VV$-graphs transports
$\Phi(x,-) : A\doublerightarrow Y$ with contact arrows mappings
$$A(a;b)\rightarrow \Phi_{\lan x,a\ran,\lan x,b\ran} (1_x(*)\sqprod A(a;b))
\subset Y(\Phi_0(x,a); \Phi_0(x,b))\kbl$$
and $\Phi(-,a): X\doublerightarrow Y$ with contact arrows mappings
$$X(x;y)\rightarrow \Phi_{\lan x,a \ran, \lan y,a\ran} (X(x;y)\sqprod 1_a(*))
\subset Y(\Phi_0(x,a);\Phi_0(y,a))\tsk$$
Then this proposition can be red:
If we have coincidence of contact arrows mappings
$$X(x;y)\times A(a;b) \rightarrow \Phi(X(x;y),a)\circ \Phi(y,A(a;b))=
$$$$ \Phi(x,A(a;b))\circ \Phi(X(x;y),b) \subset Y(\Phi_0(x,a);\Phi_0(y;b))$$
then these  $\VV$-graphs transforms can be get as partial ones
from some $\VV$-graphs transport $\Phi: X\times A \doublerightarrow Y$.
We can choose such $\VV$-graphs transport defined by  these equal values
$$  \Phi(X(x;y), A(a;b))=
$$
$$\Phi(X(x;y),a) \circ \Phi(y,A(a;b))=
 \Phi(x,A(a;b))\circ \Phi (X(x;y),b)\tsk$$
%

This properties of name appointment
remains in smaller categories of $\VV$-graphs. It may be
in the category  of original $\VV$-graphs
$\OGrph_{\VV}$ or the category of $\VV$-enriched categories with natural
 functors
$\Cat_{\VV}^=$.

We remark that having families of functors
 $\Phi(x,-): A\doublerightarrow Y$
and $\Phi(-,a): X\doublerightarrow Y$  with coherent vertexes mappings
$$\Phi(x,-)_0(a)= \Phi(-,a)_0(x)$$
we get two forms  with  the same vertexes mappings
$$\Phi(x,-)_0(a)=\Phi_0(a,b)= \Phi(-,a)_0(x)\tsk $$
One is with predecomposition property
$$\Phi_{\lan x,a\ran,\lan y,b\ran}(X(x;y)\sqprod A(a;b))
= \Phi(X(a;y),a)\circ \Phi(y, A(a;b))
\kbl$$
another is with postdecomposition property
$$\Phi_{\lan x,a\ran,\lan y,b\ran} (X(x;y)\sqprod A(a;b))=
\Phi((x,A(a;b))\circ \Phi(X(x;y),b)\tsk$$
Both forms has the same name $X\doublerightarrow Y^A$.
For vertex $x\in X_0$ it appoints the functor
$\Phi(x,-): A\doublerightarrow Y$
with edges set mappings
$$\Phi_{x,y} : X(x;y)\rightarrow \Prod_{a\in A_0} \Phi(X(x;y),a)$$
providing the transforms  sets between functors $\Phi(x,-)$ and $\Phi(y,-)$.
\vskip\tarpas
The situation isn't always so simple. We provide a counterexample with
Banach spaces. Arbitrary monoid $X$ can be identified with category $p$
having unique object $*\in p_0$. The edges set coincides with taken monoid
$$X= p(*;*)\tsk$$
The transport of monoids $f: X\rightarrow Y$
will be natural  functor of correspondent categories $F: p\doublerightarrow r$.
The objects mapping is obvious $F_0(*)=*$
and edges set mapping is taken transport
$$f=F_{*,*}: p(*;*)\rightarrow r(*;*) \tsk$$
For an assistant monoid $A$ we provide the category $s$.
The exponential space $r^s$ will have functors $\phi: s\doublerightarrow r$
with unique objects mapping $\phi_0(*)=*$, only the edges set mapping
can be different transports between monoids $f, g: A\rightarrow Y$.
The transform between such functors will be defined
by one member of target monoid $u\in Y$. It is natural exactly when
we have commutation
$$f(a)\circ u= u\circ f(a) \uparrow a\in A\tsk$$

We shall take Banach space $X$ as  a category with one object.
For them we have projective tensor product $X\otimes Y$ which
with exponential space of continuous linear mappings $Y^A$ provides
truly adjoint pair of functors, i. e.
we have bijective name appointment
$$\Ban (X\otimes A;Y) =\rightarrow \Ban (X;Y^A) \tsk$$
So for such tensor product we have an evaluation mapping
$$ \ev_Y: Y^A \otimes A\rightarrow Y \tsk$$
In \baf G. Valiukevi\v cius 2022* we constructed a relator $X\sqprod A$
with biequicontinuous tensor product. The contact arrows mapping
is defined with extension of sum
$+ : X\sqprod X \rightarrow X$
without any difficulty. However extended evaluation mapping
$$\ev_Y: Y^A\sqprod A\rightarrow Y$$
can be defined only in smaller exponential space of integrable
linear mappings $f: A\rightarrow Y$.

The composition of arrows is the same for both tensor product,
but  bijective name appointment is get in the smaller category of Banach
spaces with integrable linear mappings
$$\SBan(X\sqprod A; Y) = \rightarrow \SBan (X;Y^A) \tsk$$



%Uýbaigiau traukõ callatice/oneda.teû


==> yoneda.tex <==
%2021.05.30. Pradójau traukõ clattice/yoneda.tex
%2022.02.17. Taisiau
%2022.05.09. Trumpinau
%2022.06.02 Perra÷iau
%2022.08.05 Taisiau
%2022.08.31. Taisiau
%2023.03.12. Taisiau
\Skyr Yoneda lemma for enriched categories. Yoneda lemma..

We are going  to define the joint pair of superfunctors
$X\otimes T$ and $Y^T$ in
the category $\Cat_V$ of all $V$-enriched categories.
For a values category $\VV$ we demand existence of ^{truly =joint pair}
of functors. One  adjoint is  defined with the biproduct
$r\otimes s$ and another coadjoint is an  exponential functor $t^s$.
As usually it provides the bijective^{=name appointment}
$$\VV(r\times s; t) \rightarrow \VV(r;t^s)$$
with commuting diagrams for arrows $u: r\rightarrow r'$ and
$v: t\rightarrow t'$
$$\matrix {\VV(r\otimes s;t) & \rightarrow &V(r;t^S) \cr
\mapupk (u\otimes 1_s)^* &   & \mapdownd (v^s)_* \cr
V(r'\otimes s; t) & \rightarrow  & \VV(r';(t')^s) \cr}  $$
\vskip\tarpas

For concreteness we can take some examples of values categories $\VV$.
At this moment we don't need of large sets. All sets will be small sets,
i. e. the members of some ^{=universe}.

The first  example is a category of small sets $\Set$. We take the ^{Carte
tensor =product}  $X\times Y$ of two sets $X$ and $Y$ as an example of
^{=biproduct}.  It will be called a ^{Carte =biproduct}. For some
^{=assistant set} $T$  it provides a functor $X\times T$ within the category
of sets $\Set$. This functor has the ^{coadjoint =functor} called
^{exponential =functor} $Y^T$.  It is defined with the ^{functional
=space}  $Y^T= \Set(T;Y)$
compounded of all mappings $\phi: T\rightarrow Y$  as points.
The  arrows  will be defined by ^{=changing of target space}.
For a mapping $f:X\rightarrow Y$ exponential functor will appoint the mapping
$f^T: X^T \rightarrow Y^T$  defined by ^{=composition of mappings}. For
a mapping $\phi: T\rightarrow X$ it appoints the
composed mapping $\phi\circ f: T\rightarrow Y$.

For such joint pair of functors the ^{unit =transform} is
 defined by collection of ^{=sections mappings}
$$\lambda_X: X \rightarrow (X\times T)^T$$
which for  a point $x\in X$ appoints the ^{=section}
$\lambda_X(x): T\rightarrow X\times T$. It is a mapping
which for a point $s\in T$ appoints the  ^{=couple}
$\lan x,s\ran\in X\times T$, we shall write
$$\lambda_X(x)_t= \lan x,t\ran \in X\times T\tsk$$

The ^{counit =transform} is defined by collection  of ^{=evaluation mappings}
$$\ev_Y: Y^T\times T \rightarrow Y$$ which for a couple $\lan \phi,s\ran$
of mapping
$\phi\in Y^T$ and point $s\in T$ appoints as ^{=value}
the point $\phi(s)\in Y$.

For such ^{joint =pair of functors} we have bijective ^{=name appointment}
$$\Set(X\times T; Y)=\rightarrow \Set (X; Y^T) \tsk$$
It for a mapping over Carte product $f:X\times T\rightarrow Y$,
which will be called a ^{=form}, appoints
another mapping to the functional space  $g: X\rightarrow Y^T$.
It will be called a ^{=name form}. Its values will be called
 ^{partial =forms}. .

Another example will be the category of ordered spaces $\Mn$.
 Its objects
will be ^{ordered =spaces} $X$ and arrows will be ^{monotone =mappings}
 between
ordered spaces $f: X\doublerightarrow Y$.

An ordered space can be considered as
a ^{=convergence space}. In this space for  ^{onepoint =sequence}
$x\in X$ we appoint a ^{=limit set} compounded of all bigger points
$$\lim x= \lbrace y: x\mzl y \rbrace\subset X\tsk$$
The ^{=monotone mappings} $f:X\rightarrow Y$  then coincide with
continuous mappings defined by inclusion of limit's image
$$ f(\lim x)\subset \lim f(x) \tsk$$
Such  convention allows us to use the same ^{=nomenclature} for different
areas of mathematics.

We take the ^{=Carte tensor product} of ordered spaces $X\times Y$ defined as
Carte tensor product of sets $X\times Y$ with ^{=initial order relation} for
the projections $p_1: X\times Y\rightarrow X$ and $p_2: X\times Y\rightarrow Y$.
It will be again Carte tensor product of corresponding convergence space.

For some ^{=assistant ordered space} $T$ defined functor  $X\times T$ has
a coadjoint exponential functor defined with a new  functional space
$Y^T= \Mn (T;Y) $ compounded of all monotone mappings
$\phi: T\doublerightarrow Y$.
The functional space in the category of sets $\Set$
for a small set $T$ coincides with infinite
Carte tensor product
$$\Set (T;Y) = \Prod_{t\in T}  Y $$
i. e. each mapping $\phi: T\rightarrow Y$
can be considered as collection of values
$$\lan \phi(t)\uparrow t\in T\ran  \in \Prod _{t\in T} Y \tsk$$
For ordered space $Y$ we get an order relation in such product defined again
as the  order relation  ^{=initial for these  projections} $p_t: \Prod_{t\in T} Y\rightarrow Y$.
The monotone mappings compound a ^{partial =space}  in  such ordered space
$$\Mn(T;Y)\subset \Prod_{t\in T} Y\tsk$$
Such situation can be red also for the convergence spaces.

The unit transform will be defined by  the collection of the same
sections  mappings $\lambda_X: X\rightarrow (X\times T)^T $. We need only
to check that it will be monotone or continuous for corresponding convergence
spaces
$$\lambda_X : X\rightarrow (X\times T)^T\subset \Prod_{t\in T} (X\times T)
\tsk$$
First we shall check that every section $\lambda_X(x): T\rightarrow X\times T$
is continuous. We need to check the continuity only for each projection.

The composition with the first projection is get as composition with
the  unique continuous mapping to the final ^{onepoint =space}
$$\lambda_X(x)\circ p_1: T\rightarrow X\times T \rightarrow \lbrace x\rbrace
\subset X \kbl$$
so it again coincides with the unique arrow to onepoint set.

The composition with the second projection coincides with the identic mapping
over assistant space
$$\lambda_X(x)\circ p_2: T\rightarrow X\times T\rightarrow T =
\Identity_T: T\rightarrow T \tsk$$
So both projections provide continuous mappings, therefore sections are
continuous.

The continuity of sections mapping $\lambda_X: X\rightarrow (X\times T)^T$
must be checked again for every projection
$p_t: (X\times T)^T\rightarrow X\times T$  and further
for two projections over Carte tensor product  $X\times T$.
We get the identity mapping $\Identity_X: X\rightarrow X$
 for the first projection
$$\lambda_X \circ p_t \circ p_1=\Identity_X: X\rightarrow (X\times T)^T
\rightarrow
X\times T \rightarrow X\kbl$$
and we get unique arrow to the onepoint set $!: X\rightarrow \lbrace t\rbrace$
for the second projection
$$\lambda_X\circ p_t\circ p_2=!: X\rightarrow (X\times T)^T \rightarrow
X\times T \rightarrow \lbrace t\rbrace \tsk$$
So we get the  continuous projection $\lambda_X\circ p_t: X\rightarrow X\times T$,
consequently also the  sections mapping  $\lambda_X: X\rightarrow
(X\times T)^T $ itself is continuous.

The counit transform in the category $\Set$ was
defined by collection of evaluation mappings
$$\ev_Y: (\Prod_{t\in T} Y )\times T  \rightarrow Y\tsk$$
Now we want to restrict  such mapping over smaller set of continuous mappings
$$ \ev_Y: Y^T\times T \rightarrow Y \tsk$$
In functional space $Y^T$ we have defined an initial convergence, which
usually is named as a weak convergence. There are  only special cases when
we can get continuous evaluation for weak convergence in functional space.
But for the ordered spaces evaluation mapping becomes  monotone.
Let we have inequality for monotone mappings
$$\phi(t)\mzl \psi(t)\uparrow t\in T \tsk$$
For pair of arguments $s\mzl t$ we can check inequality between
acquired values
$$\phi(s)\mzl \psi(t) \tsk$$
Indeed.  For transitive relation we get
$$\phi(s)\mzl \phi(t) \mzl \psi(t)\tsk$$

For taken  joint pair of functors we  get  again the  bijective name
appointment
$$\Mn(X\times T; Y)=\rightarrow \Mn (X; Y^T) $$
which for arbitrary  form as monotone mapping over the product
of ordered spaces
$f:X\times T\rightarrow Y$ appoints
the monotone mapping of ^{=partial forms }  over
the source space $X$.

\vskip\tarpas
The ordered space is an instance of a set $X$ with binary relation
$R\subset X\times X$, or more generally an instance of a graph $X$.
We can  understand the inequality  $a\dgl b$ as an  edge $f: a\rightarrow b$
between the vertexes.
Otherwise sometimes is useful with the sign of inequality to denote the
arrows  from some another category.
Such  simplified notation can be applied
when we want to work with different sorts of arrows
as we see for the ^{$\two$-=categories}.  Usually  somebody prefer to speak
 about ^{=maps} and ^{=cells}, but that
language  can be applied only
for special class of our considered ^{=superfunctors}.

The graph $X$ is understood as a set of ^{=edges}  between the ^{=vertexes}.
The set of vertexes will be denoted $X_0$. We shall work with
^{directed =graphs}. Every edge has its direction.
A ^{graphs =transport} between two graphs $f: X\doublerightarrow Y$
is defined by the ^{vertexes =mapping} $f_0: X_0\rightarrow Y_0$
and the family of ^{edges =mappings}
$f_{x,y}: X(x;y)\rightarrow Y(f_0(x);f_0(y))$.
They are composed  with usual rules
$$ (f\circ g)_0=f_0\circ g_0\kbl (f\circ g)_{x,y}= f_{x,y}\circ
g_{f_0(x),f_0(y)} \kbl$$
and  we have  an ^{identity =transport} defined with identity mappings
$$\Identity_{X_0}: X_0\rightarrow X_0\kbl
 \Identity_{X(x,y)}: X(x;y)\rightarrow X(x;y)\tsk$$
Identity transports are  neutral for composition of graphs transports.
They will be denoted as identity graphs transport
 $\Identity_X: X\doublerightarrow X$.

The graphs transports will be arrows in the category of graphs $\Grph$.
We define a ^{=Carte biproduct}
$X\times Y$. It has the Carte tensor product of
vertexes sets  $X_0\times Y_0$ and the Carte tensor product of edges set
$$X\times Y(\lan x,y\ran;\lan x',y'\ran ) = X(x;x')\times Y(y;y') \uparrow
\lan x,y\ran\in X_0\times Y_0, \lan x',y'\ran\in X_0\times Y_0\tsk$$

For chosen  ^{=assistant graph} $T$ we shall  define  a joint pair of superfunctors.
The adjoint superfunctor is defined with  the Carte biproduct
$X\times T$.
For a graph $X$ it appoints the graphs biproduct with the assistant graph
$X\times T$ and for a graphs transport $f: X\doublerightarrow X'$ it
 appoints  the graphs transport between Carte biproducts defined
by  the biproduct of taken graphs transport
 with  the identity transport  of the assistant graph
 $$f\times \Identity_T: X\times T\doublerightarrow X'\times T\tsk$$

The coadjoint superfunctor $Y^T$ is defined with the graph of all transforms
between graphs
transports over the assistant graph $\phi: T\doublerightarrow Y$.
 These graphs
transports  become  vertexes, and  edges will be transforms
$\alpha: \phi\rightarrow \psi$ between  them  defined with some  collection of edges
$$\alpha_t\in Y(\phi_0(t);\psi_0(t))\tsk$$
For an graphs transport $g: Y\doublerightarrow Y'$ it appoints the new
graphs transport defined by changing of target space with taken graphs
transport. For a graphs transport $\phi: T\doublerightarrow Y$ it appoints
the new graphs transport $\phi\circ g: T\doublerightarrow Y'$ and for
a transform between graphs transports $\alpha: \phi\rightarrow \psi$
it appoints the new transform $\alpha\ast T: \phi\circ f
\rightarrow \psi\circ f$
defined with the new collection of arrows
$$g_{\phi_0(t),\psi_0(t)} (\alpha_t)\in Y'(g_0(\phi_0(t)); g_0(\psi_0(t)))
\tsk$$
We can see that another changing of target space with another
graphs transport $h: Y'\doublerightarrow Y''$ provides the same result
as changing of target space with composition of graphs transports
$g\circ h: Y\doublerightarrow Y''$.
Also the  changing of target space with identity transport
$\Identity_Y: Y\doublerightarrow Y$ provides the identity graphs
transport again.
So we have got indeed the superfunctor $Y^T$.

We get a  ^{=partial unit transform} for such joint pair of superfunctors
 defined with the collection of sections transports
$\lambda_X: X\doublerightarrow  (X\times T)^T$ 
          for the assistant graph $T$ and the source graph $X$ with chosen
unit arrows $1_s\in T(s;s)$ and
$1_a\in X(a;a)$.
For vertexes we take ordinary sections mappings
 $$\lambda_{X_0}: X_0\rightarrow X_0^{T_0}\tsk$$

For the edge $\alpha\in X(x,y)$ we appoint the transform between  two
sections $\lambda_X(x): T\doublerightarrow X\times T$ and
$\lambda_X(y): T\doublerightarrow X\times T$. These sections are graphs
transports with the mappings for vertexes
$\lambda_{X_0}(x):T_0\rightarrow X_0\times T_0$ defined
$$\lambda_{X_0}(x)_t= \lan x,t\ran\in X_0\times T_0$$  and
the edges mappings are provided
$$\lambda_X(\alpha)= \lan \alpha, 1_s\ran \in X(x;y)\times T(s;t) \uparrow
\alpha\in X(x;y) \tsk$$
 The unit transform allows us to define a ^{=name appointment}
  for the forms over the Carte biproduct
$$\Grph(X\times T;Y) \rightarrow \Grph (X; Y^T)\tsk$$
For a graphs transport $f: X\times Y \doublerightarrow Y$ it appoints
the composition  of sections mapping with the graphs transport provided
by changing of target space  with taken graphs transport
     $$g=\lambda_X \circ f^T  : X\doublerightarrow Y^T\tsk$$
For a vertex $x\in X_0$ it appoints the section which for a
vertex $t\in T_0$
appoints the couple $\lan x,t\ran \in X_0\times T_0$, and further
the changing of target space will appoint  the graphs transport
$T\doublerightarrow Y$ which for a vertex $t\in T$ appoints the
vertex in the target space $f(x,t)\in Y_0$ and for an edge $u\in T(s;t)$
it will appoint  the image of couple
$\lan 1_x,u\ran \in X\times T(\lan x,s\ran;\lan x,t\ran)$
by taken graphs transport
$$f( 1_x,u)\in Y(f_0(x,s);f_0(x,t))\tsk$$
For an edge $\alpha\in X(a;b)$ it appoints the transform between two
sections  defined with collection of edges
$\lan \alpha,1_s\ran\in X\times T(\lan a,s\ran;\lan b,s\ran) $ and further
the transform between graphs transports to the target graph $Y$
defined with collection of edges $f(\alpha,1_s)\in Y(f_0(a,s);f_0(b,s))$.

The partial 
counit transform is defined with collection of evaluation transports
$\ev_Y: Y^T\times T\doublerightarrow Y$  in the target graph  $Y$
with mappings of contact arrows
$$Y_{c,d,e}: Y(c;d)\times Y(d;e)\rightarrow  Y(c;d)\circ Y(d;e)\subset Y(c;e)\tsk$$
Evaluation transport can be defined  in two ways.

For the couple $\lan \alpha, u\ran $ of a transform
$\alpha: \phi\rightarrow \psi$ between to graphs transports
$\phi, \psi: T\doublerightarrow  Y$ and an edge between two vertexes in
source graph $u\in T(s;t)$  we  can define the ^{precontact =arrow }
$$\ev_{Y}^+(\lan \alpha,u\ran )= \alpha_s\circ \psi_{s,t}(u)\kbl$$
and another ^{postcontact =arrow}
$$\ev_Y^- (\lan \alpha, u\ran) = \phi_{s,t}(u)\circ \alpha_t \tsk$$

The counit transport allows us to define the ^{=realization appointment}
for partial forms transport  over the source graph $X$
$$\Grph(X; Y^T) \rightarrow \Grph(X\times T;Y)\tsk$$
With precontact arrows we get the ^{=prerealization}, and with
postcontact arrows we define the ^{=postrealization}.

For a graphs transport $g: X\doublerightarrow Y^T$ it appoints the
biproduct
  of taken graphs transport with
the identity transport of the assistant graph
$g\times \Identity_T : X\times T\doublerightarrow Y^T\times T$
composed with the evaluation transport  $\ev_Y: Y^T\times T\doublerightarrow Y$
$$f= (g\times \Identity_Y)\circ \ev_Y: X\times T\doublerightarrow Y\tsk$$
For a couple $\lan x,t\ran$ of $x\in X_0$ and $t\in T_0$
it appoints the couple $\lan g_0(x),t\ran$ of the  graphs transport
$g_0(x)\in (Y^T)_0$ and the same vertex in the assistant graph $t\in T_0$.
Further we get the value of this graphs transport over taken vertex
$g_0(x)_t\in Y_0 $.
For a couple $\lan \alpha, u\ran $ of an edge in the source graph
$\alpha\in X(a;b)$ and an edge in the assistant graph $u\in T(s;t)$
we get the couple $\lan g(\alpha),u\ran$ of transform
$g(\alpha): g_0(a)\rightarrow g_0(b)$
between
graphs transports $g_0(a), g_0(b): T\doublerightarrow Y$
defined with collection of edges $g(\alpha)_s\in Y(g_0(a)_s;g_0(b)_s)$
and the same edge $u\in T(s;t)$.
Further
the evaluation  transport appoints the precontact arrow
$$g(\alpha)_s\circ g_0(b)_{u}\in Y(g_0(a)_s;g_0(b)_t)$$
or the postcontact arrow
$$g_0(a)_u\circ g(\alpha)_t \in Y(g_0(a)_s;g_0(b)_t)\tsk$$

Earlier in \baf G. Valiukevi\v cius 2022* we have checked
when realization appointment ^{=reverses}  name
of graphs transport
$f\in \Grph( X\times T;Y)$.
For the preevaluation we have used the ^{=predecomposable  property}
$$f(\alpha,1_s)\circ f(1_b,u)= f(\alpha,u) \kbl$$
and for the postevaluation we have used  the ^{=postdecomposable property}
$$f(1_a,u)\circ f(\alpha,1_t)= f(\alpha,u)\tsk$$
In these cases we get that the realization appointment  is ^{=surjective} and the
name appointment is ^{=injective}.

Also we have checked  when the name appointment reverses the realization of
graphs transports $g:X\doublerightarrow Y^T$.
For the preevaluation we have  used the ^{=preneutral  properties}
$$g(1_a)_s\circ g_0(a)_u= g_0(a)_u)\kbl
g(\alpha)_s\circ g_0(b)_{1_s} = g(\alpha)_s \kbl$$
and for the postevaluation we have used the ^{=postneutral properties}
$$g_0(a)_u \circ g(1_a)_t=g_0(a)_u\kbl g_0(a)_{1_s}\circ g(\alpha)_s=
g(\alpha)_s \tsk$$
In these cases we get that the name appointment is surjective and the
realization appointment
is injective.

 A transform
$\alpha: \phi\rightarrow \psi$  is called ^{=natural} if we get
commuting  quadrats from equality of precontact and postcontact
arrows
$$\alpha_s \circ \psi_0(u)= \phi_0(u)\circ \alpha_t\tsk$$
\vskip\tarpas
$$\matrix { \phi_0(s) &\mapright \phi_{s,t}(u) & \phi_0(t) \cr
           \mapdownk \alpha_s & \searrow  & \mapdownd \alpha_t \cr
           \psi_0(s) & \maprightap \psi_{s,t}(u) & \psi_0(t) \cr } $$
\vskip\tarpas

For two graphs transports $\phi, \psi: T\doublerightarrow Y$ we shall
 denote the set of natural transforms $\alpha: \phi\rightarrow \psi$
 with  a  new sign $Y^{(T)}(\phi;\psi)$. These will be edges sets for
a new exponential graph $Y^{(T)}$. At this moment we are not
interested can such new exponential graphs  to define a superfunctor.

Having predecomposable and postdecomposable properties we get injective name
appointment  to the set $\Grph(X; Y^T)$
 of all transports to the exponential graph.
 We shall say that taken graphs transport $f: X\times T\doublerightarrow Y$
is ^{=decomposable}.
We have seen that such graphs transport can be ^{=corestrained }
in the new exponential graph of natural transforms $Y^{(T)}$.

Both preevaluation  and postevaluation transports coincide over the
exponential  graph of natural transforms.
This is easy to see from equality
$$f(\alpha, 1_s)\circ f(1_b,u)= f(1_a,u)\circ f(\alpha,1_s)\tsk$$
In this case both  realization 
mappings also coincide and their image contains all decomposable graphs
transports.

Having graphs transport $g: X\doublerightarrow Y^T$ with preneutral and
postneutral properties we get that both prerealization and postrealization
mappings reverses the
name of taken graphs transport. We shall say that taken graphs transport
$g: X\doublerightarrow Y^T$ has ^{=neutral properties}.
Such properties can be visualized by ^{splitting =diagrams}
$$ \matrix { g_0(a)_s & \mapright g_0(a)_{1_s} & g_0(a)_s \cr
\mapdownk g(\alpha)_s & \searrow & \mapdownd g(\alpha) _s \cr
g_0(b)_{1_s}  & \maprightap g_0(b)_{1_s} & g_0(b)_s \cr } \hskip 10 pt
\matrix { g_0(a) & \mapright g_0(a)_u & g_0(a)_t \cr
\mapdownk g(1_a)_s & \searrow  & \mapdownd g(1_a)_t \cr
g_0(a)_s  & \maprightap g_0(a)_u  & g_0(a)_t \cr } $$
\vskip \tarpas
Such diagrams were applied by \baf P. Freyd, A. Scedrov 1990* \S 1.28
to define $g_0(a)_{1_s}$ and $g(1_a)_s$ as splitting idempotents.

In this case the name
mapping is surjective and both realization  are injective.
For the decomposable graphs transport $f: X\times T\doublerightarrow Y$
having name  $g: X\doublerightarrow Y^T$ with neutral properties
we get bijective name appointment
$$\Grph(X\times T;Y)=\rightarrow \Grph(X; Y^{(T)})\tsk $$

\vskip\tarpas
We shall restrict the general category of graphs as we want
to get  superfunctor $Y^{(T)} $
for the exponential graphs of natural transforms.
First we shall define the  ^{original =graphs}.
In \baf J. Freyd, A. Scedrov 1990* \S 1.263 we can see a name ^{pointed
=sets} for the sets with chosen origin point. However in 1.4(11)4
is defined the point in arbitrary object from some category, so we
don't want to use the name of pointed set for objects in
arbitrary category.

In original graph  $X$ we choose  unit arrows $1_a\in X(a;a)$.
The ^{original  graphs  =transports} $f: X\doublerightarrow Y$
must maintain chosen unit arrows
$$f(1_a)= 1_{f_0(a)} \tsk$$
They will be called also as ^{crude =functors}.
Such category of original graphs we shall denote $\OGrph$.  The letter $\VO$
must denote the graphs with origin point.

We can take yet a smaller category  compounded of all
original graphs transports
between original graphs with contact arrows mappings
 $$\alpha\circ \beta \in X(a;c)\uparrow \alpha\in X(a;b), \beta\in X(b;c)
 \tsk$$
They define a graphs transport over ^{pullbacked =product}
$X\times_p X \subset X\times X\tsk$
$$\circ: X\times _p X\doublerightarrow X\tsk$$
In original graph $X$ we demand a neutral properties for chosen unit arrows
 $$1_a\circ \alpha= \alpha= \alpha\circ 1_b\uparrow \alpha\in X(a;b)\tsk$$
For the category $\OGrph^=$
we take original graphs transports
with additional property  to maintain the contact arrows mappings
$$f(\alpha\circ \beta)= f(\alpha)\circ f(\beta) \uparrow \alpha\in X(a;b),
\beta\in X(b;c) \tsk$$
Such graphs transports can  be called as ^{usual =functors}, with more
concrete language we
can call them as ^{natural  =functors}.
The choosing of unit arrows or contact arrows mappings can be announced
as some algebraic operations and special graphs transforms must maintain
such operations.

We have the Carte biproduct $X\times Y$
 of two original graphs defined with initial structure of operations.
 For a couple of vertexes $\lan x,y\ran\in X_0\times Y_0$ we appoint
 the couple of unit arrows
 $$\lan 1_x,1_y\ran\in X(x;x)\times Y(y;y) \tsk$$
For  two couples of edges
$$\lan \alpha, \alpha'\ran\in X(a;b)\times Y(a';b'),
\lan \beta',\beta' \ran \in X(b,c)\times Y(c';d') $$
we can define  a contact arrow
$$\lan \alpha,\alpha'\ran\circ \lan \beta ,\beta'\ran=
\lan \alpha\circ\beta,\alpha'\circ\beta'\ran\in
X(a;c)\times Y(a';c') \tsk$$

So for arbitrary  assistant original graph $T$ we define
superfunctor $X\times T$
in the category
of original  graphs  $\OGrph$ or in the smaller category  $\OGrph^=$ of
^{natural  =functors} between original  graphs.

For an original  graph $X$ it appoints the Carte biproduct
$X\times T$ and for an  original graphs transports
$f: X\doublerightarrow X'$  it appoints the Carte biproduct  with the
identity transport of the assistant graph
$\Identity_T:T\doublerightarrow T$
$$f\times \Identity_T : X\times T\doublerightarrow X' \times T \tsk$$

Another superfunctor will be defined with  the graph of all
transforms
$Y^T$.  The unit arrows and contact arrows mappings will be taken
as initial structure in the  product  $\Prod_{t\in T_0}  Y$.
The unit transform $1_\phi: \phi\rightarrow \phi$
is defined with the collection of unit arrows
$$1_{\phi_0(s)} \in Y(\phi_0 (s );\phi_0(s)) \uparrow s\in T_0\tsk$$
The contact arrows mapping  also is  defined by  collection of contact edges
$$(\alpha\circ\beta)_s = \alpha_s\circ \beta_s \uparrow s\in T_0 \tsk$$

The unit arrow $1_\phi: \phi\rightarrow \phi$ will be a natural transform,
but the composition of natural transforms doesn't need to remain a natural
transform. However for the natural  original  graphs functor
over the Carte biproduct
$f: X\times T\doublerightarrow Y$  the name form $g: X\doublerightarrow Y^T$
will be corestricted in the exponential space a natural transform.

Finally we restrict ourselves with the ^{=categories}.
The original  graph  $X$ becomes a category  if its contact arrows are get
with associative composition of arrows, i. e. we have the
identity  provided with associativity isomorphism
$$\alpha\circ (\beta\circ \gamma)= (\alpha\circ \beta)\circ \gamma
\uparrow  \alpha\in X(a;b), \beta\in X(b;c), \gamma\in X(c;d)\tsk$$
Vertexes of category will be called  ^{=objects} $x\in X_0$
and edges will be called ^{=arrows} $\alpha\in X(a;b)$.
The functors between categories  $f: X\doublerightarrow Y$
will compound the category $\Cat$.

For the category of small categories $\Cat$ we can define an exponential
 superfunctor  $Y^{(T)}$  of natural transforms.
First we  need to check that the composition of two natural transforms
remains a natural transform.

Let we have three functors $\phi,\psi,\xi: T\doublerightarrow Y$
and two natural transforms $\alpha: \phi\rightarrow \psi$
and $\beta: \psi\rightarrow \xi$.
Having ^{commuting =quadrats}  for arbitrary edge in assistant category
$u\in T(s;t)$
$$\phi(u)\circ \alpha_t= \alpha_s\circ \psi(u)\kbl$$$$
\psi(u)\circ \beta_t= \beta_s\circ \xi(u)\kbl$$
we get a new commuting quadrat
$$\phi(u)\circ (\alpha_t\circ \beta_t)= (\alpha_s\circ \beta_s)\circ \xi(u)
\tsk$$
$$\matrix {
\phi_0(s)  & \mapright \alpha_s & \psi_0(s) & \mapright \beta_s  & \xi_0(s)\cr
\mapdownk \phi(u) &  & \mapdownk \beta(u) & & \mapdownd \xi(u)  \cr
\phi_0(t) & \maprightap \alpha_y & \psi_0(t) & \maprightap \beta_t
 & \xi_0(t)  \cr } $$
\vskip \tarpas
The  proving  uses three ways from a vertex $\phi_0(s)$ to the vertex
$\psi_0(t)$
$$(\alpha_s\circ \beta_s )\circ \xi (u)=
\alpha_s \circ (\beta_s \circ \xi(u))=
\alpha_s\circ (\psi(u)\circ \beta_t)=$$$$
(\alpha_s\circ \psi(u))\circ \beta_t=
(\phi(u)\circ \alpha_t)\circ \beta_t=
\phi(u)\circ (\alpha_t\circ \beta_t)\tsk$$

We also can prove that the space of natural transforms $Y^{(T)}$ defines
a superfunctor for the graphs transports   $f: X\doublerightarrow Y$
 maintaining contact arrows mappings
$$f(u\circ v)= f(u)\circ f(v)\uparrow u\in X(a;b), v\in X(b;c)\tsk$$
The changing of target space $f^T: Y^T\doublerightarrow (Y')^T$
will maintain the commuting diagrams for natural transform
$\alpha: \phi\rightarrow \psi$, i. e. we get commuting diagram again
in the new target space $Y'$
$$ \matrix{ f_0(\phi_0(s)) &\mapright f(\alpha_s) & f_0(\psi_0(s)\cr
           \mapdownk f(\phi(u)) & & \mapdownd f(\psi(u)) \cr
          f_0( \phi_0(t)) & \maprightap f(\alpha_t) &  f_0(\psi_0(t)) \cr}$$
\vskip\tarpas
For the original graphs transport $f:X\doublerightarrow Y$ we get
the changing of target space again maintaining unit transform defined by
by collection of chosen unit arrows $1_{\phi_0(x)}\in X(\phi_0(x);\phi_0(x))$.
Also for the natural  functor between original graphs we get
again the changing of target space
maintaining the composition of transforms
$$f(\alpha \circ \beta)=\Prod_{s\in T_0} f(\alpha_s\circ \beta_s)=
\Prod_{s\in T_0} (f(\alpha_s)\circ f(\beta_s))= f(\alpha)\circ f(\beta) \tsk$$
\vskip\tarpas

We shall prefer for some functor $F: X\doublerightarrow Y$ to use the usual
notation for points
$$F_0(x)\in Y_0\uparrow x\in X_0$$
and the exponential notation
for arrows $$f^F\in Y(F_0(x);F_0(y))\uparrow f\in X(x;y)\tsk$$

We extend  the proving of Yoneda lemma for  more general original
graphs with contact arrows mappings.
Let we have a graphs transport  to the sets  category
$F: X^\op\doublerightarrow \Set$. It will be  called a ^{=character}
 over taken original  graph $X$.
The representable character is defined by some point $x\in X_0$
$$X(-; x): X^\op \doublerightarrow \Set \tsk$$
It  can be  understood as a value for the Yoneda mapping
$$(\Yoneda_X)_0: X_0\rightarrow  (\Set^{X^\op} )_0\tsk$$
This mapping is extended as original graphs transport
$$\Yoneda_X: X\doublerightarrow \Set^{X^\op} $$
and this extension will be ^{=fullfaithful  imbedding}, i. e. we have
bijection between the edges set $X(a,b)$ and the set of transforms between
appointed representable characters
$\Set^{X^\op} (X(-;a);X(-;b))$. Later we shall
 describe such transforms as natural or continuous ones.

The choosing of unit arrow $i_x\in X(x;x)$ is a  universal arrow
from onepoint set $*\in \Set_0$  to the representable functor
$X(-;x) :X^\op \doublerightarrow \Set $, clr. \baf S. MacLane 1998* \S 3.1
Universal arrows.
The arbitrary point in the edges set
$F: *\rightarrow X(a;x)$ is get from universal
arrow $i_x: *\rightarrow X(x;x)$ with source changing
$f^*: X(x;x) \rightarrow X(a;x)$
$$\matrix { * & \mapright i_x & X(x;x) & \hskip 20pt &  x \cr
        & \searrow & \mapdownd f^* &        & \mapupd f \cr
        & & X(a;x) &                        & a \cr}$$
\vskip\tarpas
For arbitrary graphs transport $F: X^\op \doublerightarrow \Set$
we shall get a bijection between the set of points $m\in F_0(x)$ and
the set of transforms between representable character $X(-;x)$ and taken
graphs transport $F$.

\Proposition
Over an original graph $X$ with contact arrows mappings
$$X(a;b)\otimes X(b;c)\rightarrow X(a;b)\circ X(b;c) \subset  X(a;c) $$
for arbitrary graphs transport $F: X^\op \doublerightarrow \Set$
we have a bijection between the value set $ F_0(x)$
and the set of transforms between representable character $X(-;x)$
and taken graphs transport $F$.
\Proof:
A transform between two graphs transports $\alpha: X(-;x) \rightarrow F$
is defined by collection of mappings between value sets
$$\alpha_a: X(a;x) \rightarrow F_0(a)\tsk$$
We take the image of unit arrow $i_x\in X(x;x)$
$$m= \alpha_x(i_x) \in F_0(x)$$
as a point correspondent to taken transform $\alpha: X(-;x) \rightarrow F$.

Otherwise for arbitrary point $m\in F_0(x)$ we get a mapping
$$\alpha_a: X(a;x) \rightarrow F_0(a)\tsk $$
For an edge $f\in X(a;x)$ the  mapping $f^F:F_0(x)\rightarrow F_0(x)$
provides the  value of taken point $f^F(m) \in F_0(a)$.

For a unit arrow $i_x\in X(x;x)$ we get the identity mapping as
source changing
$i^*_x:=\Identity_{X(x;x)} : X(x;x) \rightarrow X(x;x)$.
So we get the same point $m= i_x^F(m)$ correspondent for
with  this point $m\in F_0(x)$ constructed transform $\alpha: X(-;x)\rightarrow F$.
 Otherwise for some transform $\alpha: X(-;x) \rightarrow F$ appointed
 point $\alpha_x(i_x)\in F_0(x)$ generates the same transform
 $\alpha: X(-;x)\rightarrow F$.

\irodymopabaiga
For an original graph $X$ with associative contact arrows mappings
the representable characters are natural  functors, and all transforms
between two characters are natural ones.
For non associative contact arrows mappings
a situation becomes more interesting.

In general the source changing isn't natural  functor. But for the unit arrow
$i_x\in X(x;x)$ we get equality
$$h\circ (f\circ i_x) = (h\circ f)\circ i_x \tsk$$
We shall say that unit arrow $i_x\in X(x;x) $ is a ^{=social point}
for source changing functor
$$h^*(f^*(i_x))= (h\circ f)^*(i_x)\tsk$$
Every natural transform $\alpha: X(-;x)  \doublerightarrow F $
is defined by  collection of mappings
$\alpha_a: X(a;x) \rightarrow F(a) $.
For a natural transform we have commuting diagrams for any edge $h\in X(b;a)$
$$\matrix{ X(a;x) & \mapright \alpha_a & F_0(a) \cr
  \mapdownk h^* &   &  \mapdownd h^F \cr
  X(b;x) & \maprightap \alpha_b  & K(b) \cr}$$
\vskip\tarpas
Therefore we get again equality of social point $m\in F_0(x)$
$$h^F (f^F (m))=(h\circ f)^F(m) \tsk$$

\Proposition
For an original graph $X$ with contact arrows mappings
$$\circ : X(a;b)\times X(b;c) \rightarrow X(a;c) $$
the choosing of social point $m\in F_0(x)$ provides
a  natural transform
$$\alpha: X(-;x)\rightarrow K$$
between representable character $X(-;x)$  and taken character $F$.
\Proof:
The natural transform   $\alpha: X(-;x)\rightarrow F$
is defined by collection  of mappings between appointed sets
$$\alpha_a: X(a;x)\rightarrow K(a)$$
with commuting diagrams for every edge $h\in X(b;a)$
$$\matrix { X(a;x) & \mapright \alpha_a  & F_0(a) \cr
\mapdownk h^* &   & \mapdownd h^F \cr
X(b;x) & \maprightap \alpha_b  & F_0(b) \cr } $$
\vskip\tarpas
For the unit arrow $1_x\in X(x;x)$  we have  a social point
$\alpha_x(1_x)\in F_0(x)$.
Otherwise each  social point $m = \alpha_x(1_x)\in F_0(x)$
can be get from some uniquely defined natural transform.
For generated transform $\alpha: X(-;x)\rightarrow F$ we need to check commuting
diagram for arbitrary edge $h\in X(b;a)$
$$\matrix{ X(a;x) & \mapright \alpha_a & F_0(a) \cr
 \mapdownk h^* &  & \mapdownd h^F \cr
 X(b;x) & \maprightap \alpha_b & F_0(b) \cr } $$
 \vskip\tarpas
 The equality of sets mappings suffice to check for each point in source set.
 Therefore we can apply the larger  commuting diagram
\vskip 30pt
$$ \matrix{  & \nearrow & & \cr
i_x\in X(x;x) &  & & \cr
     \mapdownk f^* & \searrow && \cr
     & \hskip -20pt \nearrow & & &\hskip -20pt\nearrow  \cr
     X(a;x) & \maprightap h^* & X(b;x) &\cr }  $$
      \vskip -100 pt
$$ \hskip 140pt \matrix{ m\in F_0(x) & &  \cr
    \mapdownk F(f) & \searrow  \cr
     \phantom{ \nearrow} & & \phantom{ \nearrow} \cr
     F_0(a) & \maprightap F(h) & F_0(b)  \cr }$$
\vskip 40pt
    \vskip \tarpas
\irodymopabaiga
We have got that the set of natural transforms
$\alpha: X(-;x) \rightarrow F $
can be identified with the set of social points in values set $F_(x)$.

Taking another representable character $F=X(-;y)$
we get bijection  between natural transforms
$\alpha: X(-x)\rightarrow X(-;y)$
and social edges $\theta\in X(x;y)$.
For such natural transform we appoint an image $\alpha_x(1_x)\in X(x;y)$.
Conversely for each edge $\theta\in X(x;y)$ we appoint the transform
defined with collection of mappings
$\alpha_a(f)= f\circ \theta\tsk$
$$\matrix{ 1_x\in X(x;x) & \mapright \alpha_x & \theta\in X(x;y) \cr
\mapdownk f^* & & \mapdownd f^* \cr
f\in X(a;x) & \maprightap \alpha_a & f\circ \theta \in X(a;y) \cr } $$
\vskip\tarpas
By the former proposition such transform is natural.

In general For the contact arrow
$\theta\circ \kappa\in X(x;z)\uparrow \kappa\in X(y;z)$
we  don't get
vertical composition of correspondent natural transforms.
But for composition of natural transforms we get composed contact
arrows  mappings. We need to check the composition only over unit arrows.

Let we have composable natural transforms  $\alpha: X(-;x) \rightarrow X(-;y)$
and $\beta: X(-;y)\rightarrow X(-;z)$ with corespondent edges
$\alpha_x (1_x)= \theta\in X(x;y)$ and $ \theta_y(1_y)= \kappa\in X(y;z) $.
Then for the composition $\alpha\circ \beta: X(-;x)\rightarrow X(-;z)$
we get contact arrow
$\beta_y(\alpha_x(1_x))= \theta\circ \kappa $
$$\matrix { & & 1_y\in X(y;y) & \mapright {\beta} &\kappa\in X(y;z) \cr
 & & \mapdownk \theta^* &  & \theta^* \cr
 1_x\in X(x;x) & \mapright \alpha_x & X(x;y) & \maprightap \beta_x  &
 \theta\circ \kappa \in X(x;z) \cr} $$
 \vskip\tarpas

As a consequence we deduce important property.

For the two vertexes $x\in X_0$ and $y\in X_0$ having isomorphic natural
transform between representable characters
$$ \alpha: X(-;x) =\rightarrow X(-;y) $$
defined with edge $\alpha_x(1_x)= \theta\in X(x;y) $
we get the inverse natural transform $\alpha\inv: X(-;y)\rightarrow X(-;x)$
defined with the inverse edge $\alpha\inv (1_y)= \theta\inv \in X(y;x)$,
i. e. we have equalities of contact arrows
$$\theta\circ \theta\inv= 1_x \kbl \theta\inv \circ \theta= 1_y\tsk$$

For an original graph with associative contact arrows mappings
every representable character is natural  functor, as
for composable edges $h\in X(c;b)$ and $g\in X(b;a)$ the representable
character $X(-;x): X^\op \doublerightarrow \VV$ provides
composable source changing
$$X(a;x)\mapright g^*  X(b;x) \mapright h^*  X(c;x)\kbl$$
with an equality
$$h\circ (g\circ f) = (h\circ g)\circ f \uparrow f\in X(a;x)\kbl$$
i. e. $h^*(g^*(f)) = (h\circ g)^*(f)$.

Also for associative contact arrow mappings we get composable natural
transforms defined by  arbitrary composable edges.

$$\matrix { & & 1_y\in X(y;y) & \mapright \beta_y & \kappa \in X(y;z) \cr
 & & \mapdownk \theta^* &  & \theta^* \cr
 1_x\in X(x;x) & \mapright \alpha_x & X(x;y) & \maprightap \beta_x  &
 \theta\circ \kappa \in X(x;z) \cr
 \mapdownk f^* & &\mapdownk f^* & &\mapdownd f^* \cr
 f\in X(a;x) & \maprightap {f\circ \theta} & f\circ \theta\in X(a;y) &
 \maprightap f\circ (\theta \circ \kappa)  & X(a;z) \cr }$$
\vskip\tarpas
$$(\alpha\circ \beta)_a(f) = f \circ (\theta\circ \kappa)= (f\circ \theta)
\circ \kappa \tsk$$
 \vskip\tarpas

We shall notice that Yoneda lemma can be applied for more
large stock of transforms between two characters.
For the graph $Y$ having edges sets ordered with some order relation
we get order relation for parallel  mappings of edges set. Let we have
two mappings $u,v:X(a;b) \rightarrow Y(\phi_0(a);\psi_0(b))$. Then we can take
initial order relation between such mappings, i. e. we have an inequality
between two mappings if such inequality is true for each pairs of values.
We shall  denote such inequality as an arrow
$$u\dgl v \lygiavertu u\rightarrow v\uparrow
 u,v\in \Set(X(a;b); Y(\phi_0(a);\psi_0(b))\tsk$$
We could define the set
of ^{continuous =transforms} by diagram
$$\matrix{ F_0(x) & \mapright \alpha_x  &  G_0(x) & \cr
\mapdownk f^F & &  \mapdownd f^G & \cr
F_0(y) &  \maprightap  \alpha_y  & G_0(y)&  \cr
&  &  & &\hskip -15pt \nearrow \hfill\cr } $$
\vskip\tarpas
It will  be  the ^{deformed =quadrats} $(-13)$ for ^{respecting
=reform} $\alpha$ in \baf G. Valiukevi\v cius 2009*.
The arrows $f^F$ and $f^G$  will be interpreted as ^{generalized
=convergences}.

With another direction of inequality we shall define
^{cocontinuous  =transforms}
$$\matrix{ F_0(x) & \mapright \alpha_x  &  G_0(x) & \cr
\mapdownk F(f) & &  \mapdownd G(f) & \cr
F_0(y) &  \maprightap  \alpha_y  & G_0(y)&  \cr
&  &  & &\hskip -15pt \swarrow \hfill\cr } $$
It will correspond  the ^{deformed =quadrats} $(+13)$  of ^{wasting
=reform} $\alpha$.

The deformed  quadrats provides  instances of ^{=diagrams}.
Their  edges may be
interpreted as functors between different categories.  But later we shall
define also some coherent transform of continuous quadrats, and we shall
use another sort of edges defined with arrows of natural transforms.

The Yoneda lemma for continuous or cocontinuous
transforms needs to define for the graphs transport
 $F: X^\op\doublerightarrow \Set$
lower social points or upper social points.

For the ^{lower  social =point} $m\in F_0(x)$ we demand continuous  mapping
$h^F : F_0(a) \rightarrow F_0(b)$ for every edge $h\in X^\op(a;b)$
i. e. we should have deformed triangular diagram
$$\matrix{ m & & & \cr
  \downarrow & \searrow &  &  \cr
   F_0(a) & \maprightap h^F & F_0(b) & \cr
         &  & &\hskip -10 pt   ^\nearrow  \hfill \cr}$$
\vskip\tarpas
For the upper  social point $m\in F_0(x)$ we demand that a mapping
$h^F : F_0(a) \rightarrow F_0(b)$ would be cocontinuous,  i. e.
we would have a triangular diagram with opposite order relation
$$\matrix{ m & & & \cr
  \downarrow & \searrow &  &     \cr
   F_0(a) & \maprightap h^F  & F_0(b) & \cr
         &  & &\hskip -10 pt  { ^\swarrow}  \hfill \cr}$$
\vskip\tarpas

We can check that the lower  social points generate continuous transforms,
and the upper  social points generate    cocontinuous transforms
between representable character $X(-;x)$ and some graphs transport $F$.

\Proposition
The lower social point $m\in F_0(x)$ generates continuous transform
$\alpha: X(-;x)\rightarrow F$. And vice versa continuous transforms are
generated by some lower social point.
\Proof:
The proving can be checked by chasing diagram
\vskip 30pt
$$ \matrix{  & \nearrow & & \cr
i_x\in X(x;x) &  & & \cr
     \mapdownk f^* & \searrow && \cr
     & \hskip -20pt \nearrow & & &\hskip -20pt\nearrow  \cr
     X(a;x) & \maprightap h^* & X(b;x) &\cr }  $$
      \vskip -100 pt
$$ \hskip 140pt \matrix{ m\in F_0(x) & & & \cr
    \mapdownk F(f) & \searrow & \cr
     \phantom{ \nearrow} & & &\phantom{ \nearrow} \cr
     F_0(a) & \maprightap F(h) & F_0(b) & \cr
          &     &  & \hskip -10pt { ^\nearrow}   \hfill \cr}$$
\vskip \tarpas
\irodymopabaiga

We can say that contact arrows mappings  are ^{lower =associative},
if we have  associative arrow as inequality between two $\VV$-graphs
transports
$$(h\circ f)\circ \theta\rightarrow h\circ (f\circ \theta)\uparrow
 \theta \in X(c;x), g\in X(b;c), f\in X(a;b) \tsk$$
This will provide all arrows  $\theta\in X(c;x)$
being lower social for  representable functor $X(-;x)$.
\vskip\tarpas

We can repeat the proposition about name appointment
 for graphs with ordered
edges sets.
Let we have graphs $X$ with ordered sets of edges $X(a;b)$.
We demand that for a graphs transport $F: X\doublerightarrow Y$ the
 mappings
between edges sets would be monotone
$$F_{a,b}: X(a;b)\rightarrow X(F_0(a); F_0(b))\tsk$$

In the Carte biproduct $X\times Y$ we take the initial order relation
for edges sets
$$X\times Y(\lan a, a'\ran, \lan b, b'\ran =
X(a;b)\times Y(a';b') \tsk$$

In the exponential space $Y^T$ also we can take  an initial order relation
inside the set
of transforms
$$Y^T (\phi;\psi)= \Prod_{s\in T_0} Y(\phi_0(s); \psi_0(s)) \tsk$$

We get again  a joint pair of monotone superfunctors within the categories of
graphs with ordered sets of edges.

The choosing of unit arrows in the source graph $1_a\in X(a;a)$
and in the assistant graph  $1_t\in T(t;t)$  allows us to define
the unit transform  with the collection of sections transports
$\lambda_X: X\doublerightarrow (X\times T)^T $.
The edges mappings $$\lambda_X (\alpha): \lambda_X(a)\rightarrow \lambda_X(b) $$
are  defined by  the collection of edges
$$\lan u, 1_s\ran : \lan a,s\ran \rightarrow \lan b,s\ran \uparrow
u\in X(a;b)\kbl$$
$$\lambda_X(u) = \Prod_{s\in T_0} \lan u, 1_s) :
\Prod_{s\in T_0} \lan a,1_s) \rightarrow \Prod_{s\in T_0} \lan b,; 1_s) \tsk$$
and obviously maintain the order relation.

The choosing  of monotone contact arrows in the target graph $Y$
$$Y_{c,d,e}: Y(c;d)\times Y(d;c) \rightarrow Y(c;e)$$
allows us to define  a counit transform
$\ev_Y: Y^T\times T \rightarrow Y$  with collection
of evaluation transports. The contact arrows mappings must be monotone
for every its argument. We can take  the preevaluation or postevaluation
transport. At this moment we are chosen the preevaluation
transport defined with precontact arrows
$\ev^+_{\VV} : Y^T\times T \doublerightarrow Y$.
For a transform $\alpha: \phi\rightarrow \psi$ and an edge $u\in T(s;t)$
we appoint
$$\ev_Y^+ (\alpha,u)= \alpha_s \circ \psi(u) \in Y(\phi_0(s);\psi_0(t))\tsk$$
Such appointment will be monotone by the properties of chosen monotone
contact arrows mappings.

The  unit transform  defined with sections transports
$\lambda_X: X\doublerightarrow (X\times T)^T$
provides the monotonous name appointment for forms
$$g:\Grph(X\times T; Y) \rightarrow \Grph(X;Y^T) \tsk$$
With an inequality between two graphs transports $f\dgl f'$
we get the inequality between appointed name forms $f^\#\dgl (f')^\#$
provided with composition of monotone graphs transports. Such
are the section transport and changing of target space also are monotone
for chosen inequalities in exponential spaces
$$g(f)=f^\#: X\mapright \lambda_X (X\times T)^T \mapright f^T Y^T \tsk$$
A counit transform defined with preevaluation  transports
$\ev_Y^+: Y^T\times T \doublerightarrow Y$
also is monotone appointment for name forms
$$f_+:\Grph(X;Y^T) \rightarrow \Grph (X\times T;Y) \tsk$$
With an inequality between two graphs transports  $g\dgl g'$
we get the inequality between their realizations $f_+(g) \dgl f_+(g')$
provided with composition of monotone graphs transports.
Such is the biproduct  with identity transport
$\Identity_T: T\doublerightarrow T$ and then we have monotone
 evaluation transport
$$f_+(g)=g^\flat : X\times T  \mapright g\times 1_T  Y^T\times T
\mapright \ev_Y^+ Y\tsk$$

For graphs transport $f: X\times T\doublerightarrow Y$
we can  ask ^{lower =predecomposition } property
$$ f(\alpha,u)\dgl f (\alpha, 1_s) \circ f(1_b; u) \uparrow \alpha\in X(a;b),
 u\in T(s;t)  \tsk$$
Then we get inequalities for prerealization of name form
$$f\dgl f_+(g(f))\tsk$$
It can be considered as unit inequality for joint pair of monotonous
mappings provided with the form's name and the name form's realization
$$\Grph (X\times T;Y) \rightleftarrows \Grph (X; Y^T) \tsk$$

For a graphs transport $g: X\doublerightarrow Y^T$  we ask
^{upper =preneutral} properties
$$g( 1_a)_s \circ g_0(a)_u \dgl g_0(a)_u \kbl$$
$$g(\alpha)_s \circ g_0(b)_{1_s} \dgl g_0(\alpha)_s \tsk$$
Then we get a counit inequalities for the joint pair of name and realization
appointments
$$g\mzl g(f_+(g))\tsk$$

The categorical proving is a same as for the graphs without any order relation
in the sets of edges, cl. \baf G. Valiukevi\v cius 2022*.
\vskip\tarpas

Now we shall try to study $\VV$-enriched spaces.
At first we define  the category $\Grph_{\VV}$ of ^{$\VV$-enriched =graphs}.
We shall use a shorter name ^{$\VV$-=graphs}.
In the set of arrows $ \VV(r; s)$ between two points $r,s\in \VV_0$
 we choose  some  order relation. We must note that the equality also can be
understood as an order relation.
The arrows between points of values category $r,s\in \VV_0$  will be
called as ^{=mappings}.

A  $\VV$-graph $X$ will be a set of vertexes $X$
with the sets of edges  being objects in the values category
$X(x;y)\in V_0$.

A  ^{$\VV$-graphs =transport} $f:X\doublerightarrow Y$
will be defined with an appointment of vertexes
$f_0: X_0\rightarrow Y_0$ and collection of mappings
for the edges sets
$$f_{x,y}: X(x;y)\rightarrow Y(f_0(x);f_0(y))\tsk$$

Such transports compound the category with usual composition.
The identity transports will be ^{=unit arrows} for such composition.
For two $\VV$-graphs transports $f: X\doublerightarrow Y$ and
$g: Y\doublerightarrow Z$
we have composition of vertexes appointments
$$(f\circ g)_0(x) = g_0(f_0(x))\in Z\uparrow x\in X$$
and composition of edges set  mappings
$$(f\circ g)_{x,y}=  f_{x,y} \circ g_{f_0(x),f_0(y)} \tsk$$
An identity transport $\Identity_X: X\doublerightarrow X$
is defined by identity appointment for vertexes
$$ \Identity_{X_0}: X_0\rightarrow X_0$$
and identity mappings for the edges sets
$$\Identity_{X(x,y)}: X(x;y) \rightarrow X(x;y) \tsk$$
This category will be denoted  $\Grph_{\VV}$.

We shall say that two $\VV$-graphs transports are parallel if
they have the same vertexes appointments
$$f_0(x)= g_0(s)\uparrow s\in X_0\tsk$$
The order relation in the sets of edges $V(a;b)$ will define
the order relation between ^{=parallel  $V$-graphs transports}
$$f, g: X\doublerightarrow Y\tsk$$

The inequality  $f\dgl g$ is  defined
by order relation  for
the edges set mappings
$$f_{x,y} \dgl g _{x;y} : X(a;y) \rightarrow
Y(f_0(x); f_0(y))=Y(g_0(x);g_0(y)) \tsk$$

More strong ordering could be defined by factorization property
$$g= f\circ h\tsk$$
But it is waiting for later investigations and applications.

We shall define some
^{=superfunctors} over the category $\Grph_{\VV} $. At first we have
the ^{primary  =projection}
$$\Grph_{\VV} \superrightarrow \SET\tsk$$

 For each $\VV$-graph  $X$
it appoints the set of vertexes $X_0$ and for a $\VV$-graphs transport
$f:X\doublerightarrow Y$  it appoints the
appointment  $f_0:X_0\rightarrow Y_0$
of vertexes.

We have more interesting superfunctors.
For two $\VV$-graphs $X$ and $Y$ we appoint a biproduct
$X\otimes Y$ defined with Carte product $X_0\times Y_0$ for the sets of
vertexes and biproduct from values category $\VV$  for the sets of edges
$$X\otimes Y(\lan x,y\ran;\lan x',y'\ran):= X(x;x')\otimes Y(y;y')\tsk$$
For two $\VV$-graphs transports  $f:X\doublerightarrow X'$ and
$g: Y\doublerightarrow Y'$
we take  the  biproduct  of transports
$$f\otimes g: X\otimes Y\doublerightarrow X'\otimes Y'$$
defined  with Carte tensor product of vertexes  appointments
$$f_0\times g_0: X_0\times Y_0\rightarrow X_0'\times Y_0'$$
 and biproduct of  edges set mappings
$$(f\otimes g )_{\lan x,y\ran, \lan  x',y'\ran} := f_{x,x'} \otimes
g_{ y;y'}\tsk$$
So we have defined a superfunctor  over the Carte product of categories
$$\Grph_{\VV} \times \Grph_{\VV} \superrightarrow  \Grph_{\VV} \tsk$$
We assume that the biproduct $r\otimes s$ is monotone in values category
$\VV$ for both arguments, so the tensor product of $\VV$-graphs transports
$f\otimes g$ will be monotone also.

Let we have pairs of parallel graphs transports $f\dgl f': X\doublerightarrow X'$
and $g\dgl g': Y\doublerightarrow Y'$. These means that we have
the inequalities for edges set mappings
$$f_{x,x'}: X(x;x')\rightarrow X'(f_0(x);f_0(x')) \kbl
f'_{x,x'} : X(x;x')\rightarrow X'(f'_0(x); f'_0(x'))\tsk $$
These mappings also are parallel as $f_0=f'_0$, therefore 
$$X'(f_0(x);f_0(x'))= X'(f'_0(x);f'_0(x'))\tsk$$
Also we have the inequalities for another edges set mappings
$$g_{x,x'}: Y(x;x')\rightarrow Y'(g_0(x);g_0(x')) \kbl
g'_{x,x'} : Y(x;x')\rightarrow Y'(g'_0(x); g'_0(x'))\tsk $$
These mappings are parallel as $g_0=g'_0$, therefore
$$Y'(g_0(x);g_0(x'))= Y'(g'_0(x);g'_0(x'))\tsk$$

The inequalities
$$f_{x,x'}\dgl f'_{x,x'}\kbl g_{y,y'} \dgl g'_{y,y'}  $$
provide the inequality for biproducts
$$ f_{x,x'} \otimes g_{x,x'} \dgl f'_{x,x'}\otimes g'_{y,y'} \tsk$$
This means that we have inequality of parallel graphs transports
$$f\otimes g\dgl f'\otimes g' : X\otimes Y \doublerightarrow X'\otimes Y'
\tsk$$

We shall deal with superfunctor defined by some
^{=assistant $\VV$-graph} $T$. It for
a $\VV$-graph $X$ appoints the biproduct $X\otimes T$ and for  a
$\VV$-graphs  transport $f:X\doublerightarrow Y$
appoints
the biproduct
with the identity transport  of the assistant graph
$$f\otimes \Identity_T: X\otimes T\doublerightarrow Y\otimes T\tsk$$
Such appointment will maintain  the inequality
 between  parallel $\VV$-graphs
transports
$f,g: X\doublerightarrow Y$
$$f\dgl g \duoda f\otimes \Identity_T \dgl g\otimes \Identity_T\tsk$$

We also shall define an ^{exponential =superfunctor} $Y^T$.
For  a $\VV$-graph $Y$
and a small assistant $\VV$-graph $T$ we take
the set $Y^T$ of all $\VV$-graphs transports
 $\phi: T\doublerightarrow Y$. They are defined with
the appointments of vertexes  $\phi_0: T_0\rightarrow X_0$ and the
mappings of
edges sets
$$\phi_{s,t} : T(s;t)\rightarrow Y(\phi_0(s);\phi_0(t)))\tsk$$

The edges sets $Y^T(\phi;\psi)$ are defined as sets of transforms
produced by product of edges sets in values category $\VV$
$$Y^T(\phi;\psi)= \Prod_{s\in T_0} Y(\phi_0 (s); \psi_0(s))\tsk$$
We can check that we have got indeed a superfunctor.

For  the $V$-graphs transport $g: X\doublerightarrow Y$ we appoint
the changing of target space. For a set of transforms
between two  $\VV$-graphs transports  $\phi,\psi: T\doublerightarrow X$
we appoint the  new set of transforms
between
changed transports
$$\phi\circ g, \psi\circ g: T\doublerightarrow Y\tsk$$
The edges
set mapping will be provided by the Carte product of mappings
$$\Prod_{s\in T_0} X(\phi_0(s);\psi_0(s))\rightarrow
\Prod_{s\in T_0} g_{\phi_0(s),\psi_0(s)} (X(\phi_0(s);\psi_0(s)))\subset $$$$
\Prod_{s\in T_0} Y(g_0(\phi_0(s)); g_0(\psi_0(s)))\tsk$$

This superfunctor also is   monotone for the  order relations between
^{secondary =parallel} $\VV$-graphs transports of exponential spaces.
$$g,g': Y^T(\phi;\psi) \doublerightarrow Y^T (\phi\circ g;\psi\circ g)\tsk$$

For the  inequality
between  parallel $\VV$-graphs transports
$g,g': X\doublerightarrow Y$
with an equality of   projection
$$ g_0(x)= g'_0(x)\uparrow x\in X_0$$
and inequalities for
edges set mappings
$$g_{x,y}\dgl g'_{x, y} \uparrow x,y\in X_0 $$
we get  the $\VV$-graphs transports $g^T,(g')^T: X^T\doublerightarrow Y^T$
with the equality for the ^{ secondary  =projections}
$$(g_0)^{T_0}=(g'_0)^{T_0} : (X_0)^{T_0} \rightarrow (Y_0)^{T_0} $$
and inequalities for the $\VV$-graphs transports
defining the appointment of the first projection.
For a $\VV$-graphs transport $\phi\in (X^T)_0$ it appoint the new
$\VV$-graphs transport $\phi\circ g\in (Y^T )_0$
$$\phi\circ g\dgl \phi\circ g'\uparrow \phi\in X^T $$
with inequalities   for edges set mappings
$$T(s;t)\rightarrow g_{\phi_0(s),\phi_0(t)}
(\phi_{s,t}(T(s;t))\dgl
g'_{\phi_0(s),\phi_0(t)}
(\phi_{s,t}(T(s;t)) \tsk$$
Also we get the inequalities  for edges set mappings of $\VV$-graphs transports
provided with changing of target space
$$X(x;y) \rightarrow
\Prod_{s\in T_0} g_{\phi_0(s),\psi_0(s)} (X(\phi_0(s);\psi_0(s))) \dgl
$$$$\Prod_{s\in T_0} g'_{\phi_0(s),\psi_0(s)} (X(\phi_0(s);\psi_0(s)))
\subset \Prod_{s\in T_0} Y(g_0(\phi_0(s)); g_0(\psi_0(s)))\tsk$$

We have got a joint pair of monotone superfunctors $X\otimes T$ and $Y^T$
within the category of $\VV$-graphs $\Grph_{\VV}$.
A ^{unit partial =transform} for such joint pair of superfunctors
is defined by collection
of ^{=sections transports} for $\VV$-graphs $X$
with chosen ^{unit arrow =mappings} $*\rightarrow 1_x(*)\subset X(x;x)$.
Also we need unit arrow mappings for the assistant $\VV$-graph
$*\rightarrow 1_t(*)\subset T(t;t)$.

Sections transport  $\lambda_X: X\doublerightarrow (X\otimes T)^T$
for a vertex $x\in X_0$ appoints the section $\lambda_X(x):
T\doublerightarrow X\otimes T $ which for a vertex $t\in T_0$ appoints
the couple of vertexes $\lan x,t\ran\in X_0\times T_0$ and have edges set
mappings
$$\lambda_X(a)_{s,t}: T(s;t)\rightarrow 1_a(*)\otimes T(s;t)\subset X(a;a)\otimes
T(s;t)$$
defined as a biproduct of  chosen unit arrow mappings $*\rightarrow 1_a(*)\subset X(a;a)$
 with identity mapping $\Identity_{T(s;t)}:T(s,t)\rightarrow T(s;t)$.
For the sections transport an edges set mapping will be a  product of
biproducts for identity mappings $\Identity_{X(a,b)}:
X(a,b)\rightarrow X(a;b)$ with chosen
unit arrow $*\rightarrow 1_s(*)\subset T(s;s)$
$$X(a;b)\rightarrow (\lambda_X)_{a,b}(X(a;b)) =
\Prod_{s\in T_0} (X(a;b)\otimes 1_s(*))\subset
 (X\otimes T)^T (\lambda_X(a); \lambda_X(b))\tsk$$
There is no sense to speak about monotonous property for such section
transports when we work with $\VV$-graphs. But name appointment
of forms rests monotone
$$f^\# : X\mapright \lambda_X (X\otimes T)^T \mapright f^T Y^T \tsk$$
It is enough to know that changing of target space is monotone
for inequality between parallel $\VV$-graphs transports
$$f\dgl g: X\otimes T \doublerightarrow Y \tsk$$

A ^{counit partial =transform}  is defined  by collection of ^{=evaluation
transports} for $\VV$-graphs $Y$ with ^{=contact arrows mappings}
$$Y(x;y)\otimes Y(y;z)\rightarrow Y(x;y)\circ Y(y;z)\subset Y(x;z)\tsk$$

For a couple of  $\VV$-graphs transport $\phi: T\doublerightarrow Y$
and vertex $s\in T_0$  the  evaluation transport
appoints the value $\phi_0(s)\in Y_0$, and for a set of transform
between two $\VV$-graphs transports
$\phi, \psi: T\doublerightarrow  Y$
 $$ \Prod_{s\in T_0} Y(\phi_0(s);\psi_0(s))\subset Y^T(\phi;\psi)$$
and  an edges  set $T(s;t)$ evaluation transport will be defined by mapping
of ^{=precontact arrows}
$$Y^T(\phi;\psi)\otimes T(s;t)\rightarrow
Y(\phi_0(s);\psi_0(s))\circ \psi_{s,t} (T(s;t))\subset
 Y(\phi_0(s);\psi_0(t))\tsk$$

We shall  demand that changing of target space
with  contact arrows  mappings will be monotone in values
category $\VV$. For arbitrary object $r\in \VV_0$  we ask
monotone mappings
$$V(r; Y(x;y))\rightarrow V(r; Y(x;y) \circ Y(y;z))\subset \VV(r; Y(x;z))
\kbl$$
$$\VV(r;Y(y;z)) \rightarrow \VV(r; Y(x;y)\circ Y(y;z))\subset \VV(r;Y(x;z))
\tsk$$
That provides monotone realization for name forms
$g: X\doublerightarrow Y^T$
$$g^\flat :  X\otimes T \mapright g\otimes 1_T  Y^T \otimes T \mapright \ev_Y
Y \tsk$$                           
Let we have an inequality between  the secondary parallel name forms
$g\dgl g': X\doublerightarrow Y^T $.
Then we can check the inequality between realized forms.  We shall check
inequalities for edges set  mappings
$$X(x;y) \otimes T(s;t) \rightarrow g_{x,y} (X(x;y))\otimes T(s;t)
\rightarrow
$$$$Y(g_0(x)_s ; g_0(y)_s) \circ (g_0(y))_{s,t}  (T(s;t)) \dgl
$$$$ g'_{x;y} (X(x;y)) \circ  (g_0(y))_{s,t}  (T(s;t)) \dgl
$$$$ g'_{x;y} (X(x;y)) \circ  (g'_0(y))_{s,t}  (T(s;t)) \tsk$$

We are ready to prove the properties   of name appointment
   or realization appointment between the forms
   into the  target $V$-graph $Y$.
For chosen unit arrows mappings in the source $\VV$-graph
$*\rightarrow 1_a(*)\subset X(a;a)$ and the
assistant  $\VV$-graph $*\rightarrow 1_s(*)\subset T(s;s)$,
 and contact arrows mappings  in  the target $\VV$-graph
 $$Y(x;y)\otimes  Y(y;z)\rightarrow Y(x;y) \circ Y(y;z)\subset Y(x;z)$$
 the $\VV$-graphs form $f: X\otimes Y\doublerightarrow Z$  will be
 called  ^{=lower decomposable } if we have inequality  between mappings
$$X(a;b)\otimes T(s;t) \rightarrow
f_{\lan a,s\ran,\lan b,s\ran } (X(a;b)\otimes 1_s(*) ) \circ
f_{\lan y,s\ran,\lan y,t\ran} (1_b(*) \otimes T(s;t))\mzl  $$$$
f_{\lan x,s\ran,\lan b,t\ran} (X(a;b)\otimes T(s;t))\subset
Y(f(a,s); f(b,t))$$
Otherwise we shall say that a $\VV$-enriched graphs transport
$g: X\doublerightarrow Y^T$ is ^{upper =neutral} for chosen unit arrows
if we have other inequalities between mappings

$$X(a;b)\rightarrow g_{a,b}(X(a;b))_s \circ g(b)_{s,s}(1_s(*)) \dgl$$$$
g_{a,b} (X(a;b))_s \subset Y(g(a)_s;g(b)_s) \kbl$$
$$T(s;t)\rightarrow g_{a,a}(1_a(*) )\circ g(a)_{s,t} (T(s;t))\dgl $$$$
g(a)_{s,t}(T(s;t)) \subset Y(g(a)_s;g(a)_t) \tsk$$

As name or realization  appointments aren't totally defined,
we shall use the notion of ^{=composable partial appointments}.
One partial appointment  $\Phi:A\ventrightarrow B$ is composable with
another partial appointment  $\Psi: B\ventrightarrow C$ if the first
 appointment has values in the domain of definition for the second
 appointment.

\Proposition
The choosing of unit arrow mappings in the source $\VV$-graph
$*\rightarrow 1_a(*)\subset  X(a;a)$ and in the assistant $\VV$-graph
$*\rightarrow 1_t(*)\subset T(s;s)$  allows us to define
the name appointment   between the sets of $\VV$-graphs transports
$$\Grph_{\VV} (X\otimes T; Y)\rightarrow \Grph_{\VV} (X; Y^T)\tsk$$

The contact arrows mappings in the target $\VV$-graph  $Y$
$$ Y(c;d)\otimes Y(d;e) \rightarrow Y(c;d)\circ Y(d;e)\subset Y(c;e)$$
provide evaluation transport with precontact arrows mappings
and allow us to define the realization appointment
$$\Grph_{\VV} (X;Y^T) \rightarrow \Grph_{\VV} (X\otimes T; Y) \tsk$$

If contact arrows mappings are monotone, then
the composable restriction of these appointments  provides joint pair of
monotone mappings  from
$V$-graphs transports
over the biproduct $f: X\otimes T \doublerightarrow Y$
which are lower decomposable for chosen
mapping of contact arrows in the target  $\VV$-graph  $Y$
$$X(a;b)\otimes T(s;t) \rightarrow
f_{\lan a,s\ran,\lan b,s\ran } (X(a;b)\otimes 1_s(*) ) \circ
f_{\lan y,s\ran,\lan y,t\ran} (1_b(*) \otimes T(s;t))\mzl  $$$$
f_{\lan x,s\ran,\lan b,t\ran} (X(a;b)\otimes T(s;t))\subset
Y(f(a,s); f(b,t))$$
to $\VV$-graphs transports $g: X\doublerightarrow Y^T$ which are
upper neutral for chosen unit arrows in the source $\VV$-graph $X$ and the
assistant $\VV$-graph  $T$
$$X(a;b)\rightarrow g_{a,b}(X(a;b))_s \circ g(b)_{s,s}(1_s(*)) \dgl$$$$
g_{a,b} (X(a;b))_s \subset Y(g(a)_s;g(b)_s) \kbl$$
$$T(s;t)\rightarrow g_{a,a}(1_a(*) )\circ g(a)_{s,t} (T(s;t))\dgl $$$$
g(a)_{s,t}(T(s;t)) \subset Y(g(a)_s;g(a)_t) \kbl$$
i. e. we have inequalities for unit and counit transforms
$$f\dgl f_+(g(f))\kbl g(f_+(g))\dgl g\tsk$$
\Proof:
We shall adapt the  earlier categorical proving for  the category
of graphs $\GRPH$ in \baf G. Valiukevi\v cius 2022*.
We can  see that the  name  appointment is monotone. The inequality
$f\dgl f'$ between  $\VV$-graphs transports
$f,f': X\times T\doublerightarrow  Y$ is maintained by exponential
superfunctor
$$f^T\dgl (f')^T $$
and by composition with sections transport
$$\lambda_X: X\doublerightarrow (X\otimes T)^T \tsk$$

Also the realization appointment is monotone. The inequality $g\dgl g'$ between
$\VV$-graphs transports $g,g': X\doublerightarrow Y^T$  is maintained
by superfunctor of tensor product
$$f\otimes \Identity_T \dgl g\otimes \Identity_T $$
and by composition with evaluation transport
$$\ev_Y: Y^T\otimes T \doublerightarrow Y\tsk$$
The evaluation transport is monotone  as a
 consequence of monotone  contact arrows mappings in the target
$\VV$-graph $Y$.

First we shall check that a realization of name is decreasing.
For it we construct a  continuous diagram
$$\matrix { X\otimes T & \mapright \lambda_X\otimes 1_T &
(X\otimes T)^T \otimes T & \mapright f^T\otimes 1_T  & Y^T\otimes T &\cr
& \searrow & \mapdownd \ev_{(X\otimes T)} & & \mapdownd \ev_{Y} & \cr
& & X\otimes T & \maprightap f & Y & \cr
& &            &               &  &\hskip -15 pt \nearrow  \cr } $$
\vskip \tarpas
The evaluation transport $\ev_{(X\otimes T)}:
(X\otimes T )^T\otimes T \doublerightarrow X\otimes T $  is defined by
choosing mappings  of contact arrows
$$X(a;b)\otimes T(s;t)\rightarrow (X(a;b)\otimes *)\otimes (*\otimes T(s;t))
\rightarrow $$$$(X(a;b)\otimes 1_s(*))\circ
(1_b(*)\otimes  T(s;t))= X(a;b)\otimes T(s;t) \tsk$$
This is natural choice, but we need to check that with such choice
we have got a suitable diagram.
At first we shall check the first triangular equality for arbitrary
$\VV$-graphs
$X$ and $T$ with chosen unit arrow mappings $*\rightarrow 1_a(*) \subset
X(a;a)$ and $*\rightarrow 1_t(*)\subset T(t;t)$.
We shall prove the identic transport for composition of $\VV$-graphs
transports
\vskip\tarpas
$$\Identity_{(X\otimes T)} : X\otimes T\mapright \lambda_X\otimes 1_T (X\otimes T )^T\otimes T
\mapright \ev_{(X\otimes T)}  X\otimes T \tsk$$
We apply the  projection of categories $\Grph_{\VV}\superrightarrow \SET $
which for a $\VV$-graph $X$ appoints its vertexes set $X_0$, and for a
$\VV$-graphs transport $f: X\doublerightarrow Y$
 appoints the vertexes  appointment
$f_0:X_0\rightarrow Y_0$.

 The  constructed biproduct of $\VV$-graphs   $X\otimes Y$
is projected to the Carte tensor product of sets $X_0\times Y_0$.

For an exponential $\VV$-graph $Y^T$ such projection appoints the set of all
$\VV$-graphs transports $\phi: T\doublerightarrow Y$.
It will be called a ^{primary =projection}. The ^{secondary =projection}
is defined with
deformation of each $\VV$-graphs transport
$\phi: T\doublerightarrow Y$ to its
vertexes appointment $\phi_0: T_0\rightarrow Y_0$. Later we shall need
to calculate these projections only for some $\VV$-graphs transports.

For the secondary projection we get the first triangular equality
in the category of sets $\SET$.
The evaluation appointment for a $\VV$-graphs transport
$\phi: T\doublerightarrow Y$ and vertex $s\in T_0$ appoints the value
$\phi_0(s)\in Y_0$ which
 depends only on
projection $\phi_0: T_0\rightarrow Y_0$,  so we get the
first triangular
equality also for the primary projection.

For a biproduct of  edges sets $X(a;b)\otimes T(s;t)$
the first $\VV$-graphs transport
$$\lambda_X\otimes \Identity_T: X\otimes T\doublerightarrow (X\otimes T)^T
\otimes T $$
will appoint the biproduct of  transforms set
$$\Prod_{s\in T} ( X(a;b) \otimes 1_s(*))
\subset (X\otimes T)^T(\lambda_X(a);\lambda_X(b))$$
 and the same edges set  in the assistant $\VV$-graph $T(s;t)$.
The second $\VV$-graphs transport will be the
evaluation transport on $V$-graphs biproduct $X\otimes T$.
It for the former biproduct  will appoint the contact
arrows mapping
$$X(a;b) \otimes T(s;t) \rightarrow
(X(a;b)\otimes 1_s(*))\circ (1_b(*)\otimes T(s;t))=X(a;b)\otimes T(s;t))\tsk$$
So we can  end the checking of the first triangular equality in the category of
$\VV$-graphs $\Grph_{\VV}$.

Now we shall check for what
$\VV$-graphs transport $f: X\otimes T\doublerightarrow Y$
we get continuous  quadrat
$$ \matrix{ (X\otimes T)^T\otimes T  & \mapright f^T\otimes 1_T &
 Y^T\otimes T  &\cr
 \mapdownk \ev_{(X\otimes T)} & & \mapdownd \ev_Y &\cr
  X\otimes T & \maprightap f & Y &\cr
    &  & & \hskip -15pt \nearrow\hfill  \cr       }$$
\vskip\tarpas
We have the commuting quadrat in the category of sets $\SET$ for the
secondary projection, also we have commuting quadrat for the
primary projection.  It rests to check the continuous diagram for the
edges set mappings.

We get the continuous  quadrat only for the diagram  begun with
sections mappings and with lower decomposable $\VV$-graphs transport
$f: X\otimes T\doublerightarrow Y$.

For a set of transforms between two sections
$$\Prod_{s\in T_0} (X(a;b)\otimes 1_s(*)) \subset
(X\otimes T)^T(\lambda_X(a);\lambda_X(b)) $$
 the first evaluation $\ev_{(X\otimes T)}$  will be defined with
  the contact arrows mapping
$$(X(a;b)\otimes 1_s(*)) \circ ( 1_b(*)\otimes T(s;t))=
X(a;b)\otimes T(s;t)\subset (X\otimes T) (\lan a,s\ran;\lan b,t\ran) $$
and taken  $\VV$-graphs transport
$f: X\times T\doublerightarrow Y$ will appoint
the edges set
$$ f_{\lan a,s\ran;\lan b,t\ran} (X(a;b)\otimes T(s;t))\subset
Y(f(a,s);f(b,t))\tsk$$                      
The changing of the target space with $\VV$-graphs transport
$f:X\otimes T\doublerightarrow Y$ for a set of transforms
between sections
$$\Prod_{s\in T_0} (X(a;b)\otimes 1_s(*)) \subset (X\otimes T)^T (
T\lambda_X(a);\lambda_X(b))$$
will appoint the set of transforms between changed sections
$$\Prod_{s\in T_0} f_{\lan a,s\ran,\lan b,t\ran }
(X(a;b)\otimes 1_s(*))\subset
Y^T(\lambda_X(a)\circ f;\lambda_X(b) \circ f )\kbl$$
so for the $\VV$-graphs transport $f$
with lower decomposition
the evaluation transport for a biproduct  of such set of transforms with
the same edges set in assistant graph $T(s;t)$
will appoint the smaller contact arrows mapping
$$f_{\lan a,s\ran,\lan b,s\ran } (X(a;b)\otimes 1_s(*))\circ
f_{\lan b,s\ran,\lan b,t\ran} (1_b(*)\otimes T(s,;t))\mzl  $$$$
f_{\lan a,s\ran,\lan b,t\ran } (X(a;b)\otimes T(s;t))
\subset Y(f(a,s); f(b,t))\tsk$$

Next we shall check that a name  of realization is also
 decreasing $g(f_+(g))\dgl g $.
For it we construct another cocontinuous diagram
$$\matrix { \swarrow \hskip -10pt  & & & & &\cr
& Y^T & \mapleft (\ev_Y)^T & (Y^T\times T)^T  &
\mapleft  (g\otimes 1_T)^T  & (X\otimes T)^T \cr
&&\nwarrow  & \mapupd \lambda_{Y^T}  & & \mapupd \lambda_X  \cr
&& &Y^T & \mapleftap g &X \cr} $$
\vskip\tarpas
In the $\VV$-graph $Y$ we have chosen contact
arrow  mappings
$$ Y(c;d)\otimes Y(d;e)\rightarrow Y(c;d)\circ Y(d;e)\subset Y(c;e)\tsk$$
but for the sections transport $\lambda_{Y^T}: Y^T \doublerightarrow
(Y^T\otimes T )^T\otimes T $ we have to choose the unit arrows in
exponential  graph $Y^T$. It will be defined with chosen
unit arrows mappings in $\VV$-graph $X$ composed
with arrows sets mappings of taken $V$-graphs
transport $g:X\doublerightarrow Y^T$
$$g_{a,a} (1_a(*))\subset Y^T (g_0(a);g_0(a))\tsk$$
We shall check the second triangular equality
$$ Y^T \mapright \lambda_{Y^T} (Y^T\otimes T)^T
\mapright (\ev_Y)^T Y^T \dgl \Identity_{Y^T} \tsk$$
begun with taken
$\VV$-graphs transport $g: X\doublerightarrow Y^T $ which is upper neutral
to chosen unit arrows mappings in source $V$-graph $X$

$$X(a;b)\rightarrow g_{a,b}(X(a;b))_s \circ g_0(b)_{s,s}(1_s(*)) \dgl$$$$
g_{a,b} (X(a;b))_s \subset Y(g_0(a)_s;g_0(b)_s) \kbl$$
$$T(s;t)\rightarrow g_{a,a}(1_a(*) )\circ g_0(a)_{s,t} (T(s;t))\dgl $$$$
g_0(a)_{s,t}(T(s;t)) \subset Y(g_0(a)_s;g_0(a)_t) \tsk$$

At first we shall check the second triangular equality
in the category of sets $\SET$
for the set of all $\VV$-graphs transports
$(Y^T)_0= \lbrace \phi: T\doublerightarrow  Y\rbrace $
$$(Y^T)_0\mapright (\lambda_{(Y^T)})_0 ((Y^T \times T)^T)_0 \mapright
(\ev_{Y^T}^T)_0  (Y^T)_0 $$
begun with the projection  of taken graphs transport
%negadina projection in Set
$g_0: X_0 \rightarrow (Y^T)_0 $.
It for a $\VV$-graphs transport $\phi:T\doublerightarrow Y$ appoint
the section
$$\lambda_{Y^T}(\phi): T\doublerightarrow Y^T\times T \tsk$$
We can apply the secondary projection  to get a new triangular equality
for the same $\VV$-graphs transport $\phi: T\doublerightarrow Y$, but
with  a new sections appointment in the category of sets $\SET$
$$(Y^T)_0\mapright \lambda_{(Y^T)_0} ((Y^T)_0 \times T_0)^{T_0} \mapright
\ev_{(Y^T)_0}^{T_0}  (Y^T)_0 \tsk$$
It for a $\VV$-graphs transport $\phi: T\doublerightarrow Y$ will appoint
the section in the category of sets
$$\lambda_{(Y^T)_0}(\phi): T_0\rightarrow (Y^T)_0\times T_0 $$
which for a vertex
$t\in T_0$ appoints the couple
$\lan \phi, t\ran \in (Y^T)_0\times T_0$.
This new triangular equality will provide
the triangular
equality also for the primary projection, as evaluation
allows such secondary
projection.

Indeed for a set of all mappings $\phi: T_0\rightarrow Y_0$ we have  already
checked the  second triangular equality
$$(Y_0)^{T_0}\mapright  \lambda_{(Y_0)^{T_0}} ((Y_0)^{T_0}\times T_0)^{T_0}
\mapright \ev_{(Y_0)}^{T_0}  (Y_0)^{T_0}\tsk$$
The first appointment will be sections
appointment with arbitrary appointment $\phi: T_0\rightarrow Y_0$
$$\lambda_{(Y_0)^{T_0}}:T_0\rightarrow (Y_0)^{T_0} \times T_0 \tsk$$
So it will be valid also for imbedded smaller set
$(Y^T)_0\subset (Y_0)^{T_0}$ of all appointments get from
$\VV$-graphs transforms
$\phi: T\doublerightarrow Y$.

For a $\VV$-graphs transport $g_0(a): T\doublerightarrow Y$ we need else
to check the  inequality  for  the edges set mappings.
An  edges set  $T(s;t)$ will be mapped  by such
 graphs transports to the edges set
$$g_0(a)_{s,t} (T(s;t)) \subset Y(
g_0(a)_s; g_0(a)_t)\tsk$$
The sections transport for such graphs transport will appoint a section
$$\lambda_{Y^T} (g_0(a)): T\doublerightarrow Y^T\otimes T $$
which  for an edges set  $T(s;t)$ appoints
the biproduct
$$g_{a,a}(1_a(*))\otimes T(s;t)\subset
Y^T\otimes T(\lan g_0(a),s\ran;\lan g_0(a),t\ran )\tsk$$

The changing of target space with evaluation transport is
 defined with precontact
  arrows mapping which
 for such biproduct  will appoint the composition
$$g_{a,a}(1_a(*))_s\circ g_0(a)_{s,t} (T(s;t))\dgl  g_{s,t}(T(s;t)\subset
Y(g_0(a)_s;g_0(a)_t)
\tsk$$
So for an edges set $T(s;t)$ we get decreasing mapping.

Finally we need to check the second triangular equality for the
edges set mappings. Also we must begin with edges set mappings for
taken $\VV$-graphs transport $g: X\doublerightarrow Y^T$. They for an
edges set
$X(a;b)$ appoints the set of transforms between two graphs transports
$$ g_{a,b} (X(a;b))\subset  Y^T (g_0(a); g_0(b))\tsk$$
For such set of transforms we get the set of transforms between sections
as a product
$$\Prod_{s\in T_0} (g_{a,b} (X(a;b))\otimes 1_s(*))\subset (Y^T\otimes T)^T(
\lambda_{Y^T}(g_0(a)); \lambda_{Y^T}(g_0(b)))\tsk$$
The changing of target space with  evaluation transport
$\ev_Y: Y^T\otimes T \doublerightarrow Y$
will appoint the set of precontact arrows
$$g_{a,b}(X(a;b))_s \circ g_0(b)_{s,s} (1_s(*)) \dgl g_{a,b} (X(a;b))
\subset Y(g_0(a)_s;g_0(b)_s) \tsk$$
So we get decreasing mapping for the edges set $X(a;b)$ again.

We have shown the second triangular inequality begun with taken
$\VV$-graphs transport
$g: X\doublerightarrow Y^T$.

Now we shall check the commuting quadrat
between defined sections transports
$$ \matrix { (Y^T\otimes T)^T  &
\mapleft (g\otimes 1_T)^T & (X\otimes T)^T \cr
 \mapupk \lambda_{Y^T} &   & \mapupd \lambda_X \cr
 Y^T & \mapleftap g & X\cr } $$
\vskip\tarpas
This quadrat is commuting for the projection in the category $\SET$.
For a vertex $a\in X$ we appoint the $\VV$-graphs transport $g_0(a)\in Y^T$
which provides the section
$\lambda_{Y^T}(g_0(a)): T\doublerightarrow Y^T\otimes T$
 which for a vertex  $s\in T_0$ appoints the couple
 $\lan g_a(a), s\ran$ with  edges set mappings
$$\lambda_{Y^T}(g_0(a))_{s,t}=g_{a,a}(1_a(*)\otimes \Identity_{T(s;t)}
 :T(s;t)\rightarrow g_{a,a} (1_a(*))\otimes T(s;t)
 \subset $$$$Y^T(g_0(a);g_0(a))\otimes T(s;t)\tsk$$

The same section is get from the
section $\lambda_X(a): T\doublerightarrow X\otimes T$
by changing of target space with
$\VV$-graphs transport $g\otimes \Identity_T: X\otimes T\doublerightarrow
Y^T\otimes T $.
It for a couple of vertexes $\lan a,s\ran \in X_0\times T_0$ appoints the
couple $\lan g_0(a),s\ran \in (Y^T)_0\times T_0$, and the edges set mappings
$$g_{a,a}(1_a(*))\otimes \Identity _{T(s;t)} : T(s;t)\rightarrow
g_{a,a}(1_a(*)) \otimes T(s,t) \subset
$$$$Y^T(g_0(a);g_0(a))\otimes T(s;t)\tsk$$

 For an edges set $X(a;b)$ taken $\VV$-graphs transport
$g: X\doublerightarrow Y^T$ appoints the set of transforms  between
two $\VV$-graphs transports
$$g_{a,b} (X(a;b)) \subset Y^T(g_0(a);g_0(b))$$
which is mapped by sections
transport $\lambda_{Y^T}: Y^T\doublerightarrow (T^T\otimes T)^T $
to the set of transforms between two sections
$$ \Prod_{s\in T_0} g_{a,b} ((X(a;b)) \otimes 1_s(*) \subset
(Y^T\otimes T)^T (\lambda_{Y^T}(g_0(a)); \lambda_{Y^T} (g_0(b)))\tsk$$
The same set of transform between two sections is provided
from the set of transforms
$$\Prod_{s\in T_0} X(a;b)\otimes 1_s(*)\subset
X^T(\lambda_X(a);\lambda_X(b)) $$ 
by changing of
target space with
$\VV$-graphs transport
$g\otimes \Identity_T: X\times T \doublerightarrow Y^T\otimes T$.
For an edges set $$X(a;b)\otimes 1_s(*) \subset X(a;b)\otimes T(s;s)$$
it appoints the edges set
$$g_{a,b} (X(a;b))\otimes 1_s(*)\subset Y^T(g_0(a);g_0(b))\otimes T(s;s)$$
for every vertex $s\in T$.

We have got that the  $\VV$-graphs transports $f\in \Grph (X\times T; Y)$
with lower decomposition  for chosen  contact arrows mappings in the
target graph $Y$
are ^{lower =reversing} its  name and the
$\VV$-graphs transports $g\in \Grph(X;Y^T)$
with upper neutral property for chosen unity arrow mappings in the
source $\VV$-graph  $X$ and the assistant $\VV$-graph  $T$ are ^{upper
=reversing} its realization.
For couple of composable graphs transforms $\lan f,g\ran$
with both properties together  we have get a truly joint pair of
monotone name appointment and monotone realization appointment.

\irodymopabaiga
We shall notice that in the case of decomposition equality
$$X(a;b)\otimes T(s;t) \rightarrow
f_{\lan a,s\ran,\lan b,s\ran } (X(a;b)\otimes 1_s(*) ) \circ
f_{\lan y,s\ran,\lan y,t\ran} (1_b(*) \otimes T(s;t))=  $$$$
f_{\lan x,s\ran,\lan b,t\ran} (X(a;b)\otimes T(s;t))\subset
Y(f(a,s); f(b,t))$$
we  shall get reversing the realization mapping
$$f= f_+(g(f))\tsk$$
In the case of neutral equalities
$$ X(a;b)\rightarrow g_{a,b}(X(a;b))_s
 \circ g(b)_{s,s}(1_s(*)) = $$$$
 g_{a,b} (X(a;b))_s  \subset Y(g(a)_s;g(b)_s) \kbl$$
$$T(s;t)\rightarrow g_{a,a}(1_a(*) )
\circ g(a)_{s,t} (T(s;t)) = $$$$
g(a)_{s,t}(T(s;t)) \subset Y(g(a)_s;g(a)_t)$$
we shall get reversing property for the name appointment
$$g(f_+(g))= g \tsk$$

We also want  for $\VV$-enriched graphs to define the notion of the set
 of natural transforms. However for the values category
$\VV$ with ordered edges sets more convenient  to work with
the set of continuous transforms.

 In the exponential space of all $\VV$-graphs transports $Y^T$
 we take the inverse image of order relation
 $(\dgl) \subset \VV(r;s)\times \VV(r;s) $
 for the names of two   mappings
 provided by preevaluation and postevaluation transports
$$Y^T(\phi;\psi) \otimes T(s;t) \rightarrow Y(\phi_0(s);\psi_0(s))\circ
\psi_{s,t}(T(s;t))\subset Y(\phi_0(s);\psi_0(t))\kbl$$
$$Y^T(\phi;\psi) \otimes T(s;t) \rightarrow \phi_{s,t} (T(s;t)) \circ
Y(\phi_0(s);\psi_0(s))\subset Y(\phi_0(s);\psi_0(t))\tsk$$
So we get the inverse image
$$\rightarrow Y^{(T)}_+(\phi;\psi) \rightarrow Y^T (\phi;\psi)
\tworightarrows \Prod_{s,t\in T_0} Y(\phi_0(s);\psi_0(t))^{T(s;t)}\tsk$$
For the first precontact evaluation  we get the set of cocontinuous
transforms $Y^{(T)}_+(\phi;\psi)$
$$\matrix{ \phi_0(a) & \mapright \alpha_a & \psi_0(a) &\cr
\downarrow & (+13) & \downarrow &     \cr
\phi_0(b) & \maprightap \alpha_b & \psi_0(b) & \cr
& & & \hskip -10 pt \swarrow \hfill \cr}$$
\vskip\tarpas
The sign $(+)$  must denote  the
property of deformed quadrat $(+13)$ for ^{wasting =reforms}

Otherwise for the first postcontact evaluation we shall get
the set of continuous transforms  $Y^{(T)}_-(\phi;\psi)$
$$\matrix{ \phi_0(a) & \mapright \alpha_a & \psi_0(a) &\cr
\downarrow & (+13) & \downarrow &     \cr
\phi_0(b) & \maprightap \alpha_b & \psi_0(b) & \cr
& & & \hskip -10 pt \nearrow \hfill \cr}$$
\vskip\tarpas
The sign $(-)$ must denote the property of deformed quadrat $(-13)$
for ^{respecting =reforms},
At this moment we can't to talk about new superfunctors of exponential
spaces  $Y^{(T)}_-$ or $Y^{(T)}_+$.

We repeat the proposition when the name of $\VV$-graphs transport
 can be corestricted in the new exponential
space of continuous transforms.


\Proposition
The choosing of unit arrow mappings in the source $\VV$-graph
$1_a(*)\subset X(a;a)$ and in the assistant $\VV$-graph $1_s(*)\subset T(s;s) $
allows us to define the name appointment between the sets of $\VV$-graphs
transports
$$\Grph_{\VV} (X\otimes T;Y) \rightarrow \Grph_{\VV}(X;Y^T) \tsk$$
For a  contact arrows mapping in the target $\VV$-graph $Y$
$$Y(c;d)\otimes Y(d;e) \rightarrow Y(c;d)\circ Y(d;c) \subset Y(c;e) $$
the choosing of evaluation transport defined with precontact or
postcontact arrows mappings allows us to define the prerealization
or postrealization appointments
$$\Grph_{\VV}(X;Y^T) \rightarrow \Grph_{\VV}(X\otimes T; Y) \tsk$$

The name  of $\VV$-graphs transport $f: X\otimes T \doublerightarrow Y$  which
has upper predecomposition  and lower postdecomposition  for the
contact arrows
mapping in the target $\VV$-graph  $Y$
$$f_{\lan a,s\ran,\lan b, s\ran } (X(a;b) \otimes 1_s((*)) \circ
f_{\lan b, s\ran,\lan b,t\ran} (1_b(*)\otimes T(s;t))
\dgl  $$$$
 f_{\lan a,s\ran, \lan b,t\ran} (X(a;b)\otimes T(s;t))\dgl $$$$
f_{\lan a,s\ran,\lan a,t\ran} (1_a(*)\otimes T(s;t)) \circ
f_{\lan a, t\ran,\lan b,t\ran} (X(a;b)\otimes 1_t(*)) $$
is corestricted in exponential $\VV$-graphs  of continuous transforms
$Y^{(T)}_- $.
\Proof:

We want  to check  for the  name appointment
the inclusion in inverse image of order relation
$$g_{a,b} X(a;b) \rightarrow Y^T(g_0(a); g_0(b))\tworightarrows
 \Prod_{s,t\in T_0} Y(g_0(a)_s; g_0(b)_t)^{T(s;t)} \tsk$$
provided by preevaluation and postevaluation transports

$$X\otimes T \mapright {\lambda_X\otimes 1_T} (X\otimes T)^T \otimes T
\mapright f^T\otimes 1_T Y^T \otimes T \mapright \ev^\pm_Y  Y $$

Using the cocontinuous  diagram for the preevaluation  transport
$$\matrix { X\otimes T & \mapright \lambda_X\otimes 1_T  &
 (X\otimes T)^T \otimes T  & \mapright f^T\otimes 1_T & Y^T \otimes T  &\cr
%
&\searrow &\mapdownd \ev^+_{(X\otimes T)}  & &\mapdownd \ev^+_Y & \cr
%
& &X\otimes T  & \maprightap f &  Y &\cr
&    &         &     &  &\hskip -15pt \swarrow \hfill\cr}$$
\vskip \tarpas
and the continuous diagram for the postevaluation transport

$$\matrix { X\otimes T & \mapright \lambda_X\otimes 1_T  &
 (X\otimes T)^T \otimes T  & \mapright f^T\otimes 1_T & Y^T \otimes T  &\cr
%
&\searrow &\mapdownd \ev^-_{(X\otimes T)}  & &\mapdownd \ev^-_Y & \cr
%
& &X\otimes T  & \maprightap f &  Y &\cr
&    &         &     &  &\hskip -15pt \nearrow \hfill\cr}$$
\vskip \tarpas

allows us to check  the ^{=corestriction}  of name
$$g: X\mapright \lambda_X (X\otimes T)^T \mapright f^T  Y^T$$
in exponential space of continuous  transforms  $ Y^{(T)}_-$.

This can be proved by contact arrows mappings
$$\matrix {f_0( a,s) &
 \rightarrow  &  f_0(a,t)& \cr
  \downarrow  &\searrow &  \downarrow & \cr
          f_0(b, s) & \rightarrow  &  f_0(b, t ) &\hskip-5pt  \nearrow \hfill\cr
& &\hfill \nearrow \hskip  -5pt & \cr  }$$
\vskip\tarpas
Such contact arrow is provided by
$$f_{\lan a,s\ran,\lan b,t\ran }(X(a;b)\otimes T(s;t) ): f_0(a,s)
\rightarrow f_0(b,t)$$
from continuous  diagrams drown for both evaluation transports $\ev^\pm_Y$
$$f_{\lan a,s\ran,\lan b, s\ran } (X(a;b) \otimes 1_s((*)) \circ
f_{\lan b, s\ran,\lan b,t\ran} (1_b(*)\otimes T(s;t))
\dgl  $$$$
 f_{\lan a,s\ran, \lan b,t\ran} (X(a;b)\otimes T(s;t))\dgl $$$$
f_{\lan a,s\ran,\lan a,t\ran} (1_a(*)\otimes T(s;t)) \circ
f_{\lan a, t\ran,\lan b,t\ran} (X(a;b)\otimes 1_t(*)) \kbl$$
 i. e.
we have inequalities  for the precontact and the postcontact arrows

\irodymopabaiga
We can also notice that in the case of equalities
$$f_{\lan a,s\ran,\lan b, s\ran } (X(a;b) \otimes 1_s((*)) \circ
f_{\lan b, s\ran,\lan b,t\ran} (1_b(*)\otimes T(s;t))
= $$$$
 f_{\lan a,s\ran, \lan b,t\ran} (X(a;b)\otimes T(s;t))=$$$$
f_{\lan a,s\ran,\lan a,t\ran} (1_a(*)\otimes T(s;t)) \circ
f_{\lan a, t\ran,\lan b,t\ran} (X(a;b)\otimes 1_t(*)) $$
we get a name appointment  corestricted in the exponential space of natural
transforms  $Y^{(T)}$.
\vskip\tarpas

We again shall define the ^{=category of original $\VV$-graphs}
$\OGrph_{\VV}$.
For the original $\VV$-graph we demand
the  unit arrow mappings
$e_a(*)\subset  X(a;a) $.
The ^{original $\VV$-graphs =transport} $f: X\doublerightarrow Y$ must maintain
chosen unit arrow mappings
$$f_{a,a} (e_a(*))= e_{f_0(a)}(*) \tsk$$
We shall call them also as ^{crude =functors}.
Such category will be denoted $\OGrph_{\VV} $.

For  contact arrows mappings
$$X(a;b)\otimes X(b;c)\rightarrow
 X(a;b)\circ X(b;c)\subset X(a;c)$$
we demand neutral equalities
$$e_a(*)\circ X(a;b) = X(a;b)= X(a;b)\circ 1_b(*)\tsk$$
The original
$\VV$-graphs transport $f: X\doublerightarrow Y$
will be called continuous  if we additionally have continuous
diagram  for chosen contact arrows mappings
$$\matrix{
X(a;b) \otimes X(b;c) & \mapright f_{a,b}\otimes f_{b,c} &
Y(f_0(a);f_0(b)) \otimes Y(f_0(b);f_0(c)) & \cr
\mapdownk {\circ} & &\mapdownd {\circ} & \cr
X(a;c) & \maprightap f_{a,c} & Y(f_0(a); f_0(c)) & \cr
  &        &  &\hskip-25pt \nearrow \hfill \cr} $$
\vskip \tarpas
The ^{continuous original $\VV$-graphs =transports}  will be also called
^{continuous =functors}. The category of continuous
original $\VV$-graphs transports  will be denoted
$\OGrph_{\VV}^-$.

Correspondingly we define ^{cocontinuous =functors} and the category
of cocontinuous original $\VV$-graphs transports will be denoted
$\OGrph^+_{\VV}$. ^{natural  =functors} are defined as transports of
original $\VV$-graphs transports maintaining contact arrows mappings.
Their category will be denoted $\OGrph^=_{\VV}$. They are usually considered
as functors in $\VV$-enriched categories.

\vskip\tarpas
A biproduct of original $V$-graphs $X\otimes Y$ provides the
superfunctor also
in the category of original $V$-graphs $\OGrph_V$.
The unit arrow mapping is defined by the biproduct of unit arrow mappings
$$1_{\lan x,t\ran} (*) = 1_x(*)\otimes 1_s(*)\subset X\otimes T(\lan x,s\ran;
\lan x,s\ran) \tsk$$

For the choosing of contact arrows mappings we need additionally to demand
a mapping in the values category $\VV$
$$m_{\lan p,s\ran,\lan r,t\ran } :(p\otimes s)\otimes (r\otimes t) \rightarrow (p\otimes r) \otimes
(s\otimes t) \tsk$$
We can say that such biproduct  $p\otimes r$ is a ^{=relator to itself}.
Usually such arrow is provided for associative and commuting tensor product.
We shall call it a ^{=relator's involution}. Such arrows are inverse to
their selves, therefore they define isomorphic transform.

The choosing of contact arrows mappings in the
biproduct graph $X\otimes Y$ is defined
with the biproduct of contact arrows mappings.
Let we have the contact arrows mappings
$$X_{a,b,c}: X(a;b)\otimes X(b;c)\rightarrow X(a;b)\circ X(b;c) \subset X(a;c)\kbl $$
$$Y_{a',b',c'}: Y(a';b')\otimes Y(b';c')\rightarrow Y(a';b')\circ Y(b';c') \subset
Y(a';c') \tsk $$
Then in the biproduct $X\otimes Y$ we can define the contact arrows mappings
$$(X\otimes Y(\lan a,a'\ran;\lan b,b'\ran))\otimes
(X\otimes Y(\lan b,b'\ran; \lan c, c'\ran )) = $$$$
(X(a;b)\otimes Y(a';b'))\otimes (X(b;c)\otimes Y(b';c'))
\rightarrow  $$$$
(X(a;b)\otimes X(b;c))\otimes (Y(a';b')\otimes Y(b';c')) \rightarrow   $$$$
(X(a;b)\circ X(b;c))\otimes (Y(a';b')\circ Y(b';c')) \subset $$$$
X(a;c)\otimes Y(a';c')= X\otimes Y(\lan a,a'\ran ;\lan c,c'\ran)\tsk$$

We need to check that chosen unit arrows mappings
$$1_a(*)\otimes 1_{a'}(*)\subset X(a;a)\otimes Y(a';a')$$
are neutral for such defined arrows mappings.
First we have an  equality
$$(1_a(*)\otimes 1_{a'}(*))\otimes (X(a;b)\otimes Y(a';b'))\rightarrow $$$$
(1_a(*)\otimes X(a;b))\otimes (1_{a'}(*)\otimes Y(a';b')\rightarrow $$$$
(1_a(*)\circ X(a;b) )\otimes (1_{a'}(*)\circ Y(a';b'))=
X(a;b)\otimes Y(a';')\tsk$$
In the same way we can check another equality
$$(X(a;b)\otimes Y(a';b') )\circ (1_a(*)\otimes 1_{a'}(*))= X(a;b)\otimes
Y(a'; b')\tsk$$

The biproduct with an  assistant original $\VV$-graph $T$ defines
superfunctor in various categories  of original $\VV$-graphs.
For an  original $\VV$-graph $X$ it appoints the biproduct
$X\otimes T$, and for an original $\VV$-graphs  transport
$g: X\doublerightarrow Y$ it appoints the biproduct with the identity
transport of assistant  $\VV$-graph
$$g\otimes \Identity_T: X\otimes T\doublerightarrow Y\otimes T\tsk$$
For a  general original $\VV$-graphs  transport  we need to check only
maintenance of unit arrow mappings.
For the original $\VV$-graphs transport $g: X\doublerightarrow Y$
we  shall have maintained the unit arrow mappings
$$g_{a,a} (1_a(*))= 1_{g_0(a)} \subset Y(g_0(a);g_0(a))\tsk$$
So the unit arrow mappings in the biproduct
$$1_a(*)\otimes 1_s(*) \subset X(a;a)\otimes T(s;s)$$
will be mapped to the unit arrow mapping in another  biproduct
$$(g\otimes \Identity_T)_{\lan a,s\ran,\lan a,s\ran}
(1_a\otimes 1_s)= g_{a,a} (1_a(*))\otimes 1_s(*)= 1_{g_0(a)}(*)\otimes 1_s(*)
\subset $$$$ Y(g_0(a);g_0(a))\otimes T(s;s)\tsk$$

For the continuous   original $\VV$-graphs transforms
$g: X\doublerightarrow Y$
$$\matrix{ X(a;b)\otimes X(b;c) & \mapright g_{a,b}\otimes g_{b,c} &
Y(g_0(a);g_0(b))\otimes Y(g_0(b);g_0(c)) & \cr
\mapdownk {\circ } & & \mapdownd {\circ} & \cr
X(a;c) & \maprightap g_{a,c} & Y(g_0(a);g_0(c)) & \cr
      &      &   & \hskip -25pt  \nearrow \hfill \cr}$$
\vskip\tarpas
we need to ask
that chosen  arrows $m_{\lan p,s\ran,\lan r,t\ran} $
would define cocontinuous transform for every argument
changing
$p\rightarrow p'$, $r\rightarrow r'$, $ s\rightarrow s'$, $t\rightarrow t'$,
for example we have cocontinuous quadrats
$$\matrix{  (p\otimes s)\otimes (r\otimes t ) &
\mapright m_{\lan p,s\ran,\lan r,t\ran}  &
(p\otimes r) \otimes (s\otimes t) &\cr
\downarrow &  &  \downarrow & \cr
(p'\otimes s)\otimes (r\otimes t ) &
\maprightap m_{\lan p',s\ran,\lan r,t\ran}  &
(p'\otimes r) \otimes (s\otimes t) &\cr
         & & &\hskip -5pt  \swarrow \cr}$$
\vskip\tarpas
Then the appointed biproduct
$g\otimes \Identity_T: X\otimes T\doublerightarrow Y\otimes T$
rests continuous for defined contact arrows mappings.
The proving is produced gradually by each argument.
First we shall check for the composition in the first space.
We have the cocontinuous diagrams in the values category $\VV$
$$\matrix {
(X(a;b)\otimes T(s;t) ) \otimes (X(b;c)\otimes T(t;v)) &
\mapright m_{X,T} \cr
\mapdownk (g_{a,b}\otimes 1_{T(s;t)})\otimes (g_{b,c}\otimes 1_{T(t;v)}) & \cr
(Y(g_0(a);g_0(b))\otimes (T(s;t)) \otimes Y(g_0(b);g_0(c))\otimes T(t;v)) &
\maprightap m_{Y',T}  \cr}$$
\vskip \tarpas

$$\matrix{
\rightarrow & (X(a;b)\otimes X(b;c))\otimes (T(s;t)\otimes T(t;v)) & &
\mapright {\circ} \cr
&\mapdownk (g_{a,b}\otimes g_{b,c})\otimes (1_{T(s;t)}\otimes 1_{T(t;v)}) &
&  &\cr
\rightarrow &
(Y(g_0(a);g_0(b))\otimes Y(g_0(b);g_0(c)))\otimes (T(s;t)\otimes T(t;v)) & &
\maprightap {\circ } \cr
&  & \swarrow  & \cr }$$
\vskip\tarpas

$$\matrix{
\rightarrow & X(a;c)\otimes (T(s;t)\otimes T(t;v)) & &\mapright {\circ} &
X(a;c)\otimes T(s;v) & \cr
&\mapdownk 1_{X(a;c)}\otimes (1_{T(s;t)}\otimes 1_{(T(t;v)}) & &  &
\mapdownd (1_{X(a;c)}\otimes 1_{T(s;v)}  & \cr
\rightarrow & X(a;c)\otimes (T(s;t)\otimes T(t;v)) &  &
\maprightap {\circ} & X(a;c)\otimes T(s;v)) & \cr
& & \hskip -10pt\swarrow  \hfill & & &\hskip-10pt \swarrow \hfill \cr }$$
\vskip\tarpas

In the values category the arrows composition is associative, therefore we can
compose these three cocontinuous  diagrams, and we get the continuous
diagram
for  the arrows set mappings of $\VV$-graphs transport
 $g: X\doublerightarrow Y$
$$\matrix {(X(a;b)\otimes T(s;t))\otimes (X(b;c)\otimes T(t;v)) &
\mapright (g_{a,b}\otimes 1_{T(s;t)})\otimes (g_{b,c}\otimes (1_{ T(s;v))})
\cr
\downarrow  & \cr
X(a;c)\otimes T(s,v)  & \maprightap g_{a,c}\otimes 1_{T(s;v)} \cr}$$
 \vskip\tarpas

$$\matrix{ \rightarrow & (Y(g_0(a);g_0(b))\otimes T(s;t))\otimes (
Y(g_0(b); g_0(c))\otimes T(t;v)) & \cr
 & \downarrow & \cr
\rightarrow & Y(g_0(a);g_0(c)) & \cr
 &  & \hskip -25 pt \nearrow \hfill \cr}$$
\vskip\tarpas
We remark that in the category $\OGrph_{\VV}^=$ compounded by
^{natural  =functors} between  original
$\VV$-graphs
 we need to ask that arrows $m_{\lan p,s\ran,\lan r,t\ran} $
would define a natural transform.

The ^{ exponential =space} $Y^T$
in the category of original $\VV$-graphs $\OGrph_{\VV}$
will be defined by the vertex set compounded by all
original $\VV$-graphs transports $\phi: T\doublerightarrow Y$, i. e.
these $\VV$-graphs
transports must maintain
unit arrow mappings.
However in a smaller category of continuous $\VV$-graphs transports
$\OGrph_{\VV}^-$
we shall take only continuous  original $\VV$-graphs  transports
$\phi: T\doublerightarrow Y$. Their set will be denoted
$Y^{T-}$. Also we define the set of cocontinuous original $\VV$-graphs
transports $Y^{T+}$ in the category $\OGrph_{\VV}^+$, or the set of
original $\VV$-graphs  natural transports which
maintain contact arrows mappings
 $Y^{T=} $ in the category $\OGrph_{\VV}^=$.

The edges sets in exponential space of crude functors will be taken
 the same as in the category $\Grph_{\VV}$ compounded  of all transforms
$$Y^T(\phi;\psi)= \Prod_{s\in T_0} Y(\phi_0(s);\psi_0(s))\tsk$$
We shall demand that biproduct in values category $\VV$ would maintain
such product
$$\Prod_{s\in T_0}(p_s\otimes r_s)=( \Prod_{s\in T_0} p_s )\otimes
(\Prod_{s\in T_0} r_s) \tsk$$

The unit arrow mappings in exponential space are provided  by the transform
defined with a product of unit arrow mappings in the target $\VV$-graph
$$1_\phi(*) = \Prod_{s\in T_0} 1_{\phi_0(s)} (*)
\subset
\Prod_{s\in T_0} Y(\phi_0(s);\phi_0(s))\tsk$$
The contact arrows mappings also are defined by a product of such mappings
in the target $\VV$-graph $Y$
$$Y^T(\phi;\psi)\otimes Y^T(\psi;\xi)\rightarrow (\Prod_{s\in T_0}
Y(\phi_0(s);\psi_0(s))) \circ (\Prod_{s\in T_0}
 Y(\psi_0(s);\xi_0(s)))= $$$$
 \Prod_{s\in T_0} (Y(\phi_0(s);\Psi_0(s))\circ Y(\Psi_0(s);\xi_0(s)))\subset
 \Prod_{s\in T_0} Y(\phi_0(s);\xi_0(s))\tsk$$
Easy to check that chosen unit arrow mappings are neutral for such
contact arrows mappings
 $$1_\phi(*)\circ Y^T(\phi;\psi)= \Prod_{s\in T_0} 1_{\phi_0(s)} \circ
Y(\phi_0(s);\psi_0(s))= $$$$
\Prod_{s\in T_0} Y(\phi_0(s);\psi_0(s))=
Y^T(\phi;\psi)\tsk$$
In the same way we can check another equality
$$Y^T(\phi;\psi)\circ 1_{\psi}(*) = Y^T(\phi;\psi) \tsk$$

The exponential space will define superfunctors in correspondent categories.
For a $\VV$-graphs transport $g: Y\doublerightarrow Y'$ we take
the changing of target space $f^T: Y^T\doublerightarrow (Y')^T $.
For each $\VV$-graph transport $\phi: T\doublerightarrow Y$ we get the  new
 $\VV$-graphs transport $\phi\circ g : T\doublerightarrow Y'$.
 Such composition of $\VV$-graphs transport rests in correspondent
 categories. For example for the continuous  original $\VV$-graphs
 transport $\phi: T\doublerightarrow Y$ we get
 again a continuous   original $\VV$-graphs transport
 $\phi\circ g: T\doublerightarrow Y'$.

The edges set mappings are defined in old way
$$Y^T(\phi;\psi) \rightarrow \Prod_{s\in T_0} g_{\phi_0(s),\psi_0(s)}
(Y(\phi_0(s);\psi_0(s)))  \subset $$$$
\Prod_{s\in T_0} Y'(g_0(\phi_0(s));g_0(\psi_0(s))) =
 (Y')^T (\phi\circ g;\psi\circ g)\tsk$$

Finally we shall check that continuous $\VV$-graphs transports
$f: X\doublerightarrow Y$
provides continuous
changing of target space  $f^T: X^T \doublerightarrow Y^T$.
Let we have continuous quadrat
$$\matrix{ X(x;y)\otimes X(y;z) & \mapright f_{x,y}\otimes f_{y,z} &
 Y(f_0(x);f_0(y))\otimes Y(f_0(y);f_0(z)) &\cr
 \mapdownk {\circ} & & \mapdownd {\circ} &\cr
 X(x;z) & \maprightap f  & Y(f_0(x);f_0(z)) & \cr
 & & &\hskip -10pt \nearrow\hfill \cr}$$
 \vskip\tarpas
Then for the changing of target space we get again the continuous quadrat

$$\matrix{ X^T(\phi;\psi) \otimes X^T(\psi;\xi) &
\mapright f^T_{\phi;\psi}\otimes f^T_{\psi;\xi} &
 Y^T (\phi\circ f, \psi\circ f) \circ Y^T(\psi\circ f; \xi\circ f) \cr
 \mapdownk {\circ} & & \mapdownd {\circ} &\cr
Y^T(\phi\circ f;\xi\circ f) & \maprightap f^T  & Y^T (\phi\circ f;\xi\circ f )
& \cr
 & & &\hskip -10pt \nearrow \hfill \cr}$$
 \vskip\tarpas
The needed inequality is checked for each component with $s\in T_0$.
We apply the first quadrat for the vertexes
$x=\phi_0(s) $, $y= \phi_0(s) $ and $z=\xi_0(s)$.

We have got a joint pair of superfunctors defined by biproduct
$X\otimes T$ and
exponential space $Y^T$ in correspondent categories.
For such joint pair of superfunctors we can construct
the unit transform defined with collection of sections transports
$$\lambda_X: X\doublerightarrow (X\otimes T)^T \tsk$$
We need only to check that sections
$\lambda_X(a): T\doublerightarrow  X\otimes T$ belongs to
the correspondent category.
The section for the vertex $s\in T_0$ appoints the couple
$\lan a,s\ran\in X_0\times T_0$ and has edges set mappings
$$T(s;t) \rightarrow  1_a(*)\otimes T(s;t)\subset X(a;a)\otimes T(s;t)\tsk$$

For the original $\VV$-graphs transport we need to check only maintenance of unit
arrow mappings
$$ 1_s(*)\rightarrow 1_a(*)\otimes 1_s(*) \subset X(a;a)\otimes T(s;s)\tsk$$

We shall check that section's edges set mappings  are natural for the
contact arrows mappings
$$T(s;t)\otimes T(t;v)\rightarrow (1_a(*)\otimes T(s;t) )\otimes
(1_a(*)\otimes T(t;v) ) \rightarrow  $$
$$(1_a(*)\otimes 1_a(*))\otimes
(T(s;t)\otimes T(t;v)) \rightarrow (1_a(*)\circ 1_a(*))
\otimes (T(s;t)\circ T(t;v))=
$$$$
1_a(*)\otimes (T(s,t)\circ T(t;v))\subset
 X(a;a)\otimes T(s;t)\tsk$$
This can be express with commuting diagram
$$\matrix{ T(s;t)\otimes T(t;v) & \rightarrow &
(1_a(*)\otimes T(s;t))\otimes (1_a(*)\otimes T(t;v)) \cr
\mapdownk {\circ} & & \mapdownd {\circ } \cr
T(s;v) & \rightarrow & 1_a(*) \otimes T(s;v) \cr }$$
\vskip\tarpas
The sections transport also is natural for the contact arrows mappings
$$X(x;y)\otimes X(y;z) \rightarrow (\Prod_{s\in T_0} X(x;y)\otimes 1_s(*))
\otimes (\Prod_{s\in T_0} X(y;z)\otimes 1_s(*) ) = $$$$
\Prod_{s\in T_0} (X(x;y)\otimes 1_s(*))\otimes (X(y;z))\otimes 1_s(*))
\rightarrow $$$$
\Prod_{s\in T_0} (X(x;y)\otimes X(y;z))\otimes (1_s(*)\otimes 1_s(*))
\rightarrow  $$$$
\Prod_{s\in T_0} (X(x;y)\circ X(y;z))\otimes (1_s(*)\circ 1_a(*))= $$$$
\Prod_{s\in T_0} (X(x;y)\circ X(y;z))
\otimes  1_s(*) \subset \Prod_{s\in T_0} X(x;z)\otimes T(s;s)\tsk$$
This can be express by another commuting diagram
$$\matrix{ X(x;y)\otimes X(y;z) & \rightarrow  &
\Prod_{s\in T_0} X(x;y) \otimes 1_s(*))\otimes
\Prod_{s\in T_0} X(y;z) \otimes 1_s(*) \cr
\mapdownk {\circ} &   & \mapdownd {\circ} \cr
X(x;z) & \rightarrow & \Prod_{s\in T_0} X(x;z)\otimes 1_s(*) \cr}$$
\vskip \tarpas
We also can check that collection of sections transports defines
natural transforms in the category of original $\VV$-graphs  transports
   $\Grph_{\VV}$, i. e. for arbitrary  original $\VV$-graphs   transport
  $f: X\doublerightarrow X' $ we have commuting diagram
$$\matrix { X & \mapright f & X' \cr
\mapdownk  \lambda_X & & \mapdownd  \lambda_{X'}  \cr
(X\otimes T )^T & \maprightap  (f\otimes 1_T)^T & (X'\otimes T)^T \cr }$$
\vskip\tarpas
First we shall check the commuting quadrat for appointments of vertexes.
For the vertex $x\in X_0$ we get a section
$\lambda_X(x): T\doublerightarrow  X\otimes T$ with edges mappings
$$T(s;t)\rightarrow 1_x(*)\otimes T(s;t)\subset
X\otimes T(\lan x,s\ran;\lan x,t\ran)\tsk$$
The   original $\VV$-graphs  transport  provided by changing of target
space with the original $\VV$-graphs transport
$f\otimes 1_T: X\otimes T\doublerightarrow X'\otimes T $
appoints another section $T\doublerightarrow X'\times T$ with edges set
mappings
$$T(s;t)\rightarrow f_{x;x}(1_x(*)) \otimes T(s;t)=$$$$
 1_{f_0(x)}(*)\otimes T(s;t) \subset X'(f_0(x);f_0(x))\otimes T(s;t)\tsk$$
So for the vertexes appointment we get the commuting quadrat.

For the edges set  $X(x;y)$ the sections mapping $\lambda_X: X\doublerightarrow
(X\otimes T)^T $ provides the set of transforms between two sections
$$X(x;y)\rightarrow  \Prod_{s\in T_0}X(x;y)\otimes 1_s(*)\subset
\Prod_{s\in T_0} X(x;y)\otimes T(s;s)\tsk$$

The changing of target space provided with the original $\VV$-graphs
 transport $f\times 1_T: X\times T\doublerightarrow X'\otimes T$
produces the edges set mapping
$$X(x;y)\rightarrow \Prod_{s\in T_0} f_{x,y} (X'(x;y))\otimes 1_s(*)
\subset \Prod_{s\in T_0} X'(f_0(x);f_0(y))\otimes T(s;s) \tsk$$
It is the same as the edges set mapping for composition for $\VV$-graphs
transport $f: X\doublerightarrow X'$ with sections transport
$\lambda_{X'}:X'\doublerightarrow (X'\otimes T)^T $.

This commuting diagram remains also for the transports
$f: X\doublerightarrow X'$  from smaller categories $\OGrph_{\VV}^-$,
$\OGrph_{\VV}^+$ or $\OGrph_{\VV}^=$.

The counit transform can be provided by preevaluation or postevaluation
transports. They both will be   original $\VV$-graphs transports.
For the unit arrow mappings $1_\phi\in Y^T(\phi;\phi)$
from  original $\VV$-graphs
transport $\phi: T\doublerightarrow Y$  and unit arrow mapping
$1_s(*) \subset T(s;s)$  we get preevaluation  with precontact arrows
mapping
$$1_{\phi_0(s)}(*) \circ \phi_{s,s}(1_s(*))=1_{\phi_0(s)}(*)\circ
1_{\phi_0(s)}(*)=
1_{\phi_0(s)}(*) \subset Y(\phi_0(s);\phi_0(s))\tsk$$
The same checking can be repeated for postcontact arrows mapping.

However we can't define an evaluation transport in smaller categories of
continuous or
cocontinuous  original $\VV$-graphs transports. So we have the name appointment
in such categories
$$\OGrph_{\VV}^- (X\otimes T; Y)\rightarrow \OGrph_{\VV}^-(X;Y^{T-}) $$
but we haven't any
realization appointment
$$\OGrph_{\VV}^-(X; Y^{T-}) \rightarrow \OGrph_{\VV}^-(X\otimes T; Y)\tsk$$
Later we shall need some additional properties to get continuity property
for $\VV$-graphs evaluation transports over biproduct $X\otimes T$.
\vskip \tarpas

For the original $\VV$-graphs we  may do some  useful calculations.
We shall call a
original  $\VV$-graphs transport $f: X\otimes T \doublerightarrow Y$
^{=preregular} if the prerealization  appointment  reverses its name
$$f= f_+(g(f))\tsk$$
For an  original $\VV$-graphs transport $f$  with upper predecomposition we get an inequality
with its name's  prerealization, which  will be preregular $\VV$-graphs
transport
$$ f\mzl  f_+(g(f)) =f^+\tsk$$
This upper bound is a smallest among preregular bounds.

Otherwise we shall call an original  $\VV$-graphs  transport
$f: X\otimes T \doublerightarrow Y$
^{=postregular} if the postrealization  mapping reverses its name
$$f= f_-(g(f))\tsk$$
For a original $\VV$-graphs transport $f$  with lower  postdecomposition we get an
inequality
with its name's  postrealization, which  will be postregular $\VV$-graphs
transport
$$ f\dgl  f_-(g(f)) =f^-\tsk$$
This lower  bound is a biggest  among postregular lower bounds.
Taken $\VV$-graphs transport $f: X\otimes T\doublerightarrow Y$
has a name corestricted in the space of natural transform exactly when
it coincides with its upper preregular and lower postregular bounds
$$f^-= f=f^+\tsk$$
We shall prove only one of these sentences.

\Proposition
Let we have a   original $\VV$-graphs transport
$f : X\otimes T \doublerightarrow Y$
with upper predecomposition
$$f_{\lan a,s\ran,\lan b,s\ran }(X(a;b)\otimes 1_s(*))\circ
f_{\lan b,s\ran,\lan b,t\ran} (1_b(*)\otimes T(s;t))\dgl$$$$
f_{\lan a,s\ran,\lan b,t\ran}(X(a;b)\otimes T(s;t))\tsk$$
Then appointed prerealization of name $f^+= f_+(g(f))\dgl  f $
is the   smallest preregular upper bound.
\Proof:
We have calculated $f_+(g(f): X\times T \doublerightarrow Y$ as the
composition
$$X\otimes T \mapright \lambda_X\otimes 1_T (X\otimes T)^T\otimes T
 \mapright f^T\otimes 1_T Y^T\otimes T \mapright \ev_Y^+  Y \tsk$$

First sections transport for a vertex $a\in X_0$ will appoint
the section

$\lambda_X(a): T\doublerightarrow X\otimes T$  with edges
set  mappings
$$\lambda_X(a)_{s,t} (T(s;t))= 1_a(*)\otimes T(s;t)\subset X(a;a)\otimes
T(s;t) \tsk$$
The edges set mappings for a sections transport will be
$$(\lambda_X)_{a,b}: X(a;b) \rightarrow \Prod_{s'\in T_0} X(a;b) \otimes
1_{s'}(*) \subset \Prod_{s'\in T_0} (X(a;b) \otimes T(s';s'))\tsk$$

The changing of target space with $\VV$-graphs transport
$ f: X\times T\doublerightarrow Y$
will appoint the $\VV$-graphs transport
$f^T(\lambda_X(a) ): T\doublerightarrow Y$
with edges set mappings
$$ f^T(\lambda_X(a))_{s',t'} (T(s';t'))=
f_{ \lan a,s\ran,\lan a,t\ran} (1_a(*)\otimes T(s;t)) \subset Y
(f_0(a,s);f_0(a,t) )\tsk$$
The edges set mappings of such  changing target space will be
$$(f^T(\lambda_X))_{a,b} (X(a;b))=
\Prod_{s'\in T_0} f_{\lan a,s'\ran,\lan b,s'\ran}
(X(a;b) \otimes 1_{s'}(*)) \subset $$$$
 \Prod_{s'\in T_0} Y (f_0(a,s');f_0(b,s'))\tsk$$
The preevaluation transport  for a set of transforms
between two  $\VV$-graphs transports
 $\phi,\psi: T\doublerightarrow  Y$
and edges set $T(s;t)$ appoints the precontact arrows mapping
$$Y(\phi_0(s);\psi_0(s))\circ \psi_{s,t}(T(s;t))\subset
Y(\phi_0(s);\psi_0(t))\tsk$$
So in our case we get the contact arrows mappings
$$f^+_{\lan a,s\ran,\lan b,t\ran } (X(a;b)\otimes T(s;t))=$$$$
f_{\lan a,s\ran,\lan b,s\ran} (X(a;b)\otimes 1_s(*))
 \circ f_{\lan b,s\ran ,\lan b ,t\ran}  (1_b(*)\otimes T(s;t))  \tsk$$
We can calculate its predecomposition
$$f^+_{\lan a,s\ran,\lan b,s\ran} (X(a,b)\otimes 1_s(*))\circ
f^+_{\lan b,s\ran,\lan b,t\ran} (1_b(*)\otimes T(s;t))=
$$$$
(f_{\lan a,s\ran, \lan b,s\ran} (X(a;b)\otimes 1_s(*))\circ
f_{\lan b,s\ran,\lan b,s\ran }(1_b(*)\otimes 1_s(*)))\circ
$$$$
(f_{\lan a,s\ran,\lan a,s\ran } (1_t(*)\otimes 1_s(*)) \circ
f_{\lan b,s\ran,\lan b,t\ran }(1_b(*)\otimes T(s;t)))= $$$$
f_{\lan a,s\ran,\lan b,s\ran} (X(a;b)\otimes 1_s(*))
 \circ f_{\lan b,s\ran ,\lan b ,t\ran}  (1_b(*)\otimes T(s;t))=$$$$
f^+_{\lan a,s\ran,\lan b,t\ran} (X(a;b) \otimes T(s;t))\subset
Y(f_0(a,s);f_0(b,t))\tsk$$
\irodymopabaiga

For a original $\VV$-graphs and their transports
we can announce classical result about bijective name appointment.

For original $\VV$-graphs transport $f: X\otimes T\doublerightarrow Y$
with decomposition  property
$$f_{\lan a,s\ran,\lan b,s\ran }(X(a;b)\otimes 1_s(*))\circ
f_{\lan b,s\ran,\lan b,t\ran} (1_b(*)\otimes T(s;t))=$$$$
f_{\lan a,s\ran,\lan b,t\ran}(X(a;b)\otimes T(s;t))\tsk$$
we get its name corestricted in the exponential space of natural transforms
$g: X\doublerightarrow Y^{(T)} $.

Otherwise for such partial transport of original $\VV$-graphs corestricted
in exponential space of natural transforms we get realization
with decomposition property. So name  appointment is bijective
$$\OGrph_{\VV} (X\otimes T;Y)=\rightarrow \OGrph_{\VV} (X;Y^{(T)} ) \tsk$$
But we haven't naturality for transports in the target space $Y$.


We can  generalize the notion of original $\VV$-graph $X$  to
the notion  of ^{=lax original $\VV$-graph}
demanding equalities for unit arrow mappings only up unique canonical
isomorphism
$$1_a(*)\circ X(a;b) \sim  X(a;b) \sim X(a;b) \circ
1_b(*)\tsk$$

We get a new category $\OGrphl_{\VV}$ compounded by all $\VV$-graphs
transport $f:X\doublerightarrow Y$ which maintain the unit arrow
mappings up unique canonical
isomorphism in ordered space of mappings from the values category $\VV$
$$f_{a,a} (1_a(*))\sim 1_{f_0(a)}(*)\subset Y(f_0(a);f_0(a))\tsk$$
It will be interesting in the case when such set of mappings  $\VV(r;s)$
gets its ordering from another kind of arrows of some other category,

We can repeat all consideration about original $\VV$-graphs.
We produce only last sentences.
We shall call a
 $\VV$-graphs transport $f: X\otimes T \doublerightarrow Y$
^{=preregular} if the prerealization  mapping reverses its name
up unique canonical isomorphism
$$f\sim f_+(g(f))\tsk$$
For $\VV$-graphs transport $f$  with upper predecomposition we get an inequality
with its name's  prerealization, which  will be preregular $\VV$-graphs
transport
$$ f\mzl  f_+(g(f)) =f^+\tsk$$
This upper bound is an initial in a categorical sense among preregular bounds.

Otherwise we shall call a $\VV$-graphs  transport
$f: X\otimes T \doublerightarrow Y$
^{=postregular} if the postrealization  mapping reverses its name
$$f\sim f_-(g(f))\tsk$$
For $\VV$-graphs transport $f$  with the lower  postdecomposition we get an
inequality
with its name's  postrealization, which  will be the postregular $\VV$-graphs
transport
$$ f\dgl  f_-(g(f)) =f^-\tsk$$
This lower  bound is a final in a categorical sense
among postregular lower bounds.

We can generalize the space of natural transforms  $Y^{(T)}$
demanding inverse image
of similarity relation defined by existing unique canonical isomorphism.
We shall denote  such exponential space $Y^{(T)}_l$  and it will be called
the exponential space of ^{laxly =natural transforms}.
Then  taken $\VV$-graphs transport $f: X\otimes T\doublerightarrow Y$
has name corestricted in the space of natural transform exactly when
it coincides up unique canonical isomorphism with its upper preregular
and lower postregular bounds
$$f^-\sim f\sim f^+\tsk$$
\vskip\tarpas

Now we introduce the ^{=category of $\VV$-enriched categories}.
In an original $\VV$-graph $X$ we demand that for the contact arrows mappings
would be valid associative law.

The first example will be the category $\Cat_{\Set}$  of $\Set$-enriched
categories.
The $\Set$-enriched category will be arbitrary category
 $X$ with small arrows
 sets, i. e. these sets will be objects in the category of small sets
 $\Set$. So the properties of such categories will be familiar in the
 category $\CAT$ of all categories, only the provings will be adapted to
 general $\VV$-enriched categories.
 Values category
 $\VV$ will be taken a small complete monoidal category.
The defined biproduct $r\otimes s$ must be a tensor product, i. e.
we have natural ^{=associativity isomorphism}
$$s_{r,s,v}:r\otimes (s\otimes v)=\rightarrow (r\otimes s)\otimes v$$
which meets the ^{pentagon =diagram} from \baf S. MacLane 1971*  part VII Monoids.
At this moment we don't demand symmetry for such tensor product, only
the ^{=relator's involution}
$$m_{\lan p,s\ran,\lan r,t\ran } :(p\otimes s)\otimes
 (r\otimes t) \rightarrow (p\otimes r) \otimes
(s\otimes t) \tsk$$
Later we shall ask for these arrows
some continuity properties to define a  biproduct $X\otimes Y$ of
$\VV$-enriched categories as  a superfunctor in categories of
continuous or cocontinuous functors
$\Cat_{\VV}^+$, $\Cat_{\VV}^-$.

The language of enriched categories has loosed the capital place
after we have introduced original enriched graphs for study of
joint  pairs of superfunctors. The associativity property
of tensor product in values category $\VV$ is needed to define for
enriched graphs $Y$ and $T$ the
exponential space of natural transforms $Y^{(T)}$ as a superfunctor
in the category of natural  functors $\Cat_{\VV}^=$. For the exponential
space of continuous transforms $Y^{(T)}_+$ we can
define such superfunctor  only in the category of continuous-cocontinuous
functors $\Cat_{\VV}^\pm $. It will be proved for the tensor product
in values category with natural associativity isomorphisms, also it will be true for the associativity property
defined by continuous-cocontinuous  arrows. To solve this problem
for more weak  associativity property would be a special task
for others  values categories.

As earlier we demand existence of an exponential functor $r^s$ with name
appointments $$\VV(r\otimes s;t) \rightarrow \VV(r;t^s)\kbl$$
but also we shall use the opposite realization appointments.

Arbitrary $\VV$-enriched category $X$ will be a set of points $X_0$ with
objects in values category
$X(x;y)\in \VV_0$ as ^{arrows =sets}
and arrows from values category $\VV$ as ^{=mappings between arrows sets}.

 The  structure of $\VV$-enriched category is defined by  ^{=mappings
 of arrows sets composition}
 $$X_{x,y,z}:X(x;y)\otimes X(y;z)\rightarrow X(x;z)\tsk$$
We shall simply denote them   with the sign
of composition for the image set
$$X(x;y)\otimes X(y;z) \rightarrow X(x;y)\circ X(y;z)\subset X(x;z)\tsk$$
Such mappings  must ensure the
associativity  of composition
$$s_{X(x;y),X(y;z),X(z;u)}\circ (X_{x,y,z}\otimes 1_{X(z,u)})\circ X_{x,z,u}
= $$$$
(1_{X(x,y)}\otimes X_{y,z,u})\circ X_{x,y,u}\tsk$$
\vskip\tarpas
$$\hskip -10 pt\matrix{X(x;y)\otimes (X(y;z)\otimes X(z;u)) \hskip -10 pt &
  & \mapright s & &
  (X(x;y)\otimes X(y;z))\otimes X(z,;u) \cr
%
\mapdownk {1_{X(x;y)}\otimes X_{y,z,u}} \hskip 20 pt & & & &
\mapdownd {X_{x,y,z}\otimes 1_{X(z,u)}} \cr
%
\hskip 20 pt X(x;y)\otimes X(y;u) \hskip-20 pt&   & &  &
\hskip -20pt X(x;z)\otimes X(z;u) \hskip 20 pt \cr
%
X_{x,z,u} \hskip -20pt & \searrow &  & \swarrow & \hskip -20 pt X_{x,z,u} \cr
%
& & X(x;u) & & \cr} $$
\vskip \tarpas

The choosing of unit arrow
$$X_x:*\rightarrow X(x;x)$$
can be denoted as
$$1_x: *\rightarrow 1_x(*)\subset  X(x;x)\tsk$$
The arrow from category's final object $*\rightarrow X(x;x)$
usually is understood as choosing of some point in its target space.

This unit arrow choosing  must be a neutral for the source of arrows. Such property
 is expressed  demanding the identity mapping
 for  composition
$$\hskip -10pt 1_{X(x;y)}: X(x,y)\mapright
{!\otimes 1_{X(x,y)}}
 *\otimes X(x;y)
\mapright {X_x\otimes 1_{X(x;y)}}  X(x,x)\otimes  X(x;y)
\mapright {X_{x,x,y}} X(x,y)\tsk$$
The  unit arrow choosing also must be neutral for the target of arrows. This
property  is expressed  by demanding  the identity mapping
  for another composition
$$\hskip -10pt 1_{X(x,y)}: X(x;y)\mapright {1_{X(x,y)}\otimes !}
X(x;y)\otimes *  \mapright {1_{X(x,y)} \otimes X_y}  X(x,y)\otimes  X(y;y)
\mapright {X_{x,y,y}} X(x,y)\tsk$$

The ^{natural  =functors between $\VV$-enriched categories }
$f: X\doublerightarrow Y$
will be defined by appointment of category's points $f_0: X_0\rightarrow Y_0$
and mappings for the arrows sets
$$f_{x,y}: X(x,y)\rightarrow Y(f(x);f(y)) \tsk $$
For such mappings  we shall use also more detailed notation
$$f_{x,y}= X(x;y)\rightarrow f_{x,y} (X(x;y))\subset Y(f(x);f(y))\tsk$$
These arrows sets mappings must allow the
coherence properties. For choosing of unit arrow
we have commuting diagram
$$\matrix{ \ \ \ \ \ \ \ \ \ *  & \mapright {X_x} & X(x;x) \cr
           \mapdownk  {Y_{f_0(x)}} & \swarrow & \hskip -15pt f_{x,x}\cr
           Y(f_0(x);f_0(x)) &       &  \cr }\tsk$$
\vskip \tarpas
Also we have commuting diagrams 
for arrows composition mappings
$$\matrix{X(x,y) \otimes X(y;z) & \mapright {X_{x,y,z}} & X(x,z)\cr
   \hskip -15 pt    \mapdownk {f_{x,y}\otimes f_{y,z}} & &\mapdownd {f_{x,z}} \cr
       Y(f_0(x);f_0(y)) \otimes Y(f_0(y);f_0(z)) &
       \maprightap {Y_{f_0(x),f_0(y),f_0(z)}} &
       Y(f_0(x);f_0(z))\cr} \kbl$$
\vskip \tarpas


The natural  functors between $\VV$-enriched categories compound a category.
The composition of two functors $f: X\doublerightarrow Y$ and $g: Y\doublerightarrow Z$
is defined as usual composition of
points appointments
$$(f\circ g)_0 (x)= g_0(f_0(x)) \uparrow x\in X$$
and the composition of mappings for arrows sets will be
$$(f\circ g)_{x,y}=f_{x,y}\circ g_{f_0(x),f_0(y)}:X(x;y)
\rightarrow Z(g_0(f_0(x));g_0(f_0(y)))\tsk$$
Obviously such composition is associative.

The identity functors $\Identity_X: X\doublerightarrow X$
are defined with identity appointment of points
$\Identity_X(x)= x \uparrow x\in X$
and the identity mappings for arrows sets
$\Identity_{x,y}: X(x;y)\rightarrow X(x;y)$.
They  will provide the ^{left and right =units}
for the composition of functors between $\VV$-enriched
categories.

We shall call such category as  a ^{=category of natural functors between
$\VV$-enriched categories}
and   it will be  denoted $\Cat_{\VV}^= $.
So we have embedding of
such category in the category of natural  functors between original
$\VV$-graphs
 $$\Cat_{\VV}^=\subset \OGrph_{\VV}^=\tsk$$

For values category $\VV$ with ordered arrows sets $V(p;r)$
we can define a more larger stock of continuous functors.
For them we get an imbedding in the category
of continuous functors between  original $\VV$-graphs
$$ \Cat_{\VV}^-\subset \OGrph_{\VV}^-\tsk$$

Also we can define the category of cocontinuous functors.
For them  we get  an imbedding in the category
of original $\VV$-graphs with cocontinuous functors
$$ \Cat_{\VV}^+\subset \OGrph_{\VV}^+\tsk$$

We again shall  work with functors between constructed new categories.
Such functors will be called ^{=superfunctors}, as they are
defined over larger category.

The superfunctor within the category $\Cat_{\VV}$ will be defined
by mapping $F$ over the set of all functors between $\VV$-enriched
categories. It maps arbitrary $\VV$-enriched category  $X$ to another
$\VV$-enriched category  $X^F$ and arbitrary functor $f:X\doublerightarrow Y$
  of $\VV$-enriched categories
to another functor $f^F: X^F\doublerightarrow Y^F$ between
 $\VV$-enriched categories.

It must  maintain the composition of functors
$$(f\circ g)^F= f^F\circ g^F\kbl$$
and the appointment of unit arrows
$$(\Identity_X)^F= \Identity_{X^F}\tsk$$

Now  we shall define some concrete superfunctors.
For two $\VV$-enriched categories $X$ and $Y$ we shall
define a biproduct  $X\otimes Y$
as a category with Carte tensor product of objects sets
$X\times Y$ and  biproduct  in value category $\VV$  of arrows sets
$$X\otimes Y(\lan x,y\ran;\lan x',y'\ran ):= X(x;x')\otimes Y(y;y')\tsk$$

Such biproduct has defined superfunctor in the categories of functors
between original graphs. For $\VV$-enriched categories we need
additionally to check that in the biproduct
 $X\otimes Y$ contact arrows
mappings
$$X\otimes Y(\lan a,a'\ran,\lan b, b'\ran)\circ
X\otimes Y(\lan b,b'\ran'\lan c,c'\ran)=   $$$$
(X(a;b)\circ X(b;c))\otimes (Y(a';b')\circ Y(b';c'))\subset
X(a;c)\otimes Y(a';c')$$
are associative
$$
(X(a;b)\circ (X(b;c)\circ X(c;d)))\otimes
(Y(a';b')\circ (Y(b';c')\circ Y(c';d')))=$$$$
((X(a;b)\circ X(b;c))\circ X(c;d))\otimes
((Y(a';b')\circ Y(b';c'))\circ Y(c';d'))\tsk$$
This is valid for each component, and we must remind
that relator's involution are isomorphic.

In the category of small sets $\Set$ we have used the Carte tensor product.
We can check that new tensor product for $\Set$-enriched categories
rests Carte tensor product,
i. e. its projections  $p_1, p_2: X\otimes Y\doublerightarrow X $
defines ^{final =cone}.
Such projections obviously are natural  functors of $\Set$-enriched categories,
i. e.
maintain the composition of arrows sets and unit arrows.
For arbitrary other
cone of two natural  functors
$f: Z\doublerightarrow X$ and $g: Z\doublerightarrow Y$ we unanimously get
a natural  functor of $\Set$-enriched categories
$\lan f\otimes g\ran: Z\doublerightarrow X\otimes Y_0$.
We get the unique appointment for every point $z\in Z$
$$ \lan f_0(z), g_0(z)\ran\in X_0\times Y_0\tsk$$
For the mappings of arrows sets
$$f_{z_1,z_2}: Z(z_1;z_2)\rightarrow X(f_0(z_1);f_0(z_2)) \kbl
g_{z_1;z_2}: Z(z_1;z_2) \rightarrow Y(g_0(z_1);g_0(z_2))$$
we unanimously get
a mapping
$$\lan f_{z_1,z_2} \times g_{z_1.z_2}\ran : Z(z_1;z_2)\rightarrow
X(f_0(z_1);f_0(z_2)) \times Y(g_0(z_1);g_0(z_2))\tsk$$
Such mappings of arrows sets maintain the arrows sets composition
$$f_{z_1,z_2}\times g_{z_1.z_2}: Z(z_1;z_2)\circ Z(z_2;z_3)\rightarrow
$$$$ (f_{z_1,z_2} (Z(z_1;z_2)) \times g_{z_1,z_2} (Z(z_1;z_2)))\times
(f_{z_2,z_3} (Z(z_2;z_3)) \times g_{z_2,z_3} (Z(z_2;z_3)))=$$$$
(f_{z_1,z_2} (Z(z_1;z_2)) \times f_{z_2,z_3} (Z(z_2;z_3)) \times
( g_{z_1,z_2} (Z(z_1;z_2)) \times g_{z_2,z_3} (Z(z_2;z_3)))\rightarrow $$$$
(f_{z_1,z_2}(Z(z_1;z_2))\circ f_{z_2,z_3}(Z(z_2;z_3)))\times
(g_{z_1,z_2}(Z(z_1;z_2))\circ g_{z_2,z_3}(Z(z_2;z_3)))=
$$$$ f_{z_1,z_3}(Z(z_1;z_2)\circ Z(z_2;z_3))\times
(g_{z_1,z_3}(Z(z_1;z_2)\circ g_{z_2,z_3}(Z(z_2;z_3)) \subset $$$$
f_{z_1,z_3} (Z(z_1;z_3))\times g_{z_1,z_3} (Z(z_1;z_3))
\tsk$$
%It can be expressed by commuting diagram
%$$\matrix{ Z(z_1;z_2)\otimes Z(z_2;z_3)  & \rightarrow &
% (f_{z_1,z_2}(Z(z_1;z_2)\times g_{z_1,z_2}(Z(z_1;z_2) )\times
%(f_{z_2,z_3}(Z(z_2;z_3)\times g_{z_2,z_3}(Z(z_2;z_3) ) \cr
%\mapdownk {\circ} & & \mapdownd {\circ} \cr
%Z(z_1;z_3) & \rightarrow & X(f_0(z_1);f_0(z_3)) \times Y(g_0(z_1);g_0(z_3))
%\cr }$$
%\vskip\tarpas
and also maintain the equalities for chosen unit arrows
$$1_z(*)\circ f_{z,z}= 1_{f_0(z)}(*) \kbl$$
$$1_z(*)\circ g_{z,z}=1_{g_0(z)}(*) \tsk$$
We get the equality
$$ 1_z (*)\circ \lan f_{z,z}\times g_{z,z}\ran) = 1_{\lan f_0(z),g_0(z)\ran}(*)
\tsk$$
 This ends the proving that defined tensor product of $\Set$-enriched
 categories is a Carte  tensor product in the category $\Cat_{\Set}$.

For the general values category $\VV$ we also can take the  Carte tensor product
$p\times r$, but  another biproducts.
can be also  useful. 
Now we want to define the coadjoint exponential superfunctor $Y^T$
at first in the category  of $\Set $-enriched categories, i. e. for the categories with small arrows
sets.  This will be possible only for a small assistant category $T$.

We shall say that $\Set$-enriched category  $T$ is a ^{small =category}
if its points set  $T_0$ is a small set.
For such small set $T_0$ we shall have  a products of small sets  $S_s\in \Set$
$$\Prod_{s\in T_0} S_s  \in \Set \kbl$$
as for small set $T_0$ such product remain a small set,
cl. \baf S. MacLane 1971*
part 1, \S 6, exercise 1.
We shall say that the category of small sets
$\Set$ is a ^{=complete for small
products}.

The exponential category of natural transforms $Y^{(T)}$
will be defined  as some $\Set$-enriched
category only by means of ^{structural =mappings}  $Y_{x,y,z}$ and $Y_x$.
For  a $\Set$-enriched category $Y$ and  a small assistant
$\Set$-enriched category
$T$ the exponential category
 $Y^{(T)}$ is  defined with the objects set compounded of all
 functors between
$\Set$-enriched categories  $\phi: T\doublerightarrow Y$. The
arrows set
between two functors $\phi:T\doublerightarrow Y$ and
$\psi: T\doublerightarrow Y$
will be  a set of natural transforms defined as an equalizer in the product
of arrows sets
$$\rightarrow Y^{(T)}( \phi;\psi)\rightarrow \Prod_{s\in T_0} Y(\phi_0(s);
 \psi_0(s))
\tworightarrows \Prod_{s,t\in T_0} Y(\phi_0(s);\psi_0(t))^{T(s;t)}\tsk$$

We shall use the property of truly joint functors
$r\times s$ and $t^s$ in values category $\Set$
to define such arrows.
In values category $\Set$
for the mapping
$$ f :Y(\phi_0(s);\psi_0(s))\otimes T(s;t)\rightarrow
 Y(\phi_0(s);\psi_0(t))$$
we get its name
$$g=\lceil f\rceil :Y(\phi_0(s);\psi_0(s))\rightarrow
Y(\phi_0(s);\psi_0(t))^{T(s;t)} \tsk$$

This allows us to construct two different mappings  over the product from
values category  $\Set$
$$\Prod_{s\in T_0}  Y(\phi_0(s);\psi_0(s))\tsk$$
First we shall take  an arrow set
from source category $T(s;t)$.
One mapping is defined by precontact arrows mapping
$$ Y(\phi_0(s);\psi_0(s))\otimes
T(s;t)\rightarrow  Y(\phi_0(s);\psi_0(s))\circ \psi_{s,t}(T(s;t))\subset
Y(\phi_0(s);\psi_0 (t))\kbl$$
and another mapping is defined by another postcontact arrows mapping
$$
Y(\phi_0(t);\psi_0(t)) \otimes T(s;t)\rightarrow \phi_{s,t}(T(s;t))\circ
Y(\phi_0(t);\psi_0(t))\subset
Y(\phi_0(s);\psi_0(t))\tsk$$
So we have got two mappings  over the product of two arrows sets
$$Y(\phi_0(s);\psi_0(s))\times Y(\phi_0(t);\psi_0(t))\tworightarrows
(Y(\phi_0(s);\psi_0(t)))^{T(s;t)}
\kbl$$
yet more we get two needed arrows  over the whole product
$$\Prod_{s\in T_0} Y(\phi_0(s);\psi_0(s))\tworightarrows
Y(\phi_0(s);\psi_0(t))^{T(s;t)}\kbl$$
and they all together produces  the correspondent arrows
to the product of target spaces
$$\Prod_{s\in T_0} Y(\phi_0(s);\psi_0(s))\tworightarrows
\Prod_{s,t\in T_0} Y(\phi_0(s);\psi_0(t))^{T(s;t)}\tsk$$

The notion of ^{small =category} is meaningful also for arbitrary
$\VV$-enriched category. We demand that the set of points  $T_0$
for the category  $T$ would be a small set. Let values category $\VV$
 is ^{small =complete},
i. e. we always have the small products of its objects.
Then for a small assistant category $T$ we can apply
the same construction  of various exponential categories.
For values category $\VV$ with ordered arrows sets $\VV(s;r)$
we are yet defined the set of continuous transforms
$Y^{(T))}_-(\phi;\psi)$
or cocontinuous  transforms  $Y^{(T)}_+(\phi;\psi)$ in the
category of original $\VV$-graphs $\Grph_{\VV}$. Now we intend to
define  the correspondent superfunctors
in the category of $\VV$-enriched categories $\Cat_{\VV}$.
We shall probe such construction first for the set  of continuous
transforms $Y^{(T)}_-(\phi;\psi)$.

We have an exponential superfunctor  $Y^T$ defined by the sets of all transforms
$Y^T(\phi;\psi)$  in the category of   original  $\VV$-graphs transports
$\Grph_{\VV}$. The associative composition mappings in the target
$\VV$-graph $Y$
will define the associative composition mappings in the sets of
all transforms $Y^T$. The equality of mappings
$$Y(\phi_0(s);\psi_0(s))\circ (Y(\psi_0(s);\xi_0(s))\circ
Y(\xi _0(s); \chi_0(s)))= $$$$
(Y(\phi_0(s);\psi_0(s))\circ Y(\psi_0(s);\xi_0(s)))\circ
Y(\xi _0(s); \chi_0(s)) $$
produces the equality
for their products
$$Y^T(\phi;\psi)\circ (Y^T(\psi;\xi)\circ
Y^T(\xi; \chi))=
(Y^T(\phi;\psi)\circ Y^T(\psi;\xi))\circ
Y^T(\xi; \chi) \tsk$$

We need to check that for the sets of  continuous  transforms
such composition  produces a  mapping to the correspondent set of continuous
 transforms,
i. e. lies in the inverse image  of order relation from correspondent
product
$$\Prod_{s,t\in T_0} Y(\phi_0(s);\xi_0(t))^{T(s;t)}\tsk$$
Having the inequalities
$$Y(\phi_0(s);\psi_0(t))\circ \psi_{s,t}(T(s;t))\mzl
   \phi_{s,t} (T(s;t))\circ Y(\phi_0(t);\psi_0(t))\kbl$$
$$Y(\psi_0(s);\xi_0(t))\circ \xi_{s,t}(T(s;t))\mzl
   \psi_{s,t} (T(s;t))\circ Y(\psi_0(t);\xi_0(t))\kbl$$
we shall check the inequality for composition

$$\hskip -10 pt (Y(\phi(s);\psi(s))\circ Y(\psi(s);\xi(s)))\circ \xi(T(s;t))
\mzl $$$$\phi(T(s;t))\circ (Y(\phi(t);\psi(t))\circ Y(\psi(t);\xi(t)))\tsk$$
It can be checked by steps applying an associative composition mappings
in the target space $Y$
$$(Y(\phi_0(s);\psi_0(s))\circ Y(\psi_0(s);\xi_0(s)))\circ\xi(T(s;t))\gets =
$$$$Y(\phi_0(s);\psi_0(s)) \circ (Y(\psi_0(s);\xi_0(s))\circ \xi(T(s;t)))\mzl
$$$$Y(\phi_0(s);\psi_0(s))\circ (\psi(T(s;t))\circ Y(\psi_0(t);\xi_0(t)))=\to
$$$$ (Y(\phi_0(s);\psi_0(s))\circ \psi(T(s;t)))\circ Y(\psi_0(t);\xi_0(t))\mzl
$$$$ (\phi(T(s;t))\circ Y(\phi_0(t);\psi_0(t)))\circ Y(\psi_0(t);\xi_0(t))\gets=
$$$$ \phi(T(s;t))\circ (Y(\phi_0(t);\psi_0(t))\circ Y(\psi_0(t);\xi_0(t)))
\tsk$$

So we have checked that the set of continuous transforms $Y^{(T)}_-$
is again a $\VV$-enriched category.
This proving is valid also for an equalizer defining the set  of
natural transforms
$Y^{(T)}$, as the equality is only a partial case of an inequality.

We shall check when for a small assistant $\VV$-enriched category $T$
the appointment of new narrower exponential category  $Y^{(T)}_-$  could
define a superfunctor within some category  of $\VV$-enriched categories.
 For the $\VV$-graphs transport
$f: Y\doublerightarrow Y'$ we have appointed the changing of the target space
$f^T: Y^T\doublerightarrow (Y')^T$
between functor spaces $Y^T$ and $(Y')^T$.

However we can't solve this problem in  the categories $\Cat_{\VV}^-$
or $\Cat_{\VV}^+$. We shall work in a smaller category
of $\VV$-enriched categories of functors which are continuous and
cocontinuous at once
$$\Cat_{\VV}^\mp = \Cat_{\VV}^+\cap \Cat_{\VV}^-\tsk$$
We also demand that arrows $m_{\lan p,s\ran,\lan r,t\ran}$ would define the
transform being  continuous
and cocontinuous at once.
Such property is weaker than the property of natural functors  defined
 by equality relation, i. e. we have inclusion of categories
 $$\Cat_{\VV}^=\subset \Cat_{\VV}^\mp \tsk$$
We shall prove that the changing of target space with ^{continuous-cocontinuous
=functors} $f\in \Cat_{\VV}^\pm $ maintains the exponential space of
continuous transforms  $Y^{(T)}_-$.

\Proposition
The changing of target space with ^{continuous-cocontinuous
=functors} $f\in \Cat_{\VV}^\pm $ maintains the exponential space of
continuous transforms  $Y^{(T)}_-$.
\Proof:

Let we have inequalities  for arbitrary $\VV$-graphs transports
$\phi, \psi\in  X^T$
$$X(\phi_0(s);\psi_0(s))\circ \psi_{s,t} (T(s;t))\mzl
\phi_{s,t}(T(s;t))\circ X(\phi_0(t);\psi_0(t))\tsk$$

Then we can get such inequalities again for changed $\VV$-graphs transports
$\phi\circ f, \psi\circ f\in Y^T$
$$f_{\phi_0(s),\psi_0(s)}(X(\phi_0(s);\psi_0(s)))\circ
 f_{\psi_0(s),\psi_0(t)} (\psi_{s,t}(T(s;t))) \mzl
$$$$  f_{\phi_0(s),\psi_0(t)}(X(\phi_0(s);\psi_0(s))\circ
 \psi_{s,t}(T(s;t))) \mzl
$$$$
 f_{\phi_0(s),\psi_0(t)}( \phi_{s,t}(T(s;t)) \circ
X (\phi_0(t);\psi_0(t)))\mzl
$$$$
 f_{\phi_0(s),\phi_0(t)}( \phi_{s,t}(T(s;t)))) \circ
f_{\phi_0(t),\psi_0(t)} (X (\phi_0(t);\psi_0(t)))\tsk$$
So the changed set of continuous  transforms $Y^{(T)}_-(\phi;\psi)$
is included in the inverse image
defining the set of continuous transforms between changed
$\VV$-graphs transports $Y^{(T)}_-(\phi\circ f;\psi\circ f)\tsk$

To show the proving is easier for the case of equality, defining
exponential space of natural transforms as an  equalizer
$$\rightarrow X^{(T)}(\phi;\psi) \rightarrow
\Prod_{s\in T_0} X(\phi_0(s);\psi_0(s))\tworightarrows
\Prod_{s,t\in T_0} X(\phi_0(s);\psi_0(t))^{T(s;t)} \tsk$$
The changing of target space defines mapping
$$\Prod_{s\in T_0} X(\phi_0(s);\psi_0(s))\rightarrow \Prod_{s\in T_0}
f_{\phi_0(s),\psi_0(s)} (X(\phi_0(s);\psi_0(s)))\subset $$$$
\Prod_{s\in T_0} Y(f_0(\phi_0(s));f_0(\psi_0(t)))\tsk$$
The inclusion  of $X^{(T)}(\phi;\psi)$ into the equalizer of name appointments
provides equals realizations
$$X^{(T)}(\phi;\psi)\otimes T(s;t)\rightarrow
 X(\phi_0(s);\psi_0(s))\circ \psi_{s,t} (T(s;t))\subset
 X(\phi_0(s);\phi_0(t)) \kbl $$
$$X^{(T)}(\phi;\psi)\otimes T(s;t)\rightarrow
\phi_{st} (T(s;t))\circ  X(\phi_0(t);\psi_0(t))
\subset  X(\phi_0(s);\phi_0(t)) \tsk $$
We have yet checked that these equalities provide the equalities also
for the sets of transforms between changed $\VV$-graphs transports
$\phi\circ f,\psi\circ f: T\doublerightarrow Y$
$$X^{(T)}(\phi;\psi)\otimes T(s;t)\rightarrow
 f_{\phi_0(s),\psi_0(s)} (X(\phi_0(s);\psi_0(s)))\circ
 f_{\psi_0(s),\psi_0(t)}(\psi_{s,t} (T(s;t)))\subset
$$$$ Y(f_0(\phi_0(s));f_0(\psi_0(t))) \kbl $$
$$X^{(T)}(\phi;\psi)\otimes T(s;t)\rightarrow
f_{\phi_0(s),\phi_0(t)}(\phi_{st} (T(s;t)))\circ
f_{\phi_0(t),\psi_0(t)}(X(\phi_0(t);\psi_0(t)))
\subset $$$$
Y(f_0(\phi_0(s));f_0(\psi_0(t))) \kbl $$
So we get an equal name arrows, and an arrow to their equalizer
$$\matrix{  X^{(T)}(\phi;\psi) & \rightarrow  &
\Prod_{s\in T_0} X(\phi_0(s);\psi_0(s)) & \tworightarrows   \cr
 \downarrow &      & \downarrow &    \cr
 Y^{(T)}(\phi\circ f;\psi\circ f) & \rightarrow  &
\Prod_{s\in T_0} Y(f_0(\phi_0(s));f_0(\psi_0(s))) & \tworightarrows
 \cr }$$
\vskip\tarpas
For the exponential space of continuous transforms $Y^{(T)}_-$
we need work with product mappings between product spaces
$$ X^{(T)}_-(\phi;\psi)\times X^{(T)}_-(\phi;\psi)\rightarrow
\Prod_{s\in T_0} X(\phi_0(s); \psi_0(s))\times
\Prod_{s\in T_0} X(\phi_0(s); \psi_0(s))  $$$$
\rightarrow \Prod_{s,t\in T_0} X(\phi_0(s);\psi_0(t))^{T(s;t)} \times
        \Prod_{s,t\in T_0} X(\phi_0(s);\psi_0(t))^{T(s;t)}\tsk$$
to define inverse image of order relation in the last product
$$(\mzl ) \subset
\Prod_{s,t\in T_0} X(\phi_0(s);\psi_0(t))^{T(s;t)} \times
        \Prod_{s,t\in T_0} X(\phi_0(s);\psi_0(t))^{T(s;t)}\tsk$$
\irodymopabaiga

With a small $\VV$-enriched assistant category $T$ we have constructed two
superfunctors in the category of $\VV$-enriched categories:
the  biproduct  $X\otimes T$ and the ^{exponential =space
of continuous transforms between continuous-cocontinuous functors}
$Y^{(T)\mp}_- $. We want to  check  have we got truly joint pair of
superfunctors
$$\lan F,G\ran: \Cat_{\VV}^\mp \rightleftarrows \Cat_{\VV}^\mp\tsk$$

The unit transform for such joint pair of superfunctors
is defined by collection of ^{sections =functors}  of $\VV$-enriched
categories
$$\lambda_X: X\doublerightarrow (X \otimes T)^{(T)=}_= \subset
(X\otimes T)^{(T)\pm}_- \tsk$$

Also the unit arrow mapping is corestricted in the set of naturals
transforms
$$1_{\lambda_X(x)}(*)= \Prod_{s\in T_0} (1_x(*)\otimes 1_s(*))
 \subset (X\otimes T)^{(T)=}_=(\lambda_X(x);\lambda_X(x))\tsk$$
 So indeed we have defined  natural   functor
 $\lambda_X: X\doublerightarrow
 (X\otimes T)^{(T)=}_=$.

These sections functors  $\lambda_X: X\rightarrow (X\times T)^T$
has defined a natural transform between superfunctors in the category of original
$\VV$-graphs $\OGrph_{\VV}$, so the commuting quadrats remains in imbedded
smaller category of continuous-cocontinuous functors between $\VV$-enriched
categories  $\Cat_{\VV}^\mp $ or the category of natural  functors between
$\VV$-enriched categories $\Cat_{\VV}^= $,
i. e.
for a continuous-cocontinuous functor  between $\VV$-enriched categories   $f:X\rightarrow X'$
we get commutating quadrats
$$\matrix{X &\mapright f & X'\cr
         \mapdownk \lambda_X & &\mapdownd \lambda_{X'} \cr
         (X\otimes T)^{(T)\mp}_\mp & \maprightap {(f\otimes 1_T)^{(T)}\mp} &
          (X'\otimes T)^{(T)\mp}_\mp\cr}$$
\vskip\tarpas
In the category of original
$\VV$-graphs $\Grph_{\VV}$ for the joint pair of superfunctors  defined
with the biproduct of  assistant $\VV$-graph
$X\otimes T$ and exponential  space of all transforms between 
original $\VV$-graphs transports $ Y^T$ the
counit transform was  provided
in two ways.
One is a collection of preevaluation functors
$$\ev_Y^+: Y^T\otimes T \doublerightarrow Y\tsk$$
They for a original $\VV$-graphs transport
$\phi: T\doublerightarrow Y$  and vertex $s\in T$
appoints the value $\phi_0(s)\in Y$
and for the biproduct of edges sets
$Y^T(\phi;\psi)\otimes T(a;b)$  they appoint
 the set of ^{precontact =arrow }
$$Y(\phi_0(s);\psi_0(s))\circ \psi_{s,t}(T(s;t))\subset
Y(\phi_0(s);\psi_0(t))\tsk$$

Another is a collection of postevaluation functors
$$\ev_Y^- :Y^T\otimes T \doublerightarrow Y\tsk$$
They for a original $\VV$-graphs transport
$\phi: T\doublerightarrow Y$  and vertex $s\in T$
appoints the same value $\phi_0(s)\in Y$
and for the biproduct of edges sets
$Y^T(\phi;\psi)\otimes T(a;b)$  they appoint
 the set of ^{postcontact =arrow }
$$\phi_{s,t}(T(s;t))\circ Y(\phi_0(t);\psi(_0t) ) \subset
Y(\phi_0(s);\psi_0(t))
\tsk$$

Then  with correspondent prerealization or postrealization appointments
of name from any transport $f: X\otimes T\doublerightarrow Y$
 with the properties of upper
predecomposition  and lower  postdecomposition
$$ f_{\lan a,s\ran,\lan b, s\ran } (X(a;b) \otimes 1_s((*)) \circ
f_{\lan b, s\ran,\lan b,t\ran} (1_b(*)\otimes T(s;t))
\dgl  $$$$
 f_{\lan a,s\ran, \lan b,t\ran} (X(a;b)\otimes T(s;t))\dgl $$$$
f_{\lan a,s\ran,\lan a,t\ran} (1_a(*)\otimes T(s;t)) \circ
f_{\lan a, t\ran,\lan b,t\ran} (X(a;b)\otimes 1_t(*)) $$
we have got the inequalities
$$f^+\dgl f \dgl f^-\tsk$$

If contact arrows mappings in $\VV$-enriched category $Y$ were monotone,
then these inequalities can be interpreted as unit and counit transforms
for a newly defined joint pair of monotone superfunctors.

For the categories of $\VV$-enriched categories  we shall
construct more usual truly joint pair of superfunctors.
In the category compounded by continuous functors between $\VV$-enriched
categories  $\Cat_{\VV}^-$ we can check the continuity of preevaluation
transport over the exponential spaces of continuous transforms between
continuous functors
$$\ev^+_Y: Y_-^{(T)-}\otimes T \doublerightarrow Y \tsk$$
.
Let we have three continuous transports of $\VV$-enriched graphs
$\phi,\psi,\xi: T\doublerightarrow Y$
with the correspondent sets of continuous  transforms
$Y^{(T)}_-(\phi;\psi)$, $Y^{(T)}_-(\psi;\xi)$, $Y^{(T)}_-(\phi;\xi)$.
For them we can draw the diagram
$$\matrix {\phi(s) &  & &   &  \cr
        \downarrow &\searrow &&  & \cr
        \psi(s)&\rightarrow &  \psi(t) &   &\cr
        \downarrow &    &\downarrow & \searrow && \cr
        \xi(s) & \rightarrow &  \xi(t)& \rightarrow& \xi(v)\cr}$$
\vskip\tarpas
Then we can write some  equalities with associativity isomorphisms
and inequalities for the sets of continuous transforms between
continuous functors                     
$$(Y^{(T)}_-(\phi;\psi)_s\circ \psi_{s,t}(T(s;t))) \circ
(Y^{(T)}_-(\psi;\xi)_t \circ \xi_{t,v} (T(t;v))) \gets=
$$
$$Y^{(T)}_-(\phi;\psi)_s\circ( \psi_{s,t}(T(s;t)) \circ
(Y^{(T)}_-(\psi;\xi)_t \circ \xi_{t,v} (T(t;v)))) =\to=
$$
$$ Y^{(T)}_-(\phi;\psi)_s \circ ((\psi_{s,t} (T(s;t))\circ
Y^{(T)}_-(\psi;\xi)_t) \circ \xi_{t,v} (T(t;v))) \mzl
$$
$$ Y^{(T)}_-(\phi;\psi)_s \circ ((Y^{(T)}_-(\psi;\xi))_s
\circ \xi_{s,t} (T(s;t)))
\circ  \xi_{(t,v} (T(t;v))) \gets=
$$
$$Y^{(T)}_-(\phi;\psi)_s \circ (Y^{(T)}_-(\psi;\xi)_s)\circ
(\xi_{s,t} (T(s;t))\circ \xi_{t,v} (T(t;v)))) =\to $$
$$(Y^{(T)}_-(\phi;\psi)_s \circ (Y^{(T)}_-(\psi;\xi)_s)\circ
(\xi_{s,t} (T(s;t)\circ \xi_{t,v} (T(t;v))) \tsk
$$

Otherwise in the category compounded by cocontinuous factors between
$\VV$-enriched categories $\Cat_{\VV}^+$  we can check the cocontinuity
of postevaluation transport
$\ev_Y^-: Y^{(T)+}_+\otimes T \doublerightarrow T$
$$( \phi_{s,t}(T(s;t))\circ Y^{(T)}_+(\phi;\psi)_t) \circ
(\psi_{t,v} (T(t;v))\circ Y^{(T)}_+(\psi;\xi)_v )=
$$
$$ \phi_{s,t}(T(s;t))\circ ((Y^{(T)}_+(\phi;\psi)_t) \circ
(\psi_{t,v} (T(t;v)))\circ Y^{(T)}_+(\psi;\xi)_v )\dgl
$$
$$\phi_{s,t}(T(s;t))\circ ((\phi_{t,v} (T(t;v))\circ Y^{(T)}_+(\phi;\psi)_v)
\circ  Y^{(T)}_+(\psi;\xi)_v )=
$$
$$(\phi_{s,t}(T(s;t))\circ \phi_{t,v} (T(t;v)))\circ
 (Y^{(T)}_+(\phi;\psi)_v\circ  Y^{(T)}_+(\psi;\xi)_v )\tsk$$
At this time I haven't written  used isomorphic associativity arrows.

 So in the category of continuous-cocontinuous functors between $\VV$-enriched
categories $\Cat_\mp^{(T)\mp} $ we get both inequalities between preevaluation and postevaluation
transports over the exponential category of continuous-cocontinuous transforms
between continuous-cocontinuous functors of $\VV$-enriched categories.
We get two  continuous-cocontinuous evaluation transports
$$\ev_Y^\pm: Y^{(T)\mp}_\mp \otimes T\doublerightarrow Y\tsk$$
For them we get ^{double =inequalities }
$$f^+\dgl \mzl f\dgl\mzl f^- \tsk$$
Otherwise in the category of natural  functors between $\VV$-enriched
categories $\Cat_{\VV}^=$ we get natural  evaluation functor over
exponential space of natural transforms between natural  functors
$$\ev_Y: Y^{(T)=}_=\otimes T \doublerightarrow Y\tsk$$
\vskip\tarpas
We want to check that such transforms are natural, i. e. we have commuting
quadrats  for arbitrary  functor from correspondent categories
between $\VV$-enriched  categories
 $g:Y\doublerightarrow Y'$
$$\matrix{ Y^T\otimes T & \mapright {g^T\otimes T} &{Y'}^T\otimes T\cr
   \mapdownk \ev_Y & & \mapdownd \ev_({Y')}  \cr
     Y& \maprightap g & Y'\cr }$$
\vskip\tarpas

We have shown  such commuting diagrams even in the category of $\VV$-enriched
graphs for the transports  between  $\VV$-enriched graphs
$g: Y\doublerightarrow Y'$.
Now for the continuous-cocontinuous $\VV$-graphs transports
$g: Y\doublerightarrow  Y'$  we have maintained the exponential space of
continuous transforms
$$g^T_{\phi,\psi}(Y^{(T)\mp}_-(\phi;\psi))
\subset (Y')^{(T)\mp}_-(\phi\circ g;\psi\circ g) \tsk$$
The same is true for the exponential space of cocontinuous transforms
between continuous -cocontinuous $\VV$-graphs transports
$$g^T_{\phi,\psi}(Y^{(T)\mp}_+(\phi;\psi))
\subset (Y')^{(T)\mp}_+(\phi\circ g;\psi\circ g) \kbl $$
also for the intersection of such exponential spaces
$$g^T_{\phi,\psi}(Y^{(T)\mp}_\mp)(\phi;\psi))
\subset (Y')^{(T)\mp}_\mp(\phi\circ g;\psi\circ g) \kbl $$
For the cocontinuous transform defined with arrows
$M_{\lan p,s\ran,\lan r,t\ran}$ we get a continuous biproduct
$g^T\otimes \Identity_T: Y^T\otimes T \doublerightarrow (Y')^T\otimes T$
for  the exponential spaces $Y^T$ of
all transforms between arbitrary $\VV$-graphs
transports. This is true also for smaller exponential spaces $Y^{(T)\mp}_-$
of continuous transforms between continuous-cocontinuous functors of
$\VV$-enriched   categories.

And for the cocontinuous transform defined with arrows
$M_{\lan p,s\ran,\lan r,t\ran}$ we get cocontinuous  biproduct
$g^T\otimes \Identity_T: Y^T\otimes T \doublerightarrow (Y')^T\otimes T$
for  exponential  spaces $Y^T$ of all transforms between arbitrary  $\VV$-graphs
transports. This is also true for smaller  exponential spaces $Y^{(T)\mp}_+$
cocontinuous transforms between continuous-cocontinuous functors
between $\VV$-enriched categories.

We shall get usual results for natural  functors.
Sometimes is useful  to apply more complicate notation for the
exponential space of natural transforms
$$Y^{(T)}= Y^{(T)}_= \tsk$$

\Proposition
Let we have natural transform provided by relator's involution
$$m_{\lan p,s\ran,\lan r,t\ran}: (p\otimes s)\otimes (r\otimes t)
=\rightarrow (p\otimes r)\otimes (s\otimes t)\tsk$$

Then for the category of natural  functors between
 $\VV$-enriched categories $\Cat_{\VV}^=$ we get all properties
of usual trey joint pair of superfunctors
$$\Cat_{\VV}^=\rightleftarrows \Cat_{\VV}^=\tsk$$
The biproduct $X\otimes T$ defines a superfunctor.

For a natural  functor $g: X\doublerightarrow Y$ it appoints the natural
functor provided by biproduct with identity functor of assistant $\VV$-
category $g\otimes \Identity_T: X\otimes T\doublerightarrow Y\otimes T$.

The exponential space of natural transforms between natural  functors
$Y^{(T)=}_=$ defines coadjoint superfunctor.

For a natural  functor
between $\VV$-enriched categories $f:X\doublerightarrow X$ the
changing of target source $f^T: X^T\doublerightarrow Y^T$ maintains
the imbedded exponential space of natural transforms, so we get
the transport of such exponential spaces
$g^{(T)=}_=: X^{(T)=}_=\doublerightarrow  Y^{(T)=}_= $.

The unit transform is defined by natural  sections functors
$$\lambda_X: X\doublerightarrow X^{(T)=}_=\tsk$$
 They are natural
even for arbitrary  original
$\VV$-graphs transport  $f: X\doublerightarrow Y$.

The counit transform is defined by natural  evaluation functor
$$\ev_Y: Y^{(T)=}_= \otimes T \doublerightarrow Y\tsk $$
It is also  natural for natural  functors of $\VV$-enriched categories
$g: X\doublerightarrow Y$.

The  name appointment
$ \Cat_{\VV}^= (X\otimes T;Y) \rightarrow \Cat_{\VV}^+ (X; Y^{(T)=}_= )$.
for a natural  functor $f: X\otimes T\doublerightarrow Y$ appoints the
composition
$$g(f)=f^\#:X\mapright \lambda_X  (X\otimes T)^T \mapright f^T  Y^T\tsk$$
The realization appointment $\Cat_{\VV}^= (X;Y^{(T)=}_=)\rightarrow
\Cat_{\VV}^= (X\otimes T; Y) $
for a natural  functor $g: X\doublerightarrow Y^{(T)=}_=$  appoints  the
composition
$$f(g)=g^\flat :X\otimes T \mapright g\otimes 1_T Y^{(T)=}_=\otimes T
\mapright \ev_Y  Y
\tsk$$
The name and realization appointments are  one to another inverse bijections,
also natural  for natural  functors $f: X\doublerightarrow X'$
 and $g: Y\doublerightarrow Y'$ between $\VV$-enriched categories.

So the first triangular equality is get as name  of the identity mapping
$\Identity_{X\otimes T}: X\otimes T\doublerightarrow X\otimes T$,
and the second triangular equality is get as realization of
 the identity mapping
$\Identity_{Y^{(T)=}_=}: Y^{(T)=}_=\doublerightarrow Y^{(T)=}_=$.
\Proof:
This is only partial case of truly joint pair of superfunctors
in the category $\Cat_{\VV}^\mp$
of continuous-cocontinuous functors between
$\VV$-enriched categories.

\irodymopabaiga

We can introduce lax categories demanding that in some
lax original $\VV$-graph $X$ the contact arrows mappings would define
the associative composition up to unique canonical isomorphism.
Such assumption may be almost possible. May be we shall need some coherence
theorems, as it was for tensor product in monoidal categories done by
MacLane 1970.

Now we could work with lax functors which maintained contact arrows
mappings up unique canonical isomorphisms. They will compound a new category
of ^{=lax functors} $\Catl^=_{\VV}$. Or we could work with
^{weakly =lax functors} which maintain
contact arrows nap pings up some isomorphism.
Their category we shall denote $\Catw_{\VV} $.

The biproduct with assistant lax category  $X\otimes T$
again defines a superfunctor in the category of lax functors.
 For the lax functors $\phi,\psi: T\doublerightarrow Y$
we can define the set of ^{=lax  transforms}
$Y^{(T)l=}_{l=}(\phi;\psi)$. Such sets defines superfunctor  $Y^{(T)l=}_{l=}$
in the category of lax functors $\Catl^=_{\VV}$.

We again get a joint pair of superfunctors in the category of lax
functors
$$\Catl_{\VV}^=\rightleftarrows \Catl_{\VV}^=$$
with unit transform provided by sections functors
$$\lambda_X: X\doublerightarrow (X\otimes )^{(T)=}_= $$
and two counit transforms provided by preevaluation or postevaluation
functors
$$\ev_Y^pm: Y^{(T)l=}_{l=} \otimes T \doublerightarrow Y\tsk$$

They both will be lax functors coinciding up Canonical isomorphism.
For proving we need to repeat earlier proposition about
continuous-cocontinuous functors between $\VV$-enriched categories.
The name appointment can't be bijective. We shall recognize the
equivalence between forms $f: X\otimes T \doublerightarrow Y$
having the same name form.

\Proposition
Let we have laxly natural transform provided by relator's involution
$$m_{\lan p,s\ran,\lan r,t\ran}: (p\otimes s)\otimes (r\otimes t)
=\rightarrow (p\otimes r)\otimes (s\otimes t)\tsk$$

Then in the category  $\Catl_{\VV}^=$ of laxly natural  functors between
 $\VV$-enriched categories we get the  joint pair of superfunctors.
 One adjoint is the  biproduct $X\otimes T$.
 For a laxly natural  functor $g: X\doublerightarrow Y$ it appoints the laxly
 natural functor provided by biproduct with identity functor of assistant $\VV$-
category $g\otimes \Identity_T: X\otimes T\doublerightarrow Y\otimes T$.
For a monotone biproduct from values category $p\otimes r$, we get
this superfunctor $X\otimes T$ being monotone.

The exponential space of laxly natural transforms between laxly
natural  functors
$Y^{(T)l=}_{l=}$ defines coadjoint superfunctor.
For a laxly  natural  functor
between $\VV$-enriched categories $f:X\doublerightarrow X$ the
changing of target source $f^T: X^T\doublerightarrow Y^T$ maintains
the imbedded exponential space of laxly natural transforms, so we get
the transport of such exponential spaces
$g^{(T)l=}_{l=}: X^{(T)=}_=\doublerightarrow  Y^{(T)=}_= $.
For the monotone contact arrows mappings in target space $Y$,
we get again this superfunctor monotone one.

The unit transform is defined by natural  sections functors
$$\lambda_X: X\doublerightarrow X^{(T)=}_=\tsk$$
 They are natural
even for arbitrary  original
$\VV$-graphs transport  $f: X\doublerightarrow Y$.

We have two counit transform defined by  evaluation functors
$$\ev_Y^\pm : Y^{(T)l=}_{l=} \otimes T \doublerightarrow Y \tsk$$
It is also  natural for laxly natural  functors between
$\VV$-enriched categories
$g: X\doublerightarrow Y$.

The  name appointment
$ \Cat_{\VV}^= (X\otimes T;Y) \rightarrow \Cat_{\VV}^+ (X; Y^{(T)=}_= )$.
is corestricted in the space  $Y^{(T)l=}_{l=}$
 of laxly natural transforms between laxly natural functors
 exactly when we have equalities up unique canonical isomorphism
with both realizations defined by the preevaluation and the postevaluation
functors
$$f^+\sim f\sim f^-\tsk$$
\Proof:
This is partial case of the case with continuous-cocontinuous functors
and their continuous-cocontinuous transforms.

\irodymopabaiga

% Uýbaigiau traukõ clattice/yoneda.tex

